The Role of AI in Peer Support for Young People: A Study of Preferences for Human- and AI-Generated Responses

Generative Artificial Intelligence (AI) is integrated into everyday technology, including news, education, and social media. AI has further pervaded private conversations as conversational partners, auto-completion, and response suggestions. As social media becomes young people's main method of peer support exchange, we need to understand when and how AI can facilitate and assist in such exchanges in a beneficial, safe, and socially appropriate way. We asked 622 young people to complete an online survey and evaluate blinded human- and AI-generated responses to help-seeking messages. We found that participants preferred the AI-generated response to situations about relationships, self-expression, and physical health. However, when addressing a sensitive topic, like suicidal thoughts, young people preferred the human response. We also discuss the role of training in online peer support exchange and its implications for supporting young people's well-being. Disclaimer: This paper includes sensitive topics, including suicide ideation. Reader discretion is advised.

==> Plan-ToDo.tex <==
re-arrange findings as follows:

The findings should be in three--experience of support, relatability of scenarios, and response to responses

1. experiences seeking/giving support
- mean, sd, sig. differences? 

2. reliability of scenarios

2. response preference by sourceexperiences seeking support

2. relatability of scenarios
- compare 

==> Title_Ideas.tex <==

IDEAS:
% - Peer Support Exchange Norms
% - The Online and Offline Risk Experiences of Youth: An In-Depth Examination of Self-Report Survey and Private Social Media Data
% - Peer Support Exchange Norms: Measuring Young Adults' Preferences for Responses from Human and AI Sources
- Peer Support Exchange: Understanding Preferences for Responses from Human and AI Sources
- Response Preferences for Peer Support Online: A Comparison of Human and AI-Generated Responses
% - Do AI-Generated Responses Fulfill the Same Needs as Human-Generated Responses in Peer Support?
- Response Preferences for Online Peer Support: A Comparison of Human and AI Sources
- The Role of AI in Peer Support for Young People: A Study of Preferences for Human- and AI-Generated Responses
- Do Young People Prefer AI-Generated Responses to Help-Seeking Messages? % About Sensitive Topics?
- Can AI Be a Useful Tool for Peer Support for Young People?
- The Impact of Topic and Training on Participant Preferences for AI-Generated Responses in Peer Support
- The Future of Peer Support for Young People: Can AI Replace Human Support?

Possibly pull a quote from the text responses?

==> data-distribution-tables/physical-health.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Source} & \textbf{Attribute} & \textbf{Mean} & \textbf{SD} & \textbf{Min} & \textbf{Max} \\ \hline
Peer            & like               & 2.83          & 1.19        & 1.00         & 5.00         \\ \hline
Peer            & problematic        & 2.46          & 1.28        & 1.00         & 5.00         \\ \hline
Peer            & would send         & 2.78          & 1.23        & 1.00         & 5.00         \\ \hline
Peer            & inappropriate      & 2.40          & 1.27        & 1.00         & 5.00         \\ \hline
Peer            & helpful            & 2.73          & 1.22        & 1.00         & 5.00         \\ \hline
Adult Mentor    & like               & 3.48          & 0.99        & 1.00         & 5.00         \\ \hline
Adult Mentor    & problematic        & 2.10          & 1.22        & 1.00         & 5.00         \\ \hline
Adult Mentor    & would send         & 3.44          & 0.99        & 1.00         & 5.00         \\ \hline
Adult Mentor    & inappropriate      & 2.06          & 1.16        & 1.00         & 5.00         \\ \hline
Adult Mentor    & helpful            & 3.43          & 1.01        & 1.00         & 5.00         \\ \hline
Therapist       & like               & 3.43          & 0.97        & 1.00         & 5.00         \\ \hline
Therapist       & problematic        & 2.06          & 1.19        & 1.00         & 5.00         \\ \hline
Therapist       & would send         & 3.38          & 1.01        & 1.00         & 5.00         \\ \hline
Therapist       & inappropriate      & 2.02          & 1.16        & 1.00         & 5.00         \\ \hline
Therapist       & helpful            & 3.45          & 0.99        & 1.00         & 5.00         \\ \hline
AI              & like               & 3.71          & 0.96        & 1.00         & 5.00         \\ \hline
AI              & problematic        & 1.95          & 1.16        & 1.00         & 5.00         \\ \hline
AI              & would send         & 3.64          & 0.99        & 1.00         & 5.00         \\ \hline
AI              & inappropriate      & 1.95          & 1.21        & 1.00         & 5.00         \\ \hline
AI              & helpful            & 3.67          & 0.99        & 1.00         & 5.00         \\ \hline
\end{tabular}
\end{table}

==> data-distribution-tables/relationships.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Source} & \textbf{Attribute} & \textbf{Mean} & \textbf{SD} & \textbf{Min} & \textbf{Max} \\ \hline
Peer            & like               & 3.00          & 1.15        & 1.00         & 5.00         \\ \hline
Peer            & problematic        & 2.41          & 1.24        & 1.00         & 5.00         \\ \hline
Peer            & would send         & 2.98          & 1.18        & 1.00         & 5.00         \\ \hline
Peer            & inappropriate      & 2.38          & 1.24        & 1.00         & 5.00         \\ \hline
Peer            & helpful            & 3.07          & 1.13        & 1.00         & 5.00         \\ \hline
Adult Mentor    & like               & 3.48          & 1.01        & 1.00         & 5.00         \\ \hline
Adult Mentor    & problematic        & 2.04          & 1.13        & 1.00         & 5.00         \\ \hline
Adult Mentor    & would send         & 3.43          & 1.02        & 1.00         & 5.00         \\ \hline
Adult Mentor    & inappropriate      & 2.04          & 1.21        & 1.00         & 5.00         \\ \hline
Adult Mentor    & helpful            & 3.47          & 0.99        & 1.00         & 5.00         \\ \hline
Therapist       & like               & 3.29          & 1.09        & 1.00         & 5.00         \\ \hline
Therapist       & problematic        & 2.23          & 1.24        & 1.00         & 5.00         \\ \hline
Therapist       & would send         & 3.24          & 1.15        & 1.00         & 5.00         \\ \hline
Therapist       & inappropriate      & 2.20          & 1.24        & 1.00         & 5.00         \\ \hline
Therapist       & helpful            & 3.27          & 1.07        & 1.00         & 5.00         \\ \hline
AI              & like               & 3.63          & 1.00        & 1.00         & 5.00         \\ \hline
AI              & problematic        & 2.01          & 1.16        & 1.00         & 5.00         \\ \hline
AI              & would send         & 3.65          & 0.96        & 1.00         & 5.00         \\ \hline
AI              & inappropriate      & 2.01          & 1.20        & 1.00         & 5.00         \\ \hline
AI              & helpful            & 3.63          & 0.95        & 1.00         & 5.00         \\ \hline
\end{tabular}
\end{table}

==> data-distribution-tables/self-expression.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Source} & \textbf{Attribute} & \textbf{Mean} & \textbf{SD} & \textbf{Min} & \textbf{Max} \\ \hline
Peer            & like               & 3.08          & 1.09        & 1.00         & 5.00         \\ \hline
Peer            & problematic        & 2.25          & 1.19        & 1.00         & 5.00         \\ \hline
Peer            & would send         & 3.05          & 1.15        & 1.00         & 5.00         \\ \hline
Peer            & inappropriate      & 2.26          & 1.23        & 1.00         & 5.00         \\ \hline
Peer            & helpful            & 3.12          & 1.09        & 1.00         & 5.00         \\ \hline
Adult Mentor    & like               & 3.51          & 0.94        & 1.00         & 5.00         \\ \hline
Adult Mentor    & problematic        & 2.10          & 1.16        & 1.00         & 5.00         \\ \hline
Adult Mentor    & would send         & 3.48          & 0.97        & 1.00         & 5.00         \\ \hline
Adult Mentor    & inappropriate      & 2.08          & 1.18        & 1.00         & 5.00         \\ \hline
Adult Mentor    & helpful            & 3.51          & 0.99        & 1.00         & 5.00         \\ \hline
Therapist       & like               & 3.46          & 0.97        & 1.00         & 5.00         \\ \hline
Therapist       & problematic        & 2.05          & 1.15        & 1.00         & 5.00         \\ \hline
Therapist       & would send         & 3.42          & 1.05        & 1.00         & 5.00         \\ \hline
Therapist       & inappropriate      & 2.09          & 1.19        & 1.00         & 5.00         \\ \hline
Therapist       & helpful            & 3.49          & 0.98        & 1.00         & 5.00         \\ \hline
AI              & like               & 3.70          & 0.98        & 1.00         & 5.00         \\ \hline
AI              & problematic        & 2.01          & 1.22        & 1.00         & 5.00         \\ \hline
AI              & would send         & 3.67          & 1.00        & 1.00         & 5.00         \\ \hline
AI              & inappropriate      & 1.99          & 1.18        & 1.00         & 5.00         \\ \hline
AI              & helpful            & 3.75          & 0.94        & 1.00         & 5.00         \\ \hline
\end{tabular}
\end{table}

==> data-distribution-tables/suicidal-thoughts.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[h!]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Source} & \textbf{Attribute} & \textbf{Mean} & \textbf{SD} & \textbf{Min} & \textbf{Max} \\ \hline
Peer            & like               & 3.22          & 1.08        & 1.00         & 5.00         \\ \hline
Peer            & problematic        & 2.18          & 1.24        & 1.00         & 5.00         \\ \hline
Peer            & would send         & 3.19          & 1.12        & 1.00         & 5.00         \\ \hline
Peer            & inappropriate      & 2.17          & 1.22        & 1.00         & 5.00         \\ \hline
Peer            & helpful            & 3.18          & 1.11        & 1.00         & 5.00         \\ \hline
Adult Mentor    & like               & 3.59          & 0.95        & 1.00         & 5.00         \\ \hline
Adult Mentor    & problematic        & 2.04          & 1.18        & 1.00         & 5.00         \\ \hline
Adult Mentor    & would send         & 3.56          & 0.95        & 1.00         & 5.00         \\ \hline
Adult Mentor    & inappropriate      & 2.00          & 1.21        & 1.00         & 5.00         \\ \hline
Adult Mentor    & helpful            & 3.61          & 0.94        & 1.00         & 5.00         \\ \hline
Therapist       & like               & 2.99          & 1.12        & 1.00         & 5.00         \\ \hline
Therapist       & problematic        & 2.42          & 1.27        & 1.00         & 5.00         \\ \hline
Therapist       & would send         & 2.94          & 1.20        & 1.00         & 5.00         \\ \hline
Therapist       & inappropriate      & 2.42          & 1.30        & 1.00         & 5.00         \\ \hline
Therapist       & helpful            & 2.97          & 1.15        & 1.00         & 5.00         \\ \hline
AI              & like               & 2.82          & 1.20        & 1.00         & 5.00         \\ \hline
AI              & problematic        & 2.53          & 1.26        & 1.00         & 5.00         \\ \hline
AI              & would send         & 2.71          & 1.21        & 1.00         & 5.00         \\ \hline
AI              & inappropriate      & 2.54          & 1.27        & 1.00         & 5.00         \\ \hline
AI              & helpful            & 2.93          & 1.12        & 1.00         & 5.00         \\ \hline
\end{tabular}
\end{table}

==> holding-area.tex <==
%% old table option for results %%
\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
     \hline
      & \multicolumn{4}{|c|}{Source} \\
     \hline
     \multirow{2}{4em}{ } & Researcher & Young Adult & ChatGPT & Therapist\\
     \hline
      & M (SD) & M (SD) & M (SD) & M (SD)\\
     \hline
     I like this response. & 3.53 (0.93) & 3.01 (1.09) & 3.63 (0.95) & 3.39 (1.00) \\
     This response is problematic. & 2.08 (1.10) & 2.45 (1.20) & 2.10 (1.17) & 2.22 (1.21) \\
     I would send this response. & 3.48 (0.96) & 2.99 (1.12) & 3.65 (0.92) & 3.38 (1.04) \\
     This response is inappropriate. & 2.09 (1.20) & 2.45 (1.23) & 2.06 (1.20) & 2.21 (1.21) \\
     This response contains helpful advice. & 3.51 (0.94) & 3.07 (1.10) & 3.64 (0.89) & 3.42 (0.98) \\
     \hline
    \end{tabular}
    \caption{\Jordyn{ADD CAPTION}}
    \label{tab:scenario_1}
\end{table}

\subsection{Young adults' ability to relate to, sympathize with, and help a friend who is initiating a peer support conversation across topics}
% reactions to scenarios (relate/sympathize/help) - descriptive stats (mean, sd), across scenarios (e.g., correlations between whether they could relate/sympathize/help for one scenario more than another)
The scenarios used in this study come from real-world experiences of youth who could, in theory, be peers of the sample in the present publication. As such, we unsurprisingly found that our participants felt they could relate to, sympathize with, and help the "friend" in the scenarios we presented. One-way Welch tests revealed that there were some significant differences across the four scenarios in participants' ability to relate (F(4,2483) = 13.321, p < 0.001) and sympathize (F(4,2483) = 7.4468, p < 0.001), but not for the extent to which participants felt they could help (F(4,2483) = 2.2767, p = 0.059). Furthermore, there was a significant, positive correlation between the attributes across all scenarios - this means, for example, a participant who reported they could strongly relate to the person in the scenario also tended to report a stronger ability to sympathize with and help (see Figure \ref{fig:corr-matrix-scenario-attributes}).

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{correlation-matrix_2023.8.21.png}
    \caption{Correlation matrix for participants' ability to relate, sympathize, and help across scenarios}
    \label{fig:corr-matrix-scenario-attributes}
\end{figure}

\begin{table}[]
\centering
\begin{tabular}{r|cc|cc|cc|cc|ll}
\cline{2-9}
\multicolumn{1}{l|}{} &
  \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Relationships \& \\ Complications\end{tabular}}} &
  \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Suicidal \\ Thoughts\end{tabular}}} &
  \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Self-\\ Expression\end{tabular}}} &
  \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Physical \\ Health Issues\end{tabular}}} &
   &
   \\ \hline
\multicolumn{1}{|r|}{\textit{attribute}} &
  \multicolumn{1}{c|}{\textit{M}} &
  \textit{SD} &
  \multicolumn{1}{c|}{\textit{M}} &
  \textit{SD} &
  \multicolumn{1}{c|}{\textit{M}} &
  \textit{SD} &
  \multicolumn{1}{c|}{\textit{M}} &
  \textit{SD} &
  \multicolumn{1}{l|}{\textit{p-value}} &
  \multicolumn{1}{l|}{\textit{sig.}} \\ \hline
\multicolumn{1}{|r|}{\textbf{relate}} &
  \multicolumn{1}{c|}{3.22} &
  1.02 &
  \multicolumn{1}{c|}{3.49} &
  0.97 &
  \multicolumn{1}{c|}{3.51} &
  0.92 &
  \multicolumn{1}{c|}{3.60} &
  0.90 &
  \multicolumn{1}{l|}{\textless 0.001} &
  \multicolumn{1}{l|}{yes} \\ \hline
\multicolumn{1}{|r|}{\textbf{sympathize}} &
  \multicolumn{1}{c|}{3.30} &
  1.01 &
  \multicolumn{1}{c|}{3.62} &
  0.88 &
  \multicolumn{1}{c|}{3.55} &
  0.94 &
  \multicolumn{1}{c|}{3.61} &
  0.90 &
  \multicolumn{1}{l|}{\textless 0.001} &
  \multicolumn{1}{l|}{yes} \\ \hline
\multicolumn{1}{|r|}{\textbf{help}} &
  \multicolumn{1}{c|}{3.31} &
  0.98 &
  \multicolumn{1}{c|}{3.46} &
  0.98 &
  \multicolumn{1}{c|}{3.47} &
  0.99 &
  \multicolumn{1}{c|}{3.49} &
  0.94 &
  \multicolumn{1}{l|}{0.059} &
  \multicolumn{1}{l|}{no} \\ \hline
\end{tabular}
\caption{Participants' ability to relate to, sympathize with, and help the person in each of the four situations presented. Answer choices were on a 5-point Likert scale from 1 to 5. Significance from one-way Welch tests describe differences in attributes across scenarios; * \textless 0.001, not.sig}
\label{tab:scenario-attributes}
\end{table}

\subsection{Which response are participants most likely to send?}
Next, we examine the extent to which youth peer support exchange norms align with content generated by a human or AI. To do this, we analyzed responses about whether participants would send a given response. One-way Welch tests showed that mean likelihood to send a given response was significantly different depending on the content source for all scenarios (scenario 1-relationships \& complications: F(3,1375.6) = 43.235, p < 0.001; scenario 2 - suicidal thoughts: F(3,1372.9) = 73.746, p < 0.001; scenario 3 - self-expression: F(3,1377.4) = 34.597, p < 0.001; scenario 4 - physical health issues: F(3,1375.8) = 63.915, p < 0.001). Young adults were more likely to send a response with content generated by AI than a human for 3/4 (75\%) of the scenarios presented. As shown in \ref{tab:responses-send-all}, participants indicated that they were most likely to send the response generated by AI for peer-support scenarios about relationships and complications (M = 3.65, SD = 0.96), self-expression (M = 3.67, SD = 1.00), and physical health issues (M = 3.64, SD = 0.99), but least likely for suicidal thoughts (M = 2.71, SD = 1.21). Interestingly, almost the exact opposite was true for responses generated by peer young adults. In other words, participants were least likely to send a response that was generated by a human their own age for relationships and complications (M = 2.98, SD = 1.18), self-expression (M = 3.05, SD = 1.15), and physical health issues (M = 2.78, SD = 1.23), and the young adult response was the second most likely response for suicidal thoughts (M = 3.19, SD = 0.95) behind the researcher response (M = 3.56, SD = 0.95).

\begin{table}[]
\centering
\begin{tabular}{|cll|cll|cll|cll|}
\hline
\multicolumn{3}{|c|}{\textbf{Relationships \& Complications}} &
  \multicolumn{3}{c|}{\textbf{Suicidal Thoughts}} &
  \multicolumn{3}{c|}{\textbf{Self-Expression}} &
  \multicolumn{3}{c|}{\textbf{Physical Health Issues}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} &
  \multicolumn{1}{c|}{\textit{M}} &
  \multicolumn{1}{c|}{\textit{SD}} &
  \multicolumn{1}{c|}{\textit{source}} &
  \multicolumn{1}{c|}{\textit{M}} &
  \multicolumn{1}{c|}{\textit{SD}} &
  \multicolumn{1}{c|}{\textit{source}} &
  \multicolumn{1}{c|}{\textit{M}} &
  \multicolumn{1}{c|}{\textit{SD}} &
  \multicolumn{1}{c|}{\textit{source}} &
  \multicolumn{1}{c|}{\textit{M}} &
  \multicolumn{1}{c|}{\textit{SD}} \\ \hline
\multicolumn{1}{|c|}{\textbf{ChatGPT}} &
  \multicolumn{1}{l|}{3.65} &
  0.96 &
  \multicolumn{1}{c|}{\textbf{Researcher}} &
  \multicolumn{1}{l|}{3.56} &
  0.95 &
  \multicolumn{1}{c|}{\textbf{ChatGPT}} &
  \multicolumn{1}{l|}{3.67} &
  1.00 &
  \multicolumn{1}{c|}{\textbf{ChatGPT}} &
  \multicolumn{1}{l|}{3.64} &
  0.99 \\ \hline
\multicolumn{1}{|c|}{\textbf{Researcher}} &
  \multicolumn{1}{l|}{3.43} &
  1.02 &
  \multicolumn{1}{c|}{\textbf{Young Adult}} &
  \multicolumn{1}{l|}{3.19} &
  1.12 &
  \multicolumn{1}{c|}{\textbf{Researcher}} &
  \multicolumn{1}{l|}{3.48} &
  0.97 &
  \multicolumn{1}{c|}{\textbf{Researcher}} &
  \multicolumn{1}{l|}{3.44} &
  0.99 \\ \hline
\multicolumn{1}{|c|}{\textbf{Therapist}} &
  \multicolumn{1}{l|}{3.24} &
  1.15 &
  \multicolumn{1}{c|}{\textbf{Therapist}} &
  \multicolumn{1}{l|}{2.94} &
  1.20 &
  \multicolumn{1}{c|}{\textbf{Therapist}} &
  \multicolumn{1}{l|}{3.42} &
  1.05 &
  \multicolumn{1}{c|}{\textbf{Therapist}} &
  \multicolumn{1}{l|}{3.38} &
  1.01 \\ \hline
\multicolumn{1}{|c|}{\textbf{Young Adult}} &
  \multicolumn{1}{l|}{2.98} &
  1.18 &
  \multicolumn{1}{c|}{\textbf{ChatGPT}} &
  \multicolumn{1}{l|}{2.71} &
  1.21 &
  \multicolumn{1}{c|}{\textbf{YoungAdult}} &
  \multicolumn{1}{l|}{3.05} &
  1.15 &
  \multicolumn{1}{c|}{\textbf{YoungAdult}} &
  \multicolumn{1}{l|}{2.78} &
  1.23 \\ \hline
\end{tabular}
\caption{The average responses for the extent to which participants agreed that they would send a response with content from each response source across all four scenarios. Means (M) and standard deviations (SD) are listed for each of the four scenarios in decreasing order by source within each scenario. Answer choices were on a 5-point Likert scale from 1 to 5; 1 was least likely to send and 5 was most likely to send.}
\label{tab:responses-send-all}
\end{table}

% most/least favorite response for each scenario - table with mean/sd for each attribute of 4 responses across scenarios (+ if they're significant?), and  most/least favorite responses for each scenario by demographic variable (male/female, ethnicity, etc.) (e.g., were males/females more likely to prefer a response from ChatGPT across all scenarios?)

- 5 attributes by source (e.g., for the researcher, the extent to which they like/problematic/send/inappropriate/helpful that source's response was across scenarios) and see if sig. differences


% old note from results
Double check that all numbers in table are correctly copied from R!! Add Within-subjects ANOVA + post-hoc analyses (see message from Dr. Huh-Yoo in Slack)
ANOVA for all types of responses
post-hoc analysis for different pair combinations w/t-tests
2 tables:
- most/least favorite for all scenarios
- 5 metrics for each response for all scenarios + extra column for ANOVA significance
- post-hoc analyses w/pair-wise analysis to see which pairs fo response source to see wihch are significantly different, use table format from health/epidemiology

% old results tables for scenarios attributes:
\begin{table}[]
\centering
\begin{tabular}{|r|cc|cc|cc|}
\hline
\multirow{2}{*}{\textbf{Scenario Topic}} &
  \multicolumn{2}{c|}{\textbf{Relate}} &
  \multicolumn{2}{c|}{\textbf{Sympathize}} &
  \multicolumn{2}{c|}{\textbf{Help}} \\ \cline{2-7} 
 &
  \multicolumn{1}{c|}{\textit{Mean}} &
  \textit{SD} &
  \multicolumn{1}{c|}{\textit{Mean}} &
  \textit{SD} &
  \multicolumn{1}{c|}{\textit{Mean}} &
  \textit{SD} \\ \hline
\textbf{Relationships \& Complications}   & \multicolumn{1}{c|}{3.22} & 1.02 & \multicolumn{1}{c|}{3.30} & 1.01 & \multicolumn{1}{c|}{3.31} & 0.98 \\ \hline
\textbf{Suicidal Thoughts}                & \multicolumn{1}{c|}{3.49} & 0.97 & \multicolumn{1}{c|}{3.62} & 0.88 & \multicolumn{1}{c|}{3.46} & 0.98 \\ \hline
\textbf{Self-Expression}                  & \multicolumn{1}{c|}{3.51} & 0.92 & \multicolumn{1}{c|}{3.55} & 0.94 & \multicolumn{1}{c|}{3.47} & 0.99 \\ \hline
\textbf{Physical Health Disorders/Issues} & \multicolumn{1}{c|}{3.60} & 0.90 & \multicolumn{1}{c|}{3.61} & 0.90 & \multicolumn{1}{c|}{3.49} & 0.94 \\ \hline
\end{tabular}
\caption{Participants' ability to relate to, sympathize with, and help the person in each of the four situations presented. Answer choices were on a 5-point Likert scale from 1 to 5.}
\label{tab:scenarios-attributes-descriptives}
\end{table}


\begin{table}[]
\centering
\begin{tabular}{rccc}
\textbf{Scenario attribute} & \textbf{df} & \textbf{chi-square} & \textbf{p-value} \\
\textbf{relate}             & 3           & 0.02                & 1.00             \\
\textbf{sympathize}         & 3           & 0.02                & 1.00             \\
\textbf{help}               & 3           & 0.01                & 1.00            
\end{tabular}
\caption{}
\label{tab:scenario-attributes-chi-square}
\end{table}

\begin{comment}
% ANOTHER VERSION OF RESPONSES-ALL-SEND TABLE NOT ORGANIZED BY DESCENDING MEAN
\begin{table}[]
\centering
\begin{tabular}{r|cccc|}
\cline{2-5}
\multicolumn{1}{l|}{}                          & \multicolumn{4}{c|}{\textit{\begin{tabular}[c]{@{}c@{}}Response Content Source\\ M (SD)\end{tabular}}}               \\ \cline{2-5} 
\multicolumn{1}{l|}{} &
  \multicolumn{1}{c|}{\textbf{AI}} &
  \multicolumn{1}{c|}{\textbf{human (peer)}} &
  \multicolumn{1}{c|}{\textbf{human (adult)}} &
  \textbf{human (adult/therapist)} \\ \hline
\multicolumn{1}{|r|}{\textbf{All Scenarios}}   & \multicolumn{1}{c|}{3.42 (1.12)} & \multicolumn{1}{c|}{3.00 (1.18)} & \multicolumn{1}{c|}{3.48 (0.98)} & 3.25 (1.12) \\ \hline
\multicolumn{1}{|r|}{\textbf{\begin{tabular}[c]{@{}r@{}}Relationships \& \\ Complications\end{tabular}}} &
  \multicolumn{1}{c|}{3.65 (0.96)} &
  \multicolumn{1}{c|}{2.98 (1.18)} &
  \multicolumn{1}{c|}{3.43 (1.02)} &
  3.24 (1.15) \\ \hline
\multicolumn{1}{|r|}{\textbf{\begin{tabular}[c]{@{}r@{}}Suicidal\\ Thoughts\end{tabular}}} &
  \multicolumn{1}{c|}{2.71 (1.21)} &
  \multicolumn{1}{c|}{3.19 (1.12)} &
  \multicolumn{1}{c|}{3.56 (0.95)} &
  2.94 (1.20) \\ \hline
\multicolumn{1}{|r|}{\textbf{Self-Expression}} & \multicolumn{1}{c|}{3.67 (1.00)} & \multicolumn{1}{c|}{3.05 (1.15)} & \multicolumn{1}{c|}{3.48 (0.97)} & 3.42 (1.05) \\ \hline
\multicolumn{1}{|r|}{\textbf{\begin{tabular}[c]{@{}r@{}}Physical Health\\ Issues\end{tabular}}} &
  \multicolumn{1}{c|}{3.64 (0.99)} &
  \multicolumn{1}{c|}{2.78 (1.23)} &
  \multicolumn{1}{c|}{3.44 (0.99)} &
  3.38 (1.01) \\ \hline
\end{tabular}
\caption{The average response for the extent to which participants agreed that they would send a response with content from each response source. Means and standard deviations are listed for each of the four scenarios, and overall across scenarios. Answer choices were on a 5-point Likert scale from 1 to 5; 1 was least likely to send and 5 was most likely to send.}
\label{tab:responses-all-send}
\end{table}
\end{comment}

\begin{comment}
% HORIZONTAL VERSION OF RESPONSES-ALL-SEND TABLE
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccccccccc}
\hline
\multicolumn{2}{c}{} &
  \multicolumn{2}{c}{\textbf{Relationships \& Complications}} &
  \multicolumn{2}{c}{\textbf{Suicidal Thoughts}} &
  \multicolumn{2}{c}{\textbf{Self-Expression}} &
  \multicolumn{2}{c}{{\color[HTML]{444444} \textbf{Physical Health Disorders \& Issues}}} &
  \multicolumn{2}{c}{\textbf{Overall}} \\ \hline
\multicolumn{2}{c}{\textit{Response Source}} &
  \textit{M} &
  \textit{SD} &
  \textit{M} &
  \textit{SD} &
  \textit{M} &
  \textit{SD} &
  \textit{M} &
  \textit{SD} &
  \textit{M} &
  \textit{SD} \\ \hline
\textbf{AI} &
  \textbf{chatgpt} &
  3.65 &
  0.96 &
  2.71 &
  1.21 &
  3.67 &
  1.00 &
  3.64 &
  0.99 &
  3.42 &
  1.12 \\ \hline
\textbf{human (peer)} &
  \textbf{young adult} &
  2.98 &
  1.18 &
  3.19 &
  1.12 &
  3.05 &
  1.15 &
  2.78 &
  1.23 &
  3.00 &
  1.18 \\ \hline
\textbf{human (adult)} &
  \textbf{researcher} &
  3.43 &
  1.02 &
  3.56 &
  0.95 &
  3.48 &
  0.97 &
  3.44 &
  0.99 &
  3.48 &
  0.98 \\ \hline
\textbf{human (adult/therapist)} &
  \textbf{therapist} &
  3.24 &
  1.15 &
  2.94 &
  1.20 &
  3.42 &
  1.05 &
  3.38 &
  1.01 &
  3.25 &
  1.12 \\ \hline
\end{tabular}%
}
\caption{The average response for the extent to which participants agreed that they would send a response with content from each response source. Means and standard deviations are listed for each of the four scenarios, and overall across scenarios. Answer choices were on a 5-point Likert scale from 1 to 5; 1 was least likely to send and 5 was most likely to send.}
\label{tab:responses-send}
\end{table}
\end{comment}

% OLD METHODS DRAFT FROM JORDYN
\section{Methods}

We conducted an online survey 18 - 24-year-olds in the US who are fluent in English and have access to the Internet. We received 1,096 responses from eligible participants, of which 622 were useable for analyses because they were complete and passed the built-in attention check question.

...The survey focused on...and included questions about demographic information such as age, gender, LGBTQIA+ status...

\Jordyn{Are we going to talk about responses to how AI could help? If not, should we even mention that we asked that question, or just say that this paper is based on a subset of data from a larger survey study?}
\Mari{(Jordyn writes this part?)}
\subsection{Survey Design}
\textit{Scenarios}
How we came up with the four scenarios:
These scenarios come directly from a previously published CHI paper \cite{huh2023help}; research assistants qualitatively coded a dataset of Instagram conversations from youth and identified the similarity between themes discussed in the publication. They merged the 20 most common problems that teens often encounter. These situations cover many different aspects of teens’ life: family, friends, school, relationships, and their personal lives. For each of these, a small paragraph describing the context and some sample quotes extracted from the corresponding conversations in the dataset are added.

\textit{Questions about the scenarios} To better understand how participants responded to each scenario presented, we asked participants to rate the extent to which they agreed with the following statements: (1) I can relate to the person in this situation, (2) I can sympathize with the person in this situation, and (3) I can help the person in this situation. \Jordyn{how are we going to use this in the analysis, if at all?}
We also asked participants how they would 

\Jordyn{Perhaps add a sample photo of the scenario to show how it was presented? To show that we wanted the participants to imagine themselves sending the response, so we gave them visual cues to help with that?}

\textit{Responses}
For each of the four scenarios, we presented participants with four possible responses written by (1) a researcher, (2) a young adult from the previously published CHI paper \cite{huh2023help}, (3) ChatGPT, and (4) a licensed therapist. Participants were \textit{not} given any information about the source of the responses - we simply presented the messages and asked participants to rate the extent to which they agreed with the following statements: (1) I like this response, (2) This response is problematic, (3) I would send this response, (4) This response is inappropriate, and (5) This response contains helpful advice. We measured agreement with a 5-point Likert scale (1 = not at all, 5 = extremely).
\Jordyn{Add text about how we came up with the response from ChatGPT}

\textit{Demographic Information} We also asked for demographic information about our participants that could impact their responses to the questions we asked, including their gender, ethnicity, and level of education. \Jordyn{Add citation about how we know each of these factors impacts HCI to support why we asked them}

\subsection{Procedure}
We recruited broadly on a first-come, first-serve basis using online posts on social media. Anyone interested in taking part in our study was directed to a one-time Qualtrics survey, where they began by filling out screening questions to assess eligibility (18-24 years old, currently living in the US, fluent in English, and stable access to the internet). For those who were eligible based on responses to the screening survey questions, they were presented with the study information and then the main survey instrument which took approximately 30 minutes to complete. After completing the survey, participants had the option to provide their contact information and receive \$5 as payment for their time. 

\subsection{Participant Demographics}

==> old/methods-v1.tex <==
VERSION 1 FROM MARI AND KAYLIE:
%To build on our aim of understanding young adults’ needs and design requirements for effective online social support and support exchange systems with the support of automatic systems such as Ai and answer our main research question, we developed a survey and interview, where our objective is to capture various ways in which young adults are interacting with their peers when seeking or receiving support. Our survey was designed to capture crucial information about how young adults prefer to interact with peers, their attitudes towards the different types of support and their attitudes towards receiving support with the presentation of various situations (see 4.2) while also capturing crucial insights on how AI can assist in potentially providing support. The survey helped us assess participants' views on the appropriateness of different responses, including AI-generated ones which allowed us to gauge participants openness to automatic systems and identifying information about design requirements such as what behavior, responses and interaction is expected and deemed appropriate.  % After collecting and analyzing our survey data, our next steps included conducting an interview of individuals who adhered to our Eligibility criteria  which was designed and reviewed by our researchers and principal investigators (PI’s) (4.2, 4.3). The aim of the interview was to have a more In- depth exploration and uncover the nuance that we may have missed in the survey, \Mari{to be elaborated upon once interview is completed} 

% Regarding our main survey questions, we first asked participants to share their experience with seeking and giving online support. Next, we presented 4 fictitious scenarios in randomized order, representing 4 main problems/topics that young adults often seek support for. These scenarios come directly from a previously published CHI paper on peer support among youth via Instagram Direct Messages [22]; research assistants qualitatively coded a dataset of Instagram conversations from youth and identified the similarity between themes discussed in the publication. They merged the 20 most common problems that teens often encounter. We narrowed them down to 4 typical scenarios that are suitable for the length of the survey but still cover typical problems of teens’ life. For each of these, a small paragraph describing the context and some sample quotes extracted from the corresponding conversations in the dataset are added. 

% To engage the participants into our scenarios, we showed them an image of a text message from a “friend” who was dealing with the problem. [Insert a sample image]. We asked participants to rate the extent to which they agreed with the following statements: (1) I can relate to the person in this situation, (2) I can sympathize with the person in this situation, and (3) I can help the person in this situation. We aimed to examine whether there is a correlation between teenagers’ sympathy and their ability to provide support, and whether this correlation is recorded through every scenario. We also asked participants how they would respond in each situation if the corresponding help seeker reached out to them for help. 

% For each of the four scenarios, we presented participants with four possible responses written by (1) a researcher in our project, (2) a young adult from the dataset of the previously published CHI paper [22], (3) ChatGPT, and (4) a licensed therapist. Participants were not given any information about the source of the responses - we simply presented the messages and asked participants to rate the extent to which they agreed with the following statements: (1) I like this response, (2) This response is problematic, (3) I would send this response, (4) This response is inappropriate, and (5) This response contains helpful advice. We measured agreement with a 5-point Likert scale (1 = not at all, 5 = extremely). Among 4 sources of responses, ChatGPT is the only non-human source. Acknowledging the rise of AI in this digital age, we were curious about whether and how ChatGPT, one of the most popular chatbots among young people, could advise and support them with their daily life problems. Before finalizing the ChatGPT’s response that we would put into the survey, we experimented with prompt generating with the chatbot (e.g., same prompts but at different times, prompts in first-person vs. third-person points of view) to see how different its responses for the same situation could be. 

% At the end of each scenario, we asked participants to choose the responses that they liked the most and the least and explain their answers. Furthermore, a question about how AI could possibly help in the situation was also given. We also asked for our participants’ demographic information, which could impact their responses to the questions we asked, including their age, gender, LGBTQIA+ status, ethnicity, and level of education. \Jordyn{Add citation about how we know each of these factors impacts HCI to support why we asked them}

% After 2 weeks giving out the survey, we received 1,096 responses from eligible participants, of which 622 were usable for analyses because they were complete and passed the built-in attention check question. 

% \subsection{Interview Design }

% Among 622 participants, we sorted out 105 participants qualified to take part in our interview, based 5 criteria of the first screening: 

% \textit{(1) Successfully completing the survey}  

% \textit{(2) Participants providing more than 3 words in all quantitative answers}  

% \textit{(3) ReCAPTCHA is greater than 0.55} 

% \textit{(4) Participants who scored 3 or more on questions focused on seeking support } 

% \textit{(5) Participants who scored 3 or more on questions focused on giving support} 


% We then incorporated a second screening, using prior interviewing experience from our researchers, we looked for:  


% \textit{(1) A diverse demographic background (e.g., gender, age, sexuality, level of education) }

% \textit{(2) Quality of their responses (e.g., how detailed their answers are lengthwise, how much 	effort they put into the answers, whether they expressed any interesting points of view).}  

% Our goal remained to invite a representative sample of participants with a variety of different opinions on the same questions. Their interview answers will continue to be studied in our upcoming project as an extension of this research. \Mari{In progress}

%\subsubsection{Scenarios}
%\Jina{these scenarios--> which scenarios? Need some overview of the survey before jumping in}
 
%research assistants qualitatively coded a dataset of Instagram conversations from youth and identified the similarity between themes discussed in the publication. They merged the 20 most common problems that teens often encounter. These situations cover many different aspects of teens’ life: family, friends, school, relationships, and their personal lives. For each of these, a small paragraph describing the context and some sample quotes extracted from the corresponding conversations in the dataset are added.
% \Jina{unnecessary detail} - addressed

%\subsubsection{Responses}


%\subsubsection{Demographic Information} We also asked for demographic information about our participants that could impact their responses to the questions we asked, including their gender, ethnicity, and level of education. 
% \Jordyn{Add citation about how we know each of these factors impacts HCI to support why we asked them}
% \Jina{I don't think we need to. Unnecessary detail.} - addressed

%\subsection{Procedure}

==> old/methods-v2.tex <==
\section{Methods}
\label{sec:methods}
\subsection{Overview}
We used an online survey to ask young adults about help-seeking scenarios and pre-written responses. \Jina{just make sure that the core terms of our contribution, such as 'help-seeking scenarios' and 'pre-written responses' are consistently used throughout the paper, including the research questions. Right now they are different}
% , without saying where the responses came from. 
In this section, we describe our recruitment strategy and procedure, explain our survey design, and describe our approach to data analysis. \Jordyn{Jina, do you think this addresses the point you made about stating an objective that addresses our research questions (without just re-stating them since they're in the intro)?} \Jina{let's work on this once we have a fuller paper, including introduction, because it needs to flow and not be repeated. Depending on what's written in the intro, we might move on right away or explain here. It really all depends on the rest of the paper, so hard to say yet without seeing the full draft.}
\Jina{skipping methods and going to findings}

\subsection{Recruitment Process}
% This study took place entirely online. We recruited survey participants by sharing a digital flyer with the authors' social media networks, including Instagram, Facebook, X (formerly known as Twitter), Discord, and Slack. The flyer included a quick summary of the project and a link to a screening survey for those who were interested in participating. 
We used an online screening survey 
% asked four questions 
to determine prospective participants' eligibility; 
% more specifically, we wanted to make sure they were 
including 1) being 18 to 24 years old, 2) currently living in the U.S., 3) fluent in English, and 4) had stable access to the Internet. 
% 1,451 respondents completed the screening questions, of which 1,096 met all four criteria for eligibility. 
Eligible respondents (N=1,096) continued to the study information sheet approved by IRB, which they were asked to review before continuing to the main survey (see section \Jordyn{add ref to survey design section} for additional details). Our survey included three main sections described below. After finishing the survey, participants could provide their contact information to receive \$5 as payment for their time. We received 866 complete survey responses from eligible participants, of which 622 were deemed fit for analysis because they passed a built-in attention check question (\Afsaneh{add what it was about}).

\subsection{Survey Design}
Our survey included three main sections: (1) help-seeking scenarios and responses, (2) prior experience with online peer support, and (3) demographic information. We describe each of these below.

\subsubsection{Help-seeking Scenarios and Responses}
% These questions were broken up into four sections, each dedicated to a different help-seeking scenario:
We had four help-seeking scenarios including relationships, suicidal thoughts, self-expression, and physical health. These scenarios come 
% directly from our group's previously published study 
from previous literature \cite{huh2023help} about frequent topics of private conversations for social support exchange between youth. For each scenario, there were four parts: (1) presenting a help-seeking message from a friend, (2) questions about the help-seeking message, (3) presenting pre-written responses to the help-seeking message, and (4) questions about the pre-written responses. To prevent question order bias, we randomized both the order in which the scenarios were presented and the questions within each scenario's four parts.

\textbf{(1) Presenting a help-seeking message}: 
We presented the scenarios in the form of a friend asking for help through a direct message. We asked participants to "imagine [they received] the following message from a friend as a text or direct message on social media" followed by a help-seeking messages from the paper \cite{huh2023help}). The help-seeking messages for each scenario are in Table \Jordyn{ref table when created}.   

\Jordyn{add table here with scenarios + help-seeking messages}

\begin{table}
\centering
\caption{Scenarios and Help-seeking messages.}
\begin{tabular}{|p{0.1\linewidth}|p{0.7\linewidth}|}
\hline
\textbf{Scenario} &
  \textbf{Help-Seeking Messages} \\ \hline
\begin{tabular}[c]{@{}l@{}}Relationships \\ \end{tabular} &
  \begin{tabular}[c]{@{}l@{}} ``Hey, I'm feeling pretty emotional right now. So, get this, my ex invited me over to his place and things got weird. He started touching me and kept asking for sex, even though he has a girlfriend. I don't know why he does this. It's messed up, but I'm ashamed to admit that I'm kind of falling for it. We were on the phone just now and he fell asleep. Ugh, I can't believe this is happening.''\end{tabular}
\end{tabular}
\end{table}

\begin{comment}
Relationships: \textit{Hey, I'm feeling pretty emotional right now. So, get this, my ex invited me over to his place and things got weird. He started touching me and kept asking for sex, even though he has a girlfriend. I don't know why he does this. It's messed up, but I'm ashamed to admit that I'm kind of falling for it. We were on the phone just now and he fell asleep. Ugh, I can't believe this is happening.}

Suicidal thoughts: \textit{I don't know what to do. I'm having a panic attack and these thoughts won't stop. I feel so overwhelmed and trapped by my own mind. I don't feel like I'm worth anything and I don't see a way out. I'm scared and I don't know how to cope with these feelings. It's like I'm drowning, and I can't breathe. I don't want to live like this}

Self-expression: \textit{I don't know what's wrong with me, I really struggle with communicating because of my anxiety, I don’t want to be judged and I always get so nervous when I have to share my thoughts and feelings with others. I'm afraid of not being taken seriously. I can’t seem to shake it off, I just wish I could get out of my head and stop overthinking everything.}

Physical health: \textit{I’m feeling drained both physically and emotionally... like, every morning, I wake up feeling tired and unmotivated. The thought of getting out of bed and facing the day seems like an impossible task. The other day, I went to counseling hoping it would help me feel better, but I feel the same. I still feel overwhelmed and stressed. All I want to do is to take some time to rest and recharge my energy.}
\end{comment}
 
\textbf{(2) Questions about the help-seeking message}: 
We then asked participants to rate the extent to which they agreed with the following statements: "I can relate to the person in this situation," "I can sympathize with the person in this situation," and "I can help the person in this situation." Answer choices were on a 5-point Likert scale (1 = not at all, 5 = extremely).
\Jordyn{describe why we asked these questions and why participants' reactions to the scenarios is important}

\textbf{(3) Presenting pre-written responses to the help-seeking message}: 
For each of the four scenarios (relationships, suicidal thoughts, self-expression, and physical health), we presented four pre-written responses originating from (1) a young adult, (2) a researcher, (3) a therapist, and (4) ChatGPT. 
We wanted to understand the young adult's norms and preferences about responses with various proficiency generated from different sources.
The youth responses were from the original youth conversations for each scenario \cite{huh2023help}.
We wanted to investigate a response from same age group as young adult, but with more experience and training to prorivide support. So the responses from researchers were designed by Undergraduate Research Assistant who had training in \Afsaneh{need to find what type of training channacy had}. 
Next, to provide a professional response, we had a clinical psychologist on the team who drafted the therapist response.
Given the popularity of AI LLMs among young people \Afsaneh{[CITE]} and their potential to provide support \Afsaneh{[CITE]}, we included a response from ChatGPT to each scenario.
\Afsaneh{Kaylie please add what was prompted to Chatgpt and when.}


We did not tell participants where the pre-written responses came from because we wanted to understand their reactions to the content as part of peer support exchange, not whether they felt another source would be able to engage in that exchange.
The responses are outlined in Table \Jordyn{add table with scenario, help-seeking message, responses, and response source}.

\textbf{(4) Questions about the pre-written responses}: 
To assess participants' preferences, we asked participants how much they liked each response on a 5-point Likert scale (1 = not at all, 5 = extremely). We also asked participants to select which response they like the most/least and why. To capture participants' positive and negative reactions to the responses, we asked participants to rate the extent to which they agreed with two positive statements ("I would send this response" and "This response contains helpful advice") and two negative statements ("This response is problematic" and  "This response is inappropriate"). We measured agreement with a 5-point Likert scale (1 = not at all, 5 = extremely).
% Question about how AI could possibly help in the situation was also given. 

\subsubsection{Prior experience with online peer support}
While prior experience with online peer support was not a requirement to participate in the study, we recognize that prior experience does shape human perception \Jordyn{rephrase and add reference}. To account for this, we asked "How often do you \textit{seek} support online (e.g., on social media)? 
% This includes, but is not limited to, posting a question on Reddit, direct messaging a friend for help, or asking for advice in a Facebook group. and give peer support online." 
and "How often do you \textit{give} support online (e.g., on social media)? This includes, but is not limited to, responding to a question on Reddit, direct messaging a friend who asked for help, or giving advice in a Facebook group." Answer choices were on a 5-point likert scale with standard frequency anchors\Jordyn{add reference to pew study and other papers that use same anchors} (1=never, 2=rarely, 3=sometimes, 4=often, 5=always).

\subsubsection{Demographics}
We also asked for our participants’ demographic information, including their age, gender, whether they identify as a member of the LGBTQ community, race, and education.

\subsection{Ethical Considerations}
This study was approved by the [anonymized] IRB as an exempt protocol, which meant participants were presented with the study information but not required to sign a consent document. The study information described the research objective, the procedures involved in completing the survey, the voluntary nature of the study, the potential risks involved, the anonymization process, and incentives. Only the research team members specified in the IRB protocol were granted access to the data, which was stored on a university-approved server.  

\subsection{Data Analysis}
\Jordyn{add text}
before comparing means, assessed whether variances were equal to determine which test was most appropriate for ANOVA
graphs - means with boxes to represent standard error - chose this visualization because it's easy to see significant differences (if the error bars don't overlap, the difference in means is significant)

==> old/results-v1.tex <==
VERSION 1:

\section{Results}
% \Jordyn{what do we think about referring to the sources as: AI (chatgpt), peer (young adult), adult (researcher), adult + clinically trained (therapist; or adult/clinical, or something to that effect...) }

\Jordyn{question for Afsaneh/Jina: tables are vertical because text is too small if they're horizontal - do you have any ideas for how to present the data in a way that looks good but doesn't take up too much space, or do you think the vertical tables could work for the two-column formatting CHI uses?}
\Jina{Right, except that I think you can reduce the white space and make it as compact as possible. You could also use the olympic example, just putting side by side, but not sure unless we try it out and see}

\Jordyn{RQs:
1. How do young adults engaging in peer support conversations feel about responses generated by (a) a young adult peer, (b) an adult researcher, (c) an adult mental health professional, and (d) Artifial Intelligence? % need to specify that they don't know the source?
2a. How do response preferences change depending on (1) the topic of conversation, and (2) the relatabilty of that topic?
- does relatability/ability to sympathize/ability to help impact preferences for different responses?
2b. What can young adults tell us about why those preferences vary?
- run n-gram (2-gram and 3-gram), use those top 3 grams for each open-ended question
- use open-ended questions to show why
3. How do individual differences (demographic factors and experience giving/seeking support) impact (1) preferences of responses or (2) relatability of scenarios?
}

We present our results in three sections. First, we present young adults' preferences for responses from different sources (a young adult, a researcher, a therapist, and ChatGPT) during peer support conversations (\ref{sec:results-1}). Second, we discuss how these preferences vary depending on the topic of conversation and its relatability (\ref{sec:results-2}. Lastly, we discuss how these preferences compare across scenarios. 
\Jina{these are worded in ways that we understand, but what does it mean to the readers? Why do they care? It can be reworded now that you have given the structure, speak more like when you are talking to someone in person. Like, 'We present young adults' preferences of what types of responses felt more appropriate than others'. We then discuss how these preferences might be moderated differently depending on the topic of the scenario.}

\Jina{I'm going to look over the results tonight. Sorry,}

\begin{comment}
    Ideas for:
RQ1: How do young adults feel about their ability to relate to, sympathize with, and help a friend who is initiating a peer support conversation?
RQ2a: Without knowing the content source, do young adults prefer a response generated by a human or AI? Do youth reveal anything about peer support exchange norms based on their preferences for responses written by AI or human sources?
RQ2b: without knowing the source of responses presented, do youth prefer content generated by (a) a peer, (b) an adult who is NOT a mental health professional ("researcher"), (c) a mental health professional (therapist), or (d) an AI chatbot (ChatGPT). Do preferences vary by demographic factors? 
\end{comment}

\subsection{Response preference by source}
We begin with overall preferences for responses by source during peer support exchange.
\label{sec:results-1}
\subsubsection{Overall response preference} To measure participant preferences between responses, we used their answers to the agreement Likert scale for the statement "I like this response" (see section \ref{sec:methods}). Bartlett's test tells us that the variance in response preference was significantly different based on which source the response came from (p < 0.001). A subsequent one-way Welch test with unequal variance reveals significant differences in participants' preference for a response based on which source it came from (F(3,5517.7) = 99.197, p-value < 0.001). As visualized in figure \ref{fig:plot-source-like}, participants' overall favorite response was created by a researcher (M = 3.51, SD = 0.02), followed by ChatGPT (M = 3.46, SD =  0.02), then a therapist (M = 3.29, SD = 0.02), and the young adult's response was their least favorite (M = 3.03, SD = 0.02).

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{source-like-figure_2023.8.22.png}
    \caption{Overall response preference by source.}
    \label{fig:plot-source-like}
\end{figure}

\subsubsection{Positive and negative attributes} In addition to preferences for responses from different sources, we also wanted to understand ways in which participants felt positively and negatively about responses from different sources. We explored these questions because it is possible for participants to "like" a response for paradoxical reasons, such as finding the content comically inappropriate \Jordyn{does that sentence/argument make sense?} - as we describe in the following paragraphs, this does not seem to be the case in our sample.

For positive attributes, we asked about the extent to which participants agreed (1) they would send a response, and (2) a response contained helpful information. Bartlett's test indicates that, based on the source a response came from, the variance was significantly different for both positive attributes (p < 0.001 in both cases). This information led us to conduct a one-way Welch test with unequal variance for both attributes, and the results of both were significant. This means the extent to which a participant agreed they would send a response (F(3,5513.9) = 91.085, p < 0.001) or felt a response was helpful (F(3,5519.6) = 104.37, p < 0.001)
did vary significantly by response source. These differences are visualized in Figure \ref{fig:plot-source-positive}.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{source-positive-figure_2023.8.22.png}
    \caption{Overall positive perceptions of responses by source.}
    \label{fig:plot-source-positive}
\end{figure}

For negative attributes, we asked about the extent to which participants found a response (1) problematic and (2) inappropriate. Bartlett's test indicates that, based on the source a response came from, the variance was significantly different for the extent to which participants found a response problematic (p < 0.001), but not for the extent to which they found a response inappropriate (p > 0.05). Using these findings, we conducted a one-way Welch test with equal variance for the extent to which a response was problematic, and unequal variance for the extent to which a response was inappropriate. For both tests, the results were significant, indicating that the extent to which a participant found a response problematic (F(3,1379) = 14.47, p < 0.001) or inappropriate (F(3,2484) = 12.113, p < 0.001) did vary significantly by response source. These differences are visualized in Figure \ref{fig:plot-source-negative}. \Jordyn{add note to methods that we asked about +/- responses to responses to make sure we got high quality data that makes sense}

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{source-negative-figure_2023.8.22.png}
    \caption{Overall negative perceptions of responses by source.}
    \label{fig:plot-source-negative}
\end{figure}

Taken together, these results (Figures \ref{fig:plot-source-like}, \ref{fig:plot-source-positive}, and \ref{fig:plot-source-negative}) show that negative perceptions of responses follow the opposite pattern that we see for overall preference and positive perceptions. This means that responses from sources that participants preferred more and perceived more positively were also perceived less negatively.

\subsection{Response preference by source within scenarios}
Next, we analyzed preferences by source within each individual scenario. We present these results in four sub-sections, each corresponding to a different scenario from our survey instrument (additional details are in section \ref{sec:methods}).
\label{sec:results-2}
\subsubsection{Scenario 1: relationships}
In the scenario about relationships, participants' reactions to the responses varied significantly depending on the source of the response (see Figure \ref{fig:plot-scenario-1}).
Bartlett's test indicates that, within the scenario about relationships, the variance is significantly different for the extent to which participants liked a response, found a response problematic, felt they would send a response, and found a response helpful (p < 0.001), but not for the extent to which they found a response inappropriate (p > 0.05). In the subsequent one-way Welch test, we used unequal variance for those attributes for which variance was significantly different according to Bartlett's test, and equal variance for those that were not significantly different. The results of the Welch test told us that preferences varied significantly depending on the source of the response. This finding applies to the extent to which they liked the response (F(3,1378) = 39.145, p < 0.001), the extent to which they felt the response is problematic (F(3,1379) = 14.47, p < 0.001), the extent to which they felt they would send the response (F(3,1375.6) = 43.235, p < 0.001), the extent to which they felt the response is inappropriate (F(3,2484) = 12.113, p < 0.001), and the extent to which they felt a response contains helpful advice (F(3,1379.9) = 12.011, p < 0.001). As presented in Table \ref{tab:scenario-1-responses}, the favorite response was ChatGPT (M = 3.63, SD = 1.00), followed by the researcher's response (M = 3.48, SD = 1.01), then the therapist's response (M = 3.29, SD = 1.09), and the young adult's response was participants' least favorite (M = 3.00, SD = 1.15).

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{scenario-1-figure_2023.8.22.png}
    \caption{Perceptions of responses by source for scenario 1 (Relationships).}
    \label{fig:plot-scenario-1}
\end{figure}


\begin{table}[hbt!]
\centering
\begin{tabular}{|ccc|}
\hline
\multicolumn{3}{|c|}{\textbf{I like this response}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{3.63} & 1.00 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{3.48} & 1.01 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{3.29} & 1.09 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{3.00} & 1.15 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response is problematic.}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{2.41} & 1.24 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{2.23} & 1.24 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{2.04} & 1.13 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{2.01} & 1.16 \\ \hline
\multicolumn{3}{|c|}{\textbf{I would send this response.}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{3.65} & 0.96 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{3.43} & 1.02 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{3.24} & 1.15 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{2.98} & 1.17 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response is inappropriate.}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{2.38} & 1.24 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{2.20} & 1.24 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{2.04} & 1.21 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{2.01} & 1.20 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response contains helpful advice.}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{3.63} & 0.95 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{3.47} & 0.99 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{3.27} & 1.07 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{3.07} & 1.13 \\ \hline
\end{tabular}
\caption{Perceptions of responses by source for scenario 1 (relationships), sorted by decreasing mean across attributes.}
\label{tab:scenario-1-responses}
\end{table}

% Agreement with statements about responses for scenario 1: relationships. Responses for scenario 1 by source, organized in descending order by mean for each statement. Answer choices were on a Likert scale from 1 to 5; 1 indicated no agreement with the given statement and 5 indicated extreme agreement with the given statement.

\subsubsection{Scenario 2: suicidal thoughts}
Perceptions of responses also varied significantly depending on the source of the responses for the scenario about suicidal thoughts (see Figure \ref{fig:plot-scenario-2}). 

Bartlett's test indicates that, within this scenario, the variance is significantly different for the extent to which participants liked a response, felt they would send a response, and found a response helpful (p < 0.001), but not for the extent to which they found a response problematic or inappropriate (p > 0.05) . In the subsequent one-way Welch test, we used unequal variance for those attributes for which variance was significantly different according to Bartlett's test, and equal variance for those that were not significantly different. The Welch test told us that preferences varied significantly depending on the source of the response. This finding applies to the extent to which young adults liked the response F(3,1375.3) = 64.075, p < 0.001), the extent to which they felt the response is problematic (F(3,2484) = 20.399, p < 0.001), the extent to which they felt they would send the response (F(3,1372.9) = 73.746, p < 0.001), the extent to which they felt the response is inappropriate (F(3,2484) = 23.458, p < 0.001), and the extent to which they felt a response contains helpful advice (F(3,1375.6) = 59.135, p < 0.001). Table \ref{tab:scenario-2-responses} presents participants' perceptions of the responses from each source in decreasing order by mean.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{scenario-2-figure_2023.8.22.png}
    \caption{Perceptions of responses by source for scenario 2 (Suicidal Thoughts).}
    \label{fig:plot-scenario-2}
\end{figure}

\begin{table}[hbt!]
\centering
\begin{tabular}{|ccc|}
\hline
\multicolumn{3}{|c|}{\textbf{I   like this response}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{3.59} & 0.95 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{3.22} & 1.08 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{2.99} & 1.12 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{2.82} & 1.19 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response is problematic.}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{2.53} & 1.26 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{2.42} & 1.27 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{2.18} & 1.24 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{2.04} & 1.18 \\ \hline
\multicolumn{3}{|c|}{\textbf{I would send this response.}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{3.56} & 0.94 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{3.19} & 1.12 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{2.94} & 1.20 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{2.71} & 1.21 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response is inappropriate.}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{2.54} & 1.27 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{2.42} & 1.30 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{2.17} & 1.22 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{2.00} & 1.20 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response contains helpful advice.}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{3.61} & 0.94 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{3.18} & 1.10 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{2.97} & 1.15 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{2.93} & 1.12 \\ \hline
\end{tabular}
\caption{Perceptions of responses by source for scenario 2 (suicidal thoughts), sorted by decreasing mean across attributes.}
\label{tab:scenario-2-responses}
\end{table}

\subsubsection{Scenario 3: self-expression}
Perceptions of responses also varied significantly depending on the source of the responses for the scenario about self-expression (see Figure \ref{fig:plot-scenario-3}). 

Bartlett's test indicates that, within this scenario, the variance is significantly different for the extent to which participants liked a response, felt they would send a response, and found a response helpful (p < 0.01), but not for the extent to which they found a response problematic or inappropriate (p > 0.05). In the subsequent one-way Welch test, we used unequal variance for those attributes for which variance was significantly different according to Bartlett's test, and equal variance for those that were not significantly different. The Welch test told us that preferences varied significantly depending on the source of the response. This finding applies to the extent to which young adults liked a response (F(3,1378.4) = 37.623, p < 0.001), the extent to which they felt a response is problematic (F(3,2484) = 4.8789, p < 0.01), the extent to which they felt they would send a response (F(3,1377.4) = 34.597, p < 0.001), the extent to which they felt a response is inappropriate (F(3,2484) = 5.5616, p < 0.001), and the extent to which they felt a response contains helpful advice (F(3,1378.4) = 39.531, p < 0.001). Table \ref{tab:scenario-3-responses} presents participants' perceptions of the responses from each source in decreasing order by mean.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{scenario-3-figure_2023.8.23.png}
    \caption{Perceptions of responses by source for scenario 3 (self-expression).}
    \label{fig:plot-scenario-3}
\end{figure}

\begin{table}[hbt!]
\centering
\begin{tabular}{|ccc|}
\hline
\multicolumn{3}{|c|}{\textbf{I like this response}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{3.70} & 0.98 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{3.51} & 0.94 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{3.46} & 0.97 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{3.08} & 1.09 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response is problematic.}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{2.25} & 1.19 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{2.10} & 1.16 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{2.05} & 1.15 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{2.01} & 1.22 \\ \hline
\multicolumn{3}{|c|}{\textbf{I would send this response.}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{3.67} & 1.00 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{3.48} & 0.97 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{3.42} & 1.05 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{3.05} & 1.15 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response is inappropriate.}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{2.26} & 1.23 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{2.09} & 1.19 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{2.08} & 1.18 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{1.99} & 1.18 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response contains helpful advice}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{3.75} & 0.94 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{3.51} & 0.99 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{3.49} & 0.98 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{3.12} & 1.09 \\ \hline
\end{tabular}
\caption{Perceptions of responses by source for scenario 3 (self-expression), sorted by decreasing mean across attributes.}
\label{tab:scenario-3-responses}
\end{table}

\subsubsection{Scenario 4: physical health}
Perceptions of responses also varied significantly depending on the source of the responses for the scenario about physical health (see Figure \ref{fig:plot-scenario-4}). 

Bartlett's test indicates that, within this scenario, the variance is significantly different for the extent to which participants liked a response, felt they would send a response, and found a response helpful (p < 0.01), but not for the extent to which they found a response problematic or inappropriate (p > 0.05). In the subsequent one-way Welch test, we used unequal variance for those attributes for which variance was significantly different according to Bartlett's test, and equal variance for those that were not significantly different. The Welch test told us that preferences varied significantly depending on the source of the response. This finding applies to the extent to which young adults liked a response (F(3,1376.3) = 71.062, p < 0.001), the extent to which they felt a response is problematic F(3,2484) = 20.761, p < 0.001), the extent to which they felt they would send a response (F(3,1375.8) = 63.915, p < 0.001), the extent to which they felt a response is inappropriate (F(3,2484) = 17.348, p < 0.001), and the extent to which they felt a response contains helpful advice (F(3,1376.1) = 77.939, p < 0.001). Table \ref{tab:scenario-4-responses} presents participants' perception of the responses from each source decreasing order by mean.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{scenario-4-figure_2023.8.23.png}
    \caption{Perceptions of responses by source for scenario 4 (physical health).}
    \label{fig:plot-scenario-4}
\end{figure}

% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[hbt!]
\centering
\begin{tabular}{|ccc|}
\hline
\multicolumn{3}{|c|}{\textbf{I like this response}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{3.71} & 0.96 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{3.48} & 0.99 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{3.43} & 0.97 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{2.83} & 1.19 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response is problematic.}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{2.46} & 1.28 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{2.10} & 1.22 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{2.06} & 1.18 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{1.95} & 1.16 \\ \hline
\multicolumn{3}{|c|}{\textbf{I would send this response.}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{3.64} & 0.99 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{3.44} & 0.99 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{3.38} & 1.01 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{2.78} & 1.23 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response is inappropriate.}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{2.40} & 1.27 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{2.06} & 1.15 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{2.02} & 1.16 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{1.95} & 1.21 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response contains helpful advice}} \\ \hline
\multicolumn{1}{|c|}{\textit{source}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{ChatGPT}}} & \multicolumn{1}{c|}{3.67} & 0.99 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Therapist}}} & \multicolumn{1}{c|}{3.45} & 0.99 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Researcher}}} & \multicolumn{1}{c|}{3.43} & 1.01 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Young Adult}}} & \multicolumn{1}{c|}{2.73} & 1.22 \\ \hline
\end{tabular}
\caption{Perceptions of responses by source for scenario 4 (physical health), sorted by decreasing mean across attributes.}
\label{tab:scenario-4-responses}
\end{table}

\subsection{Response preference by source across topics}
\label{sec:results-3}
Lastly, we break down preferences for responses across scenarios and compare preferred responses from each source. We present these results in four sub-sections, each corresponding to a different source for the responses used in our survey instrument (additional details are in section \ref{sec:methods}).

\subsubsection{Researcher}
Young adults found the researcher's responses significantly more helpful for some scenarios than others, and results were trending for the likelihood that young adults would send the researcher's responses, but the other attributes were not significantly different across scenarios (see Figure \ref{fig:plot-researcher}). 

Bartlett's test indicates that, for the researcher's responses, variance is not significantly different for any of the attributes (p > 0.05). This meant we used unequal variance for the subsequent one-way Welch tests, which showed that preferences varied significantly for the researchers' response across scenarios for the extent to which young adults found the researcher's responses helpful (F(3,2484) = 3.7713, p = 0.01), but not for the likelihood that young adults would send the researcher's responses (F(3,2484) = 2.2745, p > 0.05), the extent to which participants liked the researcher's responses (F(3,2484) = 1.1.9513, p > 0.05), or the extent to which they found the researcher's responses problematic (F(3,2484) = 0.46222, p > 0.05) or inappropriate (F(3,2484) = 0.5596, p > 0.05). Table \ref{tab:researcher-responses} presents participants' perceptions of the researcher's responses for each scenario in decreasing order by mean.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{researcher-figure_21023.8.23.png}
    \caption{Perceptions of researcher's responses by attribute for all scenarios.}
    \label{fig:plot-researcher}
\end{figure}

\begin{table}[hbt!]
\centering
\begin{tabular}{|ccc|}
\hline
\multicolumn{3}{|c|}{\textbf{I like this response}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{3.59} & 0.95 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{3.51} & 0.94 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{3.48} & 1.01 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{3.48} & 0.99 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response is problematic.}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{2.10} & 1.16 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{2.10} & 1.22 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{2.04} & 1.13 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{2.04} & 1.18 \\ \hline
\multicolumn{3}{|c|}{\textbf{I would send this response.}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{3.56} & 0.94 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{3.48} & 0.97 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{3.44} & 0.99 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{3.43} & 1.02 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response is inappropriate.}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{2.08} & 1.18 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{2.06} & 1.15 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{2.04} & 1.21 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{2.00} & 1.20 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response contains helpful advice}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{3.61} & 0.94 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{3.51} & 0.99 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{3.47} & 0.99 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{3.43} & 1.01 \\ \hline
\end{tabular}
\caption{Perceptions of the researcher responses by attribute for all scenarios, sorted by decreasing mean across attributes.}
\label{tab:researcher-responses}
\end{table}

\subsubsection{Young adult}
Perceptions of the young adult's responses were significantly different for all attributes across the four scenarios (see Figure \ref{fig:plot-young-adult}). 

Bartlett's test indicates that, for the young adult's responses, variance is significantly different for the extent to which participants liked the young adult's responses and found them helpful (p < 0.05), but not for the extent to which they found the young adult's responses problematic, helpful, or inappropriate (p > 0.05). This information meant we used unequal variance for the attributes with significant differences and equal variance for those without significant differences in the subsequent one-way Welch test. The Welch test indicated that preferences varied significantly for the young adult's responses across scenarios for all attributes, including the extent to which participants liked the young adult's responses (F(3,1379.1) = 13.219, p < 0.001), the extent to which they found the young adult's responses problematic (F(3,2484) = 7.1727, p < 0.001), the degree to which they felt they would send the young adult's responses (F(3,2484) = 13.063, p < 0.001), the extent to which they found the young adult's responses inappropriate (F(3,2484) = 4.605, p < 0.05), and the extent to which they found the young adult's responses helpful (F(3,1378.9) = 17.852, p < 0.001). Table \ref{tab:young-adult} presents participants' perception of the young adult's responses for each scenario in decreasing order by mean.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{young-adult-figure_2023.8.23.png}
    \caption{Perceptions of young adult's responses by attribute for all scenarios.}
    \label{fig:plot-young-adult}
\end{figure}


\begin{table}[hbt!]
\centering
\begin{tabular}{|ccc|}
\hline
\multicolumn{3}{|c|}{\textbf{I   like this response}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{3.22} & 1.08 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{3.08} & 1.09 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{3.00} & 1.15 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{2.83} & 1.19 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response is problematic.}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{2.46} & 1.28 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{2.41} & 1.24 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{2.25} & 1.19 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{2.18} & 1.24 \\ \hline
\multicolumn{3}{|c|}{\textbf{I would send this response.}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{3.19} & 1.12 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{3.05} & 1.15 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{2.98} & 1.17 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{2.78} & 1.23 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response is inappropriate.}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{2.40} & 1.27 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{2.38} & 1.24 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{2.26} & 1.23 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{2.17} & 1.22 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response contains helpful advice}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{3.18} & 1.10 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{3.12} & 1.09 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{3.07} & 1.13 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{2.73} & 1.22 \\ \hline
\end{tabular}
\caption{Perceptions of the young adult's responses by attribute for all scenarios, sorted by decreasing mean across attributes.}
\label{tab:young-adult-responses}
\end{table}

\subsubsection{ChatGPT}
Perceptions of ChatGPT's responses were significant for all attributes across scenarios (see Figure \ref{fig:plot-chatgpt}). 

Bartlett's test indicates that variance is significantly different for the extent to which young adults liked ChatGPT's responses, felt they would send ChatGPT's responses, and found ChatGPT's responses helpful (p < 0.001), but not for the extent to which they found ChatGPT's responses problematic or inappropriate (p > 0.05). This information meant we used unequal variance for the attributes with significant differences and equal variance for those without significant differences in the subsequent one-way Welch test. The Welch test indicated that preferences varied significantly for the young adult's responses across scenarios for all attributes, including the extent to which young adults liked ChatGPT's responses (F(3,1376.2) = 89.166, p < 0.001), the extent to which they found ChatGPT's responses problematic (F(3,2484) = 31.697, p < 0.001), the degree to which they felt they would send ChatGPT's responses (F(3,1375.7) = 103.49, p < 0.001), the extent to which they found ChatGPT's responses inappropriate (F(3,2484) = 32.754, p < 0.001), and the extent to which they found ChatGPT's responses helpful (F(3,1377.4) = 75.515, p < 0.001). Table \ref{tab:chatgpt} presents participants' perception of ChatGPT's responses for each scenario in decreasing order by mean.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{chatgpt-figure_2023.8.23.png}
    \caption{Perceptions of ChatGPT's responses by attribute for all scenarios.}
    \label{fig:plot-chatgpt}
\end{figure}


\begin{table}[hbt!]
\centering
\begin{tabular}{|ccc|}
\hline
\multicolumn{3}{|c|}{\textbf{I like this response}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{3.71} & 0.96 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{3.70} & 0.98 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{3.63} & 1.00 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{2.82} & 1.19 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response is problematic.}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{2.53} & 1.26 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{2.01} & 1.16 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{2.01} & 1.22 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{1.95} & 1.16 \\ \hline
\multicolumn{3}{|c|}{\textbf{I would send this response.}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{3.67} & 1.00 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{3.65} & 0.96 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{3.64} & 0.99 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{2.71} & 1.21 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response is inappropriate.}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{2.54} & 1.27 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{2.01} & 1.20 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{1.99} & 1.18 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{1.95} & 1.21 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response contains helpful advice.}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{3.75} & 0.94 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{3.67} & 0.99 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{3.63} & 0.95 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{2.93} & 1.12 \\ \hline
\end{tabular}
\caption{Perceptions of ChatGPT's responses by attribute for all scenarios, sorted by decreasing mean across attributes.}
\label{tab:chatgpt-responses}
\end{table}

\subsubsection{Therapist}
Finally, perceptions of the therapist's responses were significant for all attributes across scenarios (see Figure \ref{fig:plot-therapist}). 

Bartlett's test indicates that variance is significantly different for the extent to which young adults liked the therapist's responses, felt they would send the therapist's responses, and found the therapist's responses inappropriate or helpful (p < 0.001), but not for the extent to which they found the therapist's responses problematic (p > 0.05). This information meant we used unequal variance for the attributes with significant differences and equal variance for those without significant differences in the subsequent one-way Welch test. The Welch test indicated that preferences varied significantly for the therapist's responses across scenarios for all attributes, including the extent to which young adults liked the therapist's responses F(3,1377.5) = 24.864, p < 0.001), the extent to which they found the therapist's responses problematic (F(3,2484) = 12.679, p < 0.001), the degree to which they felt they would send the therapist's responses (F(3,1377) = 22.659, p < 0.001), the extent to which they found the therapist's responses inappropriate (F(3,1378.9) = 12.414, p < 0.001), and the extent to which they found the therapist's responses helpful (F(3,1377.5) = 29.817, p < 0.001). Table \ref{tab:therapist-responses} presents participants' perception of the therapist's responses for each scenario in decreasing order by mean.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{therapist-figure_2023.8.23.png}
    \caption{Perceptions of the therapist's responses by attribute for all scenarios.}
    \label{fig:plot-therapist}
\end{figure}

\begin{table}[hbt!]
\centering
\begin{tabular}{|ccc|}
\hline
\multicolumn{3}{|c|}{\textbf{I like this response.}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{3.46} & 0.97 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{3.43} & 0.97 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{3.29} & 1.09 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{2.99} & 1.12 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response is problematic.}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{2.42} & 1.27 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{2.23} & 1.24 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{2.06} & 1.18 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{2.05} & 1.15 \\ \hline
\multicolumn{3}{|c|}{\textbf{I would send this response.}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{3.42} & 1.05 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{3.38} & 1.01 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{3.24} & 1.15 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{2.94} & 1.20 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response is inappropriate.}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{2.42} & 1.30 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{2.20} & 1.24 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{2.09} & 1.19 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{2.02} & 1.16 \\ \hline
\multicolumn{3}{|c|}{\textbf{This response contains helpful advice.}} \\ \hline
\multicolumn{1}{|c|}{\textit{scenario}} & \multicolumn{1}{c|}{\textit{mean}} & \textit{sd} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{3}}} & \multicolumn{1}{c|}{3.49} & 0.98 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{4}}} & \multicolumn{1}{c|}{3.45} & 0.99 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{1}}} & \multicolumn{1}{c|}{3.27} & 1.07 \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{2}}} & \multicolumn{1}{c|}{2.97} & 1.15 \\ \hline
\end{tabular}
\caption{Perceptions of the therapist's responses by attribute for all scenarios, sorted by decreasing mean across attributes.}
\label{tab:therapist-responses}
\end{table}

==> old/results-v2_TOCHI_.tex <==
\section{Results}
In this section, we first describe the participant demographics, followed by young adults' reactions \Jina{need to be specific} to topics of conversations that frequently come up during peer support (RQ1). Next, we discuss young adults' reactions to responses from different sources (young adult, researcher, therapist, and ChatGPT) in response to help-seeking messages (RQ2a). \Jina{there are two different ways that the paper refers to the help-seeking messages: help-seeking messages and topics of conversation. Are they two different things?}
Then, we discuss how these preferences vary depending on previous experiences with online peer support (RQ2b), the topic of conversation (RQ2c) and the \Jina{participants'?} relatability of that topic (RQ2d). Lastly, we describe how young adults explained their preferences for certain responses over others (RQ3).

\subsection{Participant Demographics}
Of the 622 responses, the gender identity consisted of (67.05\%) identifying as male and (32.50\%) as female, with an average age of 21, the majority falling within the 18-24 age group (80.94\%). The majority identified as African American (30.05\%) and Caucasian (48.31\%). Educational attainment exhibited a range of levels, with (49.09\% ) having completed a bachelor's degree and (6.70\%) holding a master's degree. \Jina{Why are there parentheses?}
\Jordyn{check numbers and add table about participant demographics}

\subsection{RQ1: How do young adults feel about the topics that frequently come up in online peer support conversations?} \Jina{RQ1: How do young adults feel about the frequent topics in online peer support conversations? - The shorter the sentences / RQs the better for easier read. Think of adding extra word as paying extra dollar}
\Afsaneh{How much participants felt they could help in, relate to, and sympathize with the help seeking messages?}

Young adults felt the most sympathy for the scenario \Jina{Here's another term used in the paper aside from "topic" when it is referring to the same thing} about physical health, and thought it was the most relatable; however, young adults \Jina{We go back and forth between young adults and participants. need to be consistent. Otherwise it sounds like we have two different populations} felt \Jina{findings need to be past tense} they can help most when a peer is experiencing suicidal thoughts. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/plot.scenario.attributes_2023.8.28.png}
    \caption{How much young adults felt they could help in, relate to, and sympathize with the scenarios presented.} \Jina{How are these boxes so neatly all having the same vertical length? They all had same variance?}
    \label{fig:plot-scenario-attributes}
\end{figure}

\Jordyn{add text and RQ about reactions to scenarios (relabatility/sympathy/help)}
\Jina{Need to clearly establish in the methods what help, relate, sympathize mean and conclusions they can bring}
\subsection{RQ2a: What is young adults' preference about the different response origins to help-seeking messages and why?}
Young adults preferred the responses created by the researcher, and the young adult's response was their least favorite. The second favorite responses were generated by ChatGPT (M = 3.46, SD =  0.02), followed by the therapist's responses (M = 3.29, SD = 0.02), and the young adult's responses were their least favorite on average (M = 3.03, SD = 0.02). See Figure \ref{fig:plot-source-like}.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/plot.source.like_2023.8.25.png}
    \caption{RQ1a: How much young adults liked responses by source}
    \label{fig:plot-source-like}
\end{figure}
\Jordyn{figure out how to re-order facet panels for all figures - currently alphabetical}

\subsection{RQ2b: How positively (helpful, would send) and negatively (inappropriate, problematic) do young adults feel about the different responses to help-seeking messages?}
We also looked at how positively and negatively young adults felt about the responses from different sources. Overall, the responses from sources that participants preferred more and viewed more positively were also perceived less negatively. This is important because it is possible for participants to "like" a response for paradoxical reasons, such as finding the content comically inappropriate, this does not seem to be the case in our sample (see Figure \ref{fig:cor-matrix-attributes} \Jordyn{add scale to figure (darker red means closer to -1, darker blue means closer to 1, white means 0, insignificant values are crossed out (p > 0.05)}).

Positive attributes - how much they felt they \textit{would send} a response and how \textit{helpful} they thought a response was - followed the same pattern as their favorite responses. This means young adults felt the \textbf{\textit{researcher's responses were the most helpful}} (M=3.50, SD=0.99) of the responses presented and also indicated that \textbf{\textit{young adults were most likely to send the researcher's responses}} (M=3.48, SD=0.98), followed by ChatGPT's responses (how helpful: M=3.49, SD=1.05; likelihood to send: M=3.42, SD=1.12), then the therapist's responses (how helpful: M=3.29, SD=1.07; likelihood to send: M=3.25, SD=1.12), and the young adult's responses received the lowest score for positive attributes (how helpful: M=3.02, SD=1.15; likelihood to send: M=3.00, SD=1.18). See Figure \ref{fig:plot-source-pos}. The negative attributes - how \textit{problematic} and \textit{inappropriate} young adults felt the responses were - followed the exact opposite pattern as the positive attributes. The young adult's responses were, on average, the ones young adults felt were most problematic (M=2.32, SD=1.24) and inappropriate (M=2.30, SD = 1.24), followed by the therapist's responses (how problematic: M=2.19, SD=1.22; how inappropriate: M=2.18, SD=1.23). 

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/plot.source.pos_2023.8.25.png}
    \caption{RQ1b: How positive young adults felt about the responses by source}
    \label{fig:plot-source-pos}
\end{figure}

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/plot.source.neg_2023.8.25.png}
    \caption{RQ1c: How negative young adults felt about the responses by source}
    \label{fig:plot-source-neg}
\end{figure}

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.45]{figures/cor.matrix_2023.8.26.jpg}
    \caption{Correlation between ratings for positive and negative attributes of responses by source}
    \label{fig:cor-matrix-attributes}
\end{figure}

\subsection{RQ2e: How do young adults’ reactions to those responses vary depending on their previous experience giving and receiving peer support online?}
Our participants reported a decent amount of experience with online peer support. 79\% (490/622) of the young adults in our sample said they seek online peer support at least "sometimes" (M=3.20, SD=0.96), and 75\% (469/622) give online peer support at least "sometimes" (M=3.19, SD=0.97). Also, those who have more experience seeking peer support were also more likely to have experience giving peer support (r(620) = 0.51, p < 0.001), although the differences between the two were not significant (meaning they were not more likely to seek online peer support than give it, or vice versa). 

\textbf{\textit{Young adults who have more experience giving support online were more likely to find ChatGPT's responses more inappropriate}} (r(621) = 0.04, p < 0.05). Interestingly, this was the only significant correlation between experiences giving/receiving support and any of the attributes we asked about, positive or negative, for the responses from each source.

\Jordyn{figure out what other analyses to do for this question}


\subsection{RQ2c: How do young adults’ preferences for those responses vary depending on the topics for which young adults seek support?}
\textbf{\textit{Our results show that young adults prefer the response from ChatGPT for all but one of the topics (suicidal thoughts).}} In the following four sub-sections, we present young adults' preferences for responses to help-seeking messages about (1) relationships, (2) suicidal thoughts, (3) self-expression, and (4) physical health.

\subsubsection{(1) Relationships}
\label{sec:relationships}
In the scenario about relationships, participants' reactions to the responses varied significantly depending on the source of the response. When the help-seeking message is about relationships, young adults prefer the response generated by ChatGPT. Our results show that not only did young adults like ChatGPT's response the best for the scenario about relationships, but they also felt the most positive (how helpful: M=3.63, SD=1.00; likelihood to send: M=3.65, SD=0.96) and least negative (how problematic: M=2.01, SD=1.16; how inappropriate: M=2.01, SD=1.20). \textbf{\textit{When discussing relationship issues, young adults did not like the response from another young adult.}} They liked the young adult's response the least (M=3.00, SD=1.15), and felt it was the most negative (how problematic: M=2.41, SD=1.24; how inappropriate: M=2.38, SD=1.24) and least positive (how helpful: M=3.07, SD=1.13; likelihood to send: M=2.98, SD=1.17). 
See Figure \ref{fig:plot-scenario-1}. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/scenario-1-figure_2023.8.26.png}
    \caption{RQ2b(1): Perceptions of responses by source for help-seeking message about relationships.}
    \label{fig:plot-scenario-1}
\end{figure}

\subsubsection{(2) Suicidal thoughts}
\label{sec:suicidal-thoughts}
In response to help-seeking messages about suicidal thoughts, young adults preferred the response from the researcher and reacted very negatively to ChatGPT's response. Among the responses presented, young adults liked the researcher's response the most (M=3.59, SD=0.95), and felt the most positively (how helpful: M=3.61, SD=0.94; likelihood to send: M=3.56, SD=0.94) and least negatively about it (how problematic: M=2.04, SD=1.18; how inappropriate: M=2.00,	SD=1.20). At the same time, young adults liked ChatGPT's response the least (M=2.82, SD=1.19) and felt the most negative (how problematic: M=2.53, SD=1.26; how inappropriate: M=2.54, SD=1.27) and least positive about it (how helpful: M=2.93, SD=1.12; likelihood to send: M=2.71,	SD=1.21).
See Figure \ref{fig:plot-scenario-2}. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/scenario-2-figure_2023.8.26.png}
    \caption{RQ2b(2): Perceptions of responses by source for help-seeking message about suicidal thoughts.}
    \label{fig:plot-scenario-2}
\end{figure}

\subsubsection{(3) Self-expression}
\label{sec:self-expression}
Young adults' reactions to the responses about self-expression followed a similar pattern to the responses about relationships. We saw that young adults preferred the response generated by ChatGPT for the help-seeking message about self-expression, and reacted most negatively to the response from another young adult. We found that young adults liked ChatGPT's response the most (M=3.70, SD=0.98), felt the most positively about ChatGPT's response (how helpful: M=3.75, SD=0.94; likelihood to send: M=3.67, SD=1.00) and felt the least negatively about ChatGPT's response (how problematic: M=2.01, SD=1.22; how inappropriate: M=1.99, SD=1.18). Young adults also felt the most negatively, and least positively, about the response created by another young adult (how problematic: M=2.25, SD=1.19; how inappropriate: M=2.26, SD=1.23; how helpful: M=3.12, SD=1.09; likelihood to send: M=3.05, SD=1.15).
See Figure \ref{fig:plot-scenario-3}.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/scenario-3-figure_2023.8.26.png}
    \caption{RQ2b(3): Perceptions of responses by source for help-seeking message about self-expression.}
    \label{fig:plot-scenario-3}
\end{figure}

\subsubsection{(4) Physical health}
\label{sec:physical-health}
When the help-seeking message is about physical health, young adults once again prefer ChatGPT's response and do not like the young adult's response. The results show that young adults like ChatGPT's response the most (M=3.71, SD=0.96), felt the most positively about it (how helpful: M=3.67, SD=0.99; likelihood to send: M=3.64, SD=0.99), and the least negatively (how problematic: M=1.95, SD=1.16; how inappropriate: M=1.95, SD=1.21). Young adults also felt the most negatively, and least positively, about the response created by another young adult (how problematic: M=2.46, SD=1.28; how inappropriate: M=2.40, SD=1.27; how helpful: M=2.73, SD=1.22; likelihood to send: M=2.78, SD=1.23).
See Figure \ref{fig:plot-scenario-4}.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/scenario-4-figure_2023.8.26.png}
    \caption{RQ2b(4): Perceptions of responses by source for help-seeking message about physical health.}
    \label{fig:plot-scenario-4}
\end{figure}

\subsection{RQ2d: How do young adults’ preferences for those responses vary depending on the relatability of the topics for which young adults seek support?}
\Jordyn{maybe "how connected they felt to the topic" instead of "relatability of the topic"? or "how they felt about the topic itself independent of the response"?}
\Jordyn{add text to describe findings in correlation matrix}

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/RQ2c_2023.8.26.jpg}
    \caption{RQ2c: Correlations between young adults' response preferences and topic relatability.}
    \label{fig:cor-matrix-rq2c}
\end{figure}


\subsection{RQ3: What can young adults tell us about their preferences for certain responses during online peer support conversations?}
\Jordyn{n-gram, analyses pending from Kaylie}


==> old/results-v3.tex <==
\section{Results}
%  \Jordyn{maybe change "response" to "help-giving reply" or even just "reply" throughout results?...}
We first describe preferences for and reactions to different support-giving responses (peer, adult mentor, therapist, and AI). Then, we discuss how these preferences and reactions vary depending on the topic of the help-seeking message they are responding to.

% Results are organized into two sections: perceptions of help-seeking messages and preferences for responses to help-seeking messages. We use the same structure for both sections; first, we look at which messages evoked the strongest reactions and which responses are most preferred, respectively, then we examine demographic predictors of reactions to help-seeking messages and preferences for responses, respectively.

\subsection{RQ1: How do young people react to human- and AI-generated help-giving responses?}
We found that, before considering the topic of a help-seeking message, the human-generated adult-mentor response performed best overall. 

We begin by comparing the average responses from the four sources (peer, adult mentor, therapist, and AI) without separating them by topic. To do this, we looked at how much participants liked ("like") each source's responses in aggregate for all help-seeking messages. See Figure \ref{fig:plot-source-like}. These means were significantly different (\textit{F}(3.0,5517.7) = 99.20, p < 0.001), with the adult mentor responses being participants' favorite (M=3.51, SD=0.02), followed by AI (M=3.46, SD=0.02), then the therapist (M=3.29, SD=0.02), and the peer responses were their least favorite (M=3.03, SD=0.02). This means that \textbf{\textit{before considering the topic of the help-seeking message, it seemed like humans outperformed AI.}}

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale = 1]{figures/plot.source.like_2023.9.11.png}
    \caption{Preferences for responses from four sources aggregated across help-seeking topics, in descending order of average preference. The Y-axis is an averaged measure of preference from 1 (liked least/lowest preference) to 5 (liked most/highest preference).}
    \label{fig:plot-source-like}
\end{figure}

Next, we wanted to understand how participants reacted to the different responses beyond which one they "liked" the most (i.e., preferred). To do this, we looked at aggregate responses for all help-seeking messages by source to understand how helpful the responses were ("helpful"), how likely they were to send them ("would send"), and how inappropriate ("inappropriate") and problematic ("problematic") they felt the responses were. In subsequent sections and figures, we refer to these four measures as "attributes" of participants' responses.

We first looked at the correlations between the positive and negative attributes we asked about to determine whether participants "like" responses for paradoxical reasons, such as finding the content comically inappropriate - fortunately, this was not the case in our data. To do this, we used means across the two positive attributes (how helpful participants felt the responses were and how likely they were to send them) and two negative attributes (how inappropriate and problematic participants felt a response was) to get an overall idea of how positive and negative their reaction was, respectively. Overall, the responses from sources that participants preferred more and viewed more positively were also perceived less negatively (see Appendix \ref{cor-matrix}). This is also a good measure of data quality in our study because it signals that a positive reaction means participants find value in the help-giving response. Participants also tended to feel more positively than negatively about all the responses, meaning they rated higher on the Likert scales when asked about positive attributes than negative attributes, which means we avoided doing more harm than good, which is important for ethical research.

Next, we break down reactions to the different responses (peer, adult mentor, therapist, and AI) by comparing the different attributes we asked about (how helpful the response was, how likely participants were to send the response, how problematic the response was, and how inappropriate the response was). Positive attributes - how much they felt they would send a response and how helpful they thought it was - followed the same pattern as participants' favorite responses (most "liked"). This means participants felt the adult mentor's responses were the most helpful (M=3.50, SD=0.99) of the responses presented and also indicated that participants were most likely to send the adult mentor's responses (M=3.48, SD=0.98), followed by AI's responses (how helpful: M=3.49, SD=1.05; likelihood to send: M=3.42, SD=1.12), then the therapist's responses (how helpful: M=3.29, SD=1.07; likelihood to send: M=3.25, SD=1.12), and the peer's responses received the lowest score for positive attributes (how helpful: M=3.02, SD=1.15; likelihood to send: M=3.00, SD=1.18). The negative attributes - how problematic and inappropriate participants felt the responses were - followed the exact opposite pattern as the positive attributes. On average, \textbf{\textit{the peer responses were the most problematic and inappropriate}} (how problematic: M=2.32, SD=1.24; how inappropriate: M=2.30, SD = 1.24), followed by the therapist's responses (how problematic: M=2.19, SD=1.22; how inappropriate: M=2.18, SD=1.23), AI's responses (how problematic: M=2.13, SD=0.02; how inappropriate: M=2.12, SD=0.02), and the adult mentor's responses were seen as the least problematic (M=2.07, SD = 0.02) and inappropriate (M=2.05, SD = 0.02). See Figure \ref{fig:source-reactions}. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/plot.source.reactions_2023.9.11.png}
    \caption{Participant reactions to responses by source. The x-axis is how much participants agreed with the different attributes of their reaction (helpful, inappropriate, problematic, and would send).}
    \label{fig:source-reactions}
\end{figure}

Our findings from RQ1 suggest that participants may prefer a human response to help-seeking messages - however, these findings do not account for the nuance in real-life peer support exchanges. To address this, we present analyses for RQ2 to understand how reactions to human- and AI-generated responses vary depending on what they are responding to.

\subsection{RQ2: How do young people react to help-giving responses about (a) relationships, (b) suicidal thoughts, (c) self-expression, and (d) physical health?}
\textbf{\textit{Our results show that participants preferred AI-generated responses to help-seeking messages about relationships, self-expression, and physical health, but not suicidal thoughts.}} In the next four sections, we describe this finding in more detail and break down those preferences by the topic of the help-seeking messages: relationships ( section \ref{sec:relationships}), suicidal thoughts (section \ref{sec:suicidal-thoughts}), self-expression (section \ref{sec:self-expression}), and physical health (section \ref{sec:physical-health}). For each topic, we begin by with the quantitative results for each attribute of the responses, followed by quotes from open-ended responses from the participants to illustrate why they did, or did not, like each response. Results from the open-ended responses are described from most to least preferred response within each scenario.

\subsubsection{Relationships}
\label{sec:relationships}
Participants' reactions to responses about relationships did vary significantly by source, and they preferred the response generated by AI. Our results show that not only did \textbf{\textit{participants like the AI response the most}}, but they also felt it was the most helpful (M=3.63, SD=1.00), least problematic (M=2.01, SD=1.16), least inappropriate (M=2.01, SD=1.20), and that they were most likely to send it (M=3.65, SD=0.96).

\textbf{\textit{When discussing relationship issues, participants did not like the peer response.}} They liked the peer's response the least (M=3.00, SD=1.15) and felt it was the most negative (how problematic: M=2.41, SD=1.24; how inappropriate: M=2.38, SD=1.24) and least positive (how helpful: M=3.07, SD=1.13; likelihood to send: M=2.98, SD=1.17). 
See Figure \ref{fig:plot-scenario-1}. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.75]{figures/plot.relationships_2023.9.11.png}
    \caption{Reactions to responses by source for help-seeking message about relationships.}
    \label{fig:plot-relationships}
\end{figure}

\Jordyn{add participant ID\#, gender, and ethnicity for all quotes!}

This sentiment was reflected in the free-response questions, where participants noted that they liked the balance and empathy in the AI-generated responses but wanted more acknowledgment of the others' perspectives (which this AI did not have the context for, as the "ex" was not involved in the conversation). Participants noted that they liked how the AI response both offered support and presented actionable solutions: \textit{“This particular response says it all, it's absolutely what I'd say. What I like the most is that it tells [the friend] how to deal with the situation and still encourages [them].”} The response was \textit{"helpful...
%The response has facts that are hard to hear but they are helpful. The message is 
[and] also supportive and feels like a safe space."}
    %it also has ways of how to cope with the situation.
Some participants even said the AI-generated response seemed like it came from someone who is a good friend: \textit{“They are really trying to help the friend so much and we all need such friends."} There were also mentions of qualities participants associated with the AI response, including that they thought it was "[empathetic]...supportive and caring." Even though participants did favor the AI-generated response to the help-seeking message about relationships, they did note some room for improvement. Namely, that the response doesn't consider the entire context of the situation and "accuses the ex without listening to his side of the story."

Participants noted that the human-generated responses from the adult mentor also provided acknowledgment and validation, but it was potentially less useful and lacked clear solutions. Those who liked this response noted that \textit{“it is respectful and...made [them] feel like the person understood [the help-seeker's] feelings"}. Participants also noted a sense of maturity in how the response did not judge the help-seeker: “...the [response] answered the question in a mature way by making the victim not feel offended by going back to the ex. The response is just showing him or her that is what we [humans] go through in terms of love life.” Despite these positive attributes of the adult mentor's response, some participants felt it was \textit{"just about beating around the bush"} and that \textit{"it didn't provide a way of how to solve the situation clearly."}

Participants liked the therapist's response because they felt it was extremely understanding and non-judgmental but noted that it seemed to delay giving actionable advice. Even though they did not know a therapist wrote one of the responses, they picked up on the professional tone: \textit{"This person provides professional remedy and ... [asks] the victim to share their mixed emotions and from there she/he will be in a position to offer strategies.”} They saw the response as "very empathetic without shaming the friend," but noted that it felt like " scheduling [giving] help to next time when the [help-seeker] is in need of it now.” They appreciated the supportive tone but would have liked more concrete and immediate advice rather than beating around the bush and delaying support.

We received the most negative comments about the peer's response because participants felt it was terse, suggested hasty actions, and was not encouraging. While some appreciated the response's brevity, the way it was written came across as \textit{"too direct with no empathy.”} This lack of empathy made participants feel like the sender had a bad attitude and was being too tough on the help-seeker: \textit{"It sounds harsh and rude, and also it doesn't consider the feelings of the victim."}

\subsubsection{Suicidal thoughts}
\label{sec:suicidal-thoughts}
In response to help-seeking messages about suicidal thoughts, participants preferred the response from the adult mentor and reacted most negatively to AI's response. Among the responses presented, participants liked the adult mentor's response the most (M=3.59, SD=0.95) and felt the most positively (how helpful: M=3.61, SD=0.94; likelihood to send: M=3.56, SD=0.94) and least negatively about it (how problematic: M=2.04, SD=1.18; how inappropriate: M=2.00,	SD=1.20). They also liked AI's response the least (M=2.82, SD=1.19) and felt the most negative (how problematic: M=2.53, SD=1.26; how inappropriate: M=2.54, SD=1.27) and least positive about it (how helpful: M=2.93, SD=1.12; likelihood to send: M=2.71,	SD=1.21).
See Figure \ref{fig:plot-suicidal-thoughts}. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.75]{figures/plot.suicidal.thoughts_2023.9.11.png}
    \caption{Reactions to responses by source for help-seeking message about suicidal thoughts.}
    \label{fig:plot-suicidal-thoughts}
\end{figure}

When describing why they preferred the adult mentor's response to this sensitive topic, participants noted that they liked how it conveyed genuine concern by inviting the help-seeker to share more details and put effort over providing more support. \textit{"There’s a feeling of relating with the individual here. There’s a feeling of care and [that they're] really interested and [want] to understand the individual }
% plus boosting the individual’s confidence and also wanting to understand the individual’s 
\textit{[and their] situation."}
% It’s the best to do in such situation, for someone who wants to really be there for such person.” 
The only area of improvement that participants mentioned for the adult mentor response is that the message could have been a little shorter, but did not note what content should be cut. The second most preferred response came from a peer, and participants felt it was \textit{"very shallow"}, inconsiderate, and would leave the help-seeker feeling unseen. Interestingly, they likened this type of message to a computer-generated response, saying it sounded \textit{"...typical of a bot"}. Unlike the adult mentor's response, participants did not like how the peer's response was \textit{"so shallow [and] does not give the victim...much [detail] on how to tackle the situation and [get] helped."} Participants noted that the therapist's response immediately asked for more information in an attempt to ensure the help-seeker's safety - not knowing that this message was written by a clinician, some thought this sounded \textit{"professional"} while many others took it as intrusively asking for more information right away instead of offering support. \textit{“I think this response makes the person in need sink deeper into her trouble rather than pull her out. It's a bit inappropriate.”} Since the initial help-seeking message did not use the word "suicide," many participants also did not like that the therapist's response immediately drew that conclusion and felt that calling it out could com across as judgemental: \textit{“I hate the assumption about self harm and suicide. It feels really I'm going to insert myself into your life to fix it and doesn't feel friendly at all.”} The AI-generated response overall performed the worst. While some felt the response was \textit{"genuine"} and \textit{"actually truthful about the person's ability,"} most saw the referral to a healthcare provider as a lack of desire to help. \textit{“Fine, you can’t provide help but that’s not the best way to put it. You could always have the right choice of words and making the right sentence in this situation before suggesting a mental health professional and not everybody will like the fact that they are referring to them as going crazy. Not really cool though.”}

\subsubsection{Self-expression}
\label{sec:self-expression}
Participants' reactions to the responses about self-expression followed a similar pattern to the responses about relationships. We saw that participants preferred the response generated by AI for the help-seeking message about self-expression and reacted most negatively to the peer response. We found that participants liked AI's response the most (M=3.70, SD=0.98), felt the most positively about AI's response (how helpful: M=3.75, SD=0.94; likelihood to send: M=3.67, SD=1.00) and felt the least negatively about AI's response (how problematic: M=2.01, SD=1.22; how inappropriate: M=1.99, SD=1.18). Participants also felt the most negatively and least positively about the peer response (how problematic: M=2.25, SD=1.19; how inappropriate: M=2.26, SD=1.23; how helpful: M=3.12, SD=1.09; likelihood to send: M=3.05, SD=1.15).
See Figure \ref{fig:plot-self-expression}.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.75]{figures/plot.self.expression_2023.9.11.png}
    \caption{Reactions to responses by source for help-seeking message about self-expression.}
    \label{fig:plot-self-expression}
\end{figure}

Participants liked that the AI-generated response conveyed guidance, support, empathy, and understanding. \textit{"I think a response like this can make the person feel like they've all been in this situation before, and there are points of empathy that they can draw on to guide them to be braver by drawing on the respondent's situation.”} Similar to the relationships message, participants liked that this response \textit{"[empathizes] with the friend while also providing practical solutions”}. They felt the adult mentor did this as well, but to a lesser extent. They liked that \textit{"it starts with sympathy,”} but the overall tone felt \textit{"unattached."} and the message \textit{"[gave] the impression that someone should act rudely and not care what others think.”} Participants seemed to suspect that this message came from a clinician, \textit{"The message looks like one a professional therapist would send..."} As one participant said, “The response is appropriate because [it] is from [a] counselor, someone who has been able to tackle much of the issues by being exposed to different clients and knowing what to do for certain client till they reach a point of believing in themselves and having that courage to talk to anyone without any fear.” The peer's response quite simply did not feel supportive enough to participants and did not do enough to calm the help-seeker, "I think that's too casual a response to really consider the issue from the perspective of the person pouring it out.” 

\subsubsection{Physical health}
\label{sec:physical-health}
When the help-seeking message was about physical health, participants once again preferred AI's response and did not like the peer response. The results show that participants liked AI's response the most (M=3.71, SD=0.96), felt the most positively about it (how helpful: M=3.67, SD=0.99; likelihood to send: M=3.64, SD=0.99), and the least negatively (how problematic: M=1.95, SD=1.16; how inappropriate: M=1.95, SD=1.21). Participants also felt the most negatively and least positively about the peer response (how problematic: M=2.46, SD=1.28; how inappropriate: M=2.40, SD=1.27; how helpful: M=2.73, SD=1.22; likelihood to send: M=2.78, SD=1.23).
See Figure \ref{fig:plot-physical-health}.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.75]{figures/plot.physical.health_2023.9.11.png}
    \caption{Reactions to responses by source for help-seeking message about physical health.}
    \label{fig:plot-physical-health}
\end{figure}

This AI-generated response once again performed the best because 
\textit{"its an all round genuine answer [that] shows you care[,] Understand the problem and offer the right solutions.”} The adult mentor response seemed to \textit{"[make] the person feel as if it's OK to just relax and not do anything."} While the therapist response did offer a solution, participants did not think it was necessarily the right one: \textit{“It's very unclear whether this respondent wants to help out. They are telling the victim to keep pursuing the same course that ain't working for them.”} Participants also noted the extra cost that therapy would incur: \textit{"Counselling can be [quite] expensive,"} which they did not think were necessary since \textit{"Although yes counseling helps sometimes but at this time it wont work cause at this point he/she needs love and support from family and friends who would be available to support them.”}

\begin{table}[]
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Topic of Help-Seeking Message} & \textbf{Source of Best Response} \\ \hline
Relationships & AI \\ \hline
Suicidal Thoughts & Human \\ \hline
Self-Expression & AI \\ \hline
Physical Health & AI \\ \hline
\end{tabular}
\caption{Source of the best-performing response (human or AI) to help-seeking messages about different topics.}
\label{tab:best-source}
\end{table}

We summarize these findings to answer RQ2 in table \ref{tab:best-source}, which outlines which source (human or AI) performed the best for all attributes of participants' responses for each scenario. The best-performing response was the most preferred, most likely to be sent, most helpful, least problematic, and least inappropriate.


==> old/results-v4.tex <==
\section{Results}
Our results are organized into two sections: perceptions of help-seeking messages about frequent topics about which peers exchange support (RQ1) and preferences for human- and AI-generated responses for those help-seeking messages (RQ2). We begin with the same structure for both sections; first, we look at which messages evoked the strongest reactions and which responses participants liked most, respectively, then we examine how those reactions to help-seeking messages and preferences for responses vary by demographic factors (gender, ethnicity, and education).

% Next, we discuss young adults' reactions to responses from different sources (young adult, researcher, therapist, and ChatGPT) in response to help-seeking messages (RQ2a).

\subsection{RQ1: How do young people react to help-seeking messages about frequent topics of peer support exchange?}

Participants' overall reported abilities to relate, help, and sympathize with the help-seeking messages were moderate (i.e., close to the mid-range answer choice).
%, but there were no topics that participants did not feel they could relate, help, or sympathize with. 
Participants felt the most sympathy for the help-seeking message about suicidal thoughts but could relate and help most with the help-seeking message about physical health (see Figure \ref{fig:messages-reactions}). Interestingly, the message about relationships, not the one about suicidal thoughts, was the least relatable. See Figure \ref{fig:messages-reactions}.

\begin{figure}
    \centering
    \includegraphics[scale = 0.4]{figures/plot.messages.react_2023.9.11.png}
    \caption{Perceptions of help-seeking messages about four topics: relationships, suicidal thoughts, self-expression, and physical health. Answers were on a 5-point Likert scale about agreement with statements on the x-axis. 1 was the lowest agreement, and 5 was the highest agreement.}
    \label{fig:messages-reactions}
\end{figure}

% \textit{Differences by gender}: The only reaction for all the help-seeking messages that varied significantly by gender was reported ability to help with the help-seeking message was about physical health. For this topic, male participants felt they could help more than did female participants (male: M=3.52, SD=0.05; female: M=3.35, SD=0.07; T(396.72) = 1.95, p = 0.05).

% \textit{Differences by ethnicity}: There were no significant differences by ethnicity for participants' reported ability to relate, sympathize, or help with any of the help-seeking messages.

% \textit{Differences by education}: \Jordyn{add a description here - lots of significant differences by education!} See table \ref{tab:messages-reaction-education}. A subsequent test for correlations indicated...\Jordyn{add info about whether more education was +/- correlated w/different measures}


% \begin{table}[]
% \centering
% \begin{tabular}{l|cccccc|}
% \cline{2-7}
%  & \multicolumn{6}{l|}{\textbf{Participants' reported ability to...}} \\ \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{\textit{Topic of Help-Seeking Message}}} & \multicolumn{2}{c|}{\textbf{Relate}} & \multicolumn{2}{c|}{\textbf{Sympathize}} & \multicolumn{2}{c|}{\textbf{Help}} \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\textit{Mean}} & \multicolumn{1}{c|}{\textit{SD}} & \multicolumn{1}{c|}{\textit{Mean}} & \multicolumn{1}{c|}{\textit{SD}} & \multicolumn{1}{c|}{\textit{Mean}} & \textit{SD} \\ \hline
% \multicolumn{1}{|l|}{\textbf{Relationships}} & \multicolumn{1}{c|}{3.22} & \multicolumn{1}{c|}{1.02} & \multicolumn{1}{c|}{3.30} & \multicolumn{1}{c|}{1.01} & \multicolumn{1}{c|}{3.31} & 0.98 \\ \hline
% \multicolumn{1}{|l|}{\textbf{Suicidal Thoughts}} & \multicolumn{1}{c|}{3.49} & \multicolumn{1}{c|}{0.97} & \multicolumn{1}{c|}{3.62} & \multicolumn{1}{c|}{0.88} & \multicolumn{1}{c|}{3.46} & 0.98 \\ \hline
% \multicolumn{1}{|l|}{\textbf{Self-Expression}} & \multicolumn{1}{c|}{3.51} & \multicolumn{1}{c|}{0.92} & \multicolumn{1}{c|}{3.55} & \multicolumn{1}{c|}{0.94} & \multicolumn{1}{c|}{3.47} & 0.99 \\ \hline
% \multicolumn{1}{|l|}{\textbf{Physical Health}} & \multicolumn{1}{c|}{3.60} & \multicolumn{1}{c|}{0.90} & \multicolumn{1}{c|}{3.61} & \multicolumn{1}{c|}{0.90} & \multicolumn{1}{c|}{3.49} & 0.94 \\ \hline
% \end{tabular}
% \caption{The extent to which participants felt they could relate, sympathize, and help with the four help-seeking messages presented, which were about four different topics (relationships, suicidal thoughts, self-expression, and physical health). Answers were on a 5-point Likert scale.}
% \label{tab:messages-reactions}
% \end{table}

% \begin{landscape}
% \begin{table}[]
% \centering
% \begin{tabular}{|r|c|cccccccc|c|}
% \hline
% \textit{} & \textbf{} & \multicolumn{8}{c|}{\textit{Education}} & \textbf{} \\ \hline
% \textit{Topic of Help-Seeking Message} & \textit{Participants' ability to...} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Some high\\ school\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}High school \\ or equivalent\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Trade\\ school\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Bachelor's\\ degree\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Master's\\ degree\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Doctoral\\ degree\end{tabular}}} & \multicolumn{1}{c|}{\textbf{Other}} & \textbf{\begin{tabular}[c]{@{}c@{}}Prefer\\ not to say\end{tabular}} & \textit{\textbf{Sig.}} \\ \hline
% \multirow{3}{*}{\textbf{Relationships}} & \textbf{Relate} & \multicolumn{1}{c|}{3.24} & \multicolumn{1}{c|}{3.01} & \multicolumn{1}{c|}{3.25} & \multicolumn{1}{c|}{3.24} & \multicolumn{1}{c|}{3.46} & \multicolumn{1}{c|}{3.92} & \multicolumn{1}{c|}{4.33} & 2.86 & \textit{\textbf{**}} \\ \cline{2-11} 
%  & \textbf{Sympathize} & \multicolumn{1}{c|}{3.53} & \multicolumn{1}{c|}{3.16} & \multicolumn{1}{c|}{3.27} & \multicolumn{1}{c|}{3.33} & \multicolumn{1}{c|}{3.56} & \multicolumn{1}{c|}{3.58} & \multicolumn{1}{c|}{4.00} & 2.86 & \textit{\textbf{***}} \\ \cline{2-11} 
%  & \textbf{Help} & \multicolumn{1}{c|}{3.24} & \multicolumn{1}{c|}{3.02} & \multicolumn{1}{c|}{3.23} & \multicolumn{1}{c|}{3.40} & \multicolumn{1}{c|}{3.82} & \multicolumn{1}{c|}{4.17} & \multicolumn{1}{c|}{4.00} & 2.43 & \textit{\textbf{-}} \\ \hline
% \multirow{3}{*}{\textbf{Suicidal Thoughts}} & \textbf{Relate} & \multicolumn{1}{c|}{3.35} & \multicolumn{1}{c|}{3.39} & \multicolumn{1}{c|}{3.40} & \multicolumn{1}{c|}{3.53} & \multicolumn{1}{c|}{3.67} & \multicolumn{1}{c|}{3.92} & \multicolumn{1}{c|}{4.67} & 3.43 & \textit{\textbf{-}} \\ \cline{2-11} 
%  & \textbf{Sympathize} & \multicolumn{1}{c|}{3.41} & \multicolumn{1}{c|}{3.54} & \multicolumn{1}{c|}{3.47} & \multicolumn{1}{c|}{3.68} & \multicolumn{1}{c|}{3.82} & \multicolumn{1}{c|}{3.58} & \multicolumn{1}{c|}{4.33} & 4.00 & \textit{\textbf{**}} \\ \cline{2-11} 
%  & \textbf{Help} & \multicolumn{1}{c|}{3.29} & \multicolumn{1}{c|}{3.29} & \multicolumn{1}{c|}{3.39} & \multicolumn{1}{c|}{3.48} & \multicolumn{1}{c|}{3.92} & \multicolumn{1}{c|}{3.92} & \multicolumn{1}{c|}{4.33} & 3.71 & \textit{\textbf{**}} \\ \hline
% \multirow{3}{*}{\textbf{Self-Expression}} & \textbf{Relate} & \multicolumn{1}{c|}{3.47} & \multicolumn{1}{c|}{3.37} & \multicolumn{1}{c|}{3.46} & \multicolumn{1}{c|}{3.57} & \multicolumn{1}{c|}{3.44} & \multicolumn{1}{c|}{4.08} & \multicolumn{1}{c|}{4.33} & 3.57 & \textit{\textbf{*}} \\ \cline{2-11} 
%  & \textbf{Sympathize} & \multicolumn{1}{c|}{3.29} & \multicolumn{1}{c|}{3.43} & \multicolumn{1}{c|}{3.48} & \multicolumn{1}{c|}{3.63} & \multicolumn{1}{c|}{3.54} & \multicolumn{1}{c|}{4.00} & \multicolumn{1}{c|}{4.33} & 3.57 & \textit{\textbf{**}} \\ \cline{2-11} 
%  & \textbf{Help} & \multicolumn{1}{c|}{3.41} & \multicolumn{1}{c|}{3.29} & \multicolumn{1}{c|}{3.38} & \multicolumn{1}{c|}{3.53} & \multicolumn{1}{c|}{3.74} & \multicolumn{1}{c|}{3.83} & \multicolumn{1}{c|}{4.33} & 3.57 & \textit{\textbf{**}} \\ \hline
% \multirow{3}{*}{\textbf{Physical Health}} & \textbf{Relate} & \multicolumn{1}{c|}{4.00} & \multicolumn{1}{c|}{3.53} & \multicolumn{1}{c|}{3.43} & \multicolumn{1}{c|}{3.61} & \multicolumn{1}{c|}{3.87} & \multicolumn{1}{c|}{3.92} & \multicolumn{1}{c|}{4.33} & 4.00 & \textit{\textbf{*}} \\ \cline{2-11} 
%  & \textbf{Sympathize} & \multicolumn{1}{c|}{3.71} & \multicolumn{1}{c|}{3.51} & \multicolumn{1}{c|}{3.48} & \multicolumn{1}{c|}{3.67} & \multicolumn{1}{c|}{3.69} & \multicolumn{1}{c|}{3.75} & \multicolumn{1}{c|}{4.33} & 4.14 & \textit{\textbf{*}} \\ \cline{2-11} 
%  & \textbf{Help} & \multicolumn{1}{c|}{4.06} & \multicolumn{1}{c|}{3.39} & \multicolumn{1}{c|}{3.27} & \multicolumn{1}{c|}{3.52} & \multicolumn{1}{c|}{3.64} & \multicolumn{1}{c|}{3.83} & \multicolumn{1}{c|}{4.33} & 3.86 & \textit{\textbf{\textasciicircum{}}} \\ \hline
% \end{tabular}
% \caption{The extent to which participants felt they could relate, sympathize, and help with the four help-seeking messages presented by education. Answers were on a 5-point Likert scale. Significance indicators: - not significant, \textasciicircum trending, * \textless{}0.05, ** \textless{}0.01, *** \textless{}0.001.}
% \label{tab:messages-reaction-education}
% \end{table}
% \end{landscape}




\subsection{RQ2: How much do young people like different help-giving responses created by humans and AI?}

We found that participants preferred AI-generated responses to help-seeking messages about relationships, self-expression, and physical health, but not suicidal thoughts (see table \ref{tab:like-responses}).

\begin{landscape}
\begin{table}[]
\centering
\begin{tabular}{|ccc|ccc|ccc|ccc|}
\hline
\multicolumn{3}{|c|}{\textbf{Relationships}} & \multicolumn{3}{c|}{\textbf{Suicidal Thoughts}} & \multicolumn{3}{c|}{\textbf{Self-Expression}} & \multicolumn{3}{c|}{\textbf{Physical Health}} \\ \hline
\multicolumn{1}{|c|}{\textit{Response Source}} & \multicolumn{1}{c|}{\textit{M}} & \textit{SD} & \multicolumn{1}{c|}{\textit{Response Source}} & \multicolumn{1}{c|}{\textit{M}} & \textit{SD} & \multicolumn{1}{c|}{\textit{Response Source}} & \multicolumn{1}{c|}{\textit{M}} & \textit{SD} & \multicolumn{1}{c|}{\textit{Response Source}} & \multicolumn{1}{c|}{\textit{M}} & \textit{SD} \\ \hline
\multicolumn{1}{|c|}{AI} & \multicolumn{1}{c|}{3.65} & 0.96 & \multicolumn{1}{c|}{Adult Mentor} & \multicolumn{1}{c|}{3.56} & 0.95 & \multicolumn{1}{c|}{AI} & \multicolumn{1}{c|}{3.67} & 1.00 & \multicolumn{1}{c|}{AI} & \multicolumn{1}{c|}{3.64} & 0.99 \\ \hline
\multicolumn{1}{|c|}{Adult Mentor} & \multicolumn{1}{c|}{3.43} & 1.02 & \multicolumn{1}{c|}{Peer} & \multicolumn{1}{c|}{3.19} & 1.12 & \multicolumn{1}{c|}{Adult Mentor} & \multicolumn{1}{c|}{3.48} & 0.97 & \multicolumn{1}{c|}{Adult Mentor} & \multicolumn{1}{c|}{3.44} & 0.99 \\ \hline
\multicolumn{1}{|c|}{Therapist} & \multicolumn{1}{c|}{3.24} & 1.15 & \multicolumn{1}{c|}{Therapist} & \multicolumn{1}{c|}{2.94} & 1.20 & \multicolumn{1}{c|}{Therapist} & \multicolumn{1}{c|}{3.42} & 1.05 & \multicolumn{1}{c|}{Therapist} & \multicolumn{1}{c|}{3.38} & 1.01 \\ \hline
\multicolumn{1}{|c|}{Peer} & \multicolumn{1}{c|}{2.98} & 1.18 & \multicolumn{1}{c|}{AI} & \multicolumn{1}{c|}{2.71} & 1.21 & \multicolumn{1}{c|}{Peer} & \multicolumn{1}{c|}{3.05} & 1.15 & \multicolumn{1}{c|}{Peer} & \multicolumn{1}{c|}{2.78} & 1.23 \\ \hline
\end{tabular}
\caption{How much participants liked the human- and AI-generated responses from four different sources (human peer, human adult mentor, human therapist, and AI) by help-seeking topic (relationships, suicidal thoughts, self-expression, and physical health). Within each topic, response sources are listed from most to least liked, with most liked at the top of the list and least liked at the bottom.}
\label{tab:like-responses}
\end{table}
\end{landscape}




% % \textit{Differences by gender}: The only significant difference by gender was that female participants liked the adult mentor response significantly more than male participants did for the help-seeking message about physical health (female: M=3.60, SD=0.07; male: M=3.41, SD=0.05; T(446.89) = 2.30, p = 0.02).

% % \textit{Differences by ethnicity}: There were two significant differences in response preferences by participants' ethnicity, specifically for the extent to which different groups like the AI responses to the help-seeking messages about relationships and self-expression. African-American participants liked the AI response about relationships the most, while participants who identified as Native Hawaiian/Pacific Islander liked it the least. For the AI response about self-expression, individuals who identified as mixed race liked the AI response the most and participants who identified as Native Hawaiian/Pacific Islander liked it the least. See table \ref{tab:like-responses-ethnicity}.

% % \textit{Differences by education}: There were seven significant differences in response preferences by participants' level of education, including the extent to which participants liked the adult mentor and AI responses about relationships, the adult mentor response about suicidal thoughts, the adult mentor, therapist, and AI response about self-expression, and the AI response about physical health. See table \ref{tab:like-responses-education}.

% \Jordyn{discussion idea: possible implications for testing AI systems? need to consider level of education when evaluating how systems perform? what is there to say about this? what's the implication?...}

% \begin{table}[]
% \centering
% \begin{tabular}{|c|c|cccccccccc|c}
% \cline{1-12}
% \textbf{} & \textbf{} & \multicolumn{10}{c|}{\textit{Ethnicity}} & \multicolumn{1}{l}{} \\ \cline{1-12}
% \textit{Topic of Help-Seeking Message} & \textit{Response source} & \multicolumn{1}{c|}{\textbf{Caucasian}} & \multicolumn{1}{c|}{\textbf{African American}} & \multicolumn{1}{c|}{\textbf{Native American}} & \multicolumn{1}{c|}{\textbf{Latino or Hispanic}} & \multicolumn{1}{c|}{\textbf{Mixed Race}} & \multicolumn{1}{c|}{\textbf{Asian}} & \multicolumn{1}{c|}{\textbf{Multiple}} & \multicolumn{1}{c|}{\textbf{Prefer not to say}} & \multicolumn{1}{c|}{\textbf{Native Hawaiian or Pacific Islander}} & \textbf{Other} & \multicolumn{1}{l}{\textit{\textbf{Significance}}} \\ \cline{1-12}
% \multirow{4}{*}{\textbf{Relationships}} & \textbf{Peer} & \multicolumn{1}{c|}{3.11} & \multicolumn{1}{c|}{2.95} & \multicolumn{1}{c|}{2.79} & \multicolumn{1}{c|}{2.77} & \multicolumn{1}{c|}{2.88} & \multicolumn{1}{c|}{3.00} & \multicolumn{1}{c|}{3.38} & \multicolumn{1}{c|}{2.33} & \multicolumn{1}{c|}{2.67} & 1.00 & \textit{\textbf{-}} \\ \cline{2-12}
%  & \textbf{Adult Mentor} & \multicolumn{1}{c|}{3.44} & \multicolumn{1}{c|}{3.59} & \multicolumn{1}{c|}{3.53} & \multicolumn{1}{c|}{3.19} & \multicolumn{1}{c|}{3.58} & \multicolumn{1}{c|}{3.12} & \multicolumn{1}{c|}{3.56} & \multicolumn{1}{c|}{3.33} & \multicolumn{1}{c|}{3.17} & 5.00 & \textit{\textbf{-}} \\ \cline{2-12}
%  & \textbf{Therapist} & \multicolumn{1}{c|}{3.42} & \multicolumn{1}{c|}{3.20} & \multicolumn{1}{c|}{3.03} & \multicolumn{1}{c|}{3.27} & \multicolumn{1}{c|}{3.21} & \multicolumn{1}{c|}{2.94} & \multicolumn{1}{c|}{3.38} & \multicolumn{1}{c|}{2.89} & \multicolumn{1}{c|}{2.83} & 3.00 & \textit{\textbf{-}} \\ \cline{2-12}
%  & \textbf{AI} & \multicolumn{1}{c|}{3.53} & \multicolumn{1}{c|}{3.88} & \multicolumn{1}{c|}{3.53} & \multicolumn{1}{c|}{3.38} & \multicolumn{1}{c|}{3.71} & \multicolumn{1}{c|}{3.18} & \multicolumn{1}{c|}{3.81} & \multicolumn{1}{c|}{3.44} & \multicolumn{1}{c|}{2.83} & 4.00 & \textit{\textbf{*}} \\ \cline{1-12}
% \multirow{4}{*}{\textbf{Suicidal Thoughts}} & \textbf{Peer} & \multicolumn{1}{c|}{3.24} & \multicolumn{1}{c|}{3.21} & \multicolumn{1}{c|}{3.41} & \multicolumn{1}{c|}{3.23} & \multicolumn{1}{c|}{3.04} & \multicolumn{1}{c|}{3.18} & \multicolumn{1}{c|}{3.38} & \multicolumn{1}{c|}{2.56} & \multicolumn{1}{c|}{3.17} & 4.00 & \textit{\textbf{-}} \\ \cline{2-12}
%  & \textbf{Adult Mentor} & \multicolumn{1}{c|}{3.54} & \multicolumn{1}{c|}{3.70} & \multicolumn{1}{c|}{3.41} & \multicolumn{1}{c|}{3.69} & \multicolumn{1}{c|}{3.92} & \multicolumn{1}{c|}{3.00} & \multicolumn{1}{c|}{3.75} & \multicolumn{1}{c|}{3.44} & \multicolumn{1}{c|}{3.00} & 5.00 & \textit{\textbf{-}} \\ \cline{2-12}
%  & \textbf{Therapist} & \multicolumn{1}{c|}{3.09} & \multicolumn{1}{c|}{2.87} & \multicolumn{1}{c|}{2.85} & \multicolumn{1}{c|}{3.27} & \multicolumn{1}{c|}{2.96} & \multicolumn{1}{c|}{2.88} & \multicolumn{1}{c|}{3.13} & \multicolumn{1}{c|}{2.78} & \multicolumn{1}{c|}{2.83} & 1.00 & \textit{\textbf{-}} \\ \cline{2-12}
%  & \textbf{AI} & \multicolumn{1}{c|}{2.87} & \multicolumn{1}{c|}{2.76} & \multicolumn{1}{c|}{3.09} & \multicolumn{1}{c|}{2.85} & \multicolumn{1}{c|}{2.21} & \multicolumn{1}{c|}{3.41} & \multicolumn{1}{c|}{2.81} & \multicolumn{1}{c|}{2.56} & \multicolumn{1}{c|}{2.00} & 1.00 & \textit{\textbf{-}} \\ \cline{1-12}
% \multirow{4}{*}{\textbf{Self-Expression}} & \textbf{Peer} & \multicolumn{1}{c|}{3.06} & \multicolumn{1}{c|}{3.16} & \multicolumn{1}{c|}{3.09} & \multicolumn{1}{c|}{3.19} & \multicolumn{1}{c|}{2.92} & \multicolumn{1}{c|}{2.94} & \multicolumn{1}{c|}{3.50} & \multicolumn{1}{c|}{2.56} & \multicolumn{1}{c|}{2.33} & 1.00 & \textit{\textbf{-}} \\ \cline{2-12}
%  & \textbf{Adult Mentor} & \multicolumn{1}{c|}{3.52} & \multicolumn{1}{c|}{3.51} & \multicolumn{1}{c|}{3.44} & \multicolumn{1}{c|}{3.42} & \multicolumn{1}{c|}{3.88} & \multicolumn{1}{c|}{3.47} & \multicolumn{1}{c|}{3.44} & \multicolumn{1}{c|}{2.67} & \multicolumn{1}{c|}{2.83} & 5.00 & \textit{\textbf{-}} \\ \cline{2-12}
%  & \textbf{Therapist} & \multicolumn{1}{c|}{3.47} & \multicolumn{1}{c|}{3.40} & \multicolumn{1}{c|}{3.53} & \multicolumn{1}{c|}{3.58} & \multicolumn{1}{c|}{3.75} & \multicolumn{1}{c|}{3.18} & \multicolumn{1}{c|}{3.75} & \multicolumn{1}{c|}{3.11} & \multicolumn{1}{c|}{2.83} & 5.00 & \textit{\textbf{-}} \\ \cline{2-12}
%  & \textbf{AI} & \multicolumn{1}{c|}{3.51} & \multicolumn{1}{c|}{3.98} & \multicolumn{1}{c|}{3.74} & \multicolumn{1}{c|}{3.69} & \multicolumn{1}{c|}{4.04} & \multicolumn{1}{c|}{3.12} & \multicolumn{1}{c|}{4.00} & \multicolumn{1}{c|}{3.56} & \multicolumn{1}{c|}{2.83} & 5.00 & \textit{\textbf{*}} \\ \cline{1-12}
% \multirow{4}{*}{\textbf{Physical Health}} & \textbf{Peer} & \multicolumn{1}{c|}{2.83} & \multicolumn{1}{c|}{2.82} & \multicolumn{1}{c|}{2.82} & \multicolumn{1}{c|}{2.77} & \multicolumn{1}{c|}{2.46} & \multicolumn{1}{c|}{3.29} & \multicolumn{1}{c|}{2.94} & \multicolumn{1}{c|}{2.67} & \multicolumn{1}{c|}{3.33} & 1.50 & \textit{\textbf{-}} \\ \cline{2-12}
%  & \textbf{Adult Mentor} & \multicolumn{1}{c|}{3.44} & \multicolumn{1}{c|}{3.58} & \multicolumn{1}{c|}{3.32} & \multicolumn{1}{c|}{3.42} & \multicolumn{1}{c|}{3.54} & \multicolumn{1}{c|}{3.29} & \multicolumn{1}{c|}{3.75} & \multicolumn{1}{c|}{3.11} & \multicolumn{1}{c|}{3.67} & 2.00 & \textit{\textbf{-}} \\ \cline{2-12}
%  & \textbf{Therapist} & \multicolumn{1}{c|}{3.35} & \multicolumn{1}{c|}{3.56} & \multicolumn{1}{c|}{3.44} & \multicolumn{1}{c|}{3.50} & \multicolumn{1}{c|}{3.63} & \multicolumn{1}{c|}{3.12} & \multicolumn{1}{c|}{3.31} & \multicolumn{1}{c|}{3.22} & \multicolumn{1}{c|}{3.33} & 5.00 & \textit{\textbf{-}} \\ \cline{2-13} 
%  & \textbf{AI} & \multicolumn{1}{c|}{3.57} & \multicolumn{1}{c|}{3.96} & \multicolumn{1}{c|}{3.62} & \multicolumn{1}{c|}{3.58} & \multicolumn{1}{c|}{4.00} & \multicolumn{1}{c|}{3.06} & \multicolumn{1}{c|}{3.81} & \multicolumn{1}{c|}{3.56} & \multicolumn{1}{c|}{3.83} & 5.00 & \multicolumn{1}{c|}{\textit{\textbf{\textasciicircum{}}}} \\ \hline
% \end{tabular}
% \caption{Average answer for how much participants liked the human- and AI-generated responses from four different sources (human peer, human adult mentor, human therapist, and AI) for each help-seeking topic (relationships, suicidal thoughts, self-expression, and physical health) by ethnicity. Answers were on a 5-point Likert scale. Significance indicators: - not significant, \textasciicircum trending, * \textless{}0.05.}
% \label{tab:like-responses-ethnicity}
% \end{table}

% \begin{table}[!ht]
% \resizebox{0.5\textwidth}{!}{
% \centering
% \small
% \begin{tabular}{|c|c|cccccccc|c|}
% \hline
% \textbf{} & \textbf{} & \multicolumn{8}{c|}{\textit{Education}} & \textbf{} \\ \hline
% \textit{Topic of Help-Seeking Message} & \textit{Response source} & \multicolumn{1}{c|}{\textbf{Some high school}} & \multicolumn{1}{c|}{\textbf{High school or equivalent}} & \multicolumn{1}{c|}{\textbf{Trade school}} & \multicolumn{1}{c|}{\textbf{Bachelor's degree}} & \multicolumn{1}{c|}{\textbf{Master's degree}} & \multicolumn{1}{c|}{\textbf{Doctoral degree}} & \multicolumn{1}{c|}{\textbf{Other}} & \textbf{Prefer not to say} & \textit{\textbf{Significance}} \\ \hline
% \multirow{4}{*}{\textbf{Relationships}} & \textbf{Peer} & \multicolumn{1}{c|}{2.41} & \multicolumn{1}{c|}{3.18} & \multicolumn{1}{c|}{3.03} & \multicolumn{1}{c|}{2.94} & \multicolumn{1}{c|}{2.79} & \multicolumn{1}{c|}{3.58} & \multicolumn{1}{c|}{1.33} & 3.71 & \textit{\textbf{-}} \\ \cline{2-11} 
%  & \textbf{Adult Mentor} & \multicolumn{1}{c|}{3.71} & \multicolumn{1}{c|}{3.35} & \multicolumn{1}{c|}{3.29} & \multicolumn{1}{c|}{3.55} & \multicolumn{1}{c|}{3.72} & \multicolumn{1}{c|}{3.83} & \multicolumn{1}{c|}{4.67} & 3.00 & \textit{\textbf{*}} \\ \cline{2-11} 
%  & \textbf{Therapist} & \multicolumn{1}{c|}{3.06} & \multicolumn{1}{c|}{3.30} & \multicolumn{1}{c|}{3.14} & \multicolumn{1}{c|}{3.35} & \multicolumn{1}{c|}{3.13} & \multicolumn{1}{c|}{3.58} & \multicolumn{1}{c|}{4.00} & 3.29 & \textit{\textbf{-}} \\ \cline{2-11} 
%  & \textbf{AI} & \multicolumn{1}{c|}{3.82} & \multicolumn{1}{c|}{3.43} & \multicolumn{1}{c|}{3.56} & \multicolumn{1}{c|}{3.70} & \multicolumn{1}{c|}{3.69} & \multicolumn{1}{c|}{4.00} & \multicolumn{1}{c|}{4.67} & 3.86 & \textit{\textbf{**}} \\ \hline
% \multirow{4}{*}{\textbf{Suicidal Thoughts}} & \textbf{Peer} & \multicolumn{1}{c|}{3.29} & \multicolumn{1}{c|}{3.29} & \multicolumn{1}{c|}{3.04} & \multicolumn{1}{c|}{3.21} & \multicolumn{1}{c|}{3.18} & \multicolumn{1}{c|}{3.92} & \multicolumn{1}{c|}{4.00} & 3.43 & \textit{\textbf{-}} \\ \cline{2-11} 
%  & \textbf{Adult Mentor} & \multicolumn{1}{c|}{3.18} & \multicolumn{1}{c|}{3.39} & \multicolumn{1}{c|}{3.55} & \multicolumn{1}{c|}{3.70} & \multicolumn{1}{c|}{3.82} & \multicolumn{1}{c|}{3.58} & \multicolumn{1}{c|}{4.00} & 3.71 & \textit{\textbf{***}} \\ \cline{2-11} 
%  & \textbf{Therapist} & \multicolumn{1}{c|}{2.82} & \multicolumn{1}{c|}{2.95} & \multicolumn{1}{c|}{2.89} & \multicolumn{1}{c|}{3.08} & \multicolumn{1}{c|}{2.87} & \multicolumn{1}{c|}{3.25} & \multicolumn{1}{c|}{4.00} & 1.86 & \textit{\textbf{-}} \\ \cline{2-11} 
%  & \textbf{AI} & \multicolumn{1}{c|}{2.76} & \multicolumn{1}{c|}{2.93} & \multicolumn{1}{c|}{2.96} & \multicolumn{1}{c|}{2.72} & \multicolumn{1}{c|}{2.62} & \multicolumn{1}{c|}{3.50} & \multicolumn{1}{c|}{2.00} & 2.86 & \textit{\textbf{-}} \\ \hline
% \multirow{4}{*}{\textbf{Self-Expression}} & \textbf{Peer} & \multicolumn{1}{c|}{3.35} & \multicolumn{1}{c|}{3.14} & \multicolumn{1}{c|}{2.83} & \multicolumn{1}{c|}{3.09} & \multicolumn{1}{c|}{3.13} & \multicolumn{1}{c|}{3.75} & \multicolumn{1}{c|}{4.00} & 2.43 & \textit{\textbf{-}} \\ \cline{2-11} 
%  & \textbf{Adult Mentor} & \multicolumn{1}{c|}{3.24} & \multicolumn{1}{c|}{3.31} & \multicolumn{1}{c|}{3.40} & \multicolumn{1}{c|}{3.61} & \multicolumn{1}{c|}{3.77} & \multicolumn{1}{c|}{3.92} & \multicolumn{1}{c|}{4.00} & 3.14 & \textit{\textbf{***}} \\ \cline{2-11} 
%  & \textbf{Therapist} & \multicolumn{1}{c|}{3.18} & \multicolumn{1}{c|}{3.41} & \multicolumn{1}{c|}{3.18} & \multicolumn{1}{c|}{3.51} & \multicolumn{1}{c|}{3.92} & \multicolumn{1}{c|}{3.75} & \multicolumn{1}{c|}{4.67} & 3.29 & \textit{\textbf{**}} \\ \cline{2-11} 
%  & \textbf{AI} & \multicolumn{1}{c|}{3.82} & \multicolumn{1}{c|}{3.53} & \multicolumn{1}{c|}{3.47} & \multicolumn{1}{c|}{3.81} & \multicolumn{1}{c|}{3.79} & \multicolumn{1}{c|}{4.08} & \multicolumn{1}{c|}{5.00} & 3.29 & \textit{\textbf{**}} \\ \hline
% \multirow{4}{*}{\textbf{Physical Health}} & \textbf{Peer} & \multicolumn{1}{c|}{2.53} & \multicolumn{1}{c|}{2.87} & \multicolumn{1}{c|}{2.68} & \multicolumn{1}{c|}{2.84} & \multicolumn{1}{c|}{2.77} & \multicolumn{1}{c|}{3.92} & \multicolumn{1}{c|}{2.67} & 2.86 & \textit{\textbf{-}} \\ \cline{2-11} 
%  & \textbf{Adult Mentor} & \multicolumn{1}{c|}{3.29} & \multicolumn{1}{c|}{3.35} & \multicolumn{1}{c|}{3.41} & \multicolumn{1}{c|}{3.59} & \multicolumn{1}{c|}{3.33} & \multicolumn{1}{c|}{3.83} & \multicolumn{1}{c|}{4.33} & 2.71 & \textit{\textbf{-}} \\ \cline{2-11} 
%  & \textbf{Therapist} & \multicolumn{1}{c|}{3.53} & \multicolumn{1}{c|}{3.34} & \multicolumn{1}{c|}{3.39} & \multicolumn{1}{c|}{3.45} & \multicolumn{1}{c|}{3.59} & \multicolumn{1}{c|}{3.50} & \multicolumn{1}{c|}{4.33} & 3.57 & \textit{\textbf{-}} \\ \cline{2-11} 
%  & \textbf{AI} & \multicolumn{1}{c|}{3.41} & \multicolumn{1}{c|}{3.54} & \multicolumn{1}{c|}{3.63} & \multicolumn{1}{c|}{3.79} & \multicolumn{1}{c|}{3.79} & \multicolumn{1}{c|}{4.08} & \multicolumn{1}{c|}{4.67} & 4.00 & \textit{\textbf{***}} \\ \hline
% \end{tabular}
% \caption{Average answer for how much participants liked the human- and AI-generated responses from four different sources (human peer, human adult mentor, human therapist, and AI) for each help-seeking topic (relationships, suicidal thoughts, self-expression, and physical health) by education. Answers were on a 5-point Likert scale. Significance indicators: - not significant, \textasciicircum trending, * \textless{}0.05, ** \textless{}0.01, *** \textless{}0.001.}
% \label{tab:like-responses-education}
% }
% \end{table}

For each topic, we begin by with the quantitative results for each attribute of the responses, followed by quotes from open-ended responses from the participants to illustrate why they did, or did not, like each response. Results from the open-ended responses are described from most to least preferred response within each scenario.

\subsubsection{Relationships}
\label{sec:relationships}
Participants' reactions to responses about relationships did vary significantly by source, and they preferred the response generated by AI. Our results show that not only did \textbf{\textit{participants like the AI response the most}}, but they also felt it was the most helpful (M=3.63, SD=1.00), least problematic (M=2.01, SD=1.16), least inappropriate (M=2.01, SD=1.20), and that they were most likely to send it (M=3.65, SD=0.96).

\textbf{\textit{When discussing relationship issues, participants did not like the peer response.}} They liked the peer's response the least (M=3.00, SD=1.15) and felt it was the most negative (how problematic: M=2.41, SD=1.24; how inappropriate: M=2.38, SD=1.24) and least positive (how helpful: M=3.07, SD=1.13; likelihood to send: M=2.98, SD=1.17). 
See Figure \ref{fig:plot-scenario-1}. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.75]{figures/plot.relationships_2023.9.11.png}
    \caption{Reactions to responses by source for help-seeking message about relationships.}
    \label{fig:plot-relationships}
\end{figure}

\Jordyn{add participant ID\#, gender, and ethnicity for all quotes!}

This sentiment was reflected in the free-response questions, where participants noted that they liked the balance and empathy in the AI-generated responses but wanted more acknowledgment of the others' perspectives (which this AI did not have the context for, as the "ex" was not involved in the conversation). Participants noted that they liked how the AI response both offered support and presented actionable solutions: \textit{“This particular response says it all, it's absolutely what I'd say. What I like the most is that it tells [the friend] how to deal with the situation and still encourages [them].”} The response was \textit{"helpful...
%The response has facts that are hard to hear but they are helpful. The message is 
[and] also supportive and feels like a safe space."}
    %it also has ways of how to cope with the situation.
Some participants even said the AI-generated response seemed like it came from someone who is a good friend: \textit{“They are really trying to help the friend so much and we all need such friends."} There were also mentions of qualities participants associated with the AI response, including that they thought it was "[empathetic]...supportive and caring." Even though participants did favor the AI-generated response to the help-seeking message about relationships, they did note some room for improvement. Namely, that the response doesn't consider the entire context of the situation and "accuses the ex without listening to his side of the story."

Participants noted that the human-generated responses from the adult mentor also provided acknowledgment and validation, but it was potentially less useful and lacked clear solutions. Those who liked this response noted that \textit{“it is respectful and...made [them] feel like the person understood [the help-seeker's] feelings"}. Participants also noted a sense of maturity in how the response did not judge the help-seeker: “...the [response] answered the question in a mature way by making the victim not feel offended by going back to the ex. The response is just showing him or her that is what we [humans] go through in terms of love life.” Despite these positive attributes of the adult mentor's response, some participants felt it was \textit{"just about beating around the bush"} and that \textit{"it didn't provide a way of how to solve the situation clearly."}

Participants liked the therapist's response because they felt it was extremely understanding and non-judgmental but noted that it seemed to delay giving actionable advice. Even though they did not know a therapist wrote one of the responses, they picked up on the professional tone: \textit{"This person provides professional remedy and ... [asks] the victim to share their mixed emotions and from there she/he will be in a position to offer strategies.”} They saw the response as "very empathetic without shaming the friend," but noted that it felt like " scheduling [giving] help to next time when the [help-seeker] is in need of it now.” They appreciated the supportive tone but would have liked more concrete and immediate advice rather than beating around the bush and delaying support.

We received the most negative comments about the peer's response because participants felt it was terse, suggested hasty actions, and was not encouraging. While some appreciated the response's brevity, the way it was written came across as \textit{"too direct with no empathy.”} This lack of empathy made participants feel like the sender had a bad attitude and was being too tough on the help-seeker: \textit{"It sounds harsh and rude, and also it doesn't consider the feelings of the victim."}

\subsubsection{Suicidal thoughts}
\label{sec:suicidal-thoughts}
In response to help-seeking messages about suicidal thoughts, participants preferred the response from the adult mentor and reacted most negatively to AI's response. Among the responses presented, participants liked the adult mentor's response the most (M=3.59, SD=0.95) and felt the most positively (how helpful: M=3.61, SD=0.94; likelihood to send: M=3.56, SD=0.94) and least negatively about it (how problematic: M=2.04, SD=1.18; how inappropriate: M=2.00,	SD=1.20). They also liked AI's response the least (M=2.82, SD=1.19) and felt the most negative (how problematic: M=2.53, SD=1.26; how inappropriate: M=2.54, SD=1.27) and least positive about it (how helpful: M=2.93, SD=1.12; likelihood to send: M=2.71,	SD=1.21).
See Figure \ref{fig:plot-suicidal-thoughts}. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.75]{figures/plot.suicidal.thoughts_2023.9.11.png}
    \caption{Reactions to responses by source for help-seeking message about suicidal thoughts.}
    \label{fig:plot-suicidal-thoughts}
\end{figure}

When describing why they preferred the adult mentor's response to this sensitive topic, participants noted that they liked how it conveyed genuine concern by inviting the help-seeker to share more details and put effort over providing more support. \textit{"There’s a feeling of relating with the individual here. There’s a feeling of care and [that they're] really interested and [want] to understand the individual }
% plus boosting the individual’s confidence and also wanting to understand the individual’s 
\textit{[and their] situation."}
% It’s the best to do in such situation, for someone who wants to really be there for such person.” 
The only area of improvement that participants mentioned for the adult mentor response is that the message could have been a little shorter, but did not note what content should be cut. The second most preferred response came from a peer, and participants felt it was \textit{"very shallow"}, inconsiderate, and would leave the help-seeker feeling unseen. Interestingly, they likened this type of message to a computer-generated response, saying it sounded \textit{"...typical of a bot"}. Unlike the adult mentor's response, participants did not like how the peer's response was \textit{"so shallow [and] does not give the victim...much [detail] on how to tackle the situation and [get] helped."} Participants noted that the therapist's response immediately asked for more information in an attempt to ensure the help-seeker's safety - not knowing that this message was written by a clinician, some thought this sounded \textit{"professional"} while many others took it as intrusively asking for more information right away instead of offering support. \textit{“I think this response makes the person in need sink deeper into her trouble rather than pull her out. It's a bit inappropriate.”} Since the initial help-seeking message did not use the word "suicide," many participants also did not like that the therapist's response immediately drew that conclusion and felt that calling it out could com across as judgemental: \textit{“I hate the assumption about self harm and suicide. It feels really I'm going to insert myself into your life to fix it and doesn't feel friendly at all.”} The AI-generated response overall performed the worst. While some felt the response was \textit{"genuine"} and \textit{"actually truthful about the person's ability,"} most saw the referral to a healthcare provider as a lack of desire to help. \textit{“Fine, you can’t provide help but that’s not the best way to put it. You could always have the right choice of words and making the right sentence in this situation before suggesting a mental health professional and not everybody will like the fact that they are referring to them as going crazy. Not really cool though.”}

\subsubsection{Self-expression}
\label{sec:self-expression}
Participants' reactions to the responses about self-expression followed a similar pattern to the responses about relationships. We saw that participants preferred the response generated by AI for the help-seeking message about self-expression and reacted most negatively to the peer response. We found that participants liked AI's response the most (M=3.70, SD=0.98), felt the most positively about AI's response (how helpful: M=3.75, SD=0.94; likelihood to send: M=3.67, SD=1.00) and felt the least negatively about AI's response (how problematic: M=2.01, SD=1.22; how inappropriate: M=1.99, SD=1.18). Participants also felt the most negatively and least positively about the peer response (how problematic: M=2.25, SD=1.19; how inappropriate: M=2.26, SD=1.23; how helpful: M=3.12, SD=1.09; likelihood to send: M=3.05, SD=1.15).
See Figure \ref{fig:plot-self-expression}.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.75]{figures/plot.self.expression_2023.9.11.png}
    \caption{Reactions to responses by source for help-seeking message about self-expression.}
    \label{fig:plot-self-expression}
\end{figure}

Participants liked that the AI-generated response conveyed guidance, support, empathy, and understanding. \textit{"I think a response like this can make the person feel like they've all been in this situation before, and there are points of empathy that they can draw on to guide them to be braver by drawing on the respondent's situation.”} Similar to the relationships message, participants liked that this response \textit{"[empathizes] with the friend while also providing practical solutions”}. They felt the adult mentor did this as well, but to a lesser extent. They liked that \textit{"it starts with sympathy,”} but the overall tone felt \textit{"unattached."} and the message \textit{"[gave] the impression that someone should act rudely and not care what others think.”} Participants seemed to suspect that this message came from a clinician, \textit{"The message looks like one a professional therapist would send..."} As one participant said, “The response is appropriate because [it] is from [a] counselor, someone who has been able to tackle much of the issues by being exposed to different clients and knowing what to do for certain client till they reach a point of believing in themselves and having that courage to talk to anyone without any fear.” The peer's response quite simply did not feel supportive enough to participants and did not do enough to calm the help-seeker, "I think that's too casual a response to really consider the issue from the perspective of the person pouring it out.” 

\subsubsection{Physical health}
\label{sec:physical-health}
When the help-seeking message was about physical health, participants once again preferred AI's response and did not like the peer response. The results show that participants liked AI's response the most (M=3.71, SD=0.96), felt the most positively about it (how helpful: M=3.67, SD=0.99; likelihood to send: M=3.64, SD=0.99), and the least negatively (how problematic: M=1.95, SD=1.16; how inappropriate: M=1.95, SD=1.21). Participants also felt the most negatively and least positively about the peer response (how problematic: M=2.46, SD=1.28; how inappropriate: M=2.40, SD=1.27; how helpful: M=2.73, SD=1.22; likelihood to send: M=2.78, SD=1.23).
See Figure \ref{fig:plot-physical-health}.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.75]{figures/plot.physical.health_2023.9.11.png}
    \caption{Reactions to responses by source for help-seeking message about physical health.}
    \label{fig:plot-physical-health}
\end{figure}

This AI-generated response once again performed the best because 
\textit{"its an all round genuine answer [that] shows you care[,] Understand the problem and offer the right solutions.”} The adult mentor response seemed to \textit{"[make] the person feel as if it's OK to just relax and not do anything."} While the therapist response did offer a solution, participants did not think it was necessarily the right one: \textit{“It's very unclear whether this respondent wants to help out. They are telling the victim to keep pursuing the same course that ain't working for them.”} Participants also noted the extra cost that therapy would incur: \textit{"Counselling can be [quite] expensive,"} which they did not think were necessary since \textit{"Although yes counseling helps sometimes but at this time it wont work cause at this point he/she needs love and support from family and friends who would be available to support them.”}

\begin{table}[]
\centering
\begin{tabular}{|c|c|}
\hline
\textbf{Topic of Help-Seeking Message} & \textbf{Source of Best Response} \\ \hline
Relationships & AI \\ \hline
Suicidal Thoughts & Human \\ \hline
Self-Expression & AI \\ \hline
Physical Health & AI \\ \hline
\end{tabular}
\caption{Source of the best-performing response (human or AI) to help-seeking messages about different topics.}
\label{tab:best-source}
\end{table}

% \subsection{RQ3: How does young people's ability to relate, sympathize, and help with different help-seeking topics (RQ1) impact how much they like help-giving responses from different sources (RQ2)?}

% % To answer RQ3, we wanted to understand how much participants' ability to relate, sympathize, and help with different help-seeking topics impacted how much they liked help-giving responses from different sources. 
% We ran linear regressions for each topic (relationships, suicidal thoughts, self-expression, and physical health) with how much participants liked help-giving responses from different human sources (peer, adult mentor, therapist) and AI as dependent variables and ability to relate, sympathize, and help with different help-seeking topics as independent variables (4 responses x 3 reactions to help-seeking message = 12 models per topic). This means we ran 48 preference analyses in total (12 models per topic x 4 topics).


% \begin{figure}
%     \centering
%     \includegraphics[scale = 0.5]{figures/heatmap_2023.9.11.png}
%     \caption{Heatmap of regression coefficients of how much participants liked responses from each source by ability to relate, sympathize, and help with each help-seeking topic. Darker blue is a higher r-squared value, and white is a lower r-squared value.}
%     \label{fig:enter-label}
% \end{figure}




==> old/results-v5.tex <==
\section{Results}
% Our findings indicate that human-generated responses perform better when analyses do not take the topic into account, but topic-based analyses reveal that young people prefer AI-generated responses for less sensitive topics. In this section, we describe our findings that led us to this conclusion. 
We first describe perceptions of help-seeking messages for frequent topics about which peers exchange support, and how those perceptions were related to how much participants liked the different responses (RQ1). Then, we describe participants' preferences for, and reactions, to different support-giving responses (peer, adult mentor, therapist, and AI) across all topics (RQ2-a) and how these preferences and reactions vary depending on the topic of the help-seeking message they are responding to (relationships, suicidal thoughts, self-expression, or physical health; RQ2-b).

\subsection{Statistic about Reactions to Help-seeking Messages about Frequent Topics of Peer Support Exchange and Demographic Characteristics}/Jina{I feel like we dont have any significant findings here that is too novel and is very short. it passed without much learned. It also shows very little demographic results. I feel like this section is just confusing without much highlights and not comprehensive either. usually the first section should be most fun and motivating for the readers and this section doesnt do that}

Participants' overall reported abilities to relate, help, and sympathize with the help-seeking messages were moderate (i.e., close to the mid-range answer choice, which was three on a five-point Likert scale with a range of one to five).
%, but there were no topics that participants did not feel they could relate, help, or sympathize with. 
Participants felt the most sympathy for the help-seeking message about suicidal thoughts but could relate and help most with the help-seeking message about physical health. Interestingly, the message about relationships, not the one about suicidal thoughts, was the least relatable. See Figure \ref{fig:messages-reactions}. /Jina{these conclusions are weird to say after having declared none of the results were significant}
There were no significant differences between topics for participants' ability to relate, sympathize, or help. However, there were significant, albeit modest, correlations between their ability /Jina{how much they can relate..?}to relate, sympathize, or help and the extent to which they liked each response. /Jina{this sentence is redundant with next sentence and next sentence is way better. i would delete this prior sentence} Regardless of the source of response (peer, adult mentor, AI, therapist), we noticed that the more participants could relate, sympathize, and help, the more they liked the responses, the more positively they felt about them, and the less negatively they felt about them. See Appendix \ref{cor-messages-responses}.

\begin{figure}[!t]
    \centering
    \includegraphics[scale = 0.5]{figures/plot.messages.react_2023.9.11.png}
    \caption{Perceptions of help-seeking messages about four topics: relationships, suicidal thoughts, self-expression, and physical health. Answers were on a 5-point Likert scale about agreement with statements on the x-axis. 1 was the lowest agreement, and 5 was the highest agreement.}
    \label{fig:messages-reactions}
\end{figure}

Next, we describe our findings regarding differences found based on demographics (gender, ethnicity, and education). The only reaction for all the help-seeking messages that varied significantly by gender was the ability to help with the help-seeking message about physical health. For this topic, male participants felt they could help more than did female participants (male: M=3.52, SD=0.05; female: M=3.35, SD=0.07; T(396.72) = 1.95, p = 0.05). There were no significant differences by ethnicity in participants' reported ability to relate, sympathize, or help with any of the help-seeking messages. Finally, we found some significant differences based on education 
% for all but two of the variables (ability to help with relationships and ability to relate to suicidal thoughts; 
(see Appendix \ref{messages-reaction-education-means}), and a subsequent test for correlations indicated that participants with a higher level of education felt they could relate, sympathize, and help more with all of the help-seeking messages (see Appendix \ref{messages-reaction-education-correlations}).

% Our findings did 

% \begin{table}[hbt!]
% \centering
% \begin{tabular}{l|cccccc|}
% \cline{2-7}
%  & \multicolumn{6}{l|}{\textbf{Participants' reported ability to...}} \\ \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{\textit{Topic of Help-Seeking Message}}} & \multicolumn{2}{c|}{\textbf{Relate}} & \multicolumn{2}{c|}{\textbf{Sympathize}} & \multicolumn{2}{c|}{\textbf{Help}} \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\textit{Mean}} & \multicolumn{1}{c|}{\textit{SD}} & \multicolumn{1}{c|}{\textit{Mean}} & \multicolumn{1}{c|}{\textit{SD}} & \multicolumn{1}{c|}{\textit{Mean}} & \textit{SD} \\ \hline
% \multicolumn{1}{|l|}{\textbf{Relationships}} & \multicolumn{1}{c|}{3.22} & \multicolumn{1}{c|}{1.02} & \multicolumn{1}{c|}{3.30} & \multicolumn{1}{c|}{1.01} & \multicolumn{1}{c|}{3.31} & 0.98 \\ \hline
% \multicolumn{1}{|l|}{\textbf{Suicidal Thoughts}} & \multicolumn{1}{c|}{3.49} & \multicolumn{1}{c|}{0.97} & \multicolumn{1}{c|}{3.62} & \multicolumn{1}{c|}{0.88} & \multicolumn{1}{c|}{3.46} & 0.98 \\ \hline
% \multicolumn{1}{|l|}{\textbf{Self-Expression}} & \multicolumn{1}{c|}{3.51} & \multicolumn{1}{c|}{0.92} & \multicolumn{1}{c|}{3.55} & \multicolumn{1}{c|}{0.94} & \multicolumn{1}{c|}{3.47} & 0.99 \\ \hline
% \multicolumn{1}{|l|}{\textbf{Physical Health}} & \multicolumn{1}{c|}{3.60} & \multicolumn{1}{c|}{0.90} & \multicolumn{1}{c|}{3.61} & \multicolumn{1}{c|}{0.90} & \multicolumn{1}{c|}{3.49} & 0.94 \\ \hline
% \end{tabular}
% \caption{The extent to which participants felt they could relate, sympathize, and help with the four help-seeking messages presented, which were about four different topics (relationships, suicidal thoughts, self-expression, and physical health). Answers were on a 5-point Likert scale.}
% \label{tab:messages-reactions}
% \end{table}



\subsection{RQ2-a: Reactions to Human and AI-generated Help-giving Responses Across Scenarios}
We found that the human-generated adult-mentor response performed best when we combined responses across all help-seeking topics and compared the average responses from the four sources (peer, adult mentor, therapist, and AI).
% without separating them by topic. 
How much participants liked each source's responses (see Appendix \ref{plot-source-like})/Jina{what will the appendix show? see appendix for x y z}, were significantly different (\textit{F}(3.0,5517.7) = 99.20, p < 0.001) across all help-seeking messages.  /Jina{double check it I made a correct revision. Did you mean it} The post-hoc analysis showed that the adult mentor's responses were participants' the most liked response (M=3.51, SD=0.02), followed by AI (M=3.46, SD=0.02), then the therapist's (M=3.29, SD=0.02). The peer responses were their least favorite (M=3.03, SD=0.02). This means that before considering the topic of the help-seeking message, it seemed like humans, specifically that of adult mentor,  outperformed AI in generating help-giving responses, although peer responses were not as liked by the participants. /Jina{this level of finding, with this level of clarity and detail and its interpretation is perfect} However, such responses varied after considering help-seeking topics, which we will discuss further in **. 
% Next, we wanted to understand how participants reacted to the different responses beyond which one they "liked" the most (i.e., preferred). We looked at aggregate responses for all help-seeking messages by the source to understand how helpful the responses were ("helpful"), how likely they were to send them ("would send"), and how inappropriate ("inappropriate") and problematic ("problematic") they felt the responses were. In subsequent sections and figures, we refer to these four measures as "attributes" of participants' responses.

Next, we break down reactions to the different responses (peer, adult mentor, therapist, and AI) by comparing: how helpful the response was, how likely participants were to send the response, how problematic the response was, and how inappropriate the response was). Positive attributes - how much they felt they would send a response and how helpful they thought it was - /Jina{this should have been in methods and here just go theough the findings. also it is confusing. what is positive attributes? you should just say helpful ess etc that was tested. readers dont have to learn more things and remember them for understadning the findings} followed the same pattern as participants' favorite/Jina{this should just be the most liked} responses. This means/Jina{notnsure jf I understand following the same pattern. Just say only what happened. like removing the previous sentence and right away saying the next sentence here} participants felt the adult mentor's responses were the most helpful (M=3.50, SD=0.99) of the responses presented and also indicated that participants were most likely to send the adult mentor's responses (M=3.48, SD=0.98), followed by AI's responses (how helpful: M=3.49, SD=1.05; likelihood to send: M=3.42, SD=1.12), then the therapist's responses (how helpful: M=3.29, SD=1.07; likelihood to send: M=3.25, SD=1.12), and the peer's responses receiving the lowest score for positive attributes (how helpful: M=3.02, SD=1.15; likelihood to send: M=3.00, SD=1.18). The negative attributes - how problematic and inappropriate participants felt the responses were - followed the exact opposite pattern as the positive attributes. According to our analyses, the peer responses were the most problematic and inappropriate (how problematic: M=2.32, SD=1.24; how inappropriate: M=2.30, SD = 1.24), followed by the therapist's responses (how problematic: M=2.19, SD=1.22; how inappropriate: M=2.18, SD=1.23), AI's responses (how problematic: M=2.13, SD=0.02; how inappropriate: M=2.12, SD=0.02), and the adult mentor's responses were seen as the least problematic (M=2.07, SD = 0.02) and inappropriate (M=2.05, SD = 0.02). See Figure \ref{fig:source-reactions}. 

\begin{figure}[!t]
    \centering
    \includegraphics[scale = 0.5]{figures/plot.source.reactions_2023.9.11.png}
    \caption{Participant reactions to responses by source. The x-axis is how much participants agreed with the different attributes of their reaction (helpful, inappropriate, problematic, and would send).}
    \label{fig:source-reactions}
\end{figure}

Our findings from RQ2-a suggest that participants may prefer a human response to help-seeking messages - however, these findings do not account for the nuance in real-life peer support exchanges. To address this, we present RQ2-b results on how reactions to human- and AI-generated responses vary depending on what they are responding to.

\subsection{RQ2-b: How do young people react to help-giving responses about 1) relationships, 2) suicidal thoughts, 3) self-expression, and 4) physical health?}
\textbf{\textit{Our results show that participants preferred AI-generated responses to help-seeking messages about relationships, self-expression, and physical health, but not suicidal thoughts.}} In the next four sections, we describe this finding in more detail and break down those preferences by the topic of the help-seeking messages: relationships ( section \ref{sec:relationships}), suicidal thoughts (section \ref{sec:suicidal-thoughts}), self-expression (section \ref{sec:self-expression}), and physical health (section \ref{sec:physical-health}). For each topic, we begin by with the quantitative results for each attribute of the responses, followed by quotes from open-ended responses from the participants to illustrate why they did, or did not, like each response. Results from the open-ended responses are described from most to least preferred responses within each scenario.

\subsubsection{Relationships}
\label{sec:relationships}
Participants' reactions to responses about relationships did vary significantly by source, and they preferred the response generated by AI. Our results show that not only did participants like the AI response the most, but they also felt it was the most helpful (M=3.63, SD=1.00), least problematic (M=2.01, SD=1.16), least inappropriate (M=2.01, SD=1.20), and that they were most likely to send it (M=3.65, SD=0.96). When discussing relationship issues, participants did not like the peer response. They liked the peer's response the least (M=3.00, SD=1.15) and felt it was the most negative (how problematic: M=2.41, SD=1.24; how inappropriate: M=2.38, SD=1.24) and least positive (how helpful: M=3.07, SD=1.13; likelihood to send: M=2.98, SD=1.17). See Figure \ref{fig:plot-relationships}. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/plot.relationships_2023.9.11.png}
    \caption{Reactions to responses by source for help-seeking message about relationships.}
    \label{fig:plot-relationships}
\end{figure}

This sentiment was reflected in the free-response questions, where participants noted that they liked the balance and empathy in the \textbf{AI-generated} responses. They felt the AI-generated response invited the help-seeker to share additional information without being overly intrusive or demanding. As one participant put it, the response was \textit{``helpful...
%The response has facts that are hard to hear but they are helpful. The message is 
[and] also supportive and feels like a safe space.''} (P453, Female, African American).
    %it also has ways of how to cope with the situation.. Participants noted that they liked how the AI response both offered support and presented actionable solutions: \textit{“This particular response says it all, it's absolutely what I'd say. What I like the most is that it tells [the friend] how to deal with the situation and still encourages [them].”} The response was \textit{"helpful...
%The response has facts that are hard to hear but they are helpful. The message is 
    %it also has ways of how to cope with the situation.
Some participants described anthropomorphic reasons, such as the AI-generated response seemed like it came from someone who is a good friend: \textit{``They are really trying to help the friend so much and we all need such friends.''} (P434, Female, African American). There were also mentions of qualities participants associated with the AI response, including that they thought it was \textit{``[empathetic]...supportive and caring.''} (P46, Male, Prefer not to say). Even though participants did favor the AI-generated response to the help-seeking message about relationships, they did note some room for improvement. Namely, that the response doesn't consider the entire context of the situation and \textit{``accuses the ex without listening to his side of the story.''} (P118, Male, Latino/Hispanic).

Participants noted that the
% human-generated responses 
\textbf{adult mentor's responses} also provided acknowledgment and validation, but it was potentially less useful and lacked clear direction. Those who liked this response noted that \textit{``it is respectful and...made [them] feel like the person understood [the help-seeker's] feelings.''} (P50, Male, African American). Participants also noted a sense of maturity in how the response did not judge the help-seeker: \textit{``...the [response] answered the question in a mature way by making the victim not feel offended by going back to the ex. The response is just showing him or her that is what we [humans] go through in terms of love life.''} (P403, Male, African American). Despite these positive attributes of the adult mentor's response, some participants felt it lacked concrete advice and did not give specific suggestions for what to do next. As mentioned in the previous paragraph, participants liked that the AI-generated response guided the help-seeker to provide additional detail in a gentle way - they did not feel the adult mentor's response had this same quality. Instead, participants felt the adult mentor's response was, as one participant said, \textit{``
%just about 
beating around the bush''} (P341, Male, Latino/Hispanic) and \textit{``
%it 
didn't provide a way of how to solve the situation clearly.''}

Participants liked the \textbf{therapist's response} because they felt it was extremely understanding and non-judgmental but noted that it seemed to delay giving actionable advice. Even though they did not know a therapist wrote one of the responses, they picked up on the professional tone: \textit{``This person provides professional remedy and ... [asks] the victim to share their mixed emotions and from there she/he will be in a position to offer strategies.''} (P481, Female, African American). They saw the response as \textit{``very empathetic without shaming the friend''} (P587, Female, African American), but noted that it felt like \textit{``scheduling [giving] help to next time when the [help-seeker] is in need of it now.''} (P503, Female, Native American). They appreciated the supportive tone but would have liked more concrete and immediate advice rather than beating around the bush and delaying support.

We received the most negative comments about the \textbf{peer's response} because participants felt it was terse, suggested hasty actions, and was not encouraging. While some appreciated the response's brevity, the way it was written came across as \textit{``too direct with no empathy.''} (P163, Male, African American). This lack of empathy made participants feel like the sender had a bad attitude and was being too tough on the help-seeker: \textit{``It sounds harsh and rude, and also it doesn't consider the feelings of the victim.''} (P452, Female, African American).

\subsubsection{Suicidal Thoughts}
\label{sec:suicidal-thoughts}
In response to help-seeking messages about suicidal thoughts, participants preferred the response from the adult mentor and reacted most negatively to AI's response. Among the responses presented, participants liked the adult mentor's response the most (M=3.59, SD=0.95) and felt the most positively (how helpful: M=3.61, SD=0.94; likelihood to send: M=3.56, SD=0.94) and least negatively about it (how problematic: M=2.04, SD=1.18; how inappropriate: M=2.00,	SD=1.20). They also liked AI's response the least (M=2.82, SD=1.19) and felt the most negative (how problematic: M=2.53, SD=1.26; how inappropriate: M=2.54, SD=1.27) and least positive about it (how helpful: M=2.93, SD=1.12; likelihood to send: M=2.71,	SD=1.21).
See Figure \ref{fig:plot-suicidal-thoughts}. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/plot.suicidal.thoughts_2023.9.11.png}
    \caption{Reactions to responses by source for help-seeking message about suicidal thoughts.}
    \label{fig:plot-suicidal-thoughts}
\end{figure}

When describing why they preferred the \textbf{adult mentor's response} to this sensitive topic, participants noted that they liked how it conveyed genuine concern by inviting the help-seeker to share more details and put effort over providing more support. \textit{``There’s a feeling of relating with the individual here. There’s a feeling of care and [that they're] really interested and [want] to understand the individual }
% plus boosting the individual’s confidence and also wanting to understand the individual’s 
\textit{[and their] situation.''} (P124, Male, African American).
% It’s the best to do in such situation, for someone who wants to really be there for such person.” 
The only area of improvement that participants mentioned for the adult mentor response is that the message could have been a little shorter, but did not note what content should be cut. 

The second most preferred response came from a \textbf{peer}, and participants felt it was superficial, inconsiderate, and did not sufficiently acknowledge the help-seeker's struggles. Interestingly, participants likened the peer response to an AI-generated response, saying it sounded \textit{``...typical of a bot''} (P478, Female, Asian). Unlike the adult mentor's response, participants did not like how the peer's response was \textit{``so shallow [and] does not give the victim...much [detail] on how to tackle the situation and [get] helped.''} (P403, Male, African American). 

Participants noted that the \textbf{therapist's response} immediately asked for more information in an attempt to ensure the help-seeker's safety - not knowing that this message was written by a clinician, some thought this sounded \textit{``professional''} while many others took it as intrusively asking for more information right away instead of offering support. \textit{``I think this response makes the person in need sink deeper into her trouble rather than pull her out. It's a bit inappropriate.''} (P451, Female, Native Hawaiian/Pacific Islander). Since the initial help-seeking message did not use the word "suicide," many participants also did not like that the therapist's response immediately drew that conclusion and felt that calling it out could come across as judgemental: \textit{``I hate the assumption about self harm and suicide. It feels really I'm going to insert myself into your life to fix it and doesn't feel friendly at all.''} (P621, Non-binary, Asian).

The \textbf{AI-generated} response overall performed the worst. While some appreciated that the response was \textit{``actually truthful about the person's ability,''} (P52, Male, African American) most thought the referral to a healthcare provider conveyed less desire to help in that moment. \textit{``Fine, you can’t provide help but that’s not the best way to put it. You could always have the right choice of words and making the right sentence in this situation before suggesting a mental health professional and not everybody will like the fact that they are referring to them as going crazy. Not really cool though.''} (P124, Male, African American).

\subsubsection{Self-Expression}
\label{sec:self-expression}
Participants' reactions to the responses about self-expression followed a similar pattern to the responses about relationships. We saw that participants preferred the response generated by AI for the help-seeking message about self-expression and reacted most negatively to the peer response. We found that participants liked AI's response the most (M=3.70, SD=0.98) and felt the most positively (how helpful: M=3.75, SD=0.94; likelihood to send: M=3.67, SD=1.00) and least negatively (how problematic: M=2.01, SD=1.22; how inappropriate: M=1.99, SD=1.18) about it. Participants also felt the least positively and most negatively about the peer response (how helpful: M=3.12, SD=1.09; likelihood to send: M=3.05, SD=1.15, how problematic: M=2.25, SD=1.19; how inappropriate: M=2.26, SD=1.23).
See Figure \ref{fig:plot-self-expression}.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/plot.self.expression_2023.9.11.png}
    \caption{Reactions to responses by source for help-seeking message about self-expression.}
    \label{fig:plot-self-expression}
\end{figure}

Participants liked that the \textbf{AI-generated response} conveyed guidance, support, and understanding. \textit{``I think a response like this can make the person feel like they've all been in this situation before, and there are points of empathy that they can draw on to guide them to be braver by drawing on the respondent's situation.''} (P43, Male, Caucasian). Similar to the message about relationships, participants liked that this response \textit{``[empathizes] with the friend while also providing practical solutions''} (P587, Female, African American). 

They felt the response from the \textbf{adult mentor} also conveyed some affirmation of the help-seeker's struggles, but to a lesser extent. They liked that \textit{``it starts with sympathy''} (P160, Male, Prefer not to say), but the overall tone felt \textit{``unattached.''} This distinction between sympathy and empathy is important to note - as sympathy is feeling for someone else while empathy is feeling with them. The adult mentor's response conveyed "sympathy," meaning they can see where the help-seeker is coming from, but \textit{not empathy}, which implies less personal experience with the matter at hand. Participants clearly communicated this sentiment by saying that \textit{``the victim is not understood''} (P383, Male, African American) and that the message indicates \textit{``the person [who wrote it] has no idea of what the [help-seeker] is going through.''} (P611, Female, African American).
% the message \textit{"[gave] the impression that someone should act rudely and not care what others think.”} 

Similar to the relationship help-seeking message, participants suspected that the \textbf{therapist's} message came from a clinician, \textit{``The message looks like one a professional therapist would send...''} (P350, Male, Mixed Race). As one participant said, \textit{``The response is appropriate because [it] is from [a] counselor, someone who has been able to tackle much of the issues by being exposed to different clients and knowing what to do for certain client till they reach a point of believing in themselves and having that courage to talk to anyone without any fear.''} (P403, Male, African American).

The \textbf{peer's response} simply did not feel supportive enough to participants and did not do enough to calm the help-seeker, \textit{``I think that's too casual a response to really consider the issue from the perspective of the person pouring it out.''} (P21, Male, Caucasian). Moreover, they felt this response lacked depth and oversimplified the help-seeker's fear of self-expression, \textit{"I think that's too casual a response to really consider the issue from the perspective of the person pouring it out.”} Like the adult mentor response, participants also felt there was not enough of an indication that the person who wrote the response truly understands what the help-seeker is going through, but less so because they can't empathize and more because they do not want to put effort into conveying that empathy, \textit{``It was too brief and nothing more of empathy felt in it. It was more like this person wanted to help but didn’t really put much % of 
effort [into] it...
% Though it was having 
[it had] a little spark of encouragement[,] but it could be better.''} (P124, Male, African American).

\subsubsection{Physical Health}
\label{sec:physical-health}
When the help-seeking message was about physical health, participants once again preferred AI's response and did not like the peer response. The results show that participants liked AI's response the most (M=3.71, SD=0.96), felt the most positively about it (how helpful: M=3.67, SD=0.99; likelihood to send: M=3.64, SD=0.99), and the least negatively (how problematic: M=1.95, SD=1.16; how inappropriate: M=1.95, SD=1.21). Participants also felt the most negatively and least positively about the peer's response (how problematic: M=2.46, SD=1.28; how inappropriate: M=2.40, SD=1.27; how helpful: M=2.73, SD=1.22; likelihood to send: M=2.78, SD=1.23).
See Figure \ref{fig:plot-physical-health}.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/plot.physical.health_2023.9.11.png}
    \caption{Reactions to responses by source for help-seeking message about physical health.}
    \label{fig:plot-physical-health}
\end{figure}

The \textbf{AI-generated} response once again performed the best, and participants raved about how much they liked it - as one participant said, "I didn't just like this response. I love this response."
% because apart from being there for the person, you even helping and suggesting professional help for the person.” because 
Participants describe how the answer contained all the important components: empathy, acknowledgment, and concrete suggestions for next steps, \textit{"its an all round genuine answer [that] shows you care[,] understand the problem and offer the right solutions.”} The "right solution," in this case, was to continue with ongoing self-care work (i.e., talking to a counselor), and participants liked that this response acknowledged doing so is not easy. \textit{"The fact that he empathized with the person and encouraged them to further try [counseling] because you cannot get the intended results after one trial.”} Participants also liked that counseling was just one of the multiple solutions the response discussed and
%"the response 
\textit{"shows the [help-seeker] how they can use other strategies to be okay."} The comprehensive and deeply empathetic nature of this response seems to be what set it apart from the others.
% apart from counseling. it's also empathetic and it has words of affirmations .” 

Participants did like that the \textbf{adult mentor}'s response \textit{"[validated] wanting rest"}, but also felt that it \textit{"[made] the [help-seeker] feel as if it's OK to just relax and not do anything."} They discussed how the adult mentor's message did not acknowledge that self-care is more than relaxation. In doing so, this response seemed to convey that there is nothing more the help-seeker can do, \textit{“I feel like it's not addressing the issue at hand and makes the victim feel like they are doing great of which they are not.”} While participants thought \textit{"praising the [help-seeker] for small achievement[s]”} and \textit{"positive energy"} were good, they were not enough, \textit{"because 
% I think that 
it doesn't contain enough [advice] that can help the victimized person”} in this situation.

While the \textbf{therapist}'s response did offer a solution, participants did not think it was the right one: \textit{“It's very unclear whether this respondent wants to help out. They are telling the victim to keep pursuing the same course that ain't working for them.”} Unlike the AI-generated response, which suggested continued counseling in addition other solutions, participants did not like that the therapist's response was \textit{"just
% practically 
telling the person in question to [continue]
% base only on 
counselling, [with] no other options to explore.” } Therapy also incurs a cost for the help-seeker, which participants were not shy to mention in their feedback for this response. They noted that \textit{"counselling can be [quite] expensive,"} and increasing those costs might not be necessary because \textit{"
%although yes counseling helps sometimes but at this time it wont work cause 
at this point [the help-seeker] needs love and support from family and friends who would be available to support them.”} This does not mean participants wanted the response to suggest the help-seeker stop counseling altogether, but rather that there should be additional non-clinical suggestions.


% \begin{table*}[]
% \centering
% \begin{tabular}{|c|c|}
% \hline
% \textbf{Topic of Help-Seeking Message} & \textbf{Source of Best Response} \\ \hline
% Relationships & AI \\ \hline
% Suicidal Thoughts & Human \\ \hline
% Self-Expression & AI \\ \hline
% Physical Health & AI \\ \hline
% \end{tabular}
% \caption{Source of the best-performing response (human or AI) to help-seeking messages about different topics.}
% \label{tab:best-source}
% \end{table*}

% We summarize these findings to answer RQ2 in table \ref{tab:best-source}, which outlines which 
% source (human or AI) performed the best for all attributes of participants' responses for each scenario. The best-performing response was the most preferred, most likely to be sent, most helpful, least problematic, and least inappropriate.

In summary, our findings revealed that participants preferred AI-generated responses about less sensitive topics (relationships, self-expression, and physical health). For more sensitive discussions (suicidal thoughts), participants preferred responses from the adult mentor. In the next section, we discuss the implications of these findings.

==> original-submission/0-Abstract-old.tex <==

Generative artificial intelligence (AI) is integrated into everyday technology, including news, education, and social media. AI has further pervaded private conversations as conversational partners, auto-completion, and response suggestions. As social media becomes young people's main method of peer support exchange, we need to understand when and how AI can facilitate and assist in such exchanges in a beneficial, safe, and socially appropriate way. We asked 622 young people to complete an online survey and evaluate blinded human- and AI-generated responses to help-seeking messages. We found that participants preferred the AI-generated response to situations about relationships, self-expression, and physical health. However, when addressing a sensitive topic, like suicidal thoughts, young people preferred the human response. We also discuss the role of training in online peer support exchange and its implications for supporting young people's well-being. Note: This paper includes sensitive topics, including suicide ideation. Reader discretion is advised.

% Tools and systems using generative AI models are pervading every sector of our society, including education, finance, and health. Especially when it comes to AI models being used for younger populations,

% CHI researchers increasingly explore the role of and people’s perceptions toward generative AI models in various tools and contexts. Given the explosion of possibilities of AI-enabled solutions for sensitive topics and populations such as young people’s mental health, it is critical to examine how young people perceive of AI…

% The internet provides many opportunities for youth peer support exchange, but there is limited knowledge about the most helpful responses to offer in such situations. To address this, we asked 622 young people to complete an online survey and evaluate human- and AI-generated responses to help-seeking messages. We found that participants preferred the AI-generated response to situations about relationships, self-expression, and physical health. However, when the help-seeking message was about a sensitive topic, like suicidal thoughts, participants preferred the researcher's response. We also discuss the role of training in online peer support exchange and its implications for supporting young people's well-being. Note: This paper includes sensitive topics, including suicide ideation. Reader discretion is advised.

% In aggregate, we found that participants liked the researcher's responses the most, with AI as a close second. However, nuances emerged depending on the context of the help-seeking message, and 
% rather than the sources, which represent different types and levels of training. 

==> original-submission/1-Introduction-old.tex <==
\section{Introduction}
% As the number of individuals connecting to the internet continues to grow, driven by the steady expansion of social media platforms, it's noteworthy that 
Young people are at the forefront of online interactions, both in terms of 
% how often they use the internet 
frequency and the speed at which they use online tools.
% so with adolescents and young adults being the most avid users of social media 
An estimated 90\% of young adults are active on social media ~\cite{perrin2015social}, and they
% , a staggering increase from the mere 12\% recorded in 2005— making it a substantial 78-percentage point surge in usage rates (source: "Adolescent and Young Adult Use of Social Media for Health and Its Implications"). . 
% A recent study conducted by Pew Research Center found that 92\% of teenagers access the internet on a daily basis, with 24\% describing their online presence as "almost constant."
% In recent years, young adults have 
harness the power of these platforms in diverse ways. Notably, 79\% of young adults have turned to the web to seek health-related information, and 33\% have sought information pertaining to mental health. \cite{vogels2022teens} 
% \Afsaneh{(source: **https://pdxscholar.library.pdx.edu/cgi/viewcontent.cgi?article=1074&context=rri_facpubs**).}
However, various barriers exist, hindering young people's access to mental health care. These barriers include the difficulty of seeking professional support for mental health issues with more young people seeking information on how to receive professional support for their mental health while asking to be ‘taken seriously’ as described by Lavis and Winter\cite{lavis2020online}.
% (#Online harms or benefits? An ethnographic analysis of the positives and negatives of peer-support around self-harm on social media) 
Moreover, young adults are dealing with a pervasive stigma surrounding mental health diagnoses, and challenges related to accessing mental health services \cite{gowen2013online}. Consequently, researchers~\cite{gowen2013online,best2016seeking,burns2014enhancing} have determined that young individuals are increasingly exploring alternatives, such as online forums and social media groups, where they can find support and advice from peers who have encountered similar challenges\cite{ali2015online,gowen2013online}. 
In doing so, they naturally form communities or join one.
% and with peer-to-peer connections on the rise, young adults seeking to engage with one another and turning to social media platforms as a space to share their experiences with illness, seek guidance, and provide mutual support.  

SIGCHI researchers~\cite{razi2023aCSCW,naslund2016future,armstrong2009patient}, have thoroughly investigated the significance of online peer support in the lives of youth, discovering that while peers would like to offer support they sometimes do not know how to help or feel the disclosure was inauthentic~\cite{huh2023help}. Furthermore, peer support providers also struggle to maintain boundaries to express their difficulties in writing supportive and empathic responses due to lack of role clarity~\cite{kemp2012}. The notation of education as a solution to the lack of expertise was validated by a later study where researchers \cite{sharma2023human} developed an AI system called '\textit{Hailey'} which helped develop more empathetic responses to support seekers in a  mental health peer support platform.
% ; they found the human -AI collaboration enables more emphatic conversation in text based peer to peer mental health support. 
AI limitations such as their inability to understand human nuances~\cite{bishop2021artificial} have led to continued efforts to explore the potential of AI as a supplementary source of support for youth. AI-driven systems, such as Large Language Models (LLMs), chatbots, or virtual assistants, hold promise in providing accessible and non-judgmental support, filling gaps where traditional peer support may fall short\cite{ahn2020chatbot}.   However, the youth's norms around peer support providing and the extent to which AI can effectively address the support needs of youth based on the frequent support-seeking topics of youth and the practical considerations remain areas of ongoing investigation \cite{fulmer2019artificial}.
% (Fulmer, Russell. (2019). Artificial intelligence and counseling: Four levels of implementation. Theory & Psychology. 29. 095935431985304. 10.1177/0959354319853045.)

To address these gaps in the literature, we proposed the following research question: 
\textit{What are young people's preferences regarding human- and AI-generated help-giving responses (a) overall, (b) by topic, and (c) why?}
% \item [RQ1:] \textit{ What are young people's preferences regarding human and AI-generated help-giving responses?}
% \item [RQ2:] \textit{How do young people's preferences for help-giving responses vary depending on the topic of the initial help-seeking message?}
% \item \textit{a)How do these preferences vary depending on the topic of the help-seeking messages?}
% \item \textit{b)What are the potential reasons behind this preference?}
To answer our research question, we analyzed 622 survey responses from young people with their preferences about pre-written responses (from AI, therapist, adult mentor, and peer)  to four help-seeking messages on topics of relationships, suicidal thoughts, self-expression, or physical health. 
We found that young adults preferred AI-generated responses about less sensitive topics (relationships, self-expression, and physical health). For more sensitive discussions (suicidal thoughts), participants preferred responses from the adult mentor.
Our study contributes to the Human-Computer Interaction (HCI) research community in several ways. This paper provides insights into how young people perceive AI-generated responses in peer support situations. Our results also identify the popular conversational topics among young people where AI-generated responses are, and are not, well received. The findings bring implications for designing AI-powered systems to safely and effectively help youth to support each other.
% \begin{itemize}
%     \item This paper provides insights into how young people perceive AI-generated responses in peer support situations.
%     \item Our results identify the popular conversational topics among young people where AI-generated responses are, and are not, well received.
%     \item The findings bring implications for designing AI-powered systems to safely and effectively help youth to support each other.
% \end{itemize}

% How do young adults perceive different responses to different help-seeking messages:
% - what is the overall preference?
% - does that change depending on the topic?
% - why? what are potential reasons behind these preferences?


% Motivation: 1 paragraph about stats for how young adults use social media, how it's beneficial and detrimental, how young adults seek support + stats for that, give overview for topics discussed with stats
% previous research/gaps to motivate study: 1 paragraph about what previous research has done in terms of support-seeking of youth and how peers sometimes can't provide support per help me paper and how AI might be helpful to provide support. 
% End with "in order to address these gaps, we have xyz research questions, then to address these research questions we did ABC then outline main important findings then contributions" 
% How participants' perceptions about the extent they could relate, help, and sympathize with the help-seeking messages were related to their demographics and how much they liked the responses from different sources? }
% To what extent could participants relate, help, and sympathize with the help-seeking messages based on their demographics? and how those perceptions were related to how much participants liked the different responses?  }
% How do young adults feel about the topics that frequently come up in online peer support conversations?
% How do young adults feel about responses generated by different sources (a young adult peer, an adult researcher, an adult mental health professional, and artificial intelligence)? % need to specify that they don't know the source?
% /Jina{react is too generic and not a strong motivation for why it is researched}


\begin{comment}
RQ ideas:
- How do individual differences (demographic factors and experience giving/seeking support) impact (1) preferences of responses or (2) relatability of scenarios?
- How do young adults feel about their ability to relate to, sympathize with, and help a friend who is initiating a peer support conversation?
- Without knowing the content source, do young adults prefer a response generated by a human or AI?
- Do youth prefer a response generated by a person, or AI? RQ2a: Do youth reveal anything about peer support exchange norms based on their preferences for responses written by AI or human sources? RQ2b: without knowing the source of responses presented, do youth prefer content generated by (a) a peer, (b) an adult who is NOT a mental health professional ("researcher"), (c) a mental health professional (therapist), or (d) an AI chatbot (ChatGPT)
% How do young adults' preferences for those responses vary depending on (a) previous experience giving and receiving peer support online, (b) the different topics for which young adults seek support, (c) the relatability of those topics? % does relatability/ability to sympathize/ability to help impact preferences for different responses?

% \item [RQ3:] \textit{What can young adults tell us about their preferences for certain responses during peer support conversations?} \Jordyn{2-gram and 3-gram for open-ended questions to explain preferences}
\end{comment}





% • This is the first study to provide insights into support exchanges shared through the social media-linked private messaging platforms (SMPM) among youth.
% • This paper provides insights into dynamics and topics youth
% discussed in their unmoderated social support exchanges
% and online self-disclosures of youth followed by implications
% for design in supporting youth mental health.
% • The results bring implications for designing systems based
% on the unique benefits and potential challenges of SMPMbased support for youth.

% \begin{itemize}
%     \item Identify conversational topics where AI-generated responses can help in peer support.
%     \item Discuss 
% \end{itemize}

==> original-submission/2-Related_Work-old.tex <==
% 1.5 pages total
\section{Related Work}
% \subsection{Online Peer Support for Youth}
% what is social support and why is it important
% Digitization of social support
% In the 21st century, social support interactions are moving to digital spaces. 

% In the pre-smartphone era, texting was the preferred method of communication among youth \cite{nabi2013facebook}. However, now that roughly 96\% of young adults in America have a smartphone \cite{perrin2021mobile}, social media has emerged as the preferred locus of communication exchange.

\subsection{Mental Well-Being of Young Adults and Online Social Support}
% problems around mental well-being and how support is needed
More than 450 million people around the world struggle with mental illness \cite{saraceno2002world}, and young adults are disproportionately likely to be among those who are suffering \cite{jurewicz2015mental}. In a cross-country survey, 
% of 13,984 students from 19 colleges across eight countries, the 
World Health Organization found that nearly one-third of college students tested positive for at least one mental health disorder \cite{auerbach2018world}. Furthermore, mental illnesses like depression, substance use disorders, and psychosis are some of the biggest risk factors for suicide \cite{braadvik2018suicide}, which is the second-leading cause of death for teens and young adults \cite{curtin2022provisional}. With professional treatment being less affordable and less accessible than ever before \cite{kanagaraj2020why}, internet interventions are emerging as a promising avenue for formal treatment \cite{cunningham2014internet} and informal peer support \cite{woodruff2007evaluation}.

% HCI and online support
Social media platforms are some of the most-visited websites on the internet, with some sites getting an estimated 1.7 billion visits every 6 months \cite{statista2021}. 
Researchers \cite{ridout2018use} suggested that young people can benefit from online support exchanges on social medi platforms; for example, actively engaging with peers online about mental health concerns is associated with an increased likelihood of seeking formal mental health care \cite{ridout2018use}. Unique platform affordances, like anonymity, can help users feel more comfortable being honest about their experiences and feedback \cite{de2014mental}. Also, support exchange on social media can lead to increased quality of life, heightened perceived support, and increased self-efficacy \cite{uehara1990dual}.
Peer support is a system of giving and receiving help founded on the principles of respect, shared responsibility, and an agreement of what is helpful \cite{mead2001peer}. 

% - discuss two paragraphs of problems around mental well-being and how support is needed
% - https://bmjopen.bmj.com/content/12/8/e061336.abstract
% - use this to talk about the wellbeing problems that are prevalent
% - and transition to the need for peer support, and how online peer support is studied increasingly at HCI


% Human-computer interaction focuses on the design of computer technology between humans and computers, with its roots being found in the 1950s\cite{card2018psychology}.  It wasn't until the 1970s when the intersection of cognitive engineering with computer science and technology brought the psychological aspects of HCI to the forefront\cite{newell1985prospects}.  However, during the early 1980s, there was skepticism regarding the adoption of automation in mental health, primarily stemming from a limited grasp of the psychological intricacies involved\cite{balcombe2022human}.   With the continuous rise and importance of HCI in technological development, its importance cannot be overstated, with more research within the last few decades emphasizing the potential for self-help methods and the need for better system design.

% Social support is a powerful and important part of youth. Years of research point to the benefits of sharing challenging experiences with loved ones who provide support through tough times \cite{reinecke2014authenticity,kim2011facebook,grieve2016psychological}. Such disclosures can help individuals feel more confident \cite{davidson1999peer, salzer2002consumer}, more empowered \cite{davidson1999peer,dumont2002findings,ochocka2006longitudinal,resnick2008integrating}, and more accepting of themselves \cite{shilo2011effects}. Studies also show that peer support can moderate prosocial behaviors \cite{lockwood2014emotion}, schooling \cite{eklund2017adolescent}, physical health \cite{la2002peer}, physical activity \cite{hamilton2017role}, and social functioning \cite{kurtz1990self,nelson2006longitudinal,ochocka2006longitudinal,trainor1997beyond,yanos2001consumer}. 
% However, in the context of mental health, peer support is referred to as the support that individuals with mental illness or learning disabilities can provide to each other \cite{shalaby2020peer}. 


% We also live in a society with the highest rates of mental illness and the lowest access to mental health resources, making people turn to social media as an accessible and free avenue for connection. There are 57.8 million Americans struggling with mental illness \cite{nimh-mental-illness}, and more than 450 million people around the world who have similar concerns \cite{saraceno2002world}, while access to treatment is less affordable and less accessible than ever before \cite{kanagaraj2020why}. As a result, we see a rise of social network-based online interventions that enable connections and support \cite{rayland2023social}.
% among 3.6 billion social media users globally \cite{kanchan2023social}.
% , we see the rise of social sharing where individuals are sharing more information with peers  and as mental heath services continues becomes more inaccessibility\cite{rayland2023social} this become increasing true in more individuals accessing free and widely available support where they mostly discover peer support and networks. 

% With individuals being more willingness to to share or reveal aspects of their identity or experiences so they are not stigmatized or socially rejected. 
% Studies have shown that online forums that allow for anonymous interactions, like Reddit, provide a conducive environment for users to connect and disclose information. 
% Anonymity makes users feel more comfortable being honest with their experiences and feedback, especially around mental health challenges \cite{de2014mental}. However, there are still challenges that hinder disclosures during online peer-to-peer interactions. Lack of professional oversight and propagation of misinformation means there is a risk of well-intentioned, but misguided, advice circulating within online peer networks \cite{swire2020public}
% One prominent challenge is the lack of professional oversight and the potential for misinformation that take place on peer to peer support platforms. Without the guidance of mental health experts, there is a risk of well-intentioned but misguided advice circulating within these peer networks \cite{swire2020public}.
% Bad actors can also take advantage of the anonymity and openness in online spaces to engage in cyberbullying and other online harms, which is detrimental to users who are there to seek support \cite{rainie2017future}

% with the encouragement of open sharing and the anonymity some platforms offer, there is a concern for instances of cyber-bullying or harmful interactions, which can have detrimental effects on individuals seeking support\cite{rainie2017future}


% challenges in online peer interactions
%Given this recent transition to online mediums, the HCI and SIGCHI community is working to understand both the risks and benefits of digitizing social support \cite{decieux2019social}.  Research does suggest that young people can benefit from support exchange on social media, which perhaps explains its increasing prevalence. For example, social media support exchange can have benefits such as heightened perceived support, increased quality of life, or increased self-efficacy \cite{uehara1990dual}. Also, actively engaging with peers online about mental health concerns is associated with an increased likelihood of seeking formal mental health care \cite{ridout2018use}. However, not all of the exchanges on these platforms are beneficial \cite{Sharma2021}

% how youth use social media and internet and some of the content analysis studies that look into those%

\subsection{AI-Powered Mental Health Support}
Artificial intelligence (AI) systems are rapidly becoming more sophisticated and have tremendous potential to transform many fields, including mental health \cite{folstad2017chatbots,brandtzaeg2018chatbots}. Generative AI systems, like ChatGPT \footnote{https://chat.openai.com/} and Google Bard \footnote{https://bard.google.com/}, are machine learning models that can create human-like responses for accessible, affordable, and individualized support \cite{singh2023artificial}. 
In the past year, various ways in which ChatGPT can support mental health have been explored and archived in non-peer-reviewed venues %\Jordyn{ADD CITE!}
, given the short time frame since the technology became available. For instance, researchers explored ChatGPT as a therapist assistant \cite{eshghie2023chatgpt}, where it can work as a companion for patients in between therapy sessions, collecting information, listening to patients attentively, offering validation and sharing potential coping strategies. Another study (again non-empirical, non-peer-reviewed) examined the possibilities of using ChatGPT for child mental health \cite{imran2023chat}. Possibilities of the use of generative AI here included medical education for children, translation and assisting in provider-child patient communication, and access to medical information. Similar possibilities have been discussed in \cite{van2023artificial} and \cite{kizito2023chatgpt}, especially when the health condition can benefit from anonymity in accessing information \cite{kizito2023chatgpt}.
Automated mental health support cannot replace human therapists due to its significant inconsistencies and low reliability \cite{farhat2023chatgpt}, and doing so would also undermine the personal connection that is the foundation for why young people engage in online peer support. 

Research about the outcomes of implementing AI systems for mental health is mixed. For example, an analysis of user review comments found that users had mostly positive experiences with AI chatbots for symptoms of anxiety and depression \cite{ahmed_thematic_2022}, and surveys of chatbot systems can suggest that they are useful reporting tools for in-person harms \cite{rita2021chatbot} and can even help to increase youth participation in societal activities \cite{vaananen2020civicbots}. 
However, Martinengo et al. examined dialogues with AI conversational agents (CAs) and found that CAs from app stores are \textit{not} fit for comprehensive suicide risk management. According to their findings, this is because AI systems follow a predefined protocol for suicidal thoughts that is only activated in response to specific phrases that suggest immediate danger, meaning they cannot identify when a conversation is moving towards a problematic topic. Another issue is that CAs cannot send an unsolicited follow-up message after the conversation concludes to ensure the user is safe \cite{martinengo2022evaluation}. 

Therefore, it is important to understand better how AI can maximize its ability to support young people by assisting in conversations \cite{Shao2023empathetic}. For instance, Sharma et al. \cite{sharma2023human} experimented with an AI agent that provides just-in-time feedback to peer support providers in an online mental health support platform and found that AI can help peers increase empathy in their support-giving messages. Although they did not focus on youth in their study and only focused on empathy. As having empathy may not always be the most helpful way to respond (e.g., when support seekers are looking for concrete actions)- best practices in peer support should also be investigated. 

% - Talk about some recent work on using chatgpt for therapy purposes
% https://www.ncbi.nlm.nih.gov/pmc/articles/PMC10187878/
% https://link.springer.com/article/10.1007/s10439-023-03326-7
% https://www.pjms.org.pk/index.php/pjms/article/view/8118
% - Any effort to automate mental health support in any forms
% - but point out that this is all trying to replace human therapists, and it's not what young people, shown from online peer support, would like doing
% - We need better novel ways to understand how AI can maximize its ability to support young people


% The early days of computer-mediated communication consisted of digitally transmitting human-generated messages \cite{kiesler1984social}, but AI systems enable humans and computers to work together to make that content. 
% what is AI and how popular is it?
% Artificial intelligence (AI) systems are rapidly becoming more sophisticated and widely used. Conversational and generative AI, like ChatGPT \footnote{https://chat.openai.com/} and Google Bard \footnote{https://bard.google.com/}, are machine learning models that can create new content by learning patterns and structures from existing data. Similar models have been deployed in a variety of contexts, including education \cite{okonkwo2021chatbots}, hospitality \cite{buhalis2022voice}, and healthcare for both physical \cite{tjiptomongsoguno2020medical} and mental \cite{folstad2017chatbots,brandtzaeg2018chatbots} concerns. 

% what do we know about the result of using AI?

% \subsection{AI and Peer Support}
% human expectations for AI
% Human-AI collaboration 
% Previous literature~\cite{sharma2023human,sannon_i_2020} has also investigated various people's expectations and behaviors in interactions with AI and conversational agents, including human-agent data-sharing practices and privacy violations~\cite{sannon_i_2020}

%
 
 
\subsection{Gaps on Perceptions Toward Supportive AI Systems}
Researchers~\cite{carlbring2023new} note the shortcomings of these technologies, lacking in personalization, ethical considerations, recalling previous sessions, and detecting body gestures and expressions. At the same time, researchers highlight the lack of accuracy, reliability, bias, and unpredictability of outputs of these generative AI systems \cite{mardikaningsih2023risk}, calling for appropriate mitigation strategies, awareness, and careful consideration of these challenges before jumping into experimenting the possibilities of generative AI on sensitive topics, such as high-risk mental health conversations (e.g., suicide ideation).

Numerous factors have been associated with the perceived trustworthiness of generative AI systems, including

The common shortcomings of these existing works include empirical testing of how end users might perceive these generative AI-powered systems that support mental health. Our study systematically investigated young adults' perceptions of how helpful, inappropriate, and problematic AI-generated responses are compared to multiple human-generated responses. These tests were conducted blinded, thus allowing us to objectively evaluate initial reactions to the style of the responses themselves rather than young adults' preconceptions around AI. 

% There are two important limitations to this growing body of work that we would like to note. First, most of the studies focus specifically on adults (e.g., \cite{boulos2021iterative,lee2023}. Young adults have their own unique support needs that they often turn to online peer support for \cite{huh2023help} - if technology is going to integrate into settings to provide help to youth specifically, we need to understand how and when they can be most effective. Second, these studies involve designs where users know they are interacting with AI, which introduces additional user expectations and preconceptions about the system rather than the content itself \cite{kocielnik2019will}. These gaps present areas of opportunity to understand how we can design AI tools to facilitate effective support for young people, which we explore in the present study

% In this paper, we address this gap in our understanding to identify popular conversational topics among young people where AI-generated responses are, and are not, well received.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% MISC OLD TEXT %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Some benefits they reported experiencing included increased confidence and affirmation, improved symptom detection, helpful recommendations, affordable consultation, and feelings of support for loneliness. Not all feedback was positive, though -- some users noted issues regarding usability, app updates, privacy issues, and non-creative conversation \cite{ahmed_thematic_2022}.
% by offering help when in-person treatment is unavailable, or the stigma is too great to overcome alone.
  
% The first of these chatbots was called ELIZA, which was designed to respond in a Rogerian style of psychotherapy \cite{weizenbaum1967contextual}. Since ELIZA, we have seen many chatbots and other AI-powered applications to provide mental health support, like Woebot \cite{fitzpatrick2017delivering} and HAILEY \cite{sharma2023human}. Cuijpers et al. analyzed 23 randomized controlled trials for conversational AI tools and found that some applications were as effective as standard face-to-face care \cite{cuijpers2009computer}.

% Human-AI collaboration literature~\cite{sannon_i_2020} has also investigated various people's expectations and behaviors interactions with AI and conversational agents including human-agent data-sharing practices and privacy violations~\cite{sannon_i_2020}


% Moreover, After conducting various research activities to explore the effectiveness of chatbot in youth mental health, Koulouri \& Macredie describe their findings as an acceptable solution to offering mental health support for young adults. With a push for user-centered approach during the development of these applications\cite{koulouri_chatbots_2022}. 

% \cite{d2017artificial}.\cite{boulos2021iterative}. ,~\cite{ahmed_thematic_2022} found that chatbot apps for anxiety and depression provided positive experiences for people, including building confidence and affirmation, symptom detection, helpful recommendations, and affordable consultation, and providing support for loneliness as a companion by analyzing users reviews on 11 apps. Although users had negative reviews regarding usability, app updates, privacy issues, and non-creative conversation.


% conversations as conversational partners, auto-completion, and response suggestions. A

% AI is a popular technology that can be used to provide support and information, especially among young people \cite{koulouri_chatbots_2022}, although it is not a current substitute for human interaction,  in a comprehensive analysis of experts' opinions on the impact of artificial intelligence and networked technology by Pew Research\cite{anderson2018artificial}, most respondents expressed optimism about the potential for AI to enhance human capabilities and empower individuals by 2030 with potential benefits of AI’s role to be seen in healthcare, education and more.

% With an increase in mobile apps using chatbots to provide support for mental health issues. More researchers are highlighting different ways in which AI can provide support within mental health and understanding the context in which AI is being used is crucial in the realm of our study. \cite{d2017artificial}.\cite{boulos2021iterative}. ,~\cite{ahmed_thematic_2022} found that chatbot apps for anxiety and depression provided positive experiences for people, including building confidence and affirmation, symptom detection, helpful recommendations, and affordable consultation, and providing support for loneliness as a companion by analyzing users reviews on 11 apps. Although users had negative reviews regarding usability, app updates, privacy issues, and non-creative conversation.



% Petter Bae Bae Brandtzæg, Marita Skjuve, Kim Kristoffer Kristoffer Dysthe, and Asbjørn Følstad. 2021. When the social becomes non-human: young people's perception of social support in chatbots. In Proceedings of the 2021 CHI Conference on Human Factors in Computing Systems (CHI'21). Association for Computing Machinery, New York, NY, USA, Article 257. 1–13.


% and that technology is increasingly integrated with generative artificial intelligence (AI). Generative AI, like ChatGPT and Google Bard, are machine learning models that use input training data to pick up on its patterns and structures and then generate new data with similar characteristics. 

% HCI researchers have also investigated \edit{the} design and implementation of moderated peer support to facilitate support for youth in specific situations such as the youth with intellectual disability~\cite{banos2018Evaluation}, children surviving cancer~\cite{Lindberg2014Designingpeercancer}, or youth living with human immunodeficiency virus (HIV)~\cite{Karusala2021Courage}.
% Although depending on the context, peer support could have different effects\edit{; for instance,} it could be distressing when the support is judgemental and disrespectful~\cite{takahashi2009potential}. Therefore, \edit{studying how youth peer support happens in social media without moderating specific topics is essential.}



% \subsection{outline - AI in Human Communication}
% AI is an exciting new tool that's being used in a lot of new areas and one of those areas is interpersonal support and mental health applications, and that that is particularly important in a time where like a lot of young people need mental health treatment and help. We know there are a lot fo barriers to young people getting mental health treatment - not knowing who to go to, limited access to health insurance, financial constraints, stigmatization, etc. like especially coming out of the pandemic there we saw so many people who needed mental health treatment that couldn't get it.

% AI is becoming so integrated into interpersonal communication, e.g. autocompletion, Grammarly, etc., so many messages are not purely human-generated content, rather they're the result of a collaboration between humans and AI - we don't understand how people are necessarily responding to that content like not knowing that it came, not knowing where it's coming from.


% AI is a scalable, lo-cost tool to help alleviate some of those challenges, and we're only beginning to understand AI's potential to help in those situations.
% insert some citations of like for example like people have explored the benefits of using like those different chatbots like woebot and Haley and all of those talk about the research behind those and kind of what we know and then.

% But within these conversations, like how our how do you, umm users feel about the actual communications and like the exchange, the details of the exchanges that they're receiving? are they helpful or trying to think like are they being designed in a way that's helpful and also like? Are they helpful across the board or are they only helpful in certain scenarios?
% And then to address that, we took a deeper dive until like the content.

% Researchers have explored many applications of AI, but few, if any, looked at how people react when they do not know what is the source of that response, how they would react to that response?


% like AI is presenting and that kind of also goes with the flow that we do with the abstract of like AI is presenting all these new opportunities for like you know application and we see people already applying it in mental health spaces insert citations of like, you know all the like, talk about those studies. human computer interaction researchers have been looking at, and then they'll be like a human AI interaction section.
% 
% But by telling people that they're interacting with AI like we're getting more of a response to like how they feel about the content, knowing that it's from AI, not just the content itself.
% So there hasn't really been an assessment of like just looking at the message itself.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% FROM DR. RAZI'S PROPOSAL %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% They are being vastly used for different applications such as education [2], healthcare [3], customer service, healthy lifestyle, wellbeing [4], and support for sexual abuse survivors [5]. For instance, CAs can engage in empathic, non-judgmental conversations to offer support to users and guide them through psychotherapeutic exercise, but suicide risk management interventions cannot be provided by conversational agents [4]. 

% Rita and Shava [13] tested a prototype of a website with a chat bot with youth around reporting sex offenders and found it useful for youth in Namibia. The study by Crutzen et al. [14] suggested that youth prefer chatbots when accessing information about sex, drugs, and alcohol. According to Fitzpatrick et al [15], conversational agents appear to be an effective way to deliver therapy to youth who need cognitive behavior therapy. In another study, Väänänen et al. [16] created a chatbot to support youth in societal development participation. They created three scenarios for the chatbot to understand youth’s perceptions in an online survey with positive and negative sides of using chatbots. They found that youth think that the chatbot can provide equality and engage with them better than a real person, but they had privacy concerns.
% [1]	A. B. Kocaballi et al., “The Personalization of Conversational Agents in Health Care: 
% Systematic Review,” J. Med. Internet Res., vol. 21, no. 11, p. e15360, Nov. 2019, doi: 
% 10.2196/15360. 
% [2]	C. W. Okonkwo and A. Ade-Ibijola, “Chatbots applications in education: A systematic review,” Comput. Educ. Artif. Intell., vol. 2, p. 100033, Jan. 2021, doi: 
% 10.1016/j.caeai.2021.100033. 
% [3]	A. R. W. Tjiptomongsoguno, A. Chen, H. M. Sanyoto, E. Irwansyah, and B. Kanigoro, “Medical Chatbot Techniques: A Review,” in Software Engineering Perspectives in Intelligent Systems, Cham, 2020, pp. 346–356. doi: 10.1007/978-3-030-63322-6_28. 
% [4]	L. Martinengo, E. Lum, and J. Car, “Evaluation of chatbot-delivered interventions for self-management of depression: Content analysis,” J. Affect. Disord., vol. 319, pp. 598– 607, Dec. 2022, doi: 10.1016/j.jad.2022.09.028. 
% [5]	H. Park and J. Lee, “Can a Conversational Agent Lower Sexual Violence Victims’ 
% Burden of Self-Disclosure?,” in Extended Abstracts of the 2020 CHI Conference on Human Factors in Computing Systems, New York, NY, USA, Apr. 2020, pp. 1–8. doi: 
% 10.1145/3334480.3383050. 
% [6]	“JMIR Mental Health - Conversational Agents in the Treatment of Mental Health Problems: Mixed-Method Systematic Review.” https://mental.jmir.org/2019/10/e14166 (accessed Feb. 21, 2023). 
% [7]	S. Atske, “Teens, Social Media and Technology 2022,” Pew Research Center: Internet, Science & Tech, Aug. 10, 2022. 
% https://www.pewresearch.org/internet/2022/08/10/teens-social-media-and-technology2022/ (accessed Feb. 21, 2023). 
% [8]	S. Atske, “Teens and Cyberbullying 2022,” Pew Research Center: Internet, Science & Tech, Dec. 15, 2022. https://www.pewresearch.org/internet/2022/12/15/teens-andcyberbullying-2022/ (accessed Feb. 21, 2023). 
% [9]	C. L. Odgers and M. Jensen, “Adolescent Mental Health in the Digital Age: Facts, Fears and Future Directions,” J. Child Psychol. Psychiatry, vol. 61, no. 3, pp. 336–348, Mar. 2020, doi: 10.1111/jcpp.13190. 
% [10]	A. Abd-Alrazaq, Z. Safi, M. Alajlani, J. Warren, M. Househ, and K. Denecke, “Technical Metrics Used to Evaluate Health Care Chatbots: Scoping Review,” J. Med. 
% Internet Res., vol. 22, no. 6, p. e18301, Jun. 2020, doi: 10.2196/18301. 
% [11]	A. Mariamo, C. E. Temcheff, P.-M. Léger, S. Senecal, and M. A. Lau, “Emotional Reactions and Likelihood of Response to Questions Designed for a Mental Health Chatbot Among Adolescents: Experimental Study,” JMIR Hum. Factors, vol. 8, no. 1, p. e24343, Mar. 2021, doi: 10.2196/24343. 
% [12]	G. Cameron et al., “Best Practices for Designing Chatbots in Mental Healthcare – A Case Study on iHelpr,” presented at the Proceedings of the 32nd International BCS Human Computer Interaction Conference, Jul. 2018. doi: 10.14236/ewic/HCI2018.129. 
% [13]	M. N. Rita and F. B. Shava, “Chatbot Driven Web-based Platform for Online Safety and Sexual Exploitation Awareness and Reporting in Namibia,” in 2021 International Conference on Artificial Intelligence, Big Data, Computing and Data Communication Systems (icABCD), Aug. 2021, pp. 1–5. doi: 10.1109/icABCD51485.2021.9519375. 
% [14]	R. Crutzen, G.-J. Y. Peters, S. D. Portugal, E. M. Fisser, and J. J. Grolleman, “An 
% Artificially Intelligent Chat Agent That Answers Adolescents’ Questions Related to Sex, Drugs, and Alcohol: An Exploratory Study,” J. Adolesc. Health, vol. 48, no. 5, pp. 514– 519, May 2011, doi: 10.1016/j.jadohealth.2010.09.002. 
% [15]	K. K. Fitzpatrick, A. Darcy, and M. Vierhile, “Delivering Cognitive Behavior Therapy to Young Adults With Symptoms of Depression and Anxiety Using a Fully Automated Conversational Agent (Woebot): A Randomized Controlled Trial,” JMIR Ment. Health, vol. 4, no. 2, p. e7785, Jun. 2017, doi: 10.2196/mental.7785. 
% [16]	K. Väänänen, A. Hiltunen, J. Varsaluoma, and I. Pietilä, “CivicBots – Chatbots for Supporting Youth in Societal Participation,” in Chatbot Research and Design, Cham, 2020, pp. 143–157. doi: 10.1007/978-3-030-39540-7_10. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% SOURCES OF SOCIAL SUPPORT %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Family is an important source of social support, but it is not the only option. 
%  There are many types of relationships in a young person's life, including peers, trusted adults, and mental health professionals, all of them can provide social support. 

% while each of these sources has their benefits, we see 

% describe the four sources we investigated here to set up the methods section
% We chose these four sources because we wanted to understand young people's norms and preferences about responses generated by sources with proficiency in different areas. A youth peer is someone who is going through or has gone through similar experiences as the help-seeker, so they can offer support and understanding to help a help-seeker feel less alone. However, they may not have the same training or experience as an adult mentor or therapist. 

% peers

% adults - mentors and professionals/clinicians/therapists
% An adult mentor can offer support and guidance, and they can help with navigating life's challenges since they have more life experience and offer a different perspective. However, they may not be able to relate to young people's experiences as well as a youth peer could.

% Therapists are adults who are specifically trained to help people with a variety of mental health issues. Not only can they provide support, guidance, and treatment, but they are also bound by confidentiality laws, which means they cannot share information about help seekers with anyone else without their consent. 





% % rephrase
% While online peer-to-peer
% platforms like TalkLife (talklife.com) and Reddit (reddit.com) enable such supportive conversations in
% non-clinical contexts, highly empathic conversations are rare on these platforms29; peer supporters are
% typically untrained in expressing complex, creative, and open-ended skills like empathy30–33 and may
% lack the required expertise. With an estimated 400 million people suffering from mental health disorders
% worldwide34, combined with a pervasive labor shortage35, 36, these platforms have pioneered avenues
% for seeking social support and discussing mental health issues for millions of people37. However, the
% challenge lies in improving conversational quality by encouraging untrained peer supporters to adopt
% complicated and nuanced skills like empathy.


% % from "Design Opportunities for Mental Health Peer Support Technologies"
% Beyond the use of texting and phone calls for support, people with mental illnesses go online to find peers. Online peer support communities are beneficial in management of illnesses such as breast cancer [14,31], rare diseases [43], and epilepsy [32]. Mental illness is no exception. Peer support is a primary motivation for people who go online for mental health [59]. Peers find each other in online communities for mental health conditions to seek information, emotional support, and advice [6,16,29,42,58]. People with mental health conditions often prefer going online for support because of the benefits of anonymity and convenience [34,49,58,59]. However, research suggests that participating in online communities for mental health can be distressing, even when people report having positive experiences [36,63,70]. Evidence of online interactions between peers with depression show that people have negative experiences with unsupportive members, negative content, and conflicts of beliefs [42]. 



\begin{comment}
    \subsection{Young people need social support}


This support can come from friends, family, teachers, mentors, and other adults. Young people need friends who accept them for who they are. They need friends who they can talk to about their problems and who will support them through tough times.
Being part of a family with a safe and stable home environment is also a major predictor of life outcomes. 
Adult mentors: Young people need adult mentors, such as teachers, who believe in them and who can help them reach their full potential. These are adults in the community who are willing to listen to them and who can help them connect with resources and opportunities.
By understanding the social support needs of youth, we can better support them and help them thrive.


Social support can help young people feel connected, loved, and accepted. It can also help them cope with stress, make healthy choices, and achieve their goals.

There are a number of factors that can affect a young person's social support needs. These include their age, gender, race, ethnicity, socioeconomic status, and sexual orientation. For example, young people who are LGBTQ+ may need more social support than their heterosexual peers.

There are a number of things that can be done to meet the social support needs of youth. These include providing opportunities for young people to connect with each other, training adults to provide social support, and developing policies and programs that promote social support.

It is important to remember that social support is not a one-size-fits-all need. What works for one young person may not work for another. It is also important to be flexible and responsive to the individual needs of young people.


Discuss the role of training in online peer support. It should consider how training can help to mitigate the risks associated with AI-assisted peer support, and how it can help to ensure that AI is used in a beneficial and safe way.

Implications of AI for peer support

Consider the potential benefits and risks of this technology, as well as the ethical considerations that need to be taken into account.

Some of the key questions to address in this section include:

How can AI be used to improve the quality of peer support?
How can we mitigate the risks associated with AI-assisted peer support?
What are the ethical implications of using AI in peer support?
This section should conclude by summarizing the key findings of the literature and by highlighting the need for further research on this topic.

\end{comment}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% FROM HELP ME PAPER: %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Related Work}

% \subsection{Social Support Needs of Youth}
% % Youth between the ages of 13-24 is the time of transition from childhood dependence to adulthood independence \cite{cordon1997youth}. During this time, depending on the social and environmental context of the youth, youth encounters biological (e.g., hormonal changes), social (e.g., bullying, community violence), and academic challenges that might coincide with mental and behavioral risks (e.g., depression, suicide, addictions, unsafe sex) \cite{mullen_defining_2021, Ogbu1990MentoringMY,karcher2006mentoring}. It is a critical developmental phase in which, depending on appropriate guidance and support availability, youth might develop a more negative or positive trajectory \cite{eccles1993parent}. 

% As youth \edit{attempt} to be more autonomous from their parents and look for peers for behavioral and social cues to model \cite{morrissey2015effect}, researchers investigated how peer support might moderate prosocial behaviors \cite{lockwood2014emotion}, schooling \cite{eklund2017adolescent}, physical health such as diabetes \cite{la2002peer} or physical activity \cite{hamilton2017role}, or self-acceptance of sexual orientation \cite{shilo2011effects}. For instance, Morrison et al.\cite{morrissey2015effect} studied Latino youth's transition to middle school and their involvement in antisocial and prosocial behaviors. They found that social support was a critical predictor of school engagement. 
% % Likewise, Morrissey et al. \cite{morrissey2015effect}, from their five-year family and friend support intervention on physical activity for girls between the ages of 13 and 17, found that increase in family and friend support increased moderate and vigorous-intensity physical activity \cite{morrissey2015effect}. Shilo et al.\cite{shilo2011effects} examined the effects of social support components and mental health and sexual orientation milestones of LGB youth. From 461 self-identified LGB youth and young adults, they found peer support and acceptance yielded the most potent positive effect on disclosing sexual orientation and well-being. 
% Similarly, researchers compared how and when these various sources of support are effective. In a sample of urban youths exposed to community violence, peer support was found to predict lower anxiety \cite{affrunti2018community}. Also, research showed actively engaging with peers online about their mental health concerns was associated with an increased likelihood of seeking formal mental health care \cite{ridout2018use}. 

% These social support exchanges can be better achieved when there are ample opportunities for self-disclosure. However, given the sensitivity, risks, and stigma of what youth often go through (e.g., sexual identity, \edit{risky behavior, unsafe sex), finding ways to enable healthy self-disclosure would be vital in facilitating the support youth needs. It would be critical to understanding healthy self-disclosure and how it related} to the effect of psychological well-being and perceived social support.

% \subsection{Self-disclosure and Psychological Well-being}
% Yang and Brown \cite{luo2020self} presented online self-disclosure and presentation to vary on four dimensions: \emph{Breadth} refers to the amount of self-information revealed; \emph{depth} indicates the intimacy of the presented information (e.g., emotions, weaknesses, etc.); \emph{positivity} reflects how positive or negative the presented information is; \emph{authenticity} relates to how \edit{authentic the self-representation is. Recent evidence showed accurate and authentic self-disclosure could} benefit general well-being and improve self-esteem \cite{reinecke2014authenticity}. Genuinely disclosing oneself can predict greater perceived social support and increased support being enacted by others \cite{kim2011facebook}. On the other hand, inaccurate and \edit{inauthentic} self-disclosure can increase perceived stress and impair social connection \cite{grieve2016psychological}. 

% The effects of self-disclosure on well-being largely depend on the valence of the content disclosed. \emph{The capitalization process} \cite{gable2010good} explains how people rearrange their memories related to the content being shared by others. This process would make people feel more positive when hearing positive emotional disclosure and more negative when hearing negative emotional disclosure \cite{ziegele2017no}. Internet culture is biased by the `positivity \edit{norm,' where people share} positive content more than negative disclosures \cite{waterloo2018norms}. Positive disclosures are often reinforced with positive feedback and more social support, leading to feelings of connectedness \cite{andalibi2017sensitive}. \edit{Negative disclosure, on the other hand, may discourage others from responding} because of the positivity norm and the capitalization process \cite{burke2016once}. Such lack of feedback can lead to feeling ostracised, and reduced well-being of the person who shared negative disclosure \cite{luo2020self}.
% %private msgs receive more support, but unsupport is happening

% In this light, such bias and reinforcement toward positive self-disclosure in online social environments bring challenges to psychological well-being, especially for populations like youth, who go through many personal psychological challenges yet pervasively use social media for much of their communications with peers \cite{subrahmanyam2008online}. Researchers consider online authenticity \edit{often unreachable} or possible only with a personal cost, especially for those with marginalized identities and challenging life experiences \cite{10.1145/3479567}. 
% These findings \edit{reveal} that we need safe platforms for youth to share authentic, negative disclosure responses with appropriate support. \edit{To such a platform, there needs to be a better understanding of how youth disclose themselves to garner and receive support.}
 
% \subsection{Online Peer Support for Youth}
% % Peer support has been shown as a robust and broad strategy for reaching groups that existing services often fail to engage. As a terminology initially developed in the contexts of addiction and substance abuse \cite{davidson1999peer}, peer support has shown to be powerful because of its ability to provide firsthand knowledge of experienced individuals and offer visible examples of individuals \cite{mead2001peer}. Peer support has been applied to various areas, including maternal and child health \cite{sokol2016peer} and diabetes and other chronic illnesses \cite{olsson2005role}. 
% % Although much research in psychology, family studies, and health fields examined peer support among youth, many of these studies have been conducted pre-internet/mobile era. A most friend and peer exchanges happen over mobile phones, specifically over social media, instead of texting \cite{nabi2013facebook}. Accordingly, it is unknown how the structure and dynamic of friend support may be shaped in today’s increasingly mobile-based communications among youth and what potential risks might be involved \cite{decieux2019social}.

% Peer support has been increasingly investigated in the HCI literature and within SIGCHI research community~\cite{oLeary2017design,andalibi2016understanding,Bellini2021fragments}, specifically in how people with similar interests exchange support over social media through videos, blogs, \edit{and online forums, or T}witter \cite{baruah2012effectiveness}. Past research showed the importance of support being exchanged through social media and how technology design can further facilitate positive experiences, leading to heightened perceived support, increased quality of life, or increased self-efficacy \cite{uehara1990dual}. However, the populations examined mainly have \edit{primarily} focused on the adult population, often for supporting specific health, such as chronic illness \cite{welch2018interactive}. 

% HCI researchers have also investigated \edit{the} design and implementation of moderated peer support to facilitate support for youth in specific situations such as the youth with intellectual disability~\cite{banos2018Evaluation}, children surviving cancer~\cite{Lindberg2014Designingpeercancer}, or youth living with human immunodeficiency virus (HIV)~\cite{Karusala2021Courage}.
% Although depending on the context, peer support could have different effects\edit{; for instance,} it could be distressing when the support is judgemental and disrespectful~\cite{takahashi2009potential}. Therefore, \edit{studying how youth peer support happens in social media without moderating specific topics is essential.}

% % youth online peer support:
% Finally, a few studies \cite{pretorius2019young,nabi2013facebook,frison_impact_2015} that considered social support for \edit{youth used self-reported data such as surveys or interviews,} which are prone to recall and social-desirability biases \cite{Gorin2001,Fisher1993}. 
% % limited to self-report:
% For instance, Frison and Eggermont~\cite{frison_impact_2015} conducted a survey and structural equation modeling. \edit{They} found that daily stress positively predicted youth social support seeking through Facebook, and if the support was received, it decreased adolescents’ depressed \edit{moods. But in case it was not precise, their depressed mood increased.
% There have} only been a few studies ~\cite{doornwaard2014young,Hartikainen2021safesexting,razi2020let,hartikainen2021care} on youth population online peer support using their digital trace data, but they are on specific issues such as youth online sexual risks~\cite{doornwaard2014young,Hartikainen2021safesexting,razi2020let,dev2022ignoring}. Thus investigating \edit{support-seeking behaviors using social media trace data would give unfiltered insights into the} natural interactions of youth.
 
% % \subsection{Analyzing Youths Public vs. Private Social Media Data}
% Accordingly, as it is \edit{essential} to investigate digital trace data to get an unfiltered view \edit{of} how social support happens in online spaces, studies examined exchanges that are publicly available, such as comments to YouTube videos \cite{naslund2014naturally}, Reddit posts \cite{de2014mental}, or other publicly available online forums \cite{smedley2021practical} partially due to logistical constraints of data collection and privacy. However, these approaches provide limited insights into how support is \edit{sought and given in private spaces}. Public conversations fundamentally differ from those happening in private space \cite{mcgregor201973}, and we know little about how support is being exchanged in private conversations, especially among youth. Collecting private user data is challenging due to the privacy and ethics of human subjects, especially for \edit{youth, since further measures such as parental consent and assent for minors younger than 18 and reporting potential child abuse should be accounted for~\cite{razi2020privacy,agha202responsible}.}

% In this paper, we address this \edit{significant} gap in the literature regarding how youth \edit{exchange} peer support through private conversations on Instagram.
% % ; we investigate the topics that youth possibly disclose and seek help from one another, the types of support they receive, as well as when they fail to receive the help they need. Given the findings, we discuss the technological design implications in enabling a safe, supportive environment for youth to receive peer support when needed.


==> original-submission/3-Methods-old.tex <==
\section{Methods}
\label{sec:methods}
\subsection{Overview}
Using an online survey, we examined how young people react to different human- and AI-generated responses to help-seeking messages. In this section, we describe our recruitment strategy and procedure, explain our survey design, and describe our approach to data analysis. 

% about frequent topics that online peer support conversations often entailed, and we selected help-seeking messages from an existing dataset to describe those topics. 
% used an online survey to ask young adults about help-seeking messages and pre-written responses.
% , without saying where the responses came from. 

\subsection{Recruitment Process}
We recruited survey participants by sharing a digital flyer with the authors' social media networks.
% on Instagram, Facebook, X (formerly known as Twitter), Discord, and Slack. 
We used an online screening survey to determine prospective participants' eligibility, which required that they are 18 to 24 years old, currently living in the U.S., fluent in English, and have stable access to the Internet. Eligible respondents (N=1,096) continued to the IRB-approved study information sheet, which they were asked to review before continuing to the main survey. To ensure the quality of the responses, within the main survey (described in section \ref{survey-design}), there was a built-in attention check question that asked participants to accurately indicate which help-seeking message topic we had previously asked about (see appendix \ref{attention-check-question} for the full question). After finishing the survey, participants could provide their contact information to receive \$5 as payment for their time. We received 866 complete survey responses from eligible participants, of which 622 were deemed fit for analysis because they were complete and passed the built-in attention check question.

\subsection{Survey Design}
\label{survey-design}
\subsubsection{Pre-written Responses to Help-Seeking Messages} We asked participants to read four help-seeking messages, then read and respond to questions about four pre-written responses (henceforth referred to as "responses") to each help-seeking message. The four help-seeking messages came from previous literature \cite{huh2023help} about frequent topics of private conversations for social support exchange between youth, including (1) relationships, (2) suicidal thoughts, (3) self-expression, and (4) physical health. We instructed participants to imagine they received these help-seeking messages from a friend as a text or direct message on social media. See figure \ref{fig:help-seeking-messages} for the text of the help-seeking messages for all four topics as they were presented in the survey.

\begin{figure}[h!]
    \centering
    \includegraphics[scale = 0.21]{figures/help-seeking-messages.png}
    \caption{Help-seeking messages presented in the survey.}
    \label{fig:help-seeking-messages}
\end{figure}

For each of the four help-seeking messages, we presented four responses that were written by four different sources: a (1) peer, (2) adult mentor, (3) therapist, and (4) artificial intelligence (AI). See appendix \ref{appendix-responses} for the full text of responses from the four sources for all help-seeking topics.
We used \textbf{peer} responses from the original youth real social media conversations for the help-seeking messages \cite{huh2023help}. The \textbf{adult mentor} responses were designed by a research assistant who had training from Crisis Text Line\footnote{\url{https://www.crisistextline.org}}, a global not-for-profit organization that provides mental health support via text. The training covered several topics: good contact techniques (empathy, tone, active listening), understanding risk, building rapport, and how to explore the crisis and risk. To capture the evidence-based professional training \textbf{therapists} complete to optimize their responses, we had a licensed clinical psychologist who also runs an APA-accredited clinical training program write the therapist responses. We used responses generated by ChatGPT for the \textbf{AI} responses. To understand how AI and LLMs could advise and support young adults, we prompted ChatGPT, a popular AI-powered chatbot used by many young adults \cite{vogels2023majority}, in May 2023 (GPT-3.5, free version) by asking it to write a response to each help-seeking message ``in the appropriate style and of the appropriate length for a mobile text message." 
% using the prompt outlined below for each help-seeking message: 

% \begin{quote}
%     ``I want you to write a message in the appropriate style and of the appropriate length for a mobile text message. To provide some context for the situation, please read the following:

%     [insert the corresponding context from appendix \ref{appendix-context}]

%     The message you received from this friend is below:
    
%     [inserted support seeking messages from figure \ref{fig:help-seeking-messages} here]''

%     % Write a message in the appropriate style and of the appropriate length for a mobile text message."
% \end{quote}

We chose this prompt after exploration with ChatGPT and some prompt engineering. Initial attempts to generate a response by providing only the help-seeking message to the chatbot repeatedly generated responses in the form of a long bulleted list of advice. 
% We gave ChatGPT an instruction in the prompt to particularly ask the chatbot for a response with "appropriate style and of the appropriate length for a mobile text message." 
Compared to our earlier exploration, ChatGPT's response to our most current prompt was considerably shorter and involved more interaction with the help seeker, which was suitable for a text message. 
% We learned that ChatGPT only provided the desired response when we clearly explained what we wanted in the prompt; otherwise, it could not understand the help seeker on a personal level, but could only give neutral, unbiased responses.

% the chatbot to provide us with advice and emotional support, then had a back-to-back conversation with the model to explore its potential responses.  
% \Afsaneh{Kaylie please add what was exactly prompted to ChatGPT (which model was it gpt 3 or 4?, what kinds of prompts and back to back conversation did we have, what did we learn? etc.} - addressed

% The peer responses were from the original youth conversations for each help-seeking message \cite{huh2023help}. The adult mentor responses were designed by a research assistant who had training in \Afsaneh{need to find what type of training Channacy had}. 
% We also wanted to investigate a response from someone in a similar age group as the source of the help-seeking message, but with more experience and training to provide support.
% To include a mental health professional's response, we had a clinical psychologist on the team who drafted the therapist response.
% Given the popularity of AI LLMs among young people \Afsaneh{[CITE]} and their potential to provide support \Afsaneh{[CITE]}, we included a response from ChatGPT to each scenario.

% \Jordyn{add image of help-seeking messages from kaylie and table of responses for each topic here!}

We wanted to understand participants' preferences for the content in each response rather than the source of the response, so participants were blinded about where the responses came from. We did this because we wanted to understand participants' perceptions of the content as part of peer support exchange, not how they felt about different sources of support engaging in the exchange. We also randomized both the order in which the scenarios were presented and the individual questions about each response to prevent question order bias.


% \textit{Response preferences}: 
To assess participants' response preferences for the different pre-written responses (henceforth referred to as "responses"), we asked a quantitative and a qualitative question. For the quantitative question, participants indicated the extent to which they agreed to the statement "I like this response" on a 5-point Likert scale (1 = not at all, 5 = extremely).
% \textit{Reasons for response preferences}: 
For the qualitative question, we asked participants to type a brief text response about what they thought about their most and least preferred response for each help-seeking message.

% \textit{Positive and negative reactions}: 
To capture participants' reactions to the responses, beyond how much they simply "liked" them, we asked participants to rate the extent to which they agreed with these statements: "I would send this response", "This response contains helpful advice", and opposite statements including "This response is problematic" and  "This response is inappropriate". We know from psychology literature \cite{dakof1990victims} that people may not always seek help or solutions when they discuss problems or concerns, rather, they may primarily seek emotional support, active listening, or validation. 
Therefore, these statements were designed in a way to capture those preferences and also to validate the cohesiveness in survey responses (i.e., a participant cannot find a response both helpful and inappropriate.)
% \Jordyn{Afsaneh/Jina, is this accurate for why we asked about problematic/would send/inappropriate/helpful specifically?}

% \subsubsection{Prior experience with online peer support}
% While prior experience with online peer support was not a requirement to participate in the study, we recognize that prior experience does shape human perception \Jordyn{rephrase and add reference}. To account for this, we asked "How often do you \textit{seek} support online (e.g., on social media)? This includes, but is not limited to, posting a question on Reddit, direct messaging a friend for help, or asking for advice in a Facebook group. and give peer support online." 
% and "How often do you \textit{give} support online (e.g., on social media)? This includes, but is not limited to, responding to a question on Reddit, direct messaging a friend who asked for help, or giving advice in a Facebook group." Answer choices were on a 5-point likert scale with standard frequency anchors\Jordyn{add reference to pew study and other papers that use same anchors} (1=never, 2=rarely, 3=sometimes, 4=often, 5=always).

% \subsubsection{Demographics}
Lastly, we asked for our participants’ demographic information depicted in Table\ref{tab:participant-demographics}.
% , including their gender, ethnicity, and education. See Table \ref{tab:participant-demographics}.
% \Jordyn{Do we need to justify why we didn't ask about age specifically, or is that assumed since we required a certain age range f`or prospective participants to take the survey so there's not enough variance within that range to draw meaningful conclusions?} \Afsaneh{We should have asked their specific age at the end of survey with the demographic questions. For now don't mention it and if reviewers asked we justify it like that.}

\begin{table}[!t]
\centering
\small
\begin{tabular}{|ccc|}
\hline
% \multicolumn{3}{|c|}{\textbf{Participant Demographics}} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Variable}}} & \multicolumn{1}{c|}{\textit{\textbf{Count (N)}}} & \textit{\textbf{Percent of total (\%)}} \\ \hline
\multicolumn{1}{|c|}{All Responses} & \multicolumn{1}{c|}{622} & 100.00\% \\ \hline
\multicolumn{3}{|c|}{\textbf{Gender}} \\ \hline
\multicolumn{1}{|c|}{Male} & \multicolumn{1}{c|}{403} & 64.79\% \\ \hline
\multicolumn{1}{|c|}{Female} & \multicolumn{1}{c|}{216} & 34.73\% \\ \hline
\multicolumn{1}{|c|}{Non-binary} & \multicolumn{1}{c|}{2} & 0.32\% \\ \hline
\multicolumn{1}{|c|}{Prefer to self-identify} & \multicolumn{1}{c|}{1} & 0.16\% \\ \hline
\multicolumn{1}{|c|}{Prefer not to say} & \multicolumn{1}{c|}{0} & 0.00\% \\ \hline
\multicolumn{1}{|c|}{Total} & \multicolumn{1}{c|}{622} & 100.00\% \\ \hline
\multicolumn{3}{|c|}{\textbf{Ethnicity}} \\ \hline
\multicolumn{1}{|c|}{Caucasian} & \multicolumn{1}{c|}{295} & 47.43\% \\ \hline
\multicolumn{1}{|c|}{African American} & \multicolumn{1}{c|}{193} & 31.03\% \\ \hline
\multicolumn{1}{|c|}{Native American} & \multicolumn{1}{c|}{34} & 5.47\% \\ \hline
\multicolumn{1}{|c|}{Latino or Hispanic} & \multicolumn{1}{c|}{26} & 4.18\% \\ \hline
\multicolumn{1}{|c|}{Mixed Race} & \multicolumn{1}{c|}{24} & 3.86\% \\ \hline
\multicolumn{1}{|c|}{Asian} & \multicolumn{1}{c|}{17} & 2.73\% \\ \hline
\multicolumn{1}{|c|}{Multiple} & \multicolumn{1}{c|}{16} & 2.57\% \\ \hline
\multicolumn{1}{|c|}{Prefer not to say} & \multicolumn{1}{c|}{9} & 1.45\% \\ \hline
\multicolumn{1}{|c|}{Native Hawaiian or Pacific Islander} & \multicolumn{1}{c|}{6} & 0.96\% \\ \hline
\multicolumn{1}{|c|}{Other} & \multicolumn{1}{c|}{2} & 0.32\% \\ \hline
\multicolumn{1}{|c|}{Total} & \multicolumn{1}{c|}{622} & 100.00\% \\ \hline
\multicolumn{3}{|c|}{\textbf{Education}} \\ \hline
\multicolumn{1}{|c|}{Some high school} & \multicolumn{1}{c|}{17} & 2.73\% \\ \hline
\multicolumn{1}{|c|}{High school or equivalent} & \multicolumn{1}{c|}{147} & 23.63\% \\ \hline
\multicolumn{1}{|c|}{Trade school} & \multicolumn{1}{c|}{100} & 16.08\% \\ \hline
\multicolumn{1}{|c|}{Bachelor's degree} & \multicolumn{1}{c|}{297} & 47.75\% \\ \hline
\multicolumn{1}{|c|}{Master's degree} & \multicolumn{1}{c|}{39} & 6.27\% \\ \hline
\multicolumn{1}{|c|}{Doctoral degree} & \multicolumn{1}{c|}{12} & 1.93\% \\ \hline
\multicolumn{1}{|c|}{Other} & \multicolumn{1}{c|}{3} & 0.48\% \\ \hline
\multicolumn{1}{|c|}{Prefer not to say} & \multicolumn{1}{c|}{7} & 1.13\% \\ \hline
\multicolumn{1}{|c|}{Total} & \multicolumn{1}{c|}{622} & 100.00\% \\ \hline
\end{tabular}
\caption{Participant demographics}
\label{tab:participant-demographics}
\end{table}

\subsection{Ethical Considerations}
This study was approved by the [anonymized] IRB as an exempt protocol, which meant participants were presented with the study information but not required to sign a consent document. The study information described the research objective, the procedures involved in completing the survey, the voluntary nature of the study, the potential risks involved, the anonymization process, and incentives. Only the research team members specified in the IRB protocol were granted access to the data, which was stored on a university-approved server.  

\subsection{Data Analysis}
To ensure we collected high-quality data, we first looked at the correlations between how much participants 'liked' the responses, felt they `would send' the message to the help-seeker, and how `helpful' they thought it was compared to how `problematic' and `inappropriate.' We did this because it is possible for participants to prefer for paradoxical reasons, such as finding the content comically inappropriate - fortunately, this was not the case in our data. Using means across the opposing attributes, we confirmed that the responses from sources that participants preferred more, said they were more likely to send, and felt were more helpful were also perceived as less inappropriate and less problematic. 
% This points to the data quality in our study because it signals that participants' reported preferences meant they find value in the help-giving response. 
Participants also tended to feel responses were more helpful than they were inappropriate or problematic, which means we avoided doing more harm than good, as is important for ethical research.

We also wanted to understand how participants reacted to the different responses beyond which one they `liked' the most (i.e., preferred). To do this, we looked at aggregate responses for all help-seeking messages by source to understand how helpful the responses were (`helpful'), how likely they were to send them (`would send'), and how inappropriate (`inappropriate') and problematic (`problematic') they felt the responses were. In subsequent sections and figures, we refer to these four measures as `attributes' of participants' responses. We also analyzed the qualitative responses using reflexive thematic analysis \cite{braun2019reflecting}.

==> original-submission/4-Results-old.tex <==
\section{Results}

% Our findings indicate that human-generated responses perform better when analyses do not take the topic into account, but topic-based analyses reveal that young people prefer AI-generated responses for less sensitive topics. In this section, we describe our findings that led us to this conclusion. 
% We first describe perceptions of help-seeking messages for frequent topics about which peers exchange support, and how those perceptions were related to how much participants liked the different responses. 
Next, we describe participants' preferences for and reactions to different support-giving responses (peer, adult mentor, therapist, and AI) across all help-seeking topics and how these preferences and reactions vary depending on the topic of the help-seeking message they are responding to (relationships, suicidal thoughts, self-expression, or physical health).

% \subsection{Statistics about Reactions to Help-seeking Topics and Demographic Characteristics}

% Participants' overall reported abilities to relate, help, and sympathize with the help-seeking messages were moderate (i.e., close to the mid-range answer choice, which was three on a five-point Likert scale with a range of one to five).
% Participants felt the most sympathy for the help-seeking message about suicidal thoughts but could relate and help most with the help-seeking message about physical health. Interestingly, the message about relationships, not the one about suicidal thoughts, was the least relatable. See Figure \ref{fig:messages-reactions}. \Jina{these conclusions are weird to say after having declared none of the results were significant}
% There were no significant differences between topics for participants' ability to relate, sympathize, or help. However, there were significant, albeit modest, correlations between how much they could relate, sympathize, or help and the extent to which they liked each response. \Jina{this sentence is redundant with next sentence and next sentence is way better. i would delete this prior sentence} 
% Regardless of the source of response (peer, adult mentor, AI, therapist), we noticed that the more participants could relate, sympathize, and help, the more they liked the responses, the more positively they felt about them, and the less negatively they felt about them. See Appendix \ref{cor-messages-responses}.

% \begin{figure}[!t]
%     \centering
%     \includegraphics[scale = 0.5]{figures/plot.messages.react_2023.9.11.png}
%     \caption{Perceptions of help-seeking messages about four topics: relationships, suicidal thoughts, self-expression, and physical health. Answers were on a 5-point Likert scale about agreement with statements on the x-axis. 1 was the lowest agreement, and 5 was the highest agreement.}
%     \label{fig:messages-reactions}
% \end{figure}

%Next, we describe our findings regarding differences found based on demographics (gender, ethnicity, and education). 
% The only reaction for all the help-seeking messages that varied significantly by gender was the ability to help with the help-seeking message about physical health. For this topic, male participants felt they could help more than did female participants (male: M=3.52, SD=0.05; female: M=3.35, SD=0.07; T(396.72) = 1.95, p = 0.05). There were no significant differences by ethnicity in participants' reported ability to relate, sympathize, or help with any of the help-seeking messages. Finally, we found some significant differences based on education 
% for all but two of the variables (ability to help with relationships and ability to relate to suicidal thoughts; 
% (see Appendix \ref{messages-reaction-education-means}), and a subsequent test for correlations indicated that participants with a higher level of education felt they could relate, sympathize, and help more with all of the help-seeking messages (see Appendix \ref{messages-reaction-education-correlations}).

% Our findings did 

% \begin{table}[hbt!]
% \centering
% \begin{tabular}{l|cccccc|}
% \cline{2-7}
%  & \multicolumn{6}{l|}{\textbf{Participants' reported ability to...}} \\ \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{\textit{Topic of Help-Seeking Message}}} & \multicolumn{2}{c|}{\textbf{Relate}} & \multicolumn{2}{c|}{\textbf{Sympathize}} & \multicolumn{2}{c|}{\textbf{Help}} \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\textit{Mean}} & \multicolumn{1}{c|}{\textit{SD}} & \multicolumn{1}{c|}{\textit{Mean}} & \multicolumn{1}{c|}{\textit{SD}} & \multicolumn{1}{c|}{\textit{Mean}} & \textit{SD} \\ \hline
% \multicolumn{1}{|l|}{\textbf{Relationships}} & \multicolumn{1}{c|}{3.22} & \multicolumn{1}{c|}{1.02} & \multicolumn{1}{c|}{3.30} & \multicolumn{1}{c|}{1.01} & \multicolumn{1}{c|}{3.31} & 0.98 \\ \hline
% \multicolumn{1}{|l|}{\textbf{Suicidal Thoughts}} & \multicolumn{1}{c|}{3.49} & \multicolumn{1}{c|}{0.97} & \multicolumn{1}{c|}{3.62} & \multicolumn{1}{c|}{0.88} & \multicolumn{1}{c|}{3.46} & 0.98 \\ \hline
% \multicolumn{1}{|l|}{\textbf{Self-Expression}} & \multicolumn{1}{c|}{3.51} & \multicolumn{1}{c|}{0.92} & \multicolumn{1}{c|}{3.55} & \multicolumn{1}{c|}{0.94} & \multicolumn{1}{c|}{3.47} & 0.99 \\ \hline
% \multicolumn{1}{|l|}{\textbf{Physical Health}} & \multicolumn{1}{c|}{3.60} & \multicolumn{1}{c|}{0.90} & \multicolumn{1}{c|}{3.61} & \multicolumn{1}{c|}{0.90} & \multicolumn{1}{c|}{3.49} & 0.94 \\ \hline
% \end{tabular}
% \caption{The extent to which participants felt they could relate, sympathize, and help with the four help-seeking messages presented, which were about four different topics (relationships, suicidal thoughts, self-expression, and physical health). Answers were on a 5-point Likert scale.}
% \label{tab:messages-reactions}
% \end{table}


\subsection{Young People's Preferences Regarding Human and AI-generated Help-Giving Responses (RQa)}
We found that the human-generated adult-mentor response performed best when we combined responses across all help-seeking topics and compared the average responses from the four sources (peer, adult mentor, therapist, and AI).
% without separating them by topic. 
How much participants liked each source's responses were significantly different (\textit{F}(3.0,5517.7) = 99.20, p < 0.001) across all help-seeking messages. 
% See Appendix \ref{plot-source-like} for a visualization of the differences between these means and their standard deviations).  
% /Jina{double check it I made a correct revision. Did you mean it} 
The post-hoc analysis showed that participants liked the adult mentor's responses the most (M=3.51, SD=0.02), followed by AI (M=3.46, SD=0.02), then the therapist's (M=3.29, SD=0.02), and the peer responses were their least favorite (M=3.03, SD=0.02). This means that before considering the topic of the help-seeking message, it seemed like humans, specifically adult mentors, outperformed AI in generating help-giving responses, although peer responses were not as liked by the participants. However, such responses varied after considering help-seeking topics, which we will discuss. 
% Next, we wanted to understand how participants reacted to the different responses beyond which one they "liked" the most (i.e., preferred). We looked at aggregate responses for all help-seeking messages by the source to understand how helpful the responses were ("helpful"), how likely they were to send them ("would send"), and how inappropriate ("inappropriate") and problematic ("problematic") they felt the responses were. In subsequent sections and figures, we refer to these four measures as "attributes" of participants' responses.

% Next, we break down reactions to the different responses (peer, adult mentor, therapist, and AI) by comparing how helpful each source's responses were, how likely participants were to send the responses from each source to the help-seeker, how problematic and inappropriate the responses were from each source.
% Positive attributes - 
% How much participants felt they would send a response and how helpful they thought it was - \Jina{this should have been in methods and here just go theough the findings. also it is confusing. what is positive attributes? you should just say helpful ess etc that was tested. readers dont have to learn more things and remember them for understadning the findings} followed the same pattern as participants' favorite
% \Jina{this should just be the most liked} responses. 
% \Jina{notnsure jf I understand following the same pattern. Just say only what happened. like removing the previous sentence and right away saying the next sentence here} 
% Participants felt the adult mentor's responses were the most helpful (M=3.50, SD=0.99) of the responses presented and said they were were most likely to send the adult mentor's responses to the help-seeker (M=3.48, SD=0.98), followed by AI's responses (how helpful: M=3.49, SD=1.05; likelihood to send: M=3.42, SD=1.12), then the therapist's responses (how helpful: M=3.29, SD=1.07; likelihood to send: M=3.25, SD=1.12), and the peer's responses receiving the lowest scores (how helpful: M=3.02, SD=1.15; likelihood to send: M=3.00, SD=1.18). 
% The opposing measures - how problematic and inappropriate participants felt the responses were - followed the exact opposite pattern as the positive attributes. 
% According to our analyses, the peer responses were also the most problematic and inappropriate (how problematic: M=2.32, SD=1.24; how inappropriate: M=2.30, SD = 1.24), followed by the therapist's responses (how problematic: M=2.19, SD=1.22; how inappropriate: M=2.18, SD=1.23), then AI's responses (how problematic: M=2.13, SD=0.02; how inappropriate: M=2.12, SD=0.02), and the adult mentor's responses were seen as the least problematic (M=2.07, SD = 0.02) and inappropriate (M=2.05, SD = 0.02). See Figure \ref{fig:source-reactions}. 

% Next, we break down reactions to the different responses (peer, adult mentor, therapist, and AI) by comparing how much participants perceived the responses as helpful and how likely they were to send the response to the help-seeker versus problematic and inappropriate. 
Participants felt the adult mentor's responses were the most helpful (M=3.50, SD=0.99) of the responses presented and also indicated that they were most likely to send the adult mentor's responses to the help-seeker (M=3.48, SD=0.98), followed by AI's responses (how helpful: M=3.49, SD=1.05; likelihood to send: M=3.42, SD=1.12), then the therapist's responses (how helpful: M=3.29, SD=1.07; likelihood to send: M=3.25, SD=1.12), and the peer's responses receiving the lowest score for those preferences (how helpful: M=3.02, SD=1.15; likelihood to send: M=3.00, SD=1.18).

How problematic and inappropriate participants felt the responses were, depending on the source of the response, followed the opposite pattern. The peer responses were perceived to be the most problematic and inappropriate (how problematic: M=2.32, SD=1.24; how inappropriate: M=2.30, SD = 1.24), followed by the therapist's responses (how problematic: M=2.19, SD=1.22; how inappropriate: M=2.18, SD=1.23), AI's responses (how problematic: M=2.13, SD=0.02; how inappropriate: M=2.12, SD=0.02), and the adult mentor's responses as the least problematic (M=2.07, SD = 0.02) and inappropriate (M=2.05, SD = 0.02). See Figure \ref{fig:source-reactions} for a visualization of means and standard deviations for participants' reactions to the responses by source.

\begin{figure}[!t]
    \centering
    \includegraphics[scale = 0.5]{figures/plot.source.reactions_2023.9.11.png}
    \caption{Participant preferences to responses by source. The x-axis is how much participants agreed with the different attributes of their reaction (helpful, inappropriate, problematic, and would send).}
    \label{fig:source-reactions}
\end{figure}

The findings so far suggest that participants regarded AI-generated responses highly, above even therapist and peer responses, although adult mentors' responses were considered most helpful and most likely to be sent in response to the help-seeking messages. %, - however, these findings do not account for the nuance in real-life peer support exchanges. To address this, we present RQ2-b results on how reactions to human- and AI-generated responses vary depending on what they are responding to.

\subsection{Young People's Preferences for Help-Giving Responses Depending on the Topic of the Initial Help-Seeking Message and Rationale Behind Them (RQb,c)}
% \textbf{\textit{Participants preferred AI-generated responses to help-seeking messages about relationships, self-expression, and physical health, but not suicidal thoughts.}} In the next four sections, we describe this finding in more detail and break down those preferences by the topic of the help-seeking messages: relationships ( section \ref{sec:relationships}), suicidal thoughts (section \ref{sec:suicidal-thoughts}), self-expression (section \ref{sec:self-expression}), and physical health (section \ref{sec:physical-health}). For each topic, we begin with the quantitative results for each attribute of the responses, followed by quotes from open-ended responses from the participants to illustrate why they did, or did not, like each response. Results from the open-ended responses are described from most to least preferred responses within each scenario.

\subsubsection{Relationships}
\label{sec:relationships}
Participants preferred the response about relationships that AI-generated more than any of the human-generated options. 
% Participants' reactions to responses about relationships as a help-seeking topic varied significantly by source, and participants preferred the response generated by AI according to 
They liked AI's response the most (M=3.63, SD=0.04) and thought it was the most helpful (M=3.63, SD=1.00), the least problematic (M=2.01, SD=1.16) or inappropriate (M=2.01, SD=1.20), and said they were most likely to send the AI's response to the help-seeker (M=3.65, SD=0.96). On the other hand, participants did not like the peer's response about relationships (M=3.00, SD=1.15) and felt it was the most problematic (M=2.41, SD=1.24) and inappropriate (M=2.38, SD=1.24), and least helpful (M=3.07, SD=1.13); consequently, they were also least likely to send the peer's response (M=2.98, SD=1.17). See Figure \ref{fig:plot-relationships} for a visual comparison of the means and standard deviations for reactions to all responses about relationships. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/plot.relationships_2023.9.11.png}
    \caption{Reactions to responses by source for help-seeking message about relationships.}
    \label{fig:plot-relationships}
\end{figure}

This sentiment was reflected in open-ended questions, where participants shared they liked the balance and empathy in the \textbf{AI-generated} responses. They felt the AI-generated response invited the help-seeker to share additional information without being overly intrusive or demanding. As one participant put it, the response was \textit{``helpful...
%The response has facts that are hard to hear but they are helpful. The message is 
[and] also supportive and feels like a safe space.''} (P453, Female).
    %it also has ways of how to cope with the situation.. Participants noted that they liked how the AI response both offered support and presented actionable solutions: \textit{“This particular response says it all, it's absolutely what I'd say. What I like the most is that it tells [the friend] how to deal with the situation and still encourages [them].”} The response was \textit{"helpful...
%The response has facts that are hard to hear but they are helpful. The message is 
    %it also has ways of how to cope with the situation.
Some participants described anthropomorphic reasons, such as the AI-generated response seemed like it came from someone who is a good friend: \textit{``They are really trying to help the friend so much and we all need such friends.''} (P434, Female). There were also mentions of qualities participants associated with the AI response, including that they thought it was \textit{``[empathetic]...supportive and caring.''} (P46, Male). Even though participants did favor the AI-generated response to the help-seeking message about relationships, they did note some room for improvement. Namely, that the response doesn't consider the entire context of the situation and \textit{``accuses the ex without listening to his side of the story.''} (P118, Male).

Participants noted that the
% human-generated responses 
\textbf{adult mentor's responses} also provided acknowledgment and validation, but it was potentially less useful and lacked clear direction. Those who liked this response noted that \textit{``it is respectful and...made [them] feel like the person understood [the help-seeker's] feelings.''} (P50, Male). Participants also noted a sense of maturity in how the response did not judge the help-seeker: \textit{``...the [response] answered the question in a mature way by making the victim not feel offended by going back to the ex. The response is just showing him or her that is what we [humans] go through in terms of love life.''} (P403, Male). Despite these positive attributes of the adult mentor's response, some participants felt it lacked concrete advice and did not give specific suggestions for what to do next. As mentioned in the previous paragraph, participants liked that the AI-generated response guided the help-seeker to provide additional detail in a gentle way - they did not feel the adult mentor's response had this same quality. Instead, participants felt the adult mentor's response was, as one participant said, \textit{``
%just about 
beating around the bush''} (P341, Male) and \textit{``
%it 
didn't provide a way of how to solve the situation clearly.''}

Participants liked the \textbf{therapist's response} because they felt it was extremely understanding and non-judgmental but noted that it seemed to delay giving actionable advice. Even though they did not know a therapist wrote one of the responses, they picked up on the professional tone: \textit{``This person provides professional remedy and ... [asks] the victim to share their mixed emotions and from there she/he will be in a position to offer strategies.''} (P481, Female). They saw the response as \textit{``very empathetic without shaming the friend''} (P587, Female), but noted that it felt like \textit{``scheduling [giving] help to next time when the [help-seeker] is in need of it now.''} (P503, Female). They appreciated the supportive tone but would have liked more concrete and immediate advice rather than beating around the bush and delaying support.

We received the most negative comments about the \textbf{peer's response} because participants felt it was terse, suggested hasty actions, and was not encouraging. While some appreciated the response's brevity, the way it was written came across as \textit{``too direct with no empathy.''} (P163, Male). This lack of empathy made participants feel like the sender had a bad attitude and was being too tough on the help-seeker: \textit{``It sounds harsh and rude, and also it doesn't consider the feelings of the victim.''} (P452, Female).

\subsubsection{Suicidal Thoughts}
\label{sec:suicidal-thoughts}
The only help-seeking topic about suicidal thoughts was the only one for which all the human-generated responses (especially the one from the adult mentor) outperformed  AI's response. Participants liked the adult mentor's response the most (M=3.59, SD=0.95) and felt it was the most helpful (M=3.61, SD=0.94), least problematic (M=2.04, SD=1.18), least inappropriate (M=2.00, SD=1.20), and that they were most likely to send it to the help-seeker (M=3.56, SD=0.94). They also least liked AI's response (M=2.82, SD=1.19) and saw it as the most problematic (M=2.53, SD=1.26), most inappropriate (M=2.54, SD=1.27), least helpful (M=2.93, SD=1.12) and identified it as the one they were least likely to send to the help-seeker (M=2.71, SD=1.21).
See Figure \ref{fig:plot-suicidal-thoughts}. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/plot.suicidal.thoughts_2023.9.11.png}
    \caption{Reactions to responses by source for help-seeking message about suicidal thoughts.}
    \label{fig:plot-suicidal-thoughts}
\end{figure}

When describing why they preferred the \textbf{adult mentor's response} to this sensitive topic, participants noted that they liked how it conveyed genuine concern by inviting the help-seeker to share more details and put effort into providing more support. \textit{``There’s a feeling of relating with the individual here. There’s a feeling of care and [that they're] really interested and [want] to understand the individual}
% plus boosting the individual’s confidence and also wanting to understand the individual’s 
\textit{[and their] situation.''} (P124, Male).
% It’s the best to do in such situation, for someone who wants to really be there for such person.” 
The only area of improvement that participants mentioned for the adult mentor response is that the message could have been a little shorter, but did not note what content should be cut. 

The \textbf{peer's} response was the second most preferred, and participants felt it was superficial, inconsiderate, and did not sufficiently acknowledge the help-seeker's struggles. Interestingly, participants likened the peer response to an AI-generated response, saying it sounded \textit{``...typical of a bot''} (P478, Female). Unlike the adult mentor's response, participants did not like how the peer's response was \textit{``so shallow [and] does not give the victim...much [detail] on how to tackle the situation and [get] helped.''} (P403, Male). 

Participants noted that the \textbf{therapist's response} immediately asked for more information in an attempt to ensure the help-seeker's safety - not knowing that this message was written by a clinician, some thought this sounded \textit{``professional''} while many others took it as intrusively asking for more information right away instead of offering support. \textit{``I think this response makes the person in need sink deeper into her trouble rather than pull her out. It's a bit inappropriate.''} (P451, Female). Since the initial help-seeking message did not use the word "suicide," many participants also did not like that the therapist's response immediately drew that conclusion and felt that calling it out could come across as judgemental: \textit{``I hate the assumption about self harm and suicide. It feels really I'm going to insert myself into your life to fix it and doesn't feel friendly at all.''} (P621, Non-binary).

The \textbf{AI-generated} response overall performed the worst for the help-seeking topic about suicidal thoughts. While some appreciated that the response was \textit{``actually truthful about the person's ability''} (P52, Male), most thought the referral to a healthcare provider conveyed less desire to help in that moment. \textit{``Fine, you can’t provide help but that’s not the best way to put it. You could always have the right choice of words and making the right sentence in this situation before suggesting a mental health professional and not everybody will like the fact that they are referring to them as going crazy. Not really cool though''} (P124, Male).

\subsubsection{Self-Expression}
\label{sec:self-expression}
Participants' reactions to the responses about self-expression followed a similar pattern to the responses about relationships, meaning AI's response outperformed all the human-generated responses, especially the peer's response. We found that participants liked AI's response the most (M=3.70, SD=0.98), felt it was the most helpful (M=3.75, SD=0.94), said they were most likely to send it to the help-seeker (M=3.67, SD=1.00), and thought it was the least problematic (M=2.01, SD=1.22) and least inappropriate (M=1.99, SD=1.18). Participants also liked the peer's response the least (M=3.08, SD=0.04), said they were least likely to send it (M=3.05, SD=1.15), and thought it was the least helpful (M=3.12, SD=1.09), the most problematic (M=2.25, SD=1.19) and the most inappropriate (M=2.26, SD=1.23).
See Figure \ref{fig:plot-self-expression} for a visual comparison of the means and standard deviations for reactions to all responses about self-expression. 

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/plot.self.expression_2023.9.11.png}
    \caption{Reactions to responses by source for help-seeking message about self-expression.}
    \label{fig:plot-self-expression}
\end{figure}

Participants liked that the \textbf{AI-generated response} conveyed guidance, support, and understanding. \textit{``I think a response like this can make the person feel like they've all been in this situation before, and there are points of empathy that they can draw on to guide them to be braver by drawing on the respondent's situation.''} (P43, Male). Similar to the message about relationships, participants liked that this response \textit{``[empathizes] with the friend while also providing practical solutions''} (P587, Female). 

They felt the response from the \textbf{adult mentor} also conveyed some affirmation of the help-seeker's struggles but to a lesser extent. They liked that \textit{``it starts with sympathy''} (P160, Male), but the overall tone felt \textit{``unattached.''} This distinction between sympathy and empathy is important to note - as sympathy is feeling for someone else while empathy is feeling with them. The adult mentor's response conveyed "sympathy," meaning they can see where the help-seeker is coming from, but \textit{not empathy}, which implies less personal experience with the matter at hand. Participants clearly communicated this sentiment by saying that \textit{``the victim is not understood''} (P383, Male) and that the message indicates \textit{``the person [who wrote it] has no idea of what the [help-seeker] is going through.''} (P611, Female).
% the message \textit{"[gave] the impression that someone should act rudely and not care what others think.”} 

Similar to the relationship help-seeking message, participants suspected that the \textbf{therapist's} message came from a clinician, \textit{``The message looks like one a professional therapist would send...''} (P350, Male). As one participant said, \textit{``The response is appropriate because [it] is from [a] counselor, someone who has been able to tackle much of the issues by being exposed to different clients and knowing what to do for certain client till they reach a point of believing in themselves and having that courage to talk to anyone without any fear.''} (P403, Male).

The \textbf{peer's response} did not feel supportive enough to participants and did not do enough to calm the help-seeker, \textit{``I think that's too casual a response to really consider the issue from the perspective of the person pouring it out.''} (P21, Male). Moreover, they felt this response lacked depth and oversimplified the help-seeker's fear of self-expression. Like the adult mentor response, participants also felt there was not enough of an indication that the person who wrote the response truly understands what the help-seeker is going through, but less so because they can't empathize and more because they do not want to put effort into conveying that empathy, \textit{``It was too brief and nothing more of empathy felt in it. It was more like this person wanted to help but didn’t really put much % of 
effort [into] it...
% Though it was having 
[it had] a little spark of encouragement[,] but it could be better.''} (P124, Male).

\subsubsection{Physical Health}
\label{sec:physical-health}
When the help-seeking message was about physical health, the AI responses once again outperformed the human-generated responses, especially the peer's. Participants liked AI's response the most (M=3.71, SD=0.96), saw it as the most helpful (M=3.67, SD=0.99), least problematic (M=1.95, SD=1.16), least inappropriate (M=1.95, SD=1.21), and overall felt they were most likely to send it to the help-seeker (M=3.64, SD=0.99). The peer response received the least favorable reaction as the least liked response (2.83, 0.05) and thought it was the most problematic (M=2.46, SD=1.28), most inappropriate (M=2.46, SD=1.28), and least helpful (M=2.73, SD=1.22), and indicated they were least likely to send it to the help-seeker (M=2.78, SD=1.23).
See Figure \ref{fig:plot-physical-health} for a visual comparison of the means and standard deviations for reactions to all responses about physical health.

\begin{figure}[hbt!]
    \centering
    \includegraphics[scale=0.5]{figures/plot.physical.health_2023.9.11.png}
    \caption{Reactions to responses by source for help-seeking message about physical health.}
    \label{fig:plot-physical-health}
\end{figure}

The \textbf{AI-generated} response once again performed the best, and participants raved about how much they liked it - as one participant said, \textit{``I didn't just like this response. I love this response.''} (P351, Male).
% because apart from being there for the person, you even helping and suggesting professional help for the person.” because 
Participants describe how the answer contained all the important components: empathy, acknowledgment, and concrete suggestions for next steps, \textit{``its an all round genuine answer [that] shows you care[,] understand the problem and offer the right solutions.''} (P592, Female). The "right solution," in this case, was to continue with ongoing self-care work (i.e., talking to a counselor), and participants liked that this response acknowledged doing so is not easy. \textit{``The fact that he empathized with the person and encouraged them to further try [counseling] because you cannot get the intended results after one trial.''} (P80, Male). Participants also liked that counseling was just one of the multiple solutions the response discussed and
%"the response 
\textit{``shows the [help-seeker] how they can use other strategies to be okay.''} (P453, Female). The comprehensive and deeply empathetic nature of this response seems to be what set it apart from the others.
% apart from counseling. it's also empathetic and it has words of affirmations .” 

Participants did like that the \textbf{adult mentor}'s response \textit{``[validated] wanting rest''} (P621, Non-binary), but also felt that it \textit{``[made] the [help-seeker] feel as if it's OK to just relax and not do anything.''} (P351, Male). They discussed how the adult mentor's message did not acknowledge that self-care is more than relaxation. In doing so, this response seemed to convey that there is nothing more the help-seeker can do, \textit{``I feel like it's not addressing the issue at hand and makes the victim feel like they are doing great of which they are not.''} (P137, Male). While participants thought \textit{``praising the [help-seeker] for small achievement[s]''} (P614, Female) and \textit{``positive energy''} were good, they were not enough, \textit{``because 
% I think that 
it doesn't contain enough [advice] that can help the victimized person''} (P125, Male) in this situation.

While the \textbf{therapist}'s response did offer a solution, participants did not think it was the right one: \textit{``It's very unclear whether this respondent wants to help out. They are telling the victim to keep pursuing the same course that ain't working for them.''} (P167, Male). Unlike the AI-generated response, which suggested continued counseling in addition other solutions, participants did not like that the therapist's response was \textit{``just
% practically 
telling the person in question to [continue]
% base only on 
counselling, [with] no other options to explore.''} (P122, Male). Therapy also incurs a cost for the help-seeker, which participants were not shy to mention in their feedback for this response. They noted that \textit{``counselling can be [quite] expensive,''} (P166, Male) and increasing those costs might not be necessary because \textit{``
%although yes counseling helps sometimes but at this time it wont work cause 
at this point [the help-seeker] needs love and support from family and friends who would be available to support them.''} (P438, Female). This does not mean participants wanted the response to suggest the help-seeker stop counseling altogether, but rather that there should be additional non-clinical suggestions.


% \begin{table*}[]
% \centering
% \begin{tabular}{|c|c|}
% \hline
% \textbf{Topic of Help-Seeking Message} & \textbf{Source of Best Response} \\ \hline
% Relationships & AI \\ \hline
% Suicidal Thoughts & Human \\ \hline
% Self-Expression & AI \\ \hline
% Physical Health & AI \\ \hline
% \end{tabular}
% \caption{Source of the best-performing response (human or AI) to help-seeking messages about different topics.}
% \label{tab:best-source}
% \end{table*}

% We summarize these findings to answer RQ2 in table \ref{tab:best-source}, which outlines which 
% source (human or AI) performed the best for all attributes of participants' responses for each scenario. The best-performing response was the most preferred, most likely to be sent, most helpful, least problematic, and least inappropriate.

In summary, our findings revealed that participants preferred AI-generated responses about less sensitive topics (relationships, self-expression, and physical health). For more sensitive discussions (suicidal thoughts), participants preferred responses from the adult mentor. In the next section, we discuss the implications of these findings.

==> original-submission/5-Discussion-old.tex <==
\section{Discussion}
% Our results provide insight about AI's potential to respond to help-seeking topics frequently represented in youth's conversations 
% % \cite{huh2023help} 
% by presenting young adults with human- and AI-content to understand their reactions. 
Our findings point to several important areas for discussion regarding the promise of AI-powered support and questions to address about handling sensitive topics, should they arise.

\subsection{Premise for AI-Powered Support}
% Our results also provide unique insight into how young people react to AI-generated content when they do not know it came from AI. In their qualitative responses, participants likened AI's responses to something a "good friend" might say and used anthropomorphic characteristics (caring, friendship, etc.) to describe why they liked the AI response while comparing the peer-generated responses to "bots." Researchers expect that empathetically interacting AI systems will increase the level of acceptance of social robots \cite{jesin2018artificial}, and our analyses point to other anthropomorphic characteristics to consider.

Our results provide insight about AI's potential to respond to help-seeking topics frequently represented in youth's conversations, which previous literature stated that they sometimes left without supportive responses \cite{huh2023help}, by presenting young adults with human- and AI-content to understand their reactions. These findings also provide a premise for using generative AI-to-power support-giving conversations as long as they maintain the characteristics that participants identified as helpful, empathetic, constructive, and non-judgemental. However, AI is a constantly moving target, where its characteristics, functionalities, and abilities constantly evolve over time. For instance, for Open AI's GPT models, the level of memorizing past conversations is limited, but recent updates enable the system to remember user preferences and tailor responses accordingly \cite{openai2023release}. Furthermore, depending on the version of GPT models, the prompt engineering techniques might work differently. Accordingly, the lesson we should take away from this study is to apply the rationale provided by the participants and devise ways that future generative AIs can maintain the preferred styles through customization, personalization, prompt engineering, and manipulation of training data. Doing so can help the model's output come across as trustworthy \cite{cabrero2023perceived}, which affects reliance on AI systems \cite{kim2022perceived}.
% For instance, **CAN YOU GIVE SPECIFIC EXAMPLES WITH FINDINGS**


% participants knew it was AI would, they still be open to receiving suggestions from AI to support their peers better?
% Concurrent with efforts to improve AI-literacy \cite{lee2021developing}

% \Jordyn{add something about how we're so concerned with machines ability to detect ai-generated responses, but according to our results humans might not even be able ot ell the difference - especially youth (make case for adding this to AI literacy lessons/pedagogy?)}







% -- discuss how participants used anthropomorphic characteristics (caring, friendship, etc) describing why they liked the AI response. if participants knew it was AI would, they still be open to receiving suggestions from AI to support their peers better? Cite other studies on how people perceive AI suggestions when AI writing style includes different human characteristics such being more empathetic or friendly (refs needed from Afsaneh). some implications of our findings here is that AI has the capability to help the peer supporter to write a better response to those support-seeking topics.



\subsection{AI as Complimentary Response based on the Context and Sensitivity of Topics}
Before considering the context of the help-seeking message, it would appear that young people prefer the adult mentor's response. However, a closer look reveals a strong preference for the adult mentor's response to the sensitive help-seeking message about suicidal thoughts while they preferred the AI-generated response to all other help-seeking messages. 
In a research article by Shao \cite{Shao2023empathetic}, a similar encounter takes place where their results indicate human-operated counselors provide higher quality results during empathetic counseling sessions than AI, but upon further investigation, it was clear that the way in which AI-supported an individual became crucial to its success in being rated helpful. 
As indicated by our findings and as previous research \cite{Saha2022towards,ahn2020chatbot} has uncovered participants usually preferred responses that offered support and comfort within the scope of positivity to feel comfortable enough to continue to share. 

We do not intend for our results to imply that AI-generated content is sufficient to replace a therapist or clinical expertise. As we found, participants did not like AI's response about sensitive topics,
%In sensitive situations where AI could not help, 
for which ChatGPT's response specified that the kind of support required was outside the model's capabilities. While some participants appreciated the honest answer that reflected this limitation, others noted that referral to someone else felt dismissive because the help-seeker could have gone to that other source to begin with, but they did not. This points to two interesting follow-up questions: 1. if young adults are experiencing suicidal thoughts, would they go to an AI system for help in a real-world situation? 2. if the answer to question 1 is yes, then how should an AI system respond when a user asks for help it cannot provide for sensitive matters? 
% it is ethical for an AI system to recognize and convey its limits, our participants did not like that the response did not offer additional guidance about what to do next beyond reaching out to a professional. 
% This begs the question of how an AI system should respond when a user asks for help it cannot provide. 
Researchers\cite{mahmood2022owning} have begun to explore how AI should own up to its faults during user interactions, such as when it may provide incorrect information. Our work highlights that similar frameworks should be explored for sensitive topics -- for example, is it more helpful for the AI to respond with links and contact information for resources? If so, which resources are most helpful to share and why? The goal is for AI to convey its limitations constructively, ensuring the user is safe.
% \Afsaneh{Can potentially mention that when we gave our scenario to chagpt now, it prompts that it cannot provide an answer because it is a sensitive topic and you should get professional help and why this is not enough}

%with potential imminent risks to the people. However, the idea that AI-generated content can be helpful for less sensitive issues is powerful in increasing access to resources. Not all mental health professionals handle clinical cases with a diagnosed mental illness, and youth need many non-clinical mental health resources. These include, but are not limited to, learning how to have healthy relationships with emotions \cite{greenberg2003enhancing}, social decision making \cite{elias1988teaching}, resilience and grit in the face of adversity \cite{arias2022can}, and more. However, the availability of these resources can depend on factors that are out of young people's control, like school district curricula and financial resources. AI-generated content presents an opportunity to disseminate this content in a low-cost, accessible way that can help increase access to mental health tools for overall well-being.



The highly sensitive and complex issue of suicidal thoughts demands careful consideration of ethical, legal, and moral concerns, which the current AI technologies cannot address. In creating AI-based risk detection and prevention techniques, we need to keep humans in the loop, such as using AI as an assistant to peer support giver rather than directly having AI interact with struggling individuals as an all-in-one solution. Current AI technology may misinterpret language and is not able to understand the context of the situation, and nuances of human emotional state, which can lead to misidentification. Those false positives or negatives could have catastrophic results depending on the context. Having higher false alarms may burden resources depending on the types of interventions being implemented after detection, such as connecting them to mental health professionals. At the same time, missing instances may leave individuals in distress who may need help. 

% To avoid being legally responsible when an AI intervention goes wrong, companies such as OpenAI do not provide intervention when someone discloses such harmful behaviors, leaving them behind. We call the practitioners and policymakers to hold companies accountable to provide better responses in such cases.

Furthermore, even though our results indicate that young adults prefer responses from an adult mentor, it is possible that participants did not like the idea that a potential peer would interact like a clinician. Participants often noted that the therapist's responses sounded "clinical," which is not a type of interaction that they would expect from peers. That violation of expectations could be what they responded negatively to. We want to stress that cases at risk of suicide require crisis intervention and professional solutions, such as therapy. AI conversational agents could be helpful in identifying users at risk of suicide and self-harm, but it is imperative that we not rely on AI alone to detect imminent risks. Furthermore, there are open questions about monitoring stigmatized topics like suicide, as it can perpetuate algorithmic stigmatization~\cite{Andalibi2023conceptualizing} for individuals struggling with mental health issues and create an environment where they feel constantly surveilled.










%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% FROM JINA %%%%%%
%%%%%%%%%%%%%%%%%%%%%%% 

% - The overtrust and undertrust of AI--what is most recent literature on chatgpt and people's perceptions on them
% - First study to blind test chatgpt?
% - reasoning behind why they preferred AI over others
% - surprising finding about preference for AI
% > Our finding that generative AI responses were well-received for providing help compared to various human sources provides implications for generative AI's ability to be helpful in providing youth with additional support. 
% > % not saying GAI works, great let's all use it...people unexpectedly really liked GAI, even more than clinician responses

% - but does it really mean that AI can replace the help?
% - what can we learn about peer support least preferred and AI preferred the most?
% > As those responses were from real-world responses youth gave in their social media conversations \cite{huh2023help}, this finding highlights how youth are not always able to provide the support that their peers need. Previous studies had also found 
% > support seekers were left without helpful responses in those situations.
% - assistive, training peers?
% > However, we found adult-mentor responses performed best when we combined responses across all help-seeking topics. This shows the need for education and training of youth to provide better support to their peers.
% - interactive ways for people to give feedback, which then can help AI to learn what people like and train peers?
% > \Afsaneh{ discuss and cite more literature about this: Participants also reflected on why they had these preferences, pointing to positive attributes like empathy, a non-judgemental tone, rational suggestions, and avoiding terse messages with hasty recommendations.}
% - What do we know about training writing with chatgpt?
% - How can we apply what we know about training writing to the peer support context?

% - exception: sensitive topics? What happened?
% - AI preferred on non-sensitive topics. What does it mean?


% Below, we expand on the meaning of our findings, followed by implications for design, and ending with limitations and future directions.
% \subsection{Research Implications regarding Overall Reactions to Human and AI-generated Help-giving Responses \Afsaneh{-RENAME}}
% By studying young people's perceptions of pre-written responses from various human sources and generative AI, we found that the AI-generated responses were well-received for providing help with non-sensitive topics.

%  We found that young adults perceived peers' responses as least helpful and most problematic and inappropriate. We also found that participants preferred the responses that acknowledged the help-seeker's situation with empathy, a non-judgemental tone, rational suggestions, and while avoiding terse messages with hasty recommendations. more tangible suggestions for next steps, acknowl 
% not saying GAI works, great let's all use it...people unexpectedly really liked GAI, even more than clinician responses

% \subsection{Research implications based on Nuances of Help-seeking Topics \Afsaneh{-RENAME}}
% \Jordyn{add something about how we're so concerned with machines ability to detect ai-generated responses, but according to our results humans might not even be able ot ell the difference - especially youth (make case for adding this to AI literacy lessons/pedagogy?)}


 
%\Afsaneh{ discuss and cite more literature about this: Participants also reflected on why they had these preferences, pointing to positive attributes like empathy, a non-judgemental tone, rational suggestions, and avoiding terse messages with hasty recommendations.}%

% \Afsaneh{add results on relationship, self-expression, physical health results that were interesting to discuss here}
% \subsection{AI for Clinical vs Non-Clinical Cases}
% - unexpectedly, people really liked the generative AI response - implication is we don't have much control over it and depending on teh training data/how the algorithm works, its going to change the result of the model. so our results are interesting, but where do we go from here to implement it? it's not like GAI has a certain style. our results might not even help people use GAI out of the box, but we have model number and when we generated it we're 

% Suicide
% Afsaneh mentioned she has a paper about how AI shouldn't help with suicide, should we add that citation here? If so, how to connect it?...


% \subsection{When AI Can't Help}

% With the advent of generative AI systems (e.g., ChatGPT) being intertwined in everyday tools,
% % , such as smart home devices, smart-phones, and automobile interfaces, 
% researchers increasingly explore ways that these generative AI systems can support mental health.


\subsection{Design Implications}
% \subsubsection{Opportunities for Human-AI Collaboration}
Our findings show how AI-generated responses could be helpful, therefore AI-generated responses could be used to train or nudge youth to support their peers. AI and LLMs could be specifically trained with best peer support practices, such as providing specialized recommendations for youth.%~\cite{}. 
 Also, human collaboration with AI can help facilitate the expression of empathy in textual supportive conversations in noncritical settings~\cite{sharma2023human}.
This can help young adults to be mentors in their social networks. Previous literature has looked into different types of recommendations that are accepted by people about AI.
Although there are specific clinical services that peer supporters cannot provide that the AI should also acknowledge including diagnostic assessment, psychosocial evaluation, medication management, and therapy~\footnote{\url{https://edis.ifas.ufl.edu}}.
Similar to how SAMHSA~\footnote{\url{https://www.samhsa.gov/brss-tacs/recovery-support-tools/peers}} defines effective peer support for trauma survivors for those in recovery, it is important that in the design of effective peer support interventions we consider the following: providing a sense of safety; trustworthiness and transparency; collaboration and mutuality; empowerment, voice and choice; and awareness of cultural, historical, and gender issues.
Also, for having AI as an assistant for peer support givers, more research in explainable AI to make sure these models can provide the right explanations to users in those situations is warranted.

% - - communication literature (references?) has looked at AI OR humans, but that's too simple - what kind of human? what kind of AI? What kind of situation/context? These are opportunities for Human-AI collaboration to understand users' preferences, experiences, and backgrounds in those situations to create more personalized feedback/help for peer support-giver to be more effective


% ethical implications:

% Stigmatization and Trust:


% - do we just follow participant preferences? Should we just do what help-seeking people want, or does there have to be some kind of moderation/top-down approach to how we
% - just because a person said I wanted this kind of advice, should we listen to everything they're saying or should there be some limitations?
% - there are some things peer supporters should NOT provide - e.g., diagnostic assessment, medication management, etc., so we need to make sure AI doesn't provide those things
% - there are some good practices like empathic listening, encouraging them to speak to an adult/counselor, which AI could be safeguarded to nudge peer supporter in those directions



% AI-powered peer support
% - qualitative results showed gaps of skillsets that might be missing in certain types of peers, and AI can help fill that gap. call for future research to design AI-powered peer support. 
% - qualitative results helped us identify what they liked/didn't like about GAI responses, so these areimplications for how we might generate AI-based peer support tools
% if we were incorporate 
% possibility of being able to customize GAI - these people have found ways to customize/modify GAI to address customization needs of users, we can use these to customize ai-powered tools of users
% - possibly test one response vs "choose your own journey" type of experience - see "Talking to a bot or a wall? How chatbots vs. human agents affect anticipated communication quality" paper by Zhou et al (https://doi.org/10.1016/j.chb.2023.107674)
% 

\subsection{Limitations and Future Directions}
We recruited participants from our networks and snowball sampling, therefore we acknowledged that our dataset may not be a generalizable sample that accurately represents the young adult population in the US. 
% - we didn't recruit for specific makeup by sex, gender, location, etc.), but we did meet min sample size from power analysis...paper about sample size at CHI: https://dl-acm-org.ezproxy2.library.drexel.edu/doi/epdf/10.1145/2858036.2858498 
Also, we asked participants about static conversation responses, not continuous interactions. Therefore, future research should investigate youth preference in real-time conversations with additional levels of exchange.
Although we included prevalent support-seeking topics from youth real social media interactions, we were not able to present various topics, and our study is limited to the topics we presented. Future research should study more comprehensive scenarios and also more in-depth studies on specific support-seeking topics to provide deeper insights into each topic. Also in case if participants knew they were interacting with AI and the origin of the responses, that might have changed their preferences for those responses. 
To further understand youth's norms around peer support and perceptions of how AI could be helpful or inappropriate, we are planning to conduct interviews with some of the young people who participated in our study. 
% - Discuss future analyses w/this dataset (based on experiences with giving/seeking support, perceptions of situations, demographic predictors, anything else?), follow-up interviews, and other future studies, like...
% % What do we still not know? What do we need/want to learn? How are we going to do that?
% - continue to test this and see how consistent generative AI is - maybe test different models to see which is most effective for support and why?
% - How would results change if participants knew they were interacting with AI? mention ongoing follow-up interviews


==> original-submission/6-Conclusion-old.tex <==
\section{Conclusion}
To explore the potential for AI-powered peer support, we studied how young adults react to different human- and AI-generated responses to online help-seeking messages. Our findings revealed that participants preferred AI-generated responses about less sensitive topics (relationships, self-expression, and physical health), but not for sensitive discussions about suicidal thoughts. These findings point to the promise of AI-powered tools to help peers support each other during challenging times.


% \Afsaneh{Drop the mic Jordyn!!}

==> r_r/0-Abstract-rr.tex <==

Generative artificial intelligence (AI) is integrated into everyday technology, including news, education, and social media. AI has further pervaded private conversations as conversational partners, auto-completion, and response suggestions. As social media becomes young people's main method of peer support exchange, we need to understand when and how AI can facilitate and assist in such exchanges in a beneficial, safe, and socially appropriate way. We asked 622 young people to complete an online survey and evaluate blinded human- and AI-generated responses to help-seeking messages. We found that participants preferred the AI-generated response to situations about relationships, self-expression, and physical health. However, when addressing a sensitive topic, like suicidal thoughts, young people preferred the human response. We also discuss the role of training in online peer support exchange and its implications for supporting young people's well-being. Note: This paper includes sensitive topics, including suicide ideation. Reader discretion is advised.

% Tools and systems using generative AI models are pervading every sector of our society, including education, finance, and health. Especially when it comes to AI models being used for younger populations,

% CHI researchers increasingly explore the role of and people’s perceptions toward generative AI models in various tools and contexts. Given the explosion of possibilities of AI-enabled solutions for sensitive topics and populations such as young people’s mental health, it is critical to examine how young people perceive of AI…

% The internet provides many opportunities for youth peer support exchange, but there is limited knowledge about the most helpful responses to offer in such situations. To address this, we asked 622 young people to complete an online survey and evaluate human- and AI-generated responses to help-seeking messages. We found that participants preferred the AI-generated response to situations about relationships, self-expression, and physical health. However, when the help-seeking message was about a sensitive topic, like suicidal thoughts, participants preferred the researcher's response. We also discuss the role of training in online peer support exchange and its implications for supporting young people's well-being. Note: This paper includes sensitive topics, including suicide ideation. Reader discretion is advised.

% In aggregate, we found that participants liked the researcher's responses the most, with AI as a close second. However, nuances emerged depending on the context of the help-seeking message, and 
% rather than the sources, which represent different types and levels of training. 

==> r_r/1-Introduction-rr.tex <==
\section{Introduction}
% Generative artificial intelligence (AI) permeates various facets of our daily lives by seamlessly integrating into commonplace technologies such as news dissemination, educational platforms, and social media engagement. The omnipresence of AI is particularly evident in text-based interactions, where it facilitates auto-completion, provides response suggestions, and even operates as a conversational partner. Amidst these technological advancements, technology-mediated communication has emerged as a primary conduit for peer support exchanges among young people. Recognizing the pivotal role of these technologies in shaping the contemporary landscape of interpersonal connections, it becomes imperative to comprehensively understand the nuanced interplay between AI and peer support interactions. This paper aims to explore the multifaceted ways in which AI can serve as a facilitator and enhancer of peer support exchanges on social media, shedding light on the potential benefits, challenges, and the imperative need for ensuring safety and social appropriateness in the utilization of AI-driven interventions within these digital spaces. By addressing these considerations, this research endeavors to contribute to a more informed and ethically grounded integration of AI into the realm of online peer support for young individuals.}


% of people seek support online for a variety of topics, such as XYZ. Research shows that online support can be effective for XYZ reasons (cite substance use research and others ). however, support can come from a lot of different types of people. there's professional networks where people can ask doctors medical questions online (add citation), there's trained peer specialists (add substance use reference), and friends in your network whoa re people you know that may share age/other demographic variables but don' have specific training or life experience to help in certain situations (cite help me paper). 
% Amon the recent, rapid advancements in AI applications, we're also seeing applications for mental health support. As we said, the types of online support users encounter are not all the same, and comparing "humans" in general to AI is too simple. We need to compare AI to the types of human support youth can encounter, which is an area that hasn't been explored. To address these gaps...RQ's



\edit{Today's generation of youth is the first to grow up with ubiquitous internet access. Most} (92\%) young people access the internet daily, with 24\% describing their online presence as "almost constant" \cite{vogels2022teens}. \edit{Support is an important reason why young people engage online \cite{bae2021social, pretorius2019young}. Research suggests this is because online help-seeking interactions offer many benefits, including anonymity and privacy \cite{pretorius2019young, best2016seeking, bradford2014adolescent}, ease of access and immediacy \cite{bell2018suicide, best2016seeking, burns2016role, burns2010internet}, connection with others with similar experiences \cite{frost2015self, horgan2010young, mar2014exploring},
% gateways to further help-seeking, 
increased perceived control of one's help-seeking journey \cite{pretorius2019young, best2016seeking, mar2014exploring}, capabilities for self-reliance \cite{pretorius2019young, ellis2013young, mar2014exploring}, early access \cite{pretorius2019young, birnbaum2017role, frost2015self}, and inclusivity \cite{pretorius2019young, best2016seeking}. The wide reach of the internet also means that young people can connect with support-givers from various backgrounds. These interactions can be with professionals in specific areas (e.g., medical doctors \cite{khandpur2017telemedicine}), trained support specialists (e.g., people recovered from substance abuse \cite{fruitman2023online}), or peers they may otherwise encounter in school or other parts of daily life \cite{huh2023help}.} 

\edit{Now, a new evolution of technology is entering the landscape of online support -- artificial intelligence (AI) -- and young people are picking it up fast. Approximately 65\% of youth use generative AI tools \cite{salesforce2023new}, such as Large Language Models (LLMs), chatbots, and virtual assistants. Preliminary work suggests that AI-driven systems hold promise to build on the previously described benefits of online interactions by providing accessible, convenient, and personalized support \cite{haque2023overview}. Young people recognize this promise, as more than two-thirds of them have experience with AI-informed mental health apps \cite{gotzl2022artificial}, and many view AI as an acceptable solution to offer mental health support \cite{koulouri2022chatbots}.} 

SIGCHI researchers~\cite{razi2023aCSCW,naslund2016future,armstrong2009patient}, have thoroughly investigated the significance of online peer support in the lives of youth, discovering that while peers would like to offer support, they sometimes do not know how to help or feel the disclosure was inauthentic~\cite{huh2023help}. Furthermore, peer support providers sometimes struggle to maintain boundaries to express their difficulties in writing supportive and empathic responses due to lack of role clarity~\cite{kemp2012}. 
The notation of education as a solution to the lack of expertise \edit{of support givers} was validated by a later study where researchers \cite{sharma2023human} developed an AI system called '\textit{Hailey'} which helped develop more empathetic responses to support seekers in a mental health peer support platform.
\edit{Although,} AI limitations, such as their inability to understand human nuances~\cite{bishop2021artificial} \edit{and the ethical issues related to using AI in sensitive topics such as risks of misclassification~\cite{razi2021human} and potential algorithmic stigmatization and harms~\cite{Andalibi2023conceptualizing}}
% , social implications of deploying them~\cite{folstad2018sig}} 
have led to continued efforts to explore the potential of AI as a supplementary source of support for youth.
However, the youth's norms around peer support and the extent to which AI can effectively address the support needs of youth based on the frequent support-seeking topics of youth and the practical considerations remain areas of ongoing investigation \cite{fulmer2019artificial}.

\edit{Therefore, our goal is to understand how AI compares to the different types of support young people encounter online within the context of the topics that young people specifically seek support about.}
To address the aforementioned gaps in the literature, we ask the following research question\edit{s}: 

\edit{\textbf{(RQ1)} \textit{What are young people's preferences regarding help-giving responses created by humans with various help-giving skills versus AI-generated?}} 

\edit{\textbf{(RQ2)} \textit{How do young people's preferences for help-giving responses vary depending on the topic (relationships, suicidal thoughts, self-expression, or physical health) of the initial help-seeking message?}}

% \item [RQ1:] \textit{ What are young people's preferences regarding human and AI-generated help-giving responses?}
% \item [RQ2:] \textit{How do young people's preferences for help-giving responses vary depending on the topic of the initial help-seeking message?}
% \item \textit{a)How do these preferences vary depending on the topic of the help-seeking messages?}
% \item \textit{b)What are the potential reasons behind this preference?}
To answer our research question\edit{s}, we analyzed 622 survey responses from young people \edit{to understand} their preferences about pre-written responses (from AI, therapist, adult mentor, and peer) to four help-seeking messages on topics \edit{that young people frequently seek support about (}relationships, suicidal thoughts, self-expression, and physical health\edit{) \cite{huh2023help}}. 
We found that young adults preferred AI-generated responses about less sensitive topics (relationships, self-expression, and physical health). For more sensitive discussions (suicidal thoughts), participants preferred responses from the adult mentor.
Our study contributes to the Human-Computer Interaction (HCI) research community in several ways. This paper provides insights into how young people perceive AI-generated responses in peer support situations. Our results also identify the popular conversational topics among young people where AI-generated responses are, and are not, well received. The findings bring implications for designing AI-powered systems to safely and effectively help youth \edit{during online support interactions}.




% Generative artificial intelligence (AI) is seamlessly integrated into everyday technology. , transforming how we consume news, access education, and even engage in private conversations. 

% Artificial intelligence (AI) systems are rapidly becoming more sophisticated and have tremendous potential to transform many fields, including mental health \cite{folstad2017chatbots,brandtzaeg2018chatbots}.

% and approximately 65\% of Gen Z (today's generation of youth) use generative AI \cite{salesforce2023new}. 


% However, the youth's norms around peer support providing and the extent to which AI can effectively address the support needs of youth based on the frequent support-seeking topics of youth and the practical considerations remain areas of ongoing investigation \cite{fulmer2019artificial}.


% Generative artificial intelligence (AI) is rapidly advancing and increasingly integrated into daily life, from customer support and virtual assistants to writing aids and educational tools. AI-driven systems, such as Large Language Models (LLMs), chatbots, or virtual assistants, hold promise to provide accessible and non-judgmental support

% , filling gaps where traditional peer support may fall short\cite{ahn2020chatbot}.   However, the youth's norms around peer support providing and the extent to which AI can effectively address the support needs of youth based on the frequent support-seeking topics of youth and the practical considerations remain areas of ongoing investigation \cite{fulmer2019artificial}.


% This digitization of daily life has changed how young people interact with others, replacing in-person conversations with internet-facilitated options like online forums, social media groups, and direct messaging. 

% blurring the lines between physical and virtual interactions. 

% Generation Z is inextricably bonded with the internet and prioritize their access to technology above in-person experiences. (pew research center teens and technology report)

% These young users harness the power of digital platforms in diverse ways. Notably, 79\% of young adults have turned to the web to seek health-related information, and 33\% have sought information pertaining to mental health. \cite{gowen2013online}. 

% In addition to smartphones and social media, youth now have access to an even more powerful evolution of technology: artificial intelligence (AI).


% However, various barriers exist, hindering young people's access to mental health care. These barriers include the difficulty of seeking professional support for mental health issues with more young people seeking information on how to receive professional support for their mental health while asking to be ‘taken seriously’ as described by Lavis and Winter\cite{lavis2020online}.
% (#Online harms or benefits? An ethnographic analysis of the positives and negatives of peer-support around self-harm on social media) 
% Moreover, young adults are dealing with a pervasive stigma surrounding mental health diagnoses, and challenges related to accessing mental health services \cite{gowen2013online}. Consequently, researchers~\cite{gowen2013online,best2016seeking,burns2014enhancing} have determined that young individuals are increasingly exploring alternatives, such as online forums and social media groups, where they can find support and advice from peers who have encountered similar challenges\cite{ali2015online,gowen2013online}. 
% In doing so, they naturally form communities or join one.
% and with peer-to-peer connections on the rise, young adults seeking to engage with one another and turning to social media platforms as a space to share their experiences with illness, seek guidance, and provide mutual support.  



% \begin{itemize}
%     \item This paper provides insights into how young people perceive AI-generated responses in peer support situations.
%     \item Our results identify the popular conversational topics among young people where AI-generated responses are, and are not, well received.
%     \item The findings bring implications for designing AI-powered systems to safely and effectively help youth to support each other.
% \end{itemize}

% How do young adults perceive different responses to different help-seeking messages:
% - what is the overall preference?
% - does that change depending on the topic?
% - why? what are potential reasons behind these preferences?


% Motivation: 1 paragraph about stats for how young adults use social media, how it's beneficial and detrimental, how young adults seek support + stats for that, give overview for topics discussed with stats
% previous research/gaps to motivate study: 1 paragraph about what previous research has done in terms of support-seeking of youth and how peers sometimes can't provide support per help me paper and how AI might be helpful to provide support. 
% End with "in order to address these gaps, we have xyz research questions, then to address these research questions we did ABC then outline main important findings then contributions" 
% How participants' perceptions about the extent they could relate, help, and sympathize with the help-seeking messages were related to their demographics and how much they liked the responses from different sources? }
% To what extent could participants relate, help, and sympathize with the help-seeking messages based on their demographics? and how those perceptions were related to how much participants liked the different responses?  }
% How do young adults feel about the topics that frequently come up in online peer support conversations?
% How do young adults feel about responses generated by different sources (a young adult peer, an adult researcher, an adult mental health professional, and artificial intelligence)? % need to specify that they don't know the source?
% {react is too generic and not a strong motivation for why it is researched}


\begin{comment}
RQ ideas:
- How do individual differences (demographic factors and experience giving/seeking support) impact (1) preferences of responses or (2) relatability of scenarios?
- How do young adults feel about their ability to relate to, sympathize with, and help a friend who is initiating a peer support conversation?
- Without knowing the content source, do young adults prefer a response generated by a human or AI?
- Do youth prefer a response generated by a person, or AI? RQ2a: Do youth reveal anything about peer support exchange norms based on their preferences for responses written by AI or human sources? RQ2b: without knowing the source of responses presented, do youth prefer content generated by (a) a peer, (b) an adult who is NOT a mental health professional ("researcher"), (c) a mental health professional (therapist), or (d) an AI chatbot (ChatGPT)
% How do young adults' preferences for those responses vary depending on (a) previous experience giving and receiving peer support online, (b) the different topics for which young adults seek support, (c) the relatability of those topics? % does relatability/ability to sympathize/ability to help impact preferences for different responses?

% \item [RQ3:] \textit{What can young adults tell us about their preferences for certain responses during peer support conversations?} 
{2-gram and 3-gram for open-ended questions to explain preferences}
\end{comment}





% • This is the first study to provide insights into support exchanges shared through the social media-linked private messaging platforms (SMPM) among youth.
% • This paper provides insights into dynamics and topics youth
% discussed in their unmoderated social support exchanges
% and online self-disclosures of youth followed by implications
% for design in supporting youth mental health.
% • The results bring implications for designing systems based
% on the unique benefits and potential challenges of SMPMbased support for youth.

% \begin{itemize}
%     \item Identify conversational topics where AI-generated responses can help in peer support.
%     \item Discuss 
% \end{itemize}

==> r_r/2-Related_Work-rr.tex <==
% 1.5 pages total
\section{Related Work}
% \subsection{Online Peer Support for Youth}
% what is social support and why is it important
% Digitization of social support
% In the 21st century, social support interactions are moving to digital spaces. 

% In the pre-smartphone era, texting was the preferred method of communication among youth \cite{nabi2013facebook}. However, now that roughly 96\% of young adults in America have a smartphone \cite{perrin2021mobile}, social media has emerged as the preferred locus of communication exchange.

\subsection{Young Adults\edit{' Mental Health} and Online Social Support}
% problems around mental well-being and how support is needed
More than 450 million people around the world struggle with mental illness \cite{saraceno2002world}, and young adults are disproportionately likely to be among those who are suffering \cite{jurewicz2015mental}. In a cross-country survey, 
% of 13,984 students from 19 colleges across eight countries, the 
the World Health Organization found that nearly one-third of college students tested positive for at least one mental health disorder \cite{auerbach2018world}. Furthermore, mental illnesses like depression, substance use disorders, and psychosis are some of the biggest risk factors for suicide \cite{braadvik2018suicide}, which is the second-leading cause of death for teens and young adults \cite{curtin2022provisional}. With professional treatment being less affordable and less accessible than ever before \cite{kanagaraj2020why}, internet interventions are emerging as a promising avenue for formal treatment \cite{cunningham2014internet} and informal peer support \cite{woodruff2007evaluation}.

% HCI and online support
Social media platforms are some of the most-visited websites on the internet, with some sites getting an estimated 1.7 billion visits every 6 months \cite{statista2021}. 
Researchers \cite{ridout2018use} suggested that youth benefit from online support exchanges on social media platforms; for example, actively engaging with peers online about mental health concerns is associated with an increased likelihood of seeking formal mental health care \cite{ridout2018use}. Unique platform affordances, like anonymity, can help users feel more comfortable being honest about their experiences and feedback \cite{de2014mental}. Also, support exchange on social media can lead to increased quality of life, heightened perceived support, and increased self-efficacy \cite{uehara1990dual}.
% Peer support is a system of giving and receiving help founded on the principles of respect, shared responsibility, and an agreement of what is helpful \cite{mead2001peer}. 

% SIGCHI researchers \cite{razi2023aCSCW,naslund2016future,armstrong2009patient}, have thoroughly investigated the significance of online peer support in the lives of youth, discovering that while peers would like to offer support they sometimes do not know how to help or feel the disclosure was inauthentic~\cite{huh2023help}. Furthermore, peer support providers also struggle to maintain boundaries to express their difficulties in writing supportive and empathic responses due to lack of role clarity~\cite{kemp2012}. The notation of education as a solution to the lack of expertise was validated by a later study where researchers \cite{sharma2023human} developed an AI system called '\textit{Hailey'} which helped develop more empathetic responses to support seekers in a  mental health peer support platform.
% % ; they found the human -AI collaboration enables more emphatic conversation in text based peer to peer mental health support. 
% AI limitations such as their inability to understand human nuances~\cite{bishop2021artificial} have led to continued efforts to explore the potential of AI as a supplementary source of support for youth. AI-driven systems, such as Large Language Models (LLMs), chatbots, or virtual assistants, hold promise in providing accessible and non-judgmental support, filling gaps where traditional peer support may fall short\cite{ahn2020chatbot}.   However, the youth's norms around peer support providing and the extent to which AI can effectively address the support needs of youth based on the frequent support-seeking topics of youth and the practical considerations remain areas of ongoing investigation \cite{fulmer2019artificial}.
% % (Fulmer, Russell. (2019). Artificial intelligence and counseling: Four levels of implementation. Theory & Psychology. 29. 095935431985304. 10.1177/0959354319853045.)

% - discuss two paragraphs of problems around mental well-being and how support is needed
% - https://bmjopen.bmj.com/content/12/8/e061336.abstract
% - use this to talk about the wellbeing problems that are prevalent
% - and transition to the need for peer support, and how online peer support is studied increasingly at HCI


% Human-computer interaction focuses on the design of computer technology between humans and computers, with its roots being found in the 1950s\cite{card2018psychology}.  It wasn't until the 1970s when the intersection of cognitive engineering with computer science and technology brought the psychological aspects of HCI to the forefront\cite{newell1985prospects}.  However, during the early 1980s, there was skepticism regarding the adoption of automation in mental health, primarily stemming from a limited grasp of the psychological intricacies involved\cite{balcombe2022human}.   With the continuous rise and importance of HCI in technological development, its importance cannot be overstated, with more research within the last few decades emphasizing the potential for self-help methods and the need for better system design.

% Social support is a powerful and important part of youth. Years of research point to the benefits of sharing challenging experiences with loved ones who provide support through tough times \cite{reinecke2014authenticity,kim2011facebook,grieve2016psychological}. Such disclosures can help individuals feel more confident \cite{davidson1999peer, salzer2002consumer}, more empowered \cite{davidson1999peer,dumont2002findings,ochocka2006longitudinal,resnick2008integrating}, and more accepting of themselves \cite{shilo2011effects}. Studies also show that peer support can moderate prosocial behaviors \cite{lockwood2014emotion}, schooling \cite{eklund2017adolescent}, physical health \cite{la2002peer}, physical activity \cite{hamilton2017role}, and social functioning \cite{kurtz1990self,nelson2006longitudinal,ochocka2006longitudinal,trainor1997beyond,yanos2001consumer}. 
% However, in the context of mental health, peer support is referred to as the support that individuals with mental illness or learning disabilities can provide to each other \cite{shalaby2020peer}. 


% We also live in a society with the highest rates of mental illness and the lowest access to mental health resources, making people turn to social media as an accessible and free avenue for connection. There are 57.8 million Americans struggling with mental illness \cite{nimh-mental-illness}, and more than 450 million people around the world who have similar concerns \cite{saraceno2002world}, while access to treatment is less affordable and less accessible than ever before \cite{kanagaraj2020why}. As a result, we see a rise of social network-based online interventions that enable connections and support \cite{rayland2023social}.
% among 3.6 billion social media users globally \cite{kanchan2023social}.
% , we see the rise of social sharing where individuals are sharing more information with peers  and as mental heath services continues becomes more inaccessibility\cite{rayland2023social} this become increasing true in more individuals accessing free and widely available support where they mostly discover peer support and networks. 

% With individuals being more willingness to to share or reveal aspects of their identity or experiences so they are not stigmatized or socially rejected. 
% Studies have shown that online forums that allow for anonymous interactions, like Reddit, provide a conducive environment for users to connect and disclose information. 
% Anonymity makes users feel more comfortable being honest with their experiences and feedback, especially around mental health challenges \cite{de2014mental}. However, there are still challenges that hinder disclosures during online peer-to-peer interactions. Lack of professional oversight and propagation of misinformation means there is a risk of well-intentioned, but misguided, advice circulating within online peer networks \cite{swire2020public}
% One prominent challenge is the lack of professional oversight and the potential for misinformation that take place on peer to peer support platforms. Without the guidance of mental health experts, there is a risk of well-intentioned but misguided advice circulating within these peer networks \cite{swire2020public}.
% Bad actors can also take advantage of the anonymity and openness in online spaces to engage in cyberbullying and other online harms, which is detrimental to users who are there to seek support \cite{rainie2017future}

% with the encouragement of open sharing and the anonymity some platforms offer, there is a concern for instances of cyber-bullying or harmful interactions, which can have detrimental effects on individuals seeking support\cite{rainie2017future}


% challenges in online peer interactions
%Given this recent transition to online mediums, the HCI and SIGCHI community is working to understand both the risks and benefits of digitizing social support \cite{decieux2019social}.  Research does suggest that young people can benefit from support exchange on social media, which perhaps explains its increasing prevalence. For example, social media support exchange can have benefits such as heightened perceived support, increased quality of life, or increased self-efficacy \cite{uehara1990dual}. Also, actively engaging with peers online about mental health concerns is associated with an increased likelihood of seeking formal mental health care \cite{ridout2018use}. However, not all of the exchanges on these platforms are beneficial \cite{Sharma2021}

% how youth use social media and internet and some of the content analysis studies that look into those%

\subsection{AI-Powered Mental Health Support}
AI systems are rapidly becoming more sophisticated and have tremendous potential to transform many fields, including mental health \cite{folstad2017chatbots,brandtzaeg2018chatbots}. Generative AI systems, like ChatGPT \footnote{https://chat.openai.com/} and Google Bard \footnote{https://bard.google.com/}, are machine learning models that can create human-like responses for accessible, affordable, and individualized support \cite{singh2023artificial}. 
\edit{The time frame since these technologies became available is very short, but users have started to explore} various ways in which ChatGPT can support mental health and archived \edit{their findings} in non-peer-reviewed venues. 
For instance, researchers explored ChatGPT as a therapist assistant \cite{eshghie2023chatgpt}, where it can work as a companion for patients between therapy sessions, collecting information, listening to patients attentively, offering validation, and sharing potential coping strategies. Another study (again non-empirical, non-peer-reviewed) examined the possibilities of using ChatGPT for child mental health \cite{imran2023chat} \edit{with} medical education for children, translation and assisting in provider-child patient communication, and access to medical information.\cite{van2023artificial} and \cite{kizito2023chatgpt} \edit{discuss similar possibilities for} health condition\edit{s that} can benefit from anonymity in accessing information \cite{kizito2023chatgpt}.

Research about the outcomes of implementing AI systems for mental health is mixed. For example, an analysis of user review comments found that users had mostly positive experiences with AI chatbots for symptoms of anxiety and depression \cite{ahmed_thematic_2022}, and surveys of chatbot systems can suggest that they are useful reporting tools for in-person harms \cite{rita2021chatbot} and can even help to increase youth participation in societal activities \cite{vaananen2020civicbots}. 
However, Martinengo et al. examined dialogues with AI conversational agents (CAs) and found that CAs from app stores are \textit{not} fit for comprehensive suicide risk management. According to their findings, this is because AI systems follow a predefined protocol for suicidal thoughts that is only activated in response to specific phrases that suggest immediate danger, meaning they cannot identify when a conversation is moving towards a problematic topic. Another issue is that CAs cannot send an unsolicited follow-up message after the conversation concludes to ensure the user is safe \cite{martinengo2022evaluation}. 

% Automated mental health support cannot replace human therapists due to its significant inconsistencies and low reliability \cite{farhat2023chatgpt}, and doing so would also undermine the personal connection that is the foundation for why young people engage in online peer support. Therefore, 

\edit{Researchers highlight the importance of better understanding} how AI can maximize its ability to support young people by assisting in conversations \cite{Shao2023empathetic}. For instance, Sharma et al. \cite{sharma2023human} experimented with an AI agent that provides just-in-time feedback to peer support providers in an online mental health support platform and found that AI can help peers increase empathy in their support-giving messages. \edit{These findings are promising for the role of AI in peer-to-peer interactions, but the study did not focus on young people and their specific needs.} 
% Although they did not focus on youth in their study and only focused on empathy. As having empathy may not always be the most helpful way to respond (e.g., when support seekers are looking for concrete actions)- best practices in peer support should also be investigated. 

% - Talk about some recent work on using chatgpt for therapy purposes
% https://www.ncbi.nlm.nih.gov/pmc/articles/PMC10187878/
% https://link.springer.com/article/10.1007/s10439-023-03326-7
% https://www.pjms.org.pk/index.php/pjms/article/view/8118
% - Any effort to automate mental health support in any forms
% - but point out that this is all trying to replace human therapists, and it's not what young people, shown from online peer support, would like doing
% - We need better novel ways to understand how AI can maximize its ability to support young people


% The early days of computer-mediated communication consisted of digitally transmitting human-generated messages \cite{kiesler1984social}, but AI systems enable humans and computers to work together to make that content. 
% what is AI and how popular is it?
% Artificial intelligence (AI) systems are rapidly becoming more sophisticated and widely used. Conversational and generative AI, like ChatGPT \footnote{https://chat.openai.com/} and Google Bard \footnote{https://bard.google.com/}, are machine learning models that can create new content by learning patterns and structures from existing data. Similar models have been deployed in a variety of contexts, including education \cite{okonkwo2021chatbots}, hospitality \cite{buhalis2022voice}, and healthcare for both physical \cite{tjiptomongsoguno2020medical} and mental \cite{folstad2017chatbots,brandtzaeg2018chatbots} concerns. 

% what do we know about the result of using AI?

% \subsection{AI and Peer Support}
% human expectations for AI
% Human-AI collaboration 
% Previous literature~\cite{sharma2023human,sannon_i_2020} has also investigated various people's expectations and behaviors in interactions with AI and conversational agents, including human-agent data-sharing practices and privacy violations~\cite{sannon_i_2020}

%
 
 
\subsection{AI Systems \edit{and Online Support for Young Adults}}
Researchers \cite{carlbring2023new} have investigated \edit{many aspects of AI-enabled} technologies, \edit{including} personalization, ethical considerations, recalling \edit{information from} previous sessions, and detecting body gestures and expressions \cite{carlbring2023new}. At the same time, researchers highlight the lack of accuracy, reliability, bias, and unpredictability of outputs of these generative AI systems \cite{mardikaningsih2023risk}, calling for appropriate mitigation strategies, awareness, and careful consideration of these challenges before jumping into experimenting the possibilities of generative AI on sensitive topics, such as high-risk mental health conversations (e.g., suicide ideation).

% Numerous factors have been associated with the perceived trustworthiness of generative AI systems, including

The common shortcomings of these existing works include empirical testing of how end users might perceive these generative AI-powered systems that support mental health. \edit{While previous work has explored people's perceptions of AI-based agents for mental health \cite{haque2023overview, aggarwal2023artificial}, the verbal expressions and stylistic characteristics of more recent language-based AI technologies (e.g., LLMs) have more human-like characteristics than other AI agents to date \cite{pan2023llms} needs more investigation. Given this technology is new and recent, researchers have only begun to understand the nuanced perceptions of how people over-trust, under-trust, or assess the evolving nature of AI agents' abilities. Additionally, there is very little research on how specific populations, such as young adults, might react to these technologies.}


\edit{The critical role that online social support plays for the youth and young adult populations, the advent of new AI technologies that have great potential to support mental health, and the lack of understanding that we have towards young adults' perceptions around more advanced AI agents place our study into a unique position to contribute to the gaps noted in the literature. Our study is the first to investigate} young adults' perceptions of how helpful, inappropriate, and problematic AI-generated responses are compared to multiple human-generated responses. These tests were conducted blinded, thus allowing us to objectively evaluate initial reactions to the style of the responses themselves rather than young adults' preconceptions around AI. 

\edit{In summary, young people often seek support online, especially for mental health concerns \cite{bae2021social, pretorius2019young}. That support can come from individuals with varying degrees of expertise and experience, and research has shown that these interactions are beneficial \cite{pretorius2019young}. Now, AI systems are permeating digital conversations, but we do not know how young people feel about the content these systems produce. To address this gap, we studied how young people respond to AI-generated messages compared to the different types of support young people encounter online within the context of the topics that young people specifically seek support about.}

% There are two important limitations to this growing body of work that we would like to note. First, most of the studies focus specifically on adults (e.g., \cite{boulos2021iterative,lee2023}. Young adults have their own unique support needs that they often turn to online peer support for \cite{huh2023help} - if technology is going to integrate into settings to provide help to youth specifically, we need to understand how and when they can be most effective. Second, these studies involve designs where users know they are interacting with AI, which introduces additional user expectations and preconceptions about the system rather than the content itself \cite{kocielnik2019will}. These gaps present areas of opportunity to understand how we can design AI tools to facilitate effective support for young people, which we explore in the present study

% In this paper, we address this gap in our understanding to identify popular conversational topics among young people where AI-generated responses are, and are not, well received.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% MISC OLD TEXT %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Some benefits they reported experiencing included increased confidence and affirmation, improved symptom detection, helpful recommendations, affordable consultation, and feelings of support for loneliness. Not all feedback was positive, though -- some users noted issues regarding usability, app updates, privacy issues, and non-creative conversation \cite{ahmed_thematic_2022}.
% by offering help when in-person treatment is unavailable, or the stigma is too great to overcome alone.
  
% The first of these chatbots was called ELIZA, which was designed to respond in a Rogerian style of psychotherapy \cite{weizenbaum1967contextual}. Since ELIZA, we have seen many chatbots and other AI-powered applications to provide mental health support, like Woebot \cite{fitzpatrick2017delivering} and HAILEY \cite{sharma2023human}. Cuijpers et al. analyzed 23 randomized controlled trials for conversational AI tools and found that some applications were as effective as standard face-to-face care \cite{cuijpers2009computer}.

% Human-AI collaboration literature~\cite{sannon_i_2020} has also investigated various people's expectations and behaviors interactions with AI and conversational agents including human-agent data-sharing practices and privacy violations~\cite{sannon_i_2020}


% Moreover, After conducting various research activities to explore the effectiveness of chatbot in youth mental health, Koulouri \& Macredie describe their findings as an acceptable solution to offering mental health support for young adults. With a push for user-centered approach during the development of these applications\cite{koulouri_chatbots_2022}. 

% \cite{d2017artificial}.\cite{boulos2021iterative}. ,~\cite{ahmed_thematic_2022} found that chatbot apps for anxiety and depression provided positive experiences for people, including building confidence and affirmation, symptom detection, helpful recommendations, and affordable consultation, and providing support for loneliness as a companion by analyzing users reviews on 11 apps. Although users had negative reviews regarding usability, app updates, privacy issues, and non-creative conversation.


% conversations as conversational partners, auto-completion, and response suggestions. A

% AI is a popular technology that can be used to provide support and information, especially among young people \cite{koulouri_chatbots_2022}, although it is not a current substitute for human interaction,  in a comprehensive analysis of experts' opinions on the impact of artificial intelligence and networked technology by Pew Research\cite{anderson2018artificial}, most respondents expressed optimism about the potential for AI to enhance human capabilities and empower individuals by 2030 with potential benefits of AI’s role to be seen in healthcare, education and more.

% With an increase in mobile apps using chatbots to provide support for mental health issues. More researchers are highlighting different ways in which AI can provide support within mental health and understanding the context in which AI is being used is crucial in the realm of our study. \cite{d2017artificial}.\cite{boulos2021iterative}. ,~\cite{ahmed_thematic_2022} found that chatbot apps for anxiety and depression provided positive experiences for people, including building confidence and affirmation, symptom detection, helpful recommendations, and affordable consultation, and providing support for loneliness as a companion by analyzing users reviews on 11 apps. Although users had negative reviews regarding usability, app updates, privacy issues, and non-creative conversation.



% Petter Bae Bae Brandtzæg, Marita Skjuve, Kim Kristoffer Kristoffer Dysthe, and Asbjørn Følstad. 2021. When the social becomes non-human: young people's perception of social support in chatbots. In Proceedings of the 2021 CHI Conference on Human Factors in Computing Systems (CHI'21). Association for Computing Machinery, New York, NY, USA, Article 257. 1–13.


% and that technology is increasingly integrated with generative artificial intelligence (AI). Generative AI, like ChatGPT and Google Bard, are machine learning models that use input training data to pick up on its patterns and structures and then generate new data with similar characteristics. 

% HCI researchers have also investigated \edit{the} design and implementation of moderated peer support to facilitate support for youth in specific situations such as the youth with intellectual disability~\cite{banos2018Evaluation}, children surviving cancer~\cite{Lindberg2014Designingpeercancer}, or youth living with human immunodeficiency virus (HIV)~\cite{Karusala2021Courage}.
% Although depending on the context, peer support could have different effects\edit{; for instance,} it could be distressing when the support is judgemental and disrespectful~\cite{takahashi2009potential}. Therefore, \edit{studying how youth peer support happens in social media without moderating specific topics is essential.}



% \subsection{outline - AI in Human Communication}
% AI is an exciting new tool that's being used in a lot of new areas and one of those areas is interpersonal support and mental health applications, and that that is particularly important in a time where like a lot of young people need mental health treatment and help. We know there are a lot fo barriers to young people getting mental health treatment - not knowing who to go to, limited access to health insurance, financial constraints, stigmatization, etc. like especially coming out of the pandemic there we saw so many people who needed mental health treatment that couldn't get it.

% AI is becoming so integrated into interpersonal communication, e.g. autocompletion, Grammarly, etc., so many messages are not purely human-generated content, rather they're the result of a collaboration between humans and AI - we don't understand how people are necessarily responding to that content like not knowing that it came, not knowing where it's coming from.


% AI is a scalable, lo-cost tool to help alleviate some of those challenges, and we're only beginning to understand AI's potential to help in those situations.
% insert some citations of like for example like people have explored the benefits of using like those different chatbots like woebot and Haley and all of those talk about the research behind those and kind of what we know and then.

% But within these conversations, like how our how do you, umm users feel about the actual communications and like the exchange, the details of the exchanges that they're receiving? are they helpful or trying to think like are they being designed in a way that's helpful and also like? Are they helpful across the board or are they only helpful in certain scenarios?
% And then to address that, we took a deeper dive until like the content.

% Researchers have explored many applications of AI, but few, if any, looked at how people react when they do not know what is the source of that response, how they would react to that response?


% like AI is presenting and that kind of also goes with the flow that we do with the abstract of like AI is presenting all these new opportunities for like you know application and we see people already applying it in mental health spaces insert citations of like, you know all the like, talk about those studies. human computer interaction researchers have been looking at, and then they'll be like a human AI interaction section.
% 
% But by telling people that they're interacting with AI like we're getting more of a response to like how they feel about the content, knowing that it's from AI, not just the content itself.
% So there hasn't really been an assessment of like just looking at the message itself.








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% SOURCES OF SOCIAL SUPPORT %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Family is an important source of social support, but it is not the only option. 
%  There are many types of relationships in a young person's life, including peers, trusted adults, and mental health professionals, all of them can provide social support. 

% while each of these sources has their benefits, we see 

% describe the four sources we investigated here to set up the methods section
% We chose these four sources because we wanted to understand young people's norms and preferences about responses generated by sources with proficiency in different areas. A youth peer is someone who is going through or has gone through similar experiences as the help-seeker, so they can offer support and understanding to help a help-seeker feel less alone. However, they may not have the same training or experience as an adult mentor or therapist. 

% peers

% adults - mentors and professionals/clinicians/therapists
% An adult mentor can offer support and guidance, and they can help with navigating life's challenges since they have more life experience and offer a different perspective. However, they may not be able to relate to young people's experiences as well as a youth peer could.

% Therapists are adults who are specifically trained to help people with a variety of mental health issues. Not only can they provide support, guidance, and treatment, but they are also bound by confidentiality laws, which means they cannot share information about help seekers with anyone else without their consent. 





% % rephrase
% While online peer-to-peer
% platforms like TalkLife (talklife.com) and Reddit (reddit.com) enable such supportive conversations in
% non-clinical contexts, highly empathic conversations are rare on these platforms29; peer supporters are
% typically untrained in expressing complex, creative, and open-ended skills like empathy30–33 and may
% lack the required expertise. With an estimated 400 million people suffering from mental health disorders
% worldwide34, combined with a pervasive labor shortage35, 36, these platforms have pioneered avenues
% for seeking social support and discussing mental health issues for millions of people37. However, the
% challenge lies in improving conversational quality by encouraging untrained peer supporters to adopt
% complicated and nuanced skills like empathy.


% % from "Design Opportunities for Mental Health Peer Support Technologies"
% Beyond the use of texting and phone calls for support, people with mental illnesses go online to find peers. Online peer support communities are beneficial in management of illnesses such as breast cancer [14,31], rare diseases [43], and epilepsy [32]. Mental illness is no exception. Peer support is a primary motivation for people who go online for mental health [59]. Peers find each other in online communities for mental health conditions to seek information, emotional support, and advice [6,16,29,42,58]. People with mental health conditions often prefer going online for support because of the benefits of anonymity and convenience [34,49,58,59]. However, research suggests that participating in online communities for mental health can be distressing, even when people report having positive experiences [36,63,70]. Evidence of online interactions between peers with depression show that people have negative experiences with unsupportive members, negative content, and conflicts of beliefs [42]. 



\begin{comment}
    \subsection{Young people need social support}


This support can come from friends, family, teachers, mentors, and other adults. Young people need friends who accept them for who they are. They need friends who they can talk to about their problems and who will support them through tough times.
Being part of a family with a safe and stable home environment is also a major predictor of life outcomes. 
Adult mentors: Young people need adult mentors, such as teachers, who believe in them and who can help them reach their full potential. These are adults in the community who are willing to listen to them and who can help them connect with resources and opportunities.
By understanding the social support needs of youth, we can better support them and help them thrive.


Social support can help young people feel connected, loved, and accepted. It can also help them cope with stress, make healthy choices, and achieve their goals.

There are a number of factors that can affect a young person's social support needs. These include their age, gender, race, ethnicity, socioeconomic status, and sexual orientation. For example, young people who are LGBTQ+ may need more social support than their heterosexual peers.

There are a number of things that can be done to meet the social support needs of youth. These include providing opportunities for young people to connect with each other, training adults to provide social support, and developing policies and programs that promote social support.

It is important to remember that social support is not a one-size-fits-all need. What works for one young person may not work for another. It is also important to be flexible and responsive to the individual needs of young people.


Discuss the role of training in online peer support. It should consider how training can help to mitigate the risks associated with AI-assisted peer support, and how it can help to ensure that AI is used in a beneficial and safe way.

Implications of AI for peer support

Consider the potential benefits and risks of this technology, as well as the ethical considerations that need to be taken into account.

Some of the key questions to address in this section include:

How can AI be used to improve the quality of peer support?
How can we mitigate the risks associated with AI-assisted peer support?
What are the ethical implications of using AI in peer support?
This section should conclude by summarizing the key findings of the literature and by highlighting the need for further research on this topic.

\end{comment}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% FROM HELP ME PAPER: %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Related Work}

% \subsection{Social Support Needs of Youth}
% % Youth between the ages of 13-24 is the time of transition from childhood dependence to adulthood independence \cite{cordon1997youth}. During this time, depending on the social and environmental context of the youth, youth encounters biological (e.g., hormonal changes), social (e.g., bullying, community violence), and academic challenges that might coincide with mental and behavioral risks (e.g., depression, suicide, addictions, unsafe sex) \cite{mullen_defining_2021, Ogbu1990MentoringMY,karcher2006mentoring}. It is a critical developmental phase in which, depending on appropriate guidance and support availability, youth might develop a more negative or positive trajectory \cite{eccles1993parent}. 

% As youth \edit{attempt} to be more autonomous from their parents and look for peers for behavioral and social cues to model \cite{morrissey2015effect}, researchers investigated how peer support might moderate prosocial behaviors \cite{lockwood2014emotion}, schooling \cite{eklund2017adolescent}, physical health such as diabetes \cite{la2002peer} or physical activity \cite{hamilton2017role}, or self-acceptance of sexual orientation \cite{shilo2011effects}. For instance, Morrison et al.\cite{morrissey2015effect} studied Latino youth's transition to middle school and their involvement in antisocial and prosocial behaviors. They found that social support was a critical predictor of school engagement. 
% % Likewise, Morrissey et al. \cite{morrissey2015effect}, from their five-year family and friend support intervention on physical activity for girls between the ages of 13 and 17, found that increase in family and friend support increased moderate and vigorous-intensity physical activity \cite{morrissey2015effect}. Shilo et al.\cite{shilo2011effects} examined the effects of social support components and mental health and sexual orientation milestones of LGB youth. From 461 self-identified LGB youth and young adults, they found peer support and acceptance yielded the most potent positive effect on disclosing sexual orientation and well-being. 
% Similarly, researchers compared how and when these various sources of support are effective. In a sample of urban youths exposed to community violence, peer support was found to predict lower anxiety \cite{affrunti2018community}. Also, research showed actively engaging with peers online about their mental health concerns was associated with an increased likelihood of seeking formal mental health care \cite{ridout2018use}. 

% These social support exchanges can be better achieved when there are ample opportunities for self-disclosure. However, given the sensitivity, risks, and stigma of what youth often go through (e.g., sexual identity, \edit{risky behavior, unsafe sex), finding ways to enable healthy self-disclosure would be vital in facilitating the support youth needs. It would be critical to understanding healthy self-disclosure and how it related} to the effect of psychological well-being and perceived social support.

% \subsection{Self-disclosure and Psychological Well-being}
% Yang and Brown \cite{luo2020self} presented online self-disclosure and presentation to vary on four dimensions: \emph{Breadth} refers to the amount of self-information revealed; \emph{depth} indicates the intimacy of the presented information (e.g., emotions, weaknesses, etc.); \emph{positivity} reflects how positive or negative the presented information is; \emph{authenticity} relates to how \edit{authentic the self-representation is. Recent evidence showed accurate and authentic self-disclosure could} benefit general well-being and improve self-esteem \cite{reinecke2014authenticity}. Genuinely disclosing oneself can predict greater perceived social support and increased support being enacted by others \cite{kim2011facebook}. On the other hand, inaccurate and \edit{inauthentic} self-disclosure can increase perceived stress and impair social connection \cite{grieve2016psychological}. 

% The effects of self-disclosure on well-being largely depend on the valence of the content disclosed. \emph{The capitalization process} \cite{gable2010good} explains how people rearrange their memories related to the content being shared by others. This process would make people feel more positive when hearing positive emotional disclosure and more negative when hearing negative emotional disclosure \cite{ziegele2017no}. Internet culture is biased by the `positivity \edit{norm,' where people share} positive content more than negative disclosures \cite{waterloo2018norms}. Positive disclosures are often reinforced with positive feedback and more social support, leading to feelings of connectedness \cite{andalibi2017sensitive}. \edit{Negative disclosure, on the other hand, may discourage others from responding} because of the positivity norm and the capitalization process \cite{burke2016once}. Such lack of feedback can lead to feeling ostracised, and reduced well-being of the person who shared negative disclosure \cite{luo2020self}.
% %private msgs receive more support, but unsupport is happening

% In this light, such bias and reinforcement toward positive self-disclosure in online social environments bring challenges to psychological well-being, especially for populations like youth, who go through many personal psychological challenges yet pervasively use social media for much of their communications with peers \cite{subrahmanyam2008online}. Researchers consider online authenticity \edit{often unreachable} or possible only with a personal cost, especially for those with marginalized identities and challenging life experiences \cite{10.1145/3479567}. 
% These findings \edit{reveal} that we need safe platforms for youth to share authentic, negative disclosure responses with appropriate support. \edit{To such a platform, there needs to be a better understanding of how youth disclose themselves to garner and receive support.}
 
% \subsection{Online Peer Support for Youth}
% % Peer support has been shown as a robust and broad strategy for reaching groups that existing services often fail to engage. As a terminology initially developed in the contexts of addiction and substance abuse \cite{davidson1999peer}, peer support has shown to be powerful because of its ability to provide firsthand knowledge of experienced individuals and offer visible examples of individuals \cite{mead2001peer}. Peer support has been applied to various areas, including maternal and child health \cite{sokol2016peer} and diabetes and other chronic illnesses \cite{olsson2005role}. 
% % Although much research in psychology, family studies, and health fields examined peer support among youth, many of these studies have been conducted pre-internet/mobile era. A most friend and peer exchanges happen over mobile phones, specifically over social media, instead of texting \cite{nabi2013facebook}. Accordingly, it is unknown how the structure and dynamic of friend support may be shaped in today’s increasingly mobile-based communications among youth and what potential risks might be involved \cite{decieux2019social}.

% Peer support has been increasingly investigated in the HCI literature and within SIGCHI research community~\cite{oLeary2017design,andalibi2016understanding,Bellini2021fragments}, specifically in how people with similar interests exchange support over social media through videos, blogs, \edit{and online forums, or T}witter \cite{baruah2012effectiveness}. Past research showed the importance of support being exchanged through social media and how technology design can further facilitate positive experiences, leading to heightened perceived support, increased quality of life, or increased self-efficacy \cite{uehara1990dual}. However, the populations examined mainly have \edit{primarily} focused on the adult population, often for supporting specific health, such as chronic illness \cite{welch2018interactive}. 

% HCI researchers have also investigated \edit{the} design and implementation of moderated peer support to facilitate support for youth in specific situations such as the youth with intellectual disability~\cite{banos2018Evaluation}, children surviving cancer~\cite{Lindberg2014Designingpeercancer}, or youth living with human immunodeficiency virus (HIV)~\cite{Karusala2021Courage}.
% Although depending on the context, peer support could have different effects\edit{; for instance,} it could be distressing when the support is judgemental and disrespectful~\cite{takahashi2009potential}. Therefore, \edit{studying how youth peer support happens in social media without moderating specific topics is essential.}

% % youth online peer support:
% Finally, a few studies \cite{pretorius2019young,nabi2013facebook,frison_impact_2015} that considered social support for \edit{youth used self-reported data such as surveys or interviews,} which are prone to recall and social-desirability biases \cite{Gorin2001,Fisher1993}. 
% % limited to self-report:
% For instance, Frison and Eggermont~\cite{frison_impact_2015} conducted a survey and structural equation modeling. \edit{They} found that daily stress positively predicted youth social support seeking through Facebook, and if the support was received, it decreased adolescents’ depressed \edit{moods. But in case it was not precise, their depressed mood increased.
% There have} only been a few studies ~\cite{doornwaard2014young,Hartikainen2021safesexting,razi2020let,hartikainen2021care} on youth population online peer support using their digital trace data, but they are on specific issues such as youth online sexual risks~\cite{doornwaard2014young,Hartikainen2021safesexting,razi2020let,dev2022ignoring}. Thus investigating \edit{support-seeking behaviors using social media trace data would give unfiltered insights into the} natural interactions of youth.
 
% % \subsection{Analyzing Youths Public vs. Private Social Media Data}
% Accordingly, as it is \edit{essential} to investigate digital trace data to get an unfiltered view \edit{of} how social support happens in online spaces, studies examined exchanges that are publicly available, such as comments to YouTube videos \cite{naslund2014naturally}, Reddit posts \cite{de2014mental}, or other publicly available online forums \cite{smedley2021practical} partially due to logistical constraints of data collection and privacy. However, these approaches provide limited insights into how support is \edit{sought and given in private spaces}. Public conversations fundamentally differ from those happening in private space \cite{mcgregor201973}, and we know little about how support is being exchanged in private conversations, especially among youth. Collecting private user data is challenging due to the privacy and ethics of human subjects, especially for \edit{youth, since further measures such as parental consent and assent for minors younger than 18 and reporting potential child abuse should be accounted for~\cite{razi2020privacy,agha202responsible}.}

% In this paper, we address this \edit{significant} gap in the literature regarding how youth \edit{exchange} peer support through private conversations on Instagram.
% % ; we investigate the topics that youth possibly disclose and seek help from one another, the types of support they receive, as well as when they fail to receive the help they need. Given the findings, we discuss the technological design implications in enabling a safe, supportive environment for youth to receive peer support when needed.


==> r_r/3-Methods-rr.tex <==
\section{Methods}
\label{sec:methods}
Using an online survey, we examined how young people react to different human- and AI-generated responses to help-seeking messages. In this section, we describe our \edit{participant criteria and recruitment process}, explain our survey design, \edit{review ethical considerations}, and describe our approach to data analysis. 

% about frequent topics that online peer support conversations often entailed, and we selected help-seeking messages from an existing dataset to describe those topics. 
% used an online survey to ask young adults about help-seeking messages and pre-written responses.
% , without saying where the responses came from. 

\subsection{Participant Recruitment \edit{Criteria and} Process}

\edit{Our target population for this study was youth aged 18-24. While youth includes individuals aged 10-24 \cite{orenstein_eriksons_2022}, as it is a time in which physiological and psychosocial development impact well-being in ways that drastically extend the transition period to adulthood \cite{sawyer_age_2018}, we intentionally did not recruit minors. This is because of the sensitive nature of some topics in this study, and we were cautious to avoid unnecessarily exposing minors to topics like suicidal thoughts.}

\edit{We calculated the sample size for the population of youth in the U.S. of 31 million \cite{annie2023young} and determined we needed 385 participants for a 95\% confidence level with a 5\% margin of error and 664 participants for a 99\% confidence level with a 5\% margin of error. Our target was a minimum of 385, but we wanted to get as close to 664 as possible.}

We recruited participants by sharing a digital flyer \edit{on Instagram, Facebook, X (formerly known as Twitter), Discord, and Slack. The flyer included a QR code linked to} an online screening survey to determine prospective participants' eligibility, which required that they are 18 to 24 years old, currently living in the U.S., fluent in English, and have stable access to the Internet. Eligible respondents (N=1,096) continued to the IRB-approved study information sheet, which they were asked to review before continuing to the main survey. To ensure the quality of the responses, there was a built-in attention check question \edit{halfway through the main survey} that asked participants to accurately indicate which help-seeking message topic we had previously asked about.
% (see appendix \ref{attention-check-question} for the full question)
After finishing the survey, participants could provide their contact information to receive \$5 as payment for their time. We received 866 survey responses from eligible participants, of which 622 were deemed fit for analysis \edit{(see table \ref{tab:participant-demographics} for demographic information)} because they were complete and passed the built-in attention check question.

\subsection{Survey Design}
\label{survey-design}
\edit{We used a 4 x 4 study design with four help-seeking messages and four pre-written responses (henceforth referred to as "responses") to each help-seeking message (4 help-seeking messages x 4 responses = 16 total combinations). For each combination, we asked multiple questions. This section provides more details about the help-seeking messages, responses, and survey structure (see Figure \ref{fig:methods-horizontal}).}

\subsubsection{\edit{Help-Seeking Messages and Pre-Written Responses}}
\edit{The help-seeking messages came from \cite{huh2023help}, in which the authors analyzed direct message conversations between youth and categorized youth private messages for support into four main themes: (1) relationships, (2) suicidal thoughts, (3) self-expression, and (4) physical health. To capture these themes in our survey, we used the full help-seeking messages that the excerpts in \cite{huh2023help} came from.}

% \begin{figure}[h!]
%     \centering
%     \includegraphics[scale = 0.21]{figures/help-seeking-messages.png}
%     \caption{Help-seeking messages presented in the survey.}
%     \label{fig:help-seeking-messages}
% \end{figure}

The responses were written by four different sources: a (1) peer, (2) adult mentor, (3) therapist, and (4) artificial intelligence (AI).
% See appendix \ref{appendix-responses} for the full text of responses from the four sources for all help-seeking topics.
\edit{The} \textbf{peer} responses\edit{ in our survey, like the help-seeking messages, came directly from the dataset used in \cite{huh2023help} and were the real responses youth sent after receiving the corresponding help-seeking messages from \cite{huh2023help}. For the \textbf{adult mentor} responses, we wanted the message to reflect best practices for non-clinical crisis interventions. To do this, we identified an intensive, evidence-based training program through Crisis Text Line\footnote{\url{https://www.crisistextline.org}}, a global not-for-profit organization that provides mental health support via text. Given the existing research to support that this organization’s practices are effective \cite{crisis2023decade,gould2022crisis}, the second author used the training materials to generate the adult mentor’s responses to capture the appropriate tone through deliberate phrasing.}
To capture evidence-based professional training, we had a licensed clinical psychologist who also runs an APA-accredited clinical training program write the \textbf{therapist} responses. 
We used responses generated by ChatGPT for the \textbf{AI} responses. To understand how AI and LLMs could advise and support young adults, we prompted ChatGPT, a popular AI-powered chatbot used by many young adults \cite{vogels2023majority}, in May 2023 (GPT-3.5, free version) by asking it to write a response to each help-seeking message ``in the appropriate style and of the appropriate length for a mobile text message" \edit{(see Appendix \ref{appendix-context} for the full context of the prompts we used)}. We chose this prompt after exploration with ChatGPT and some prompt engineering. Initial attempts to generate a response by providing only the help-seeking message repeatedly generated responses in the form of a long bulleted list of advice. Compared to our earlier exploration, ChatGPT's response to our most current prompt was considerably shorter and involved more interaction with the help seeker, which was suitable for a text message. 
% We learned that ChatGPT only provided the desired response when we clearly explained what we wanted in the prompt; otherwise, it could not understand the help seeker on a personal level, but could only give neutral, unbiased responses.

% the chatbot to provide us with advice and emotional support, then had a back-to-back conversation with the model to explore its potential responses.  
% \{ please add what was exactly prompted to ChatGPT (which model was it gpt 3 or 4?, what kinds of prompts and back to back conversation did we have, what did we learn? etc.} - addressed

% The peer responses were from the original youth conversations for each help-seeking message \cite{huh2023help}. The adult mentor responses were designed by a research assistant who had training in \{need to find what type of training Channacy had}. 
% We also wanted to investigate a response from someone in a similar age group as the source of the help-seeking message, but with more experience and training to provide support.
% To include a mental health professional's response, we had a clinical psychologist on the team who drafted the therapist response.
% Given the popularity of AI LLMs among young people \{[CITE]} and their potential to provide support \{[CITE]}, we included a response from ChatGPT to each scenario.

% {add image of help-seeking messages from and table of responses for each topic here!}

Participants were blinded about where the responses came from because we wanted to understand participants' perceptions of the content as part of peer support exchange, not how they felt about different sources of support engaging in the exchange. We also randomized both the order in which the scenarios were presented and the individual questions about each response to prevent question order bias.  

\edit{The full text of the help-seeking messages and responses are in appendices \ref{appendix-messages} and \ref{appendix-responses}, respectively.}

\subsubsection{\edit{Survey Structure}}
\edit{At the beginning of the survey, we asked participants how often they seek and give support online. We used two multiple-choice questions, one for seeking support and one for giving support, to which the answer choices were never, rarely, sometimes, often, or always.}

\edit{Next, we presented the sixteen help-seeking message x response combinations in four sections; each section contained one help-seeking message and its four corresponding responses. Each section had the same structure. First, we instructed participants to imagine they received the help-seeking message from a friend as a text or direct message on social media. Then, we} asked participants to rate the extent to which they agreed with the following statements on a 5-point Likert scale (1 = not at all, 5 = extremely): "I like this response," "I would send this response," "This response contains helpful advice," "This response is problematic," and  "This response is inappropriate." \edit{At the end of each section,} we asked participants to type a brief text response about \edit{why they did and did not like certain combinations.}

\edit{The rationale in using the Likert scale response options was to measure the direction and intensity of the respondent’s attitude and preference toward the specific message. If attitude and preference are measured in a binary fashion (i.e., yes or no), then the data is not robust enough to capture the intensity of the attitude and preference. Because we asked respondents about their attitude and preference for each help-seeking message x response combination, it was important to capture the relative intensity of their attitude and preference for each message to allow for nuance within the data, resulting in a more accurate and representative understanding of feedback. Then, as a limitation of Likert scale responses is not understanding the "why'' behind an attitude or preference, we followed up with the qualitative question.} 

\edit{An attitude or a preference is a psychological construct. In our study, the attitude or preference we tried to measure represented the survey respondent’s predisposition to respond favorably or unfavorably to the scenario (i.e., “I like this response”). Attitudes and preferences are often - although not always - considered precursors to behavior. Numerous studies have demonstrated that individuals often express their attitudes but do not always act in accordance with those attitudes (\cite{bechler2021attitude}). In our study, we used several additional survey questions to examine whether there was consistency with what the respondents liked and what they found helpful (i.e., “I would send this response” and “This response contains helpful advice”). There is a compelling body of research in social psychology that suggests there are times of conflict between what people want (immediate gratification, for example) and what they believe they should do or what they find most helpful (longer-term benefits; \cite{bitterly2017risky}).}

\edit{We included opposing statements for the Likert scale questions for multiple reasons. First, } we know from psychology literature \cite{dakof1990victims} that people may not always seek help or solutions when they discuss problems or concerns; instead, they may primarily seek emotional support, active listening, or validation. 
Therefore, these statements were designed to capture those preferences and validate the cohesiveness in survey responses (i.e., it is unlikely that a participant finds a response both helpful and inappropriate). \edit{We also measured opposing concepts because literature in survey design suggests that participants can present acquiescence bias--the tendency to agree with statements regardless of the content. Also, social desirability bias would make participants inclined to answer in ways they believe are more socially acceptable or favorable. Accordingly, asking about opposing concepts to force participants to think more critically about their answers would increase the quality of survey responses \cite{kuru2016improving}.}

\begin{figure*}[h!]
    \centering
    \includegraphics[scale = 0.7]{figures/methods-horizontal-resized.jpg}
    \caption{\edit{Visualization of the survey structure described in section 3.2.2}}
    \label{fig:methods-horizontal}
\end{figure*}

% \begin{table}[]
% \centering
% \begin{tabular}{|cccc|}
% \hline
% \multicolumn{4}{|c|}{\textbf{How We Presented the Sixteen Help-Seeking Message x Response Combinations}} \\ \hline
% \multicolumn{2}{|c|}{\textbf{Section A}} & \multicolumn{2}{c|}{\textbf{Section B}} \\ \hline
% \multicolumn{1}{|c|}{\textit{\textbf{Help-seeking message topic}}} & \multicolumn{1}{c|}{\textit{\textbf{Response source}}} & \multicolumn{1}{c|}{\textit{\textbf{Help-seeking message topic}}} & \textit{\textbf{Response source}} \\ \hline
% \multicolumn{1}{|c|}{Relationships} & \multicolumn{1}{c|}{Peer} & \multicolumn{1}{c|}{Suicidal Thoughts} & Peer \\ \hline
% \multicolumn{1}{|c|}{Relationships} & \multicolumn{1}{c|}{Adult Mentor} & \multicolumn{1}{c|}{Suicidal Thoughts} & Adult Mentor \\ \hline
% \multicolumn{1}{|c|}{Relationships} & \multicolumn{1}{c|}{Therapist} & \multicolumn{1}{c|}{Suicidal Thoughts} & Therapist \\ \hline
% \multicolumn{1}{|c|}{Relationships} & \multicolumn{1}{c|}{AI} & \multicolumn{1}{c|}{Suicidal Thoughts} & AI \\ \hline
% \multicolumn{2}{|c|}{\textbf{Section C}} & \multicolumn{2}{c|}{\textbf{Section D}} \\ \hline
% \multicolumn{1}{|c|}{\textit{\textbf{Help-seeking message topic}}} & \multicolumn{1}{c|}{\textit{\textbf{Response source}}} & \multicolumn{1}{c|}{\textit{\textbf{Help-seeking message topic}}} & \textit{\textbf{Response source}} \\ \hline
% \multicolumn{1}{|c|}{Self-Expression} & \multicolumn{1}{c|}{Peer} & \multicolumn{1}{c|}{Physical Health} & Peer \\ \hline
% \multicolumn{1}{|c|}{Self-Expression} & \multicolumn{1}{c|}{Adult Mentor} & \multicolumn{1}{c|}{Physical Health} & Adult Mentor \\ \hline
% \multicolumn{1}{|c|}{Self-Expression} & \multicolumn{1}{c|}{Therapist} & \multicolumn{1}{c|}{Physical Health} & Therapist \\ \hline
% \multicolumn{1}{|c|}{Self-Expression} & \multicolumn{1}{c|}{AI} & \multicolumn{1}{c|}{Physical Health} & AI \\ \hline
% \end{tabular}
% \caption{\edit{We presented the sixteen help-seeking message x response combinations in four sections (A, B, C, and D), one for each topic of the help-seeking messages. To mitigate question order bias, we randomized the order in which participants viewed the sections and combinations within each section. The full text of these combinations are in appendices \ref{appendix-messages} and \ref{appendix-responses}, respectively.}}
% \label{tab:survey-structure}
% \end{table}

% % \textit{Response preferences}: 
% To assess participants' response preferences for the different pre-written responses (henceforth referred to as "responses"), we asked a quantitative and a qualitative question. For the quantitative question, participants indicated the extent to which they agreed to the statement "I like this response" on a 5-point Likert scale (1 = not at all, 5 = extremely).
% % \textit{Reasons for response preferences}: 
% For the qualitative question, we asked participants to type a brief text response about what they thought about their most and least preferred response for each help-seeking message.



% \subsubsection{Prior experience with online peer support}
% While prior experience with online peer support was not a requirement to participate in the study, we recognize that prior experience does shape human perception \{rephrase and add reference}. To account for this, we asked "How often do you \textit{seek} support online (e.g., on social media)? This includes, but is not limited to, posting a question on Reddit, direct messaging a friend for help, or asking for advice in a Facebook group. and give peer support online." 
% and "How often do you \textit{give} support online (e.g., on social media)? This includes, but is not limited to, responding to a question on Reddit, direct messaging a friend who asked for help, or giving advice in a Facebook group." Answer choices were on a 5-point likert scale with standard frequency anchors{add reference to pew study and other papers that use same anchors} (1=never, 2=rarely, 3=sometimes, 4=often, 5=always).

% \subsubsection{Demographics}
Lastly, we asked for our participants’ demographic information depicted in Table\ref{tab:participant-demographics}. \edit{See Figure \ref{fig:methods-horizontal} for a visualization of the survey structure.}

% , including their gender, ethnicity, and education. See Table \ref{tab:participant-demographics}.
% {Do we need to justify why we didn't ask about age specifically, or is that assumed since we required a certain age range f`or prospective participants to take the survey so there's not enough variance within that range to draw meaningful conclusions?} \{We should have asked their specific age at the end of survey with the demographic questions. For now don't mention it and if reviewers asked we justify it like that.}

\begin{table}[h!]
\centering
\small
\begin{tabular}{|ccc|}
\hline
% \multicolumn{3}{|c|}{\textbf{Participant Demographics}} \\ \hline
\multicolumn{1}{|c|}{\textit{\textbf{Variable}}} & \multicolumn{1}{c|}{\textit{\textbf{Count (N)}}} & \textit{\textbf{Percent of total (\%)}} \\ \hline
\multicolumn{1}{|c|}{All Responses} & \multicolumn{1}{c|}{622} & 100.00\% \\ \hline
\multicolumn{3}{|c|}{\textbf{Gender}} \\ \hline
\multicolumn{1}{|c|}{Male} & \multicolumn{1}{c|}{403} & 64.79\% \\ \hline
\multicolumn{1}{|c|}{Female} & \multicolumn{1}{c|}{216} & 34.73\% \\ \hline
\multicolumn{1}{|c|}{Non-binary} & \multicolumn{1}{c|}{2} & 0.32\% \\ \hline
\multicolumn{1}{|c|}{Prefer to self-identify} & \multicolumn{1}{c|}{1} & 0.16\% \\ \hline
\multicolumn{1}{|c|}{Prefer not to say} & \multicolumn{1}{c|}{0} & 0.00\% \\ \hline
\multicolumn{1}{|c|}{Total} & \multicolumn{1}{c|}{622} & 100.00\% \\ \hline
\multicolumn{3}{|c|}{\textbf{Ethnicity}} \\ \hline
\multicolumn{1}{|c|}{Caucasian} & \multicolumn{1}{c|}{295} & 47.43\% \\ \hline
\multicolumn{1}{|c|}{African American} & \multicolumn{1}{c|}{193} & 31.03\% \\ \hline
\multicolumn{1}{|c|}{Native American} & \multicolumn{1}{c|}{34} & 5.47\% \\ \hline
\multicolumn{1}{|c|}{Latino or Hispanic} & \multicolumn{1}{c|}{26} & 4.18\% \\ \hline
\multicolumn{1}{|c|}{Mixed Race} & \multicolumn{1}{c|}{24} & 3.86\% \\ \hline
\multicolumn{1}{|c|}{Asian} & \multicolumn{1}{c|}{17} & 2.73\% \\ \hline
\multicolumn{1}{|c|}{Multiple} & \multicolumn{1}{c|}{16} & 2.57\% \\ \hline
\multicolumn{1}{|c|}{Prefer not to say} & \multicolumn{1}{c|}{9} & 1.45\% \\ \hline
\multicolumn{1}{|c|}{Native Hawaiian or Pacific Islander} & \multicolumn{1}{c|}{6} & 0.96\% \\ \hline
\multicolumn{1}{|c|}{Other} & \multicolumn{1}{c|}{2} & 0.32\% \\ \hline
\multicolumn{1}{|c|}{Total} & \multicolumn{1}{c|}{622} & 100.00\% \\ \hline
\multicolumn{3}{|c|}{\textbf{Education}} \\ \hline
\multicolumn{1}{|c|}{Some high school} & \multicolumn{1}{c|}{17} & 2.73\% \\ \hline
\multicolumn{1}{|c|}{High school or equivalent} & \multicolumn{1}{c|}{147} & 23.63\% \\ \hline
\multicolumn{1}{|c|}{Trade school} & \multicolumn{1}{c|}{100} & 16.08\% \\ \hline
\multicolumn{1}{|c|}{Bachelor's degree} & \multicolumn{1}{c|}{297} & 47.75\% \\ \hline
\multicolumn{1}{|c|}{Master's degree} & \multicolumn{1}{c|}{39} & 6.27\% \\ \hline
\multicolumn{1}{|c|}{Doctoral degree} & \multicolumn{1}{c|}{12} & 1.93\% \\ \hline
\multicolumn{1}{|c|}{Other} & \multicolumn{1}{c|}{3} & 0.48\% \\ \hline
\multicolumn{1}{|c|}{Prefer not to say} & \multicolumn{1}{c|}{7} & 1.13\% \\ \hline
\multicolumn{1}{|c|}{Total} & \multicolumn{1}{c|}{622} & 100.00\% \\ \hline
\end{tabular}
\caption{Participant demographics}
\label{tab:participant-demographics}
\end{table}

\subsection{Ethical Considerations}
This study \edit{was submitted for full-review} to [anonymized] IRB \edit{and} was approved as an exempt study\edit{. This} meant participants were presented with the study information sheet but not required to sign a consent document. 
\edit{Despite our study's exempt status, we took multiple precautions to address potential risks due to the sensitive nature of our survey materials. We had a board-certified clinical psychologist on our research team to carefully review all language in the survey questions to minimize potential risks and monitor incoming data for concerning submissions. We also presented all participants with a study information sheet that contained the same information as a full consent document, including detailed descriptions of} the research objective, the procedures involved in completing the survey, the voluntary nature of the study, the potential risks involved, the anonymization process, and incentives. \edit{In lieu of a consent signature, we required all participants to acknowledge they read this document before beginning any study procedures.}

\edit{To protect participants' anonymity and confidentiality, o}nly the research team members specified in the IRB protocol were granted access to the data, which was stored on a university-approved server. \edit{When participants finished their participation, they were each assigned a unique identifier, known only to the researchers on the IRB protocol, that we used to identify the participant instead of their name. The PIs maintained an Excel spreadsheet containing participants’ contact information, which we did not use in our data analysis or any publication resulting from this research.}   

\subsection{Data Analysis}
To ensure we collected high-quality data, we first looked at the correlations between how much participants 'liked' the responses, felt they `would send' the message to the help-seeker, and how `helpful' they thought it was compared to how `problematic' and `inappropriate.' We did this because it is possible for participants to prefer a response for paradoxical reasons, such as finding the content comically inappropriate - fortunately, this was not the case in our data. Using means across the opposing attributes, we confirmed that the responses from sources that participants preferred more, said they were more likely to send, and felt were more helpful were also perceived as less inappropriate and less problematic. 
% This points to the data quality in our study because it signals that participants' reported preferences meant they find value in the help-giving response. 
Participants also tended to feel responses were more helpful than inappropriate or problematic, which means we avoided doing more harm than good, as is essential for ethical research.

We also wanted to understand how participants reacted to the different responses beyond which one they `liked' the most (i.e., preferred). To do this, we looked at aggregate responses for all help-seeking messages by source to understand how helpful the responses were (`helpful'), how likely they were to send them (`would send'), and how inappropriate (`inappropriate') and problematic (`problematic') they felt the responses were. In subsequent sections and figures, we refer to these four measures as `attributes' of participants' responses. \edit{Furthermore, the language we use to describe the findings for the 'would send' attribute includes the phrase “more likely.'' This refers to the extent to which participants agreed they would send the response in question, not that we performed probability or likelihood analysis as that was not part of our study methodology.}

\edit{We analyzed the quantitative data using R software.} \finaledit{Our group size (N) for all statistical tests was equal to our total number of participants, which was 622.} \edit{Before comparing means across combinations, we used Bartlett's test of homogeneity to determine whether variance was equal. When Bartlett's test was significant, indicating that variance is not equal across variables, we used Welch one-way tests for nonparametric data to compare means. When Barlett's test was not significant, meaning variance is equal across variables, we used a one-way ANOVA. We report the p-value for Bartlett's test before all F-statistics to signal which test we used.}

We analyzed the qualitative responses using reflexive thematic analysis \cite{braun2019reflecting} \edit{because it allows appropriate flexibility for inductive, iterative analysis to draw rich conclusions. We took an inductive approach to ensure conceptual coherence because our goal was to identify and develop themes directed by the content of our data, not by existing concepts or ideas. Rather than focusing on specific questions, our objective was to complement our quantitative findings and further explore reasons why participants did, or did not, like specific responses to help-seeking messages about relationships, suicidal thoughts, self-expression, and physical health. Since we conducted this qualitative analysis after analyzing participants' quantitative data, our analytical framework was situated within an essentialist perspective; in other words, we presupposed that participants' open-ended responses reflected their opinions expressed in their previous quantitative survey responses.}




% To do this, we followed the six stages outlined by Braun and Clarke: familiarization with the data, preliminary coding, generating initial themes, reviewing and developing themes, refining themes, and producing the report.
\edit{To start, the second and third authors familiarized themselves with the data by reviewing all qualitative responses and taking notes along the way. They used those notes to identify initial themes for discussion and to share with the rest of the research team. The research team met multiple times to discuss and iterate over the themes and relevant examples to produce the findings in the results section of this paper. We did not use a traditional codebook because the qualitative analyses complement our quantitative findings rather than act as a stand-alone analysis. The first, second, and third authors identified the examples used in our findings section to illustrate our main points.}


% with best practices for qualitative survey research \cite{braun2021online, braun2013shouldnt, winter2021can} 
% to develop codes and themes directly from the content of the data. Rather than focusing on specific questions, our objective was to compliment our quantitative findings and further explore reasons why participants did, or did not, like certain responses to help-seeking messages about relationships, suicidal thoughts, self-expression, and physical health. This analytical framework was situated within a constructionist perspective 

\begin{comment}

FROM ANOTHER PAPER WITH OVERLAPPING METHODOLOGIES (https://journals.sagepub.com/doi/pdf/10.1177/20563051231157297):

We analyzed data using R software. We used group means to
describe perceived harms and preferred remedies. Levene’s tests
to measure variance were significant for both harm and remedy
analyses indicating that homogeneity of variance assumption is
violated. Thus, we used Welch one-way tests for nonparametric
data and posthoc pairwise t-tests which we deemed appropriate
given our sufficiently large sample size [33]. We used the Benjamini–Hochberg (BH) test to correct for multiple comparisons
[12]. We also ran linear regressions with harassment - harm and
harassment - remedy pairings as the dependent variables and demographics and country as the independent variables (4 harassment scenarios x 4 harm types = 16 harm models; 4 harassment
scenarios x 7 remedies = 28 remedy models). We used adjusted Rsquared to identify demographic variables that were more likely to
explain model variance. Welch test and posthoc tests for harm (16
harassment-harm pairings) and remedy (28 harassment - remedy
pairings) comparisons are available in the Appendix. Regression
outputs and confidence intervals for demographic predictors are
also available in the Appendix.

We analyzed the qualitative data to the free responses question
using an iterative, inductive process. Our approach was to familiarize ourselves with the data, develop a codebook, iteratively refine
the codebook, code the data, then revisit the data to make sense of
themes from the coding process. To do this, four members of the
research team first read through a sample of responses across countries and then co-developed a draft codebook. Three members of
the team then coded a sample of responses and calculated interrater
reliability (IRR) for each code using Cohen’s Kappa. Across the 26
codes tested, Kappa values ranged from -0.1 to 1 with a median of
.35. We used the IRR values as well as our manual review of differences to refine the codebook. We removed codes that coders did
not interpret consistently, generally those with agreement below
about .4 and those that were low prevalence in the data. We revised
remaining codes, especially those that had lower agreement, and
discussed them again. The final codebook contained 21 codes (see
Appendix) that focused on moderation practices, user responsibility,
government involvement, and other areas of interest.

\end{comment}

==> r_r/4-Results-rr.tex <==
\section{Results}

% Our findings indicate that human-generated responses perform better when analyses do not take the topic into account, but topic-based analyses reveal that young people prefer AI-generated responses for less sensitive topics. In this section, we describe our findings that led us to this conclusion. 
% We first describe perceptions of help-seeking messages for frequent topics about which peers exchange support, and how those perceptions were related to how much participants liked the different responses. 
Next, we describe participants' preferences for and reactions to different support-giving responses (peer, adult mentor, therapist, and AI) across all help-seeking topics and how these preferences and reactions vary depending on the topic of the help-seeking message they are responding to (relationships, suicidal thoughts, self-expression, or physical health).

% \subsection{Statistics about Reactions to Help-seeking Topics and Demographic Characteristics}

% Participants' overall reported abilities to relate, help, and sympathize with the help-seeking messages were moderate (i.e., close to the mid-range answer choice, which was three on a five-point Likert scale with a range of one to five).
% Participants felt the most sympathy for the help-seeking message about suicidal thoughts but could relate and help most with the help-seeking message about physical health. Interestingly, the message about relationships, not the one about suicidal thoughts, was the least relatable. See Figure \ref{fig:messages-reactions}. \{these conclusions are weird to say after having declared none of the results were significant}
% There were no significant differences between topics for participants' ability to relate, sympathize, or help. However, there were significant, albeit modest, correlations between how much they could relate, sympathize, or help and the extent to which they liked each response. \{this sentence is redundant with next sentence and next sentence is way better. i would delete this prior sentence} 
% Regardless of the source of response (peer, adult mentor, AI, therapist), we noticed that the more participants could relate, sympathize, and help, the more they liked the responses, the more positively they felt about them, and the less negatively they felt about them. See Appendix \ref{cor-messages-responses}.

% \begin{figure}[!t]
%     \centering
%     \includegraphics[scale = 0.5]{figures/plot.messages.react_2023.9.11.png}
%     \caption{Perceptions of help-seeking messages about four topics: relationships, suicidal thoughts, self-expression, and physical health. Answers were on a 5-point Likert scale about agreement with statements on the x-axis. 1 was the lowest agreement, and 5 was the highest agreement.}
%     \label{fig:messages-reactions}
% \end{figure}

%Next, we describe our findings regarding differences found based on demographics (gender, ethnicity, and education). 
% The only reaction for all the help-seeking messages that varied significantly by gender was the ability to help with the help-seeking message about physical health. For this topic, male participants felt they could help more than did female participants (male: M=3.52, SD=0.05; female: M=3.35, SD=0.07; T(396.72) = 1.95, p = 0.05). There were no significant differences by ethnicity in participants' reported ability to relate, sympathize, or help with any of the help-seeking messages. Finally, we found some significant differences based on education 
% for all but two of the variables (ability to help with relationships and ability to relate to suicidal thoughts; 
% (see Appendix \ref{messages-reaction-education-means}), and a subsequent test for correlations indicated that participants with a higher level of education felt they could relate, sympathize, and help more with all of the help-seeking messages (see Appendix \ref{messages-reaction-education-correlations}).

% Our findings did 

% \begin{table}[hbt!]
% \centering
% \begin{tabular}{l|cccccc|}
% \cline{2-7}
%  & \multicolumn{6}{l|}{\textbf{Participants' reported ability to...}} \\ \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{\textit{Topic of Help-Seeking Message}}} & \multicolumn{2}{c|}{\textbf{Relate}} & \multicolumn{2}{c|}{\textbf{Sympathize}} & \multicolumn{2}{c|}{\textbf{Help}} \\ \cline{2-7} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\textit{Mean}} & \multicolumn{1}{c|}{\textit{SD}} & \multicolumn{1}{c|}{\textit{Mean}} & \multicolumn{1}{c|}{\textit{SD}} & \multicolumn{1}{c|}{\textit{Mean}} & \textit{SD} \\ \hline
% \multicolumn{1}{|l|}{\textbf{Relationships}} & \multicolumn{1}{c|}{3.22} & \multicolumn{1}{c|}{1.02} & \multicolumn{1}{c|}{3.30} & \multicolumn{1}{c|}{1.01} & \multicolumn{1}{c|}{3.31} & 0.98 \\ \hline
% \multicolumn{1}{|l|}{\textbf{Suicidal Thoughts}} & \multicolumn{1}{c|}{3.49} & \multicolumn{1}{c|}{0.97} & \multicolumn{1}{c|}{3.62} & \multicolumn{1}{c|}{0.88} & \multicolumn{1}{c|}{3.46} & 0.98 \\ \hline
% \multicolumn{1}{|l|}{\textbf{Self-Expression}} & \multicolumn{1}{c|}{3.51} & \multicolumn{1}{c|}{0.92} & \multicolumn{1}{c|}{3.55} & \multicolumn{1}{c|}{0.94} & \multicolumn{1}{c|}{3.47} & 0.99 \\ \hline
% \multicolumn{1}{|l|}{\textbf{Physical Health}} & \multicolumn{1}{c|}{3.60} & \multicolumn{1}{c|}{0.90} & \multicolumn{1}{c|}{3.61} & \multicolumn{1}{c|}{0.90} & \multicolumn{1}{c|}{3.49} & 0.94 \\ \hline
% \end{tabular}
% \caption{The extent to which participants felt they could relate, sympathize, and help with the four help-seeking messages presented, which were about four different topics (relationships, suicidal thoughts, self-expression, and physical health). Answers were on a 5-point Likert scale.}
% \label{tab:messages-reactions}
% \end{table}

\edit{Almost all of our participants (97\%) reported at least some previous experience seeking and giving support online (i.e., they did not select "never"). The relative frequency of responses was the same for both seeking and giving support. The most frequent response was "sometimes" (seeking: n = 277, 45\%; giving: n = 238, 38\%), second was "often" (seeking: n = 148, 24\%; giving: n = 174, 28\%), third was "rarely" (seeking: n = 113, 18\%; giving: n = 137, 22\%), fourth was "always" (seeking: n = 65, 10\%; giving: n = 57, 9\%), and least frequent was "never" (seeking: n = 19, 3\%; giving: n = 16, 3\%).}

\subsection{Young People's Preferences Regarding Human and AI-generated Help-Giving Responses (RQ\edit{1})}
We found that the human-generated adult-mentor response performed best when we combined responses across all help-seeking topics and compared the average responses from the four sources (peer, adult mentor, therapist, and AI).
% without separating them by topic. 
How much participants liked each source's responses were significantly different (\edit{Bartlett's test: p < 0.05;} \textit{F}(3.0,5517.7) = 99.20, p < 0.001) across all help-seeking messages. \edit{There were also significant differences in the extent to which participants found the responses helpful (Bartlett's test: p < 0.05; \textit{F}(3.0,5519.6) = 104.37, p < 0.001), problematic (Bartlett's test: p < 0.05; \textit{F}(3.0,5525.6) = 20.159, p < 0.001), inappropriate (Bartlett's test: p > 0.05; \textit{F}(3.0,9948) = 19.452, p < 0.001), and how likely they were to send the response (Bartlett's test: p < 0.05; \textit{F}(3.0,5513.9) = 91.09, p < 0.001).} 
% See Appendix \ref{plot-source-like} for a visualization of the differences between these means and their standard deviations).  
% /{double check it I made a correct revision. Did you mean it} 

The post-hoc analysis showed that participants liked the adult mentor's responses the most (M=3.51, SD=0.02), followed by AI (M=3.46, SD=0.02), then the therapist's (M=3.29, SD=0.02), and the peer responses were their least favorite (M=3.03, SD=0.02). This means that before considering the topic of the help-seeking message, it seemed like humans, specifically adult mentors, outperformed AI in generating help-giving responses, although peer responses were not as liked by the participants. However, such responses varied after considering help-seeking topics, which we will discuss. 
% Next, we wanted to understand how participants reacted to the different responses beyond which one they "liked" the most (i.e., preferred). We looked at aggregate responses for all help-seeking messages by the source to understand how helpful the responses were ("helpful"), how likely they were to send them ("would send"), and how inappropriate ("inappropriate") and problematic ("problematic") they felt the responses were. In subsequent sections and figures, we refer to these four measures as "attributes" of participants' responses.

% Next, we break down reactions to the different responses (peer, adult mentor, therapist, and AI) by comparing how helpful each source's responses were, how likely participants were to send the responses from each source to the help-seeker, how problematic and inappropriate the responses were from each source.
% Positive attributes - 
% How much participants felt they would send a response and how helpful they thought it was - \{this should have been in methods and here just go theough the findings. also it is confusing. what is positive attributes? you should just say helpful ess etc that was tested. readers dont have to learn more things and remember them for understadning the findings} followed the same pattern as participants' favorite
% \{this should just be the most liked} responses. 
% \{notnsure jf I understand following the same pattern. Just say only what happened. like removing the previous sentence and right away saying the next sentence here} 
% Participants felt the adult mentor's responses were the most helpful (M=3.50, SD=0.99) of the responses presented and said they were were most likely to send the adult mentor's responses to the help-seeker (M=3.48, SD=0.98), followed by AI's responses (how helpful: M=3.49, SD=1.05; likelihood to send: M=3.42, SD=1.12), then the therapist's responses (how helpful: M=3.29, SD=1.07; likelihood to send: M=3.25, SD=1.12), and the peer's responses receiving the lowest scores (how helpful: M=3.02, SD=1.15; likelihood to send: M=3.00, SD=1.18). 
% The opposing measures - how problematic and inappropriate participants felt the responses were - followed the exact opposite pattern as the positive attributes. 
% According to our analyses, the peer responses were also the most problematic and inappropriate (how problematic: M=2.32, SD=1.24; how inappropriate: M=2.30, SD = 1.24), followed by the therapist's responses (how problematic: M=2.19, SD=1.22; how inappropriate: M=2.18, SD=1.23), then AI's responses (how problematic: M=2.13, SD=0.02; how inappropriate: M=2.12, SD=0.02), and the adult mentor's responses were seen as the least problematic (M=2.07, SD = 0.02) and inappropriate (M=2.05, SD = 0.02). See Figure \ref{fig:source-reactions}. 

% Next, we break down reactions to the different responses (peer, adult mentor, therapist, and AI) by comparing how much participants perceived the responses as helpful and how likely they were to send the response to the help-seeker versus problematic and inappropriate. 
Participants felt the adult mentor's responses were the most helpful (M=3.50, SD=0.99) of the responses presented and also indicated that they were most likely to send the adult mentor's responses to the help-seeker (M=3.48, SD=0.98), followed by AI's responses (how helpful: M=3.49, SD=1.05; \edit{would send}: M=3.42, SD=1.12), then the therapist's responses (how helpful: M=3.29, SD=1.07; \edit{would send}: M=3.25, SD=1.12), and the peer's responses receiving the lowest score for those preferences (how helpful: M=3.02, SD=1.15; \edit{would send}: M=3.00, SD=1.18).

How problematic and inappropriate participants felt the responses were, depending on the source of the response, followed the opposite pattern. The peer responses were perceived to be the most problematic and inappropriate (how problematic: M=2.32, SD=1.24; how inappropriate: M=2.30, SD = 1.24), followed by the therapist's responses (how problematic: M=2.19, SD=1.22; how inappropriate: M=2.18, SD=1.23), AI's responses (how problematic: M=2.13, SD=0.02; how inappropriate: M=2.12, SD=0.02), and the adult mentor's responses as the least problematic (M=2.07, SD = 0.02) and inappropriate (M=2.05, SD = 0.02). See Figure \ref{fig:source-reactions} for a visualization of means and standard deviations for participants' reactions to the responses by source.

\begin{figure*}[!t]
    \centering
    \includegraphics[scale = 0.65]{figures/plot.source.reactions_2023.12.5.png}
    \caption{Participant preferences \edit{for human and AI-generated responses} by source \edit{(RQ1)}. The x-axis is how much participants agreed with the different attributes of their reaction \edit{(i.e., how strongly they agreed with the statements described in section 3.2.2). Points represent means, and the bars on either end are standard deviation.}}
    \label{fig:source-reactions}
\end{figure*}

The findings so far suggest that participants regarded AI-generated responses highly, above even therapist and peer responses, although adult mentors' responses were considered most helpful and most likely to be sent in response to the help-seeking messages. %, - however, these findings do not account for the nuance in real-life peer support exchanges. To address this, we present RQ2-b results on how reactions to human- and AI-generated responses vary depending on what they are responding to.

\subsection{Young People's Preferences for Help-Giving Responses Depending on the Topic of the Initial Help-Seeking Message and Rationale Behind Them (RQ\edit{2})}
% \textbf{\textit{Participants preferred AI-generated responses to help-seeking messages about relationships, self-expression, and physical health, but not suicidal thoughts.}} In the next four sections, we describe this finding in more detail and break down those preferences by the topic of the help-seeking messages: relationships ( section \ref{sec:relationships}), suicidal thoughts (section \ref{sec:suicidal-thoughts}), self-expression (section \ref{sec:self-expression}), and physical health (section \ref{sec:physical-health}). For each topic, we begin with the quantitative results for each attribute of the responses, followed by quotes from open-ended responses from the participants to illustrate why they did, or did not, like each response. Results from the open-ended responses are described from most to least preferred responses within each scenario.

\subsubsection{Relationships}
\label{sec:relationships}
\edit{How much participants liked each source's responses to the help-seeking message about relationships were significantly different (Bartlett's test: p < 0.05; \textit{F}(3.0,1378) = 39.145, p < 0.001) as were the extent to which participants found the responses helpful (Bartlett's test: p < 0.05; \textit{F}(3.0,1377.4) = 33.72, p < 0.001), problematic (Bartlett's test: p < 0.05; \textit{F}(3.0,1379.0) = 14.47, p < 0.001), inappropriate (Bartlett's test: p > 0.05; \textit{F}(3.0,2484) = 12.113, p < 0.001), and how likely they were to send the response (Bartlett's test: p < 0.05; \textit{F}(3.0,1375.6) = 43.24, p < 0.001).}
% Participants' reactions to responses about relationships as a help-seeking topic varied significantly by source, and participants preferred the response generated by AI according to 
Participants preferred the response about relationships that AI-generated more than any of the human-generated options.
They liked AI's response the most (M=3.63, SD=0.04) and thought it was the most helpful (M=3.63, SD=1.00), the least problematic (M=2.01, SD=1.16) or inappropriate (M=2.01, SD=1.20), and said they were most likely to send the AI's response to the help-seeker (M=3.65, SD=0.96). On the other hand, participants did not like the peer's response about relationships (M=3.00, SD=1.15) and felt it was the most problematic (M=2.41, SD=1.24) and inappropriate (M=2.38, SD=1.24), and least helpful (M=3.07, SD=1.13); consequently, they were also least likely to send the peer's response (M=2.98, SD=1.17). See Figure \ref{fig:plot-relationships} for a visual comparison of the means and standard deviations for reactions to all responses about relationships. 

\begin{figure*}[hbt!]
    \centering
    \includegraphics[scale=0.65]{figures/plot.relationships_2023.12.5.png}
    \caption{\edit{Participant preferences for human and AI-generated responses} by source for help-seeking message about relationships \edit{(RQ2, relationships)}.
    \edit{The x-axis is how much participants agreed with the different attributes of their reaction (i.e., how strongly they agreed with the statements described in section 3.2.2). Points represent means, and the bars on either end are standard deviation.}}
    \label{fig:plot-relationships}
\end{figure*}

This sentiment was reflected in open-ended questions, where participants shared they liked the balance and empathy in the \textbf{AI-generated} responses. They felt the AI-generated response invited the help-seeker to share additional information without being overly intrusive or demanding. As one participant put it, the response was \textit{``helpful...
%The response has facts that are hard to hear but they are helpful. The message is 
[and] also supportive and feels like a safe space.''} (P453, Female).
    %it also has ways of how to cope with the situation.. Participants noted that they liked how the AI response both offered support and presented actionable solutions: \textit{“This particular response says it all, it's absolutely what I'd say. What I like the most is that it tells [the friend] how to deal with the situation and still encourages [them].”} The response was \textit{"helpful...
%The response has facts that are hard to hear but they are helpful. The message is 
    %it also has ways of how to cope with the situation.
Some participants described anthropomorphic reasons, such as the AI-generated response seemed like it came from someone who is a good friend: \textit{``They are really trying to help the friend so much and we all need such friends.''} (P434, Female). There were also mentions of qualities participants associated with the AI response, including that they thought it was \textit{``[empathetic]...supportive and caring.''} (P46, Male). Even though participants did favor the AI-generated response to the help-seeking message about relationships, they did note some room for improvement. Namely, that the response doesn't consider the entire context of the situation and \textit{``accuses the ex without listening to his side of the story.''} (P118, Male).

Participants noted that the
% human-generated responses 
\textbf{adult mentor's responses} also provided acknowledgment and validation, but it was potentially less useful and lacked clear direction. Those who liked this response noted that \textit{``it is respectful and...made [them] feel like the person understood [the help-seeker's] feelings.''} (P50, Male). Participants also noted a sense of maturity in how the response did not judge the help-seeker: \textit{``...the [response] answered the question in a mature way by making the victim not feel offended by going back to the ex. The response is just showing him or her that is what we [humans] go through in terms of love life.''} (P403, Male). Despite these positive attributes of the adult mentor's response, some participants felt it lacked concrete advice and did not give specific suggestions for what to do next. As mentioned in the previous paragraph, participants liked that the AI-generated response guided the help-seeker to provide additional detail in a gentle way - they did not feel the adult mentor's response had this same quality. Instead, participants felt the adult mentor's response was, as one participant said, \textit{``
%just about 
beating around the bush''} (P341, Male) and \textit{``
%it 
didn't provide a way of how to solve the situation clearly.''}

Participants liked the \textbf{therapist's response} because they felt it was extremely understanding and non-judgmental but noted that it seemed to delay giving actionable advice. Even though they did not know a therapist wrote one of the responses, they picked up on the professional tone: \textit{``This person provides professional remedy and ... [asks] the victim to share their mixed emotions and from there she/he will be in a position to offer strategies.''} (P481, Female). They saw the response as \textit{``very empathetic without shaming the friend''} (P587, Female), but noted that it felt like \textit{``scheduling [giving] help to next time when the [help-seeker] is in need of it now.''} (P503, Female). They appreciated the supportive tone but would have liked more concrete and immediate advice rather than beating around the bush and delaying support.

We received the most negative comments about the \textbf{peer's response} because participants felt it was terse, suggested hasty actions, and was not encouraging. While some appreciated the response's brevity, the way it was written came across as \textit{``too direct with no empathy.''} (P163, Male). This lack of empathy made participants feel like the sender had a bad attitude and was being too tough on the help-seeker: \textit{``It sounds harsh and rude, and also it doesn't consider the feelings of the victim.''} (P452, Female).

\subsubsection{Suicidal Thoughts}
\label{sec:suicidal-thoughts}
\edit{How much participants liked each source's responses to the help-seeking message about suicidal thoughts were significantly different (Bartlett's test: p < 0.05; \textit{F}(3.0,1375.3) = 64.08, p < 0.001) as were the extent to which participants found the responses helpful (Bartlett's test: p < 0.05; \textit{F}(3.0,1375.6) = 59.14, p < 0.001), problematic (Bartlett's test: p > 0.05; \textit{F}(3.0,2484.0) = 20.40, p < 0.001), inappropriate (Bartlett's test: p > 0.05; \textit{F}(3.0,2484) = 23.46, p < 0.001), and how likely they were to send the response (Bartlett's test: p < 0.05; \textit{F}(3.0,1372.9) = 73.75, p < 0.001).}

The help-seeking topic of suicidal thoughts was the only one for which all the human-generated responses (especially the one from the adult mentor) outperformed  AI's response. Participants liked the adult mentor's response the most (M=3.59, SD=0.95) and felt it was the most helpful (M=3.61, SD=0.94), least problematic (M=2.04, SD=1.18), least inappropriate (M=2.00, SD=1.20), and that they were most likely to send it to the help-seeker (M=3.56, SD=0.94). They also least liked AI's response (M=2.82, SD=1.19) and saw it as the most problematic (M=2.53, SD=1.26), most inappropriate (M=2.54, SD=1.27), least helpful (M=2.93, SD=1.12) and identified it as the one they were least likely to send to the help-seeker (M=2.71, SD=1.21).
See Figure \ref{fig:plot-suicidal-thoughts}. 

\begin{figure*}[hbt!]
    \centering
    \includegraphics[scale=0.65]{figures/plot.suicidal.thoughts_2023.12.5.png}
    \caption{\edit{Participant preferences for human and AI-generated responses} by source for help-seeking message about suicidal thoughts \edit{(RQ2, suicidal thoughts)}. \edit{The x-axis is how much participants agreed with the different attributes of their reaction (i.e., how strongly they agreed with the statements described in section 3.2.2). Points represent means, and the bars on either end are standard deviation.}}
    \label{fig:plot-suicidal-thoughts}
\end{figure*}

When describing why they preferred the \textbf{adult mentor's response} to this sensitive topic, participants noted that they liked how it conveyed genuine concern by inviting the help-seeker to share more details and put effort into providing more support. \textit{``There’s a feeling of relating with the individual here. There’s a feeling of care and [that they're] really interested and [want] to understand the individual}
% plus boosting the individual’s confidence and also wanting to understand the individual’s 
\textit{[and their] situation.''} (P124, Male).
% It’s the best to do in such situation, for someone who wants to really be there for such person.” 
The only area of improvement that participants mentioned for the adult mentor response is that the message could have been a little shorter, but did not note what content should be cut. 

The \textbf{peer's} response was the second most preferred, and participants felt it was superficial, inconsiderate, and did not sufficiently acknowledge the help-seeker's struggles. Interestingly, participants likened the peer response to an AI-generated response, saying it sounded \textit{``...typical of a bot''} (P478, Female). Unlike the adult mentor's response, participants did not like how the peer's response was \textit{``so shallow [and] does not give the victim...much [detail] on how to tackle the situation and [get] helped.''} (P403, Male). 

Participants noted that the \textbf{therapist's response} immediately asked for more information in an attempt to ensure the help-seeker's safety - not knowing that this message was written by a clinician, some thought this sounded \textit{``professional''} while many others took it as intrusively asking for more information right away instead of offering support. \textit{``I think this response makes the person in need sink deeper into her trouble rather than pull her out. It's a bit inappropriate.''} (P451, Female). Since the initial help-seeking message did not use the word "suicide," many participants also did not like that the therapist's response immediately drew that conclusion and felt that calling it out could come across as judgemental: \textit{``I hate the assumption about self harm and suicide. It feels really I'm going to insert myself into your life to fix it and doesn't feel friendly at all.''} (P621, Non-binary).

The \textbf{AI-generated} response overall performed the worst for the help-seeking topic about suicidal thoughts. While some appreciated that the response was \textit{``actually truthful about the person's ability''} (P52, Male), most thought the referral to a healthcare provider conveyed less desire to help in that moment. \textit{``Fine, you can’t provide help but that’s not the best way to put it. You could always have the right choice of words and making the right sentence in this situation before suggesting a mental health professional and not everybody will like the fact that they are referring to them as going crazy. Not really cool though''} (P124, Male).

\subsubsection{Self-Expression}
\label{sec:self-expression}
\edit{How much participants liked each source's responses to the help-seeking message about self-expression were significantly different (Bartlett's test: p < 0.05; \textit{F}(3.0,1378.4) = 37.62, p < 0.001) as were the extent to which participants found the responses helpful (Bartlett's test: p < 0.05; \textit{F}(3.0,1378.4) = 39.53, p < 0.001), problematic (Bartlett's test: p > 0.05; \textit{F}(3.0,2484.0) = 4.88, p < 0.001), inappropriate (Bartlett's test: p > 0.05; \textit{F}(3.0,2484) = 5.56, p < 0.001), and how likely they were to send the response (Bartlett's test: p < 0.05; \textit{F}(3.0,1377.4) = 34.60, p < 0.001).}

Participants' reactions to the responses about self-expression followed a similar pattern to the responses about relationships, meaning AI's response outperformed all the human-generated responses, especially the peer's response. We found that participants liked AI's response the most (M=3.70, SD=0.98), felt it was the most helpful (M=3.75, SD=0.94), said they were most likely to send it to the help-seeker (M=3.67, SD=1.00), and thought it was the least problematic (M=2.01, SD=1.22) and least inappropriate (M=1.99, SD=1.18). Participants also liked the peer's response the least (M=3.08, SD=0.04), said they were least likely to send it (M=3.05, SD=1.15), and thought it was the least helpful (M=3.12, SD=1.09), the most problematic (M=2.25, SD=1.19) and the most inappropriate (M=2.26, SD=1.23).
See Figure \ref{fig:plot-self-expression} for a visual comparison of the means and standard deviations for reactions to all responses about self-expression. 

\begin{figure*}[hbt!]
    \centering
    \includegraphics[scale=0.65]{figures/plot.self.expression_2023.12.5.png}
    \caption{\edit{Participant preferences for human and AI-generated responses} by source for help-seeking message about self-expression \edit{(RQ2, self-expression)}. \edit{The x-axis is how much participants agreed with the different attributes of their reaction (i.e., how strongly they agreed with the statements described in section 3.2.2). Points represent means, and the bars on either end are standard deviation.}}
    \label{fig:plot-self-expression}
\end{figure*}

Participants liked that the \textbf{AI-generated response} conveyed guidance, support, and understanding. \textit{``I think a response like this can make the person feel like they've all been in this situation before, and there are points of empathy that they can draw on to guide them to be braver by drawing on the respondent's situation.''} (P43, Male). Similar to the message about relationships, participants liked that this response \textit{``[empathizes] with the friend while also providing practical solutions''} (P587, Female). 

They felt the response from the \textbf{adult mentor} also conveyed some affirmation of the help-seeker's struggles but to a lesser extent. They liked that \textit{``it starts with sympathy''} (P160, Male), but the overall tone felt \textit{``unattached.''} This distinction between sympathy and empathy is important to note - as sympathy is feeling for someone else while empathy is feeling with them. The adult mentor's response conveyed "sympathy," meaning they can see where the help-seeker is coming from, but \textit{not empathy}, which implies less personal experience with the matter at hand. Participants clearly communicated this sentiment by saying that \textit{``the victim is not understood''} (P383, Male) and that the message indicates \textit{``the person [who wrote it] has no idea of what the [help-seeker] is going through.''} (P611, Female).
% the message \textit{"[gave] the impression that someone should act rudely and not care what others think.”} 

Similar to the relationship help-seeking message, participants suspected that the \textbf{therapist's} message came from a clinician, \textit{``The message looks like one a professional therapist would send...''} (P350, Male). As one participant said, \textit{``The response is appropriate because [it] is from [a] counselor, someone who has been able to tackle much of the issues by being exposed to different clients and knowing what to do for certain client till they reach a point of believing in themselves and having that courage to talk to anyone without any fear.''} (P403, Male).

The \textbf{peer's response} did not feel supportive enough to participants and did not do enough to calm the help-seeker, \textit{``I think that's too casual a response to really consider the issue from the perspective of the person pouring it out.''} (P21, Male). Moreover, they felt this response lacked depth and oversimplified the help-seeker's fear of self-expression. Like the adult mentor response, participants also felt there was not enough of an indication that the person who wrote the response truly understands what the help-seeker is going through, but less so because they can't empathize and more because they do not want to put effort into conveying that empathy, \textit{``It was too brief and nothing more of empathy felt in it. It was more like this person wanted to help but didn’t really put much % of 
effort [into] it...
% Though it was having 
[it had] a little spark of encouragement[,] but it could be better.''} (P124, Male).

\subsubsection{Physical Health}
\label{sec:physical-health}
\edit{How much participants liked each source's responses to the help-seeking message about physical health were significantly different (Bartlett's test: p < 0.05; \textit{F}(3.0,1376.3) = 71.06, p < 0.001) as were the extent to which participants found the responses helpful (Bartlett's test: p < 0.05; \textit{F}(3.0,1376.1) = 77.94, p < 0.001), problematic (Bartlett's test: p > 0.05; \textit{F}(3.0,2484.0) = 20.76, p < 0.001), inappropriate (Bartlett's test: p > 0.05; \textit{F}(3.0,2484) = 17.35, p < 0.001), and how likely they were to send the response (Bartlett's test: p < 0.05; \textit{F}(3.0,1375.8) = 63.92, p < 0.001).}

When the help-seeking message was about physical health, the AI responses once again outperformed the human-generated responses, especially the peer's. Participants liked AI's response the most (M=3.71, SD=0.96), saw it as the most helpful (M=3.67, SD=0.99), least problematic (M=1.95, SD=1.16), least inappropriate (M=1.95, SD=1.21), and overall felt they were most likely to send it to the help-seeker (M=3.64, SD=0.99). The peer response received the least favorable reaction as the least liked response (2.83, 0.05) and thought it was the most problematic (M=2.46, SD=1.28), most inappropriate (M=2.46, SD=1.28), and least helpful (M=2.73, SD=1.22), and indicated they were least likely to send it to the help-seeker (M=2.78, SD=1.23).
See Figure \ref{fig:plot-physical-health} for a visual comparison of the means and standard deviations for reactions to all responses about physical health.

\begin{figure*}[hbt!]
    \centering
    \includegraphics[scale=0.65]{figures/plot.physical.health_2023.12.5.png}
    \caption{\edit{Participant preferences for human and AI-generated responses} by source for help-seeking message about physical health \edit{(RQ2, physical health)}. \edit{The x-axis is how much participants agreed with the different attributes of their reaction (i.e., how strongly they agreed with the statements described in section 3.2.2). Points represent means, and the bars on either end are standard deviation.}}
    \label{fig:plot-physical-health}
\end{figure*}

The \textbf{AI-generated} response once again performed the best, and participants raved about how much they liked it - as one participant said, \textit{``I didn't just like this response. I love this response.''} (P351, Male).
% because apart from being there for the person, you even helping and suggesting professional help for the person.” because 
Participants describe how the answer contained all the important components: empathy, acknowledgment, and concrete suggestions for next steps, \textit{``its an all round genuine answer [that] shows you care[,] understand the problem and offer the right solutions.''} (P592, Female). The "right solution," in this case, was to continue with ongoing self-care work (i.e., talking to a counselor), and participants liked that this response acknowledged doing so is not easy. \textit{``The fact that he empathized with the person and encouraged them to further try [counseling] because you cannot get the intended results after one trial.''} (P80, Male). Participants also liked that counseling was just one of the multiple solutions the response discussed and
%"the response 
\textit{``shows the [help-seeker] how they can use other strategies to be okay.''} (P453, Female). The comprehensive and deeply empathetic nature of this response seems to be what set it apart from the others.
% apart from counseling. it's also empathetic and it has words of affirmations .” 

Participants did like that the \textbf{adult mentor}'s response \textit{``[validated] wanting rest''} (P621, Non-binary), but also felt that it \textit{``[made] the [help-seeker] feel as if it's OK to just relax and not do anything.''} (P351, Male). They discussed how the adult mentor's message did not acknowledge that self-care is more than relaxation. In doing so, this response seemed to convey that there is nothing more the help-seeker can do, \textit{``I feel like it's not addressing the issue at hand and makes the victim feel like they are doing great of which they are not.''} (P137, Male). While participants thought \textit{``praising the [help-seeker] for small achievement[s]''} (P614, Female) and \textit{``positive energy''} were good, they were not enough, \textit{``because 
% I think that 
it doesn't contain enough [advice] that can help the victimized person''} (P125, Male) in this situation.

While the \textbf{therapist}'s response did offer a solution, participants did not think it was the right one: \textit{``It's very unclear whether this respondent wants to help out. They are telling the victim to keep pursuing the same course that ain't working for them.''} (P167, Male). Unlike the AI-generated response, which suggested continued counseling in addition other solutions, participants did not like that the therapist's response was \textit{``just
% practically 
telling the person in question to [continue]
% base only on 
counselling, [with] no other options to explore.''} (P122, Male). Therapy also incurs a cost for the help-seeker, which participants were not shy to mention in their feedback for this response. They noted that \textit{``counselling can be [quite] expensive,''} (P166, Male) and increasing those costs might not be necessary because \textit{``
%although yes counseling helps sometimes but at this time it wont work cause 
at this point [the help-seeker] needs love and support from family and friends who would be available to support them.''} (P438, Female). This does not mean participants wanted the response to suggest the help-seeker stop counseling altogether, but rather that there should be additional non-clinical suggestions.


% \begin{table*}[]
% \centering
% \begin{tabular}{|c|c|}
% \hline
% \textbf{Topic of Help-Seeking Message} & \textbf{Source of Best Response} \\ \hline
% Relationships & AI \\ \hline
% Suicidal Thoughts & Human \\ \hline
% Self-Expression & AI \\ \hline
% Physical Health & AI \\ \hline
% \end{tabular}
% \caption{Source of the best-performing response (human or AI) to help-seeking messages about different topics.}
% \label{tab:best-source}
% \end{table*}

% We summarize these findings to answer RQ2 in table \ref{tab:best-source}, which outlines which 
% source (human or AI) performed the best for all attributes of participants' responses for each scenario. The best-performing response was the most preferred, most likely to be sent, most helpful, least problematic, and least inappropriate.

In summary, our findings revealed that participants preferred AI-generated responses \edit{to help-seeking messages about relationships, self-expression, and physical health}. However, \edit{when the help-seeking message was about suicidal thoughts}, participants preferred responses from the adult mentor. In the next section, we discuss the implications of these findings.

==> r_r/5-Discussion-rr.tex <==
\section{Discussion}
% Our results provide insight about AI's potential to respond to help-seeking topics frequently represented in youth's conversations 
% % \cite{huh2023help} 
% by presenting young adults with human- and AI-content to understand their reactions. 
Our findings point to several important areas for discussion regarding the promise of AI-powered support and questions to address about handling sensitive topics, should they arise.

\subsection{Premise for AI-Powered Support}
% Our results also provide unique insight into how young people react to AI-generated content when they do not know it came from AI. In their qualitative responses, participants likened AI's responses to something a "good friend" might say and used anthropomorphic characteristics (caring, friendship, etc.) to describe why they liked the AI response while comparing the peer-generated responses to "bots." Researchers expect that empathetically interacting AI systems will increase the level of acceptance of social robots \cite{jesin2018artificial}, and our analyses point to other anthropomorphic characteristics to consider.

Our results provide insight about AI's potential to respond to help-seeking topics frequently represented in youth's conversations, which previous literature stated that they sometimes left without supportive responses. \edit{For instance, a study of private messages shared among youth online discovered norms of \textit{`unsupport'} when trust is hampered or when there is lack of resources or understanding of the situation by the youth peers \cite{huh2023help}. Rather than considering AI as a replacement for humans or directly giving support to the help-seeking individual, AI can play many roles in supporting the social support being exchanged among peers. Some examples include providing help-giving individuals tools to understand the intent of help-seeking individuals, ways to respond to the individuals in supportive ways, and how the responses can be stylistically modified to give better support. Our findings about participants' positive reactions to the AI-generated responses provide a premise for using generative AI to assist help-giving individuals in support-giving conversations, as long as the AI response or nudge can maintain} the characteristics that participants identified as helpful, empathetic, constructive, and non-judgemental. However, AI is a constantly moving target, where its characteristics, functionalities, and abilities constantly evolve over time. For instance, for Open AI's GPT models, the level of memorizing past conversations \edit{has been} limited, but recent updates enable\edit{d} the system to remember user preferences and tailor responses accordingly \cite{openai2023release}. Furthermore, depending on the version of GPT models, the prompt engineering techniques \edit{can generate different results}. Accordingly, the lesson we should take away from this study is to apply the rationale provided by the participants and devise ways that future generative AIs can maintain the preferred styles through customization, personalization, prompt engineering, \edit{using API wrappers to workaround shortcomings (e.g., \cite{trivedi2023openai}), and manipulation of training data. Doing so can help with improving the model's performances and transparency that leads to necessary levels of trust \cite{cabrero2023perceived} and human's reliance on AI systems \cite{kim2022perceived}}.

\edit{Some remaining questions include if participants knew it was AI, would they still be as positive as the results have shown? This question can be addressed from a future study, building on the efforts to improve AI-literacy \cite{lee2021developing} on ensuring there is no over- or under-trust of these systems. It seemed as though the participants felt genuine empathy from the AI responses, which was often missing in human-generated responses. If they find out that such genuine responses were artificially generated, it might or might not affect the trust in the system's responses. Our ongoing interview study with a subsample of these participants will address this issue.}
% For instance, **CAN YOU GIVE SPECIFIC EXAMPLES WITH FINDINGS**


% participants knew it was AI would, they still be open to receiving suggestions from AI to support their peers better?
% Concurrent with efforts to improve AI-literacy \cite{lee2021developing}

% \{add something about how we're so concerned with machines ability to detect ai-generated responses, but according to our results humans might not even be able ot ell the difference - especially youth (make case for adding this to AI literacy lessons/pedagogy?)}







% -- discuss how participants used anthropomorphic characteristics (caring, friendship, etc) describing why they liked the AI response. if participants knew it was AI would, they still be open to receiving suggestions from AI to support their peers better? Cite other studies on how people perceive AI suggestions when AI writing style includes different human characteristics such being more empathetic or friendly (refs needed). some implications of our findings here is that AI has the capability to help the peer supporter to write a better response to those support-seeking topics.



\subsection{AI as Complimentary Response based on the Context and Sensitivity of Topics}
Before considering the context of the help-seeking message, it would appear that young people prefer the adult mentor's response. However, a closer look reveals a strong preference for the adult mentor's response to the sensitive help-seeking message about suicidal thoughts while they preferred the AI-generated response to all other help-seeking messages. 
In a research article by Shao \cite{Shao2023empathetic}, a similar encounter takes place where their results indicate human-operated counselors provide higher quality results during empathetic counseling sessions than AI, but upon further investigation, it was clear that the way in which AI-supported an individual became crucial to its success in being rated helpful. 
As indicated by our findings and as previous research \cite{Saha2022towards,ahn2020chatbot} has uncovered participants usually preferred responses that offered support and comfort within the scope of positivity to feel comfortable enough to continue to share. 

We do not intend for our results to imply that AI-generated content is sufficient to replace a therapist or clinical expertise. As we found, participants did not like AI's response about sensitive topics,
%In sensitive situations where AI could not help, 
for which ChatGPT's response specified that the kind of support required was outside the model's capabilities. While some participants appreciated the honest answer that reflected this limitation, others noted that referral to someone else felt dismissive because the help-seeker could have gone to that other source to begin with, but they did not. This points to two interesting follow-up questions: 1. if young adults are experiencing suicidal thoughts, would they go to an AI system for help in a real-world situation? 2. if the answer to question 1 is yes, then how should an AI system respond when a user asks for help it cannot provide for sensitive matters? 
% it is ethical for an AI system to recognize and convey its limits, our participants did not like that the response did not offer additional guidance about what to do next beyond reaching out to a professional. 
% This begs the question of how an AI system should respond when a user asks for help it cannot provide. 
Researchers \cite{mahmood2022owning} have begun to explore how AI should own up to its faults during user interactions, such as when it may provide incorrect information. Our work highlights that similar frameworks should be explored for sensitive topics -- for example, is it more helpful for the AI to respond with links and contact information for resources? If so, which resources are most helpful to share and why? The goal is for AI to convey its limitations constructively, ensuring the user is safe.
% \{Can potentially mention that when we gave our scenario to chagpt now, it prompts that it cannot provide an answer because it is a sensitive topic and you should get professional help and why this is not enough}

%with potential imminent risks to the people. However, the idea that AI-generated content can be helpful for less sensitive issues is powerful in increasing access to resources. Not all mental health professionals handle clinical cases with a diagnosed mental illness, and youth need many non-clinical mental health resources. These include, but are not limited to, learning how to have healthy relationships with emotions \cite{greenberg2003enhancing}, social decision making \cite{elias1988teaching}, resilience and grit in the face of adversity \cite{arias2022can}, and more. However, the availability of these resources can depend on factors that are out of young people's control, like school district curricula and financial resources. AI-generated content presents an opportunity to disseminate this content in a low-cost, accessible way that can help increase access to mental health tools for overall well-being.



The highly sensitive and complex issue of suicidal thoughts demands careful consideration of ethical, legal, and moral concerns, which the current AI technologies cannot address. In creating AI-based risk detection and prevention techniques, we need to keep humans in the loop, such as using AI as an assistant to peer support giver rather than directly having AI interact with struggling individuals as an all-in-one solution. Current AI technology may misinterpret language and is not able to understand the context of the situation, and nuances of human emotional state, which can lead to misidentification. Those false positives or negatives could have catastrophic results depending on the context. Having higher false alarms may burden resources depending on the types of interventions being implemented after detection, such as connecting them to mental health professionals. At the same time, missing instances may leave individuals in distress who may need help. 

% To avoid being legally responsible when an AI intervention goes wrong, companies such as OpenAI do not provide intervention when someone discloses such harmful behaviors, leaving them behind. We call the practitioners and policymakers to hold companies accountable to provide better responses in such cases.

Furthermore, even though our results indicate that young adults prefer responses from an adult mentor, it is possible that participants did not like the idea that a potential peer would interact like a clinician. Participants often noted that the therapist's responses sounded "clinical," which is not a type of interaction that they would expect from peers. That violation of expectations could be what they responded negatively to. We want to stress that cases at risk of suicide require crisis intervention and professional solutions, such as therapy. AI conversational agents could be helpful in identifying users at risk of suicide and self-harm, but it is imperative that we not rely on AI alone to detect imminent risks. Furthermore, there are open questions about monitoring stigmatized topics like suicide, as it can perpetuate algorithmic stigmatization~\cite{Andalibi2023conceptualizing} for individuals struggling with mental health issues and create an environment where they feel constantly surveilled.
\edit{Researchers should investigate the social implications of deploying AI in sensitive contexts such as mental health support based on four algorithmic stigma elements (i.e., labeling, stereotyping, separation, status loss/discrimination)~\cite{Andalibi2023conceptualizing} which they include representational and/or allocative harms from the perspective of youth to minimize them.}









%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% FROM JINA %%%%%%
%%%%%%%%%%%%%%%%%%%%%%% 

% - The overtrust and undertrust of AI--what is most recent literature on chatgpt and people's perceptions on them
% - First study to blind test chatgpt?
% - reasoning behind why they preferred AI over others
% - surprising finding about preference for AI
% > Our finding that generative AI responses were well-received for providing help compared to various human sources provides implications for generative AI's ability to be helpful in providing youth with additional support. 
% > % not saying GAI works, great let's all use it...people unexpectedly really liked GAI, even more than clinician responses

% - but does it really mean that AI can replace the help?
% - what can we learn about peer support least preferred and AI preferred the most?
% > As those responses were from real-world responses youth gave in their social media conversations \cite{huh2023help}, this finding highlights how youth are not always able to provide the support that their peers need. Previous studies had also found 
% > support seekers were left without helpful responses in those situations.
% - assistive, training peers?
% > However, we found adult-mentor responses performed best when we combined responses across all help-seeking topics. This shows the need for education and training of youth to provide better support to their peers.
%*** - interactive ways for people to give feedback, which then can help AI to learn what people like and train peers?
% > { discuss and cite more literature about this: Participants also reflected on why they had these preferences, pointing to positive attributes like empathy, a non-judgemental tone, rational suggestions, and avoiding terse messages with hasty recommendations.}
%*** - What do we know about training writing with chatgpt?
%*** - How can we apply what we know about training writing to the peer support context?

%*** - exception: sensitive topics? What happened?
%*** - AI preferred on non-sensitive topics. What does it mean?


% Below, we expand on the meaning of our findings, followed by implications for design, and ending with limitations and future directions.
% By studying young people's perceptions of pre-written responses from various human sources and generative AI, we found that the AI-generated responses were well-received for providing help with non-sensitive topics.

%  We found that young adults perceived peers' responses as least helpful and most problematic and inappropriate. We also found that participants preferred the responses that acknowledged the help-seeker's situation with empathy, a non-judgemental tone, rational suggestions, and while avoiding terse messages with hasty recommendations. more tangible suggestions for next steps, acknowl 
% not saying GAI works, great let's all use it...people unexpectedly really liked GAI, even more than clinician responses

% \{add something about how we're so concerned with machines ability to detect ai-generated responses, but according to our results humans might not even be able ot ell the difference - especially youth (make case for adding this to AI literacy lessons/pedagogy?)}


 
%\{ discuss and cite more literature about this: Participants also reflected on why they had these preferences, pointing to positive attributes like empathy, a non-judgemental tone, rational suggestions, and avoiding terse messages with hasty recommendations.}%

% \{add results on relationship, self-expression, physical health results that were interesting to discuss here}
% \subsection{AI for Clinical vs Non-Clinical Cases}
% - unexpectedly, people really liked the generative AI response - implication is we don't have much control over it and depending on teh training data/how the algorithm works, its going to change the result of the model. so our results are interesting, but where do we go from here to implement it? it's not like GAI has a certain style. our results might not even help people use GAI out of the box, but we have model number and when we generated it we're 


% \subsection{When AI Can't Help}

% With the advent of generative AI systems (e.g., ChatGPT) being intertwined in everyday tools,
% % , such as smart home devices, smart-phones, and automobile interfaces, 
% researchers increasingly explore ways that these generative AI systems can support mental health.


\subsection{Design Implications}
% \subsubsection{Opportunities for Human-AI Collaboration}
Our findings show how AI-generated responses could be \edit{perceived as acceptable by young people. This finding provides implications for the possibility that AI-generated responses can be used to train or nudge youth to support their peers. AI could be specifically trained with best peer support practices, such as providing specialized recommendations for youth, following therapeutic approaches, or persuasive talks. For instance, behavior change literature has shown that young adults value mental, social, financial, and spiritual aspects when conceptualizing health more broadly than physical health or prevention for chronic illness \cite{molenaar2020language}. Thus, persuasion of behavior change needs to be engaging, feasible, and acceptable \cite{molenaar2020language} rather than relying on the best practices for general populations.} %~\cite{}. 

\edit{Given the unique needs young adults have about persuasion and conversations, rather than relying on expert- or other top-down approaches, humans can co-shape how AI can help in a personalized way. For instance, recent work has shown how humans can help facilitate AI's} expression of empathy in textual supportive conversations in noncritical settings~\cite{sharma2023human}. \edit{Numerous research studies have also explored efforts to generate creative content from human-AI collaborations \cite{hughes2021generative}. For instance, haiku poetry made with stimuli selected by humans were rated as more favorable than those that were generated solely by AI \cite{hitsuwari2023does}, and AI colleagues can help video game designers at various levels with design tasks \cite{lucas2017stay}. AI can provide resources and support suggestions, and young adults can in return provide feedback about what has been helpful or not, further enabling themselves to take agency in training themselves to be better supporters} in their social networks. \edit{For such usage cases of having AI as an assistant for peer support givers, we should ensure the processes and suggestions are transparent and explainable~\cite{shneiderman2020bridging}. The AI assistant should provide where the suggestion is coming from, and what the reasoning is behind it, and nudge young adults to educate themselves and also be reflective about any recommendations made. Furthermore, it would be critical to understand young adults' acceptance of AI-generated recommendations and anchor their decisions, as many researchers have examined. A systematic review of 60 articles on the acceptance of AI showed that perceived usefulness, performance expectancy, attitudes, trust, and effort expectancy significantly and positively predicted behavioral intention, willingness, and use behaviour of AI across multiple industries \cite{kelly2023factors}. However, in some scenarios involving cultural factors, the need for human contact could not be replicated or replaced by AI, regardless of the perceived usefulness or perceived ease of use. One shortcoming of these findings is that they have not engaged younger populations. As such, more research is warranted to understand how such subpopulations might react to newer forms of AI assistance.}

\edit{Also, specific clinically oriented problems cannot be sufficiently addressed by AI or peer supporters, and AI should be able to appropriately acknowledge limitations and respond with valid resources on} diagnostic assessment, psychosocial evaluation, medication management, and therapy~\footnote{\url{https://edis.ifas.ufl.edu}}. 
Similar to how SAMHSA~\footnote{\url{https://www.samhsa.gov/brss-tacs/recovery-support-tools/peers}} defines effective peer support for trauma survivors for those in recovery, it is important that in the design of effective peer support interventions researchers consider the following: providing a sense of safety; trustworthiness and transparency; collaboration and mutuality; empowerment, voice and choice; and awareness of cultural, historical, and gender issues.


% - - communication literature (references?) has looked at AI OR humans, but that's too simple - what kind of human? what kind of AI? What kind of situation/context? These are opportunities for Human-AI collaboration to understand users' preferences, experiences, and backgrounds in those situations to create more personalized feedback/help for peer support-giver to be more effective


% ethical implications:

% Stigmatization and Trust:


% - do we just follow participant preferences? Should we just do what help-seeking people want, or does there have to be some kind of moderation/top-down approach to how we
% - just because a person said I wanted this kind of advice, should we listen to everything they're saying or should there be some limitations?
% - there are some things peer supporters should NOT provide - e.g., diagnostic assessment, medication management, etc., so we need to make sure AI doesn't provide those things
% - there are some good practices like empathic listening, encouraging them to speak to an adult/counselor, which AI could be safeguarded to nudge peer supporter in those directions



% AI-powered peer support
% - qualitative results showed gaps of skillsets that might be missing in certain types of peers, and AI can help fill that gap. call for future research to design AI-powered peer support. 
% - qualitative results helped us identify what they liked/didn't like about GAI responses, so these areimplications for how we might generate AI-based peer support tools
% if we were incorporate 
% possibility of being able to customize GAI - these people have found ways to customize/modify GAI to address customization needs of users, we can use these to customize ai-powered tools of users
% - possibly test one response vs "choose your own journey" type of experience - see "Talking to a bot or a wall? How chatbots vs. human agents affect anticipated communication quality" paper by Zhou et al (https://doi.org/10.1016/j.chb.2023.107674)
% 

\subsection{Limitations and Future Directions}
We recruited participants from our networks and snowball sampling. Therefore, we acknowledged that our dataset might not be a generalizable sample that accurately represents the young adult population in the US. \edit{Although we did meet the minimum sample size for 95\% confidence based on our power analysis (see section 3.1), we did not recruit for a specific subject pool makeup by sex, gender, or location, so our demographics may not be representative of U.S. youth as a whole.} 
Also, we asked participants about static conversation responses, not continuous interactions. Therefore, future research should investigate youth preference in real-time conversations with additional levels of exchange. \edit{Our survey design also used only one response from each source for each help-seeking message, and the next iteration of this study could explore multiple responses per source for each help-seeking message to account for variability.}
Although we included support-seeking topics from real youths' social media interactions\edit{, we only focused on prevalent topics and did not present less frequent ones,} so our study is limited to the topics we \edit{included}. Future research should study more comprehensive scenarios and also go more in-depth studies on specific support-seeking topics to provide deeper insights into each topic. \edit{Future research could also address how} participants \edit{respond when they} kn\edit{o}w the origin of the responses and when they were interacting with AI and. 
\edit{We did not collect qualitative data about every help-seeking message x response combination because survey completion rates drastically reduce as the total number of questions increases \cite{liu2018examining}.} To further understand youth's norms around peer support and perceptions of how AI could be helpful or inappropriate, we are planning to conduct interviews with some of the young people who participated in our study. 
% - Discuss future analyses w/this dataset (based on experiences with giving/seeking support, perceptions of situations, demographic predictors, anything else?), follow-up interviews, and other future studies, like...
% % What do we still not know? What do we need/want to learn? How are we going to do that?
% - continue to test this and see how consistent generative AI is - maybe test different models to see which is most effective for support and why?
% - How would results change if participants knew they were interacting with AI? mention ongoing follow-up interviews


==> r_r/6-Conclusion-rr.tex <==
\section{Conclusion}
To explore the potential for AI-powered peer support, we studied how young adults react to different human- and AI-generated responses to online help-seeking messages. Our findings revealed that participants preferred AI-generated responses about less sensitive topics (relationships, self-expression, and physical health), but not for sensitive discussions about suicidal thoughts. These findings point to the promise of AI-powered tools to help peers support each other during challenging times.

==> test.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{supertabular}[c]{|cccccc|}
\hline
\multicolumn{6}{|c|}{\textbf{Scenario: Relationships}}                                                                                                                                                     \\ \hline
\endfirsthead
%
\endhead
%
\multicolumn{6}{|c|}{N = 622 for all variables}                                                                                                                                                            \\ \hline
\multicolumn{1}{|c|}{\textbf{Source}} & \multicolumn{1}{c|}{\textbf{Attribute}} & \multicolumn{1}{c|}{\textbf{Mean}} & \multicolumn{1}{c|}{\textbf{SD}} & \multicolumn{1}{c|}{\textbf{Min}} & \textbf{Max} \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{3.00}          & \multicolumn{1}{c|}{1.15}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.41}          & \multicolumn{1}{c|}{1.24}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{2.98}          & \multicolumn{1}{c|}{1.18}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.38}          & \multicolumn{1}{c|}{1.24}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{3.07}          & \multicolumn{1}{c|}{1.13}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{3.48}          & \multicolumn{1}{c|}{1.01}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.04}          & \multicolumn{1}{c|}{1.13}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{3.43}          & \multicolumn{1}{c|}{1.02}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.04}          & \multicolumn{1}{c|}{1.21}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{3.47}          & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{3.29}          & \multicolumn{1}{c|}{1.09}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.23}          & \multicolumn{1}{c|}{1.24}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{3.24}          & \multicolumn{1}{c|}{1.15}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.20}          & \multicolumn{1}{c|}{1.24}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{3.27}          & \multicolumn{1}{c|}{1.07}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{3.63}          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.01}          & \multicolumn{1}{c|}{1.16}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{3.65}          & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.01}          & \multicolumn{1}{c|}{1.20}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{3.63}          & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{6}{|c|}{\textbf{Scenario: Suicidal Thoughts}}                                                                                                                                                 \\ \hline
\multicolumn{6}{|c|}{N = 622 for all variables}                                                                                                                                                            \\ \hline
\multicolumn{1}{|c|}{\textbf{Source}} & \multicolumn{1}{c|}{\textbf{Attribute}} & \multicolumn{1}{c|}{\textbf{Mean}} & \multicolumn{1}{c|}{\textbf{SD}} & \multicolumn{1}{c|}{\textbf{Min}} & \textbf{Max} \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{3.22}          & \multicolumn{1}{c|}{1.08}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.18}          & \multicolumn{1}{c|}{1.24}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{3.19}          & \multicolumn{1}{c|}{1.12}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.17}          & \multicolumn{1}{c|}{1.22}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{3.18}          & \multicolumn{1}{c|}{1.11}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{3.59}          & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.04}          & \multicolumn{1}{c|}{1.18}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{3.56}          & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.00}          & \multicolumn{1}{c|}{1.21}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{3.61}          & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{2.99}          & \multicolumn{1}{c|}{1.12}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.42}          & \multicolumn{1}{c|}{1.27}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{2.94}          & \multicolumn{1}{c|}{1.20}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.42}          & \multicolumn{1}{c|}{1.30}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{2.97}          & \multicolumn{1}{c|}{1.15}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{2.82}          & \multicolumn{1}{c|}{1.20}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.53}          & \multicolumn{1}{c|}{1.26}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{2.71}          & \multicolumn{1}{c|}{1.21}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.54}          & \multicolumn{1}{c|}{1.27}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{2.93}          & \multicolumn{1}{c|}{1.12}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{6}{|c|}{\textbf{Scenario: Self-Expression}}                                                                                                                                                   \\ \hline
\multicolumn{6}{|c|}{N = 622 for all variables}                                                                                                                                                            \\ \hline
\multicolumn{1}{|c|}{\textbf{Source}} & \multicolumn{1}{c|}{\textbf{Attribute}} & \multicolumn{1}{c|}{\textbf{Mean}} & \multicolumn{1}{c|}{\textbf{SD}} & \multicolumn{1}{c|}{\textbf{Min}} & \textbf{Max} \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{3.08}          & \multicolumn{1}{c|}{1.09}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.25}          & \multicolumn{1}{c|}{1.19}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{3.05}          & \multicolumn{1}{c|}{1.15}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.26}          & \multicolumn{1}{c|}{1.23}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{3.12}          & \multicolumn{1}{c|}{1.09}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{3.51}          & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.10}          & \multicolumn{1}{c|}{1.16}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{3.48}          & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.08}          & \multicolumn{1}{c|}{1.18}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{3.51}          & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{3.46}          & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.05}          & \multicolumn{1}{c|}{1.15}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{3.42}          & \multicolumn{1}{c|}{1.05}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.09}          & \multicolumn{1}{c|}{1.19}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{3.49}          & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{3.70}          & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.01}          & \multicolumn{1}{c|}{1.22}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{3.67}          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{1.99}          & \multicolumn{1}{c|}{1.18}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{3.75}          & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{6}{|c|}{\textbf{Scenario: Physical Health}}                                                                                                                                                   \\ \hline
\multicolumn{6}{|c|}{N = 622 for all variables}                                                                                                                                                            \\ \hline
\multicolumn{1}{|c|}{\textbf{Source}} & \multicolumn{1}{c|}{\textbf{Attribute}} & \multicolumn{1}{c|}{\textbf{Mean}} & \multicolumn{1}{c|}{\textbf{SD}} & \multicolumn{1}{c|}{\textbf{Min}} & \textbf{Max} \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{2.83}          & \multicolumn{1}{c|}{1.19}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.46}          & \multicolumn{1}{c|}{1.28}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{2.78}          & \multicolumn{1}{c|}{1.23}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.40}          & \multicolumn{1}{c|}{1.27}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{2.73}          & \multicolumn{1}{c|}{1.22}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{3.48}          & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.10}          & \multicolumn{1}{c|}{1.22}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{3.44}          & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.06}          & \multicolumn{1}{c|}{1.16}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{3.43}          & \multicolumn{1}{c|}{1.01}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{3.43}          & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.06}          & \multicolumn{1}{c|}{1.19}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{3.38}          & \multicolumn{1}{c|}{1.01}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.02}          & \multicolumn{1}{c|}{1.16}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{3.45}          & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{3.71}          & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{1.95}          & \multicolumn{1}{c|}{1.16}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{3.64}          & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{1.95}          & \multicolumn{1}{c|}{1.21}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{3.67}          & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{6}{|c|}{\textbf{All Scenarios Combined}}                                                                                                                                                      \\ \hline
\multicolumn{6}{|c|}{N = 2488 for all variables}                                                                                                                                                           \\ \hline
\multicolumn{1}{|c|}{\textbf{Source}} & \multicolumn{1}{c|}{\textbf{Attribute}} & \multicolumn{1}{c|}{\textbf{Mean}} & \multicolumn{1}{c|}{\textbf{SD}} & \multicolumn{1}{c|}{\textbf{Min}} & \textbf{Max} \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{3.03}          & \multicolumn{1}{c|}{1.14}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.32}          & \multicolumn{1}{c|}{1.24}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{3.00}          & \multicolumn{1}{c|}{1.18}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.30}          & \multicolumn{1}{c|}{1.24}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Peer}            & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{3.02}          & \multicolumn{1}{c|}{1.15}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{3.51}          & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.07}          & \multicolumn{1}{c|}{1.17}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{3.48}          & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.05}          & \multicolumn{1}{c|}{1.19}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Adult Mentor}    & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{3.50}          & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{3.29}          & \multicolumn{1}{c|}{1.06}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.19}          & \multicolumn{1}{c|}{1.22}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{3.25}          & \multicolumn{1}{c|}{1.12}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.18}          & \multicolumn{1}{c|}{1.23}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{Therapist}       & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{3.29}          & \multicolumn{1}{c|}{1.07}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{like}               & \multicolumn{1}{c|}{3.46}          & \multicolumn{1}{c|}{1.10}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{problematic}        & \multicolumn{1}{c|}{2.13}          & \multicolumn{1}{c|}{1.22}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{would send}         & \multicolumn{1}{c|}{3.42}          & \multicolumn{1}{c|}{1.12}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{inappropriate}      & \multicolumn{1}{c|}{2.12}          & \multicolumn{1}{c|}{1.24}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\multicolumn{1}{|c|}{AI}              & \multicolumn{1}{c|}{helpful}            & \multicolumn{1}{c|}{3.49}          & \multicolumn{1}{c|}{1.05}        & \multicolumn{1}{c|}{1.00}         & 5.00         \\ \hline
\end{longtable}
